Position: Towards Bidirectional Human-AI Alignment

Recent advances in general-purpose AI underscore the urgent need to align AI systems with human goals and values. Yet, the lack of a clear, shared understanding of what constitutes "alignment" limits meaningful progress and cross-disciplinary collaboration. In this position paper, we argue that the research community should explicitly define and critically reflect on "alignment" to account for the bidirectional and dynamic relationship between humans and AI. Through a systematic review of over 400 papers spanning HCI, NLP, ML, and more, we examine how alignment is currently defined and operationalized. Building on this analysis, we introduce the Bidirectional Human-AI Alignment framework, which not only incorporates traditional efforts to align AI with human values but also introduces the critical, underexplored dimension of aligning humans with AI -- supporting cognitive, behavioral, and societal adaptation to rapidly advancing AI technologies. Our findings reveal significant gaps in current literature, especially in long-term interaction design, human value modeling, and mutual understanding. We conclude with three central challenges and actionable recommendations to guide future research toward more nuanced, reciprocal, and human-AI alignment approaches.

==> figures/literature.tex <==











% \subsection{AI Writing Support Tools}



% The improvements in large language models (LMs) like GPT3~\citep{gpt3} and Meena~\citep{meena} have provided unprecedented language generation power. This leads to an increasing interest in how these new technologies may support writers with AI-assisted writing support tools~\citep{lee2022coauthor}. 
% % 
% In these human-AI collaborative writing tasks, the writers interact with AI writing support tools not only for understanding its assessment but also aim to leverage its feedback to improve the human writing output~\citep{huang2020heteroglossia}. 
% % 
% % \hua{[DONE] lower-level writing assitance.}
% A few technologies are developed to support human writing. Many of them focused on \emph{lower-level linguistic improvement}, such as proofreading, text generation, grammar correction, auto-completion, etc. 
% % 
% For instance, Roemmele and Gordon~\citep{roemmele2015creative} proposed a Creative Help system that uses a recurrent neural network model to generate suggestions for the next sentence. 
% % 
% % 
% % 
% Furthermore, a few studies propose AI assistants that leverage the generation capability of the language models to \emph{generate inspirations} to assist the writers' ideation process~\citep{gero2022design,wang2022interpretable,coenen2021wordcraft}. 
% For instance, 
% Wordcraft~\citep{coenen2021wordcraft} is an AI-assisted editor proposed for story writing, in which a writer and a dialogue system collaborate to write a story. The system further supports natural language generation to users including planning, writing and editing the story creation.
% % 

% Additionally, there are a number of studies that design AI assistants to \emph{provide assessment and feedback} to improve human writings iteratively~\citep{du2022read,shen2023parachute}. 
% For example, Huang et al.~\citep{huang2018feedback} argue that writing, as a complex creative task, demands rich feedback in the writing revision process. They present Feedback Orchestration to guide writers to integrate feedback into revisions by a rhetorical structure. 
% More studies are proposed for AI-assisted peer review~\citep{checco2021ai}. For example, Yuan et al.~\citep{yuan2021can} automate the scientific review process that uses LLMs to generate reviews for scientific papers. 






% In this work, we apply conversational AI feedback and explanations to human-AI scientific writing tasks, in which humans submit their writings to the system and iteratively make a sequence of small decision-making processes based on AI feedback and explanations.
% As \emph{writing is a goal-directed thinking process}~\citep{gero2022design}. 
% The goal of the \convxai is to support writers to \emph{understand the feedback} and further \emph{improve their writing} outputs. 
% Particularly, \system achieves faithful scientific writing feedback by incorporating domain knowledge-embedded AI scoring, cutting-edge AI explanations, and writing suggestions.
% As a result, we aim to evaluate the effects of conversational AI feedback and explanations with domain knowledge-embedded in terms of not only helping users understand the AI prediction but also improving writing performance.







% \subsection{Conversational AI Systems}


% Our work is situated within the rich body of conversational AI or chatbots studies, which entails a long research history in the NLP~\citep{coqa,li2019acute} and HCI fields~\citep{setlur2022you,fast2018iris}. Jurafsky~\citep{jurafsky2000speech} proposes that conversation between humans is an intricate and complex join activity, which entails a set of imperative properties: {\em multiple turns}, {\em common grounding}; {\em dialogue structure},  {\em mixed-initiative}.
% % 
% By incorporating these properties, conversational interactions are also shown to significantly contribute to establishing long-term rapport and trust between humans and systems~\citep{bickmore2001relational}. 
% User interaction experience can be improved by a set of factors from the conversational AI systems~\citep{setlur2022you}. For example, Chaves and Gerosa~\citep{choudhry2020once} describe how human-like social characteristics, such as conversational intelligence and manners, may benefit the user experience.


% These principles and theories inform us to design a conversational AI explanation system that fulfills the diverse user needs in practice. Our study is deeply rooted in the conversational explanations in XAI -- the users request their demanded explanations through the chatbot-based AI assistants~\citep{sokol2018glass, tsai2021exploring}. Previous studies have explored the effectiveness of interactive dialogues in explaining online symptom checkers (OSCs)~\citep{tsai2021exploring, sun2022exploring}. For example, Tsai et al.~\citep{tsai2021exploring} intervened in the diagnostic and triage recommendations of the OSCs with three types of explanations ({\ie rationale-based, feature-based and example-based explanations}) during the conversational flows.
% The findings yield four implications for future OSC designs, which include empowering users with more control, generating multifaceted and context-aware explanations, and being cautious of the potential downsides.



% However, these existing conversational AI explanation systems are still in the preliminary stage, which only provides one type of explanation and disables users from selecting different explanation types.
% % 
% Also, these are far from being able to incorporate user feedback into producing AI explanations ({\eg enable users to choose counterfactual prediction foil}) and produce personalized explanations for users' individual needs.
% % 
% In addition, these conversational AI explanation systems are primarily applied to improve system transparency and comprehensibility, thus helping users understand and build trust in the systems.
% Little attention has been paid to examining {\em if} and {\em how} conversational AI explanations can be indeed useful for users to improve their performance in human-AI collaborative tasks.
% % 
% % 

% % \hua{[DONE] Elaborate what's the difference of ours.}
% Our work improves the conversational AI feedback and explanation systems from two perspectives: i) we focus on AI tasks where the human's goal is to improve their task performance ({\ie} scientific writing) rather than merely gain an understanding of the AI predictions; ii) we identify four design principles and incorporate them into the empirical system design for further evaluation with human tasks.
% Our work aims to further unleash the capability of conversational AI explanations and make them more useful for human tasks.










% % \begin{figure*}[!t]
% %   \includegraphics[width=0.85\textwidth]{figures/pilot.pdf}
% %   \vspace{-0.em}
% %   \caption{An overview of User Interface (UI) for the pilot study. (A) shows the recommended edits from the writing models, and (B) displays a range of XAI buttons for users to choose from for viewing AI explanations.
% %   }
% %   \label{fig:pilot}
% % \end{figure*}















% \subsection{Human-Centered AI Explanations}

% Earlier studies in the fields of Explainable Artificial Intelligence (XAI) primarily focus on developing different XAI techniques, which aims to explain \emph{why the model arrives at the predictions.} This line of studies can be broadly categorized into generating post-hoc interpretations for well-trained deep learning models~\citep{geval:2019:blackboxnlp} and designing self-explaining models~\citep{shen-etal-2022-shortest,lei-etal-2016-rationalizing,shi2016does}. 
% In specific, the majority of XAI methods aim to provide post-hoc interpretations either for each input instance ({\ie} named ``local explanations'')~
% \citep{de-cao-etal-2020-decisions,kim-etal-2020-interpretation,sankar-etal-2019-neural} or for providing a global view of how the AI model works ({\ie} named ``global explanations'')~\citep{ribeiro2018anchors}, where our study covers both of them. 
% % 
% Additionally, XAI approaches are also divided into different formats~\citep{shen2021explaining},
% including example-based~\citep{feng2019can}, feature-based~\citep{lime}, free text-based~\citep{rajani-etal-2019-explain,NEURIPS2018_4c7a167b}, rule-based explanations~\citep{ribeiro2018anchors}, etc, where our study covers a range of XAI formats.


% Despite the increasing number of XAI approaches have been proposed, evaluating AI with humans is still a challenging problem.
% Doshi-Velez and Kim~\citep{doshi:2017:towards} propose a taxonomy of interpretability evaluation including ``application-grounded'', ``human-grounded'' and ``functionally-grounded'' evaluation metrics based on different levels of human involvement and application tasks.
% % 
% The majority of the proposed XAI approaches are commonly validated effectively using the ``functionally-grounded'' evaluation methods~\citep{jacovi2020towards,promisperil,wiegreffe-pinter-2019-attention}, 
% which seek for automatic metrics ({\eg} ``plausibility'') on proxy tasks without real human participations~\citep{mohankumar2020towards,bastings-filippova-2020-elephant,10.1145/3359158}.


% Furthermore, we can see burgeoning efforts being put around involving real humans in evaluating AI explanations under the theme of ``human-centered explainable AI''. The state-of-the-art XAI methods are applied to real human tasks, such as assessing human understanding~\citep{shen2020useful}, human simulatability~\citep{ribeiro2018anchors,shen-etal-2022-shortest}, human trust and satisfaction on AI predictions~\citep{smith2020no,reasonchains:2019:emnlp}, and human-AI teamwork performance~\citep{chu2020visual}, etc~\citep{hase2020evaluating,feng2019can,ghai2020explainable}. 
% % 
% However, many human studies show that AI explanations are not always helpful for human understanding in tasks such as simulating model prediction~\citep{shen-etal-2022-shortest}, analyzing model failures~\citep{shen2020useful}, human-AI team collaboration~\citep{Bansal2021DoesTW}. For instance, \citet{Bansal2021DoesTW} conducted human studies to investigate if XAI helps achieve complementary team performance and showed that none of the explanation conditions produced an accuracy significantly higher than the simple baseline of showing confidence.

% In response, a line of work dives deep into the gaps between real-world user demands and the status quo XAI methods. Their findings reveal that users tend to ask \emph{multiple}, \emph{dynamic}, and sometimes \emph{interdependent} questions on AI explanations, whereas state-of-the-art XAI methods are mostly unable to satisfy.
% Although GUI-based XAI systems, which integrate multiple XAI into one interface, can potentially mitigate this issue, they inevitably suffer from the drawbacks, such as cognitive overload, frequent UI updates, etc.

% Therefore, prior studies envision the potential of ``Explainability as a Dialogue'' to balance the cognitive load with the diverse user needs~\citep{slack2022talktomodel,lakkaraju2022rethinking,marrakchi2021explaining,tsai2021exploring,sun2022exploring}. 
% For example, through interviews with healthcare professionals and policymakers,  \citet{lakkaraju2022rethinking} found that decision-makers strongly prefer interactive explanations with natural language dialogue forms and thereby advocated for interactive explanations. 
% % 
% Nevertheless, there has been little exploration of how a conversational XAI system should be designed in practice and how users might react to it.
% Our studies aim to resolve this problem by incorporating practical user needs into the 
% conversational XAI design, propose a user-oriented conversational universal XAI interface and investigate human behaviors during using these systems.











==> keyword.tex <==
%
% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
% Please copy and paste the code instead of the example below.
%

% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>00000000.0000000.0000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc[300]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc[100]{Do Not Use This Code~Generate the Correct Terms for Your Paper}

% %%
% %% Keywords. The author(s) should pick words that accurately describe
% %% the work being presented. Separate the keywords with commas.
% \keywords{Do, Not, Us, This, Code, Put, the, Correct, Terms, for,
%   Your, Paper}

% \received{20 February 2007}
% \received[revised]{12 March 2009}
% \received[accepted]{5 June 2009}


% https://dl.acm.org/ccs#

\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10003120.10003121.10003126</concept_id>
       <concept_desc>Human-centered computing~HCI theory, concepts and models</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[300]{Human-centered computing~HCI theory, concepts and models}




% \begin{CCSXML}
% <ccs2012>
%    <concept>
%        <concept_id>10003120.10003121</concept_id>
%        <concept_desc>Human-centered computing~Human computer interaction (HCI)</concept_desc>
%        <concept_significance>500</concept_significance>
%        </concept>
%  </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Human-centered computing~Human computer interaction (HCI)}


% \begin{CCSXML}
% <ccs2012>
% <concept>
% <concept_id>10003120.10003121.10003129</concept_id>
% <concept_desc>Human-centered computing~Interactive systems and tools</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% <concept>
% <concept_id>10003120.10003130.10003233</concept_id>
% <concept_desc>Human-centered computing~Collaborative and social computing systems and tools</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% </ccs2012>
% \end{CCSXML}


% \ccsdesc[500]{Human-centered computing~Interactive systems and tools}
% \ccsdesc[500]{Human-centered computing~Collaborative and social computing systems and tools}




% \begin{CCSXML}
% <ccs2012>
%    <concept>
%        <concept_id>10003120.10003121.10011748</concept_id>
%        <concept_desc>Human-centered computing~Empirical studies in HCI</concept_desc>
%        <concept_significance>500</concept_significance>
%        </concept>
%  </ccs2012>
% \end{CCSXML}
% \ccsdesc[500]{Human-centered computing~Empirical studies in HCI}






%
% Keywords. The author(s) should pick words that accurately describe
% the work being presented. Separate the keywords with commas.
\keywords{Human-AI Alignment, Human-AI Interaction
% Human-Centered AI Explanation and Evaluation, Personalized AI Systems
}


==> sections/acknowledgement.tex <==
% 
% 
We thank Eric Gilbert for his constructive feedback on human-centered insights on alignment, thank Eytan Adar for his valuable guidance on designing the interaction techniques for human-AI alignment,
and thank Elizabeth F. Churchill for her insightful discussion on this manuscript. We also thank Michael S Bernstein, Denny Zhou, Cliff Lampe, and Nicole Ellison 
for their encouraging feedback on this work.
% We also thank our readers for their engagement with this topic. 
% Acknowledging the rapid advancements in human-AI alignment research, 
We welcome researchers' constructive discussions and interdisciplinary efforts to achieve long-term and dynamic human-AI alignment collaboratively in the future.
%
This work was supported in part by the National Science Foundation under Grant No. IIS-2143529 and No. IIS-1949634.



==> sections/analysis.tex <==


% \begin{figure*}[!t]
%   \centering
%   \includegraphics[width=\textwidth]{figures/paper_distribution.pdf}
%   \caption{The number of papers for each dimension in the \emph{bidirectional human-AI alignment} framework. Out of papers that are relevant to each research question (\ie gray bars), we show the number of papers that are relevant to each dimension (\ie color bars). This figure illustrates the extent to which each dimension has been explored by existing research. We provide more analysis in Section~\ref{sec:trend}. }
%   \label{fig:paper_distribution}
%   % \vspace{-2em}
% \end{figure*}



% Given the proposed taxonomy of bidirectional human-AI alignment and the annotated paper codes, in this section, we are interested in analyzing the difference between the research in the NLP/AI fields (\ie which largely represents the state-of-the-art studies of AI technology) and the research in HCI fields (\ie which commonly represents the studies about individual and societal perception and behaviors). By gauging the difference between the two typical research fields, we aim to potentially identify what is the research ``misalignment'' between human and AI. Particularly, 
In this section, our aim is to consolidate key findings derived from our analysis of the framework and the current state of literature we reviewed.
We begin by analyzing the overall trends and gaps in the literature (Section~\ref{sec:trend}). We then focus on three essential aspects: the relationship between human values and alignment (Section~\ref{sec:gap_value}), the potential interaction modes used to specify human values (Section~\ref{sec:gap_interaction}).
% , and the gaps between AI model and human study evaluation (Section~\ref{sec:gap_assessment}).


% In this section,
% we first analyzed the \emph{overall trends and gaps} appeared in the literature (in Section~\ref{sec:trend}). Next, we delve deeper into inspecting three essential aspects: \emph{what are human values and their relationship?} (Section~\ref{sec:gap_value}), \emph{what are the interaction modes potentially to be used for specifying human values?} (Section~\ref{sec:gap_interaction}), and \emph{what are the gaps between AI model evaluation and human study assessment?} (Section~\ref{sec:gap_assessment}).
% 
% 
% 
% Furthermore, we discuss potential solutions as future work to mitigate these gaps (in Section~\ref{sec:discussion}), where we advocate for the collective efforts from interdisciplinary communities in the future to achieve a holistic loop of human-AI alignment.


% In this section, we share use cases for our design space, our reflections on the current literature and ethical implications, the challenges and limitations we encountered in creating the design space, and our plans for future work.



% aim to analyze the ``misalignment'' between the \emph{human} and \emph{AI} 

% identify the research gaps between the NLP/AI and HCI communities from three aspects: \emph{human value} (Section~\ref{sec:gap_value}), \emph{interaction modes} (Section~\ref{sec:gap_interaction}), \emph{evaluation approaches} (Section~\ref{sec:gap_assessment}). 
% 
% 
% 
% 
% 
% 
% 
% 
% 


\begin{figure*}[!t]
  \centering
  \includegraphics[width=\textwidth]{figures/paper_distribution.pdf}
  \caption{The number of papers for each dimension in the \emph{bidirectional human-AI alignment} framework. Out of papers that are relevant to each research question (\ie gray bars), we show the number of papers that are relevant to each dimension (\ie color bars). This figure illustrates the extent to which each dimension has been explored by existing research. We provide more analysis in Section~\ref{sec:trend}. }
  \label{fig:paper_distribution}
  \vspace{-10pt}
\end{figure*}







% \subsection{Overview of Trends and Gaps in the Literature}
\subsection{Meta Analysis of Trends and Gaps}
\label{sec:trend}


Based on our coding of all papers, we computed the number of relevant papers for each dimension in the proposed bi-directional framework. Based on the distribution in Figure~\ref{fig:paper_distribution}, we noticed that in existing literature certain dimensions are over- or under-represented. We outline the under-explored dimensions in two directions in the highlighted grey bars in the end of Section~\ref{sec:ai2human2} and Section~\ref{sec:human2ai4}, respectively, and provide more details below.
% 
% 




% \noindent
\textbf{Underexplored dimensions in AI-centered alignment research.}
Most literature \emph{\textbf{\rqadim{specified human values}}} using explicit human feedback, whereas implicit and simulated human feedback were largely under-explored. 
% We delve deeper into this analysis in Section~\ref{sec:gap_interaction}.
% 
In the \emph{\textbf{\rqbdim{integrating human specifications to AI}}} research question,
Besides, developing and customizing AI models during the inference stage or using the interactive approach is under-explored.
Also, human-in-the-loop evaluation is much less explored than automatic evaluation.





% \noindent
\textbf{Underexplored dimensions in Human-centered alignment research.}
Additionally, many studies on \emph{\textbf{\rqcdim{human cognitive adjustment to AI}}} focus on enabling AI sensemaking and explanations so that humans can better understand, trust, and rely on AI. 
% 
However, these studies often focused on explaining AI decision-making justification rather than educating people to acquire general skills and competencies required to understand, use, critique, and interact effectively with AI systems (i.e., AI literacy). 
AI literacy~\cite{long2020ai} plays a fundamental role in ensuring people understand and use AI correctly, and warrants deeper exploration. Also, we observed a wide range of studies~\cite{wu2022ai,gebreegziabher2023patat,park2023generative,ma2023hypocompass} which developed interactive mechanisms and prototypes to empower \emph{\textbf{\rqddim{human collaboration with AI}}}. However, most studies assumed that AI plays an assistant role, being less capable than humans. This situation might change over time. Moreover, the influence of AI advancements on human behavior, social relationships, and societal changes is essential but remains largely unexplored.




% However, these studies often focused on explaining AI decision-making justification rather than educating everyone to acquire the skills and competencies required to critically use AI technologies and applications (i.e., AI literacy).
% % However, these studies often focused on explaining AI decision-making justifications rather than educating everyone to acquire the skills and competencies required to critically use AI technologies and applications (i.e., AI literacy). 
% AI literacy plays a fundamental role to ensure that everyone understand and use AI correctly, but remains largely underexplored compared to other topics like explanation and trustworthiness. 
% % 
% % 
% Also, we observed a wide range of studies developing interactive mechanisms and prototypes to empower \textbf{\rqddim{humans to collaborate with AI}} in diverse roles. 
% However, most existing studies assumed that AI plays an assistant role, being less capable than humans. This situation might change in the long term. Moreover, the influence of AI advancements on human behavior, social relationships, and societal changes is important but remains largely unexplored. 





% Additionally, we observed a wide range of studies developing interactive mechanisms and prototypes to empower \textbf{\rqddim{humans to collaborate with AI}} of diverse roles. However, the existing studies mostly assumed that AI plays an assistant role collaboration, which is less capable than humans. This might potentially changed in the long-term perspective. Also, how AI advancements will influence human behavior, social relationship, and the societal change is also important yet much less explored.





% To identify the overview of the trends and gaps in the literature, we further conducted a quantitative analysis of the outcome of our rigorous codes. Particularly, we compute the number of relevant papers for each dimension presented in the \emph{Bidirectional Human-AI Alignment} framework. Figure~\ref{fig:paper_distribution} shows the distribution of paper numbers across 25 dimensions in the framework. The two dimensions of the ``human value category'' are not included but are further analyzed with details in Section~\ref{sec:gap_value}.
% % 
% % 
% As a consequence, we observed that certain dimensions are over- or under-represented. 



% To highlight a few notable phenomena, we observed that most of the literature \textbf{\rqadim{specify human values}} using the explicit human feedback. However, the interaction modes dominantly skew toward several formats (\eg rating and ranking and natural language interaction/conversations). We provide more in-depth analysis in Section~\ref{sec:gap_interaction}.
% There are some but much less studies leverage simulated human value feedback (\eg  human feedback simulators) for specification. The implicit human feedback is much under-explored but potentially contains informative values as well to be investigated.



% 
% % 
% %
% % 
% Many of the studies about \textbf{\rqcdim{human cognitive adjustment to AI}} focused on enabling AI sensemaking and explanations for humans to understand AI. However, these approaches largely focused on explaining AI decision-making justifications for humans, rather than educating humans to harness the skills and competencies required to use AI technologies and applications effectively (\ie AI literacy). This is  which is also important but large under-explored.
% % 
% AI literacy, which aims to educate everyone to critically understand and use AI, is important to ensure that humans will use AI in the correct ways. However, it's largely underexplored compared with other relevant topics like explanation and trustworthiness until now.


% Additionally, we observed a wide range of studies developing interactive mechanisms and prototypes to empower \textbf{\rqddim{humans to collaborate with AI}} of diverse roles. However, the existing studies mostly assumed that AI plays an assistant role collaboration, which is less capable than humans. This might potentially changed in the long-term perspective. Also, how AI advancements will influence human behavior, social relationship, and the societal change is also important yet much less explored.






% Based on our coding of all papers, we observe that certain dimensions in the \emph{bidirectional human-AI alignment} space are over- or under-represented. 
% % Figure~\ref{fig:paper_distribution} shows the number of papers per dimension coded as relevant.
% To highlight a few notable phenomena, we observe that \rqadim{\emph{\textbf{human values}}} are often unspecified in the literature, in which the existing studies usually mention general human values vaguely or focus on a specific set of typical human values, such as fairness, interpretability, harmlessness, etc. 
% % 
% This suggests future work may want to more explicitly specify what human values their study is examining. 
% % 
% % 
% The topic of \rqbdim{\emph{customizing AI values}} is another area that is under-represented compared to integrating general values into AI. While there has been extensive research on approaches to mitigate bias in AI models, there is a lack of studies focusing on other human values and how to steer models to generate more value-oriented outputs.
% % 
% % 
% In addition, we observe an increasing number of studies developing human-AI collaborative tools/systems, and generative agents that can simulate human behavior automatically. However, we also noticed that existing studies sometimes lack a in-depth analysis and investigation of \rqddim{critical thinking of the AI impacts} on Individuals and the society.
% % 
% We hope that the provision of our bidirectional human-AI alignment framework can help researchers to identify these issues and think about the approaches to resolve them. 
% To better support researchers understand the gaps, we delve into three common gaps we observed in the literature and our coding.
% % \hua{I will rewrite this section after our Figure~\ref{fig:paper_distribution}'s result is out.}
% % \hua{maybe we can split the figure into separate parts to be analyzed.}






% \subsubsection{A lack of customized alignment for diverse values}





% \subsubsection{A lack of studies examing the AI's impact on AI and society}




% Desired values for AI tools







\begin{figure*}[!t]
  \centering
  \includegraphics[width=\textwidth]{figures/interaction_mode.pdf}
  \caption{The interaction techniques for specifying values in human-AI alignment. We compare the common interaction techniques used for the model ``Learning'' and ``Inference'' stages in human-focused (\eg HCI) and AI-focused (\eg NLP/ML) research studies. 
% %     % 
% 
% % 
%     Discarded Options[NLP]: \cite{lu2022towards}
%   Language Analysis[NLP]: \cite{park2020scalable}  
%   Social Relationship[NLP]: \cite{isajanyan2024social}  
%   Rating[NLP]: \cite{ouyang2022training}  
%   Ranking[NLP]: \cite{yuan2024rrhf}
%   Features - Beyond Imitation[NLP]: \cite{guo2023beyond}  , HCI = \cite{feng2019can},
%   Principles[NLP]: \cite{bai2022constitutional} , [HCI]:\cite{petridis2024constitutionmaker},
%   Text Edit[NLP]: \cite{yao2023improving}, [NLP Inference]: \cite{lin2023unlocking}, [HCI]: \cite{hong2022scholastic} 
%   Conversations \cite{hwang2023aligning}, HCI=\cite{shen2023convxai}, NLP Inference: \cite{zhang2021human}
%   Multimodal [HCI]: HINT \cite{chen2022hint}, [NLP Inference]:\cite{geva2022lm}
%   Talebrush \cite{chung2022talebrush} HCI, 
%   AI Chain \cite{wu2022ai} HCI
%   Pearl \cite{jorke2023pearl} HCI,
%   % 
  % 
% \hua{read this article suggested from Eytan~\cite{brath2021surveying} \url{https://richardbrath.wordpress.com/2021/10/31/58-ways-to-visualize-alice-in-wonderland/} to improve this section.}
  }
  \label{fig:interaction}
  \vspace{-1em}
\end{figure*}
% 
% % 
% 
% 
% 
% 
\begin{table*}[!t]
\centering
% \vspace{-10pt}
\begin{tabular}[t]{@{}  !{\color[HTML]{808080}\vrule width 2pt} p{.98\textwidth} !{\color[HTML]{808080}\vrule width 2pt} @{}}
\cellcolor[HTML]{E6E6E6} 
\textbf{Takeaways of Interaction Techniques for Alignment.}
% \newline
\vspace{5pt}

1. Some common human feedback formats (rating, ranking) used in NLP/ML are not often studied in HCI.
\vspace{5pt}

2. Diverse human interactive feedbacks in HCI are not fully used in AI development in NLP/ML fields.
\end{tabular}
\end{table*}
% 



\subsection{Insights into Human Values for Alignment}
\label{sec:gap_value}


% While many papers claim to integrate or evaluate AI in relation to human values, the specific sets of human values they examine often lack clarity or comprehensiveness. 
% In order to articulate and systematically understand human values relevant to bidirectional human-AI alignment, we structured these values using a combination of top-down and bottom-up methods based on a theory of cross-cultural psychology (Section~\ref{sec:value_method}). As a result, we identified the structural relationships among human values (see Figure~\ref{fig:value_structure}) and mapped existing literature to a fine-grained taxonomy (see Figure~\ref{fig:value_taxonomy}) in Section~\ref{sec:value_outcome}. Additionally, we present our analysis findings of human values that are particularly relevant for future studies (Section~\ref{sec:value_finding}).



% While many papers claimed to integrate or evaluate AI with respect to human values, the sets of human values they studied often needed to be clarified or completed.
% To articulate and systematically understand human values related to bidirectional human-AI alignment, we structured the relevant values using a top-down and bottom-up method grounded on a theory of cross-cultural psychology (Section~\ref{sec:value_method}). As a result, we identified the structural relationship among human values (Figure~\ref{fig:value_structure}) and mapped the existing literature to the fine-grained taxonomy (Figure~\ref{fig:value_taxonomy}) in the Section~\ref{sec:value_outcome}.
% Moreover, w
% We present the findings of human values for alignment, collected during the process of adjusting the ``Schwartz Theory of Basic Values'' and conducting literature review, that are worth noting to the future studies.
% 
% 
% 
% We present the key findings for future research which are identified during our adjustment of the ``Schwartz Theory of Basic Values'' and literature review.


Our analysis, based on the adaptation of Schwartz's Theory of Basic Values and our comprehensive literature review, identifies three critical findings for future research:


\textbf{Value Prioritization in AI Systems.} Human value systems are not merely subsets of values, but ordered systems with relative priorities~\cite{schwartz1994there,schwartz2012overview}. For instance, \citet{schwartz2012overview} presented the definition for this phenomenon: \emph{\say{a value is ordered by importance relative to other values to form a system of value priorities.
The relative importance of multiple values guides action....The trade-off among relevant, competing values guides attitudes and behaviors.}}.
% 
Current AI alignment algorithms, often based on datasets of human preferences~\cite{ouyang2022training,song2024preference,rafailov2024direct}, may inadvertently prioritize majority values, potentially neglecting those of marginalized groups~\cite{fleisig2023fairprism}. Future research should address this complex interplay of values in AI systems.





\textbf{Universal vs. Personalized AI Values}. While certain values are universally expected from AI (e.g., capability, equity, responsibility), others may be undesirable in specific contexts~\cite{ngo2022alignment} (e.g., seeking power). Simultaneously, AI models should be adaptable to diverse human value systems~\cite{sorensen2024roadmap}. Research is needed to develop methods for identifying appropriate value sets for specific individuals or groups, and for customizing AI to align with user values while maintaining ethical principles.




\textbf{Disparities in Value Expectations and Evaluation}. The fundamental differences between humans and AI necessitate distinct approaches to value evaluation. For instance, assessing AI honesty may require mechanistic interpretability~\cite{bereska2024mechanistic}, a more rigorous standard than that applied to humans. Future studies should explore methods for evaluating and explaining AI values and calibrating human expectations accordingly.








% \subsubsection{\textbf{The Relative Priority of Values is as Crucial as Their Existence}}
% \label{sec:value_finding}


% Based on the definition from \citet{schwartz1994there}, we noted that a human value system is not an exclusive subset of values, but rather, an ordered system.
% % 
% \citet{schwartz2012overview} presented the definition for this phenomenon: \emph{\say{a value is ordered by importance relative to other values to form a system of value priorities.
% The relative importance of multiple values guides action....The trade-off among relevant, competing values guides attitudes and behaviors.}}
% % 
% % % 
% % \begin{quote}
% %     \say{a value is ordered by importance relative to other values to form a system of value priorities.
% %     The relative importance of multiple values guides action....The tradeoff among relevant, competing values guides attitudes and behaviors}~\cite{schwartz2012overview}.
% %     % \textit{The key to identifying the structure of value relations is the assumption that actions taken in the pursuit of each type of values have psychological, practical, and social consequences that may conflict or may be compatible with the pursuit of other value types.}~\cite{schwartz1994there}
% % \end{quote}
% % 
% % 
% % We first highlight from feature (5) and (6) that a human value system is not an exclusive subset of values, but rather, an ordered system.
% % 
% % \begin{quote}
% %     {
% %     , and (5) is ordered by importance relative to other values to form a system of value priorities.
% %     (6) The relative importance of multiple values guides action. Any attitude or behavior typically has implications for more than one value...The tradeoff among relevant, competing values guides attitudes and behaviors}~\cite{schwartz2012overview}.
% %     \textit{The key to identifying the structure of value relations is the assumption that actions taken in the pursuit of each type of values have psychological, practical, and social consequences that may conflict or may be compatible with the pursuit of other value types.}~\cite{schwartz1994there}
% % \end{quote}
% % 
% For instance, the pursuit of achievement values can possibly clash with benevolence values. 
% % In human contexts, striving for personal success often hinders efforts to improve the welfare of others who require assistance. 
% Similarly, 
% previous studies have highlighted the trade-offs between AI's state-of-the-art capabilities and their ethical performance, such as interpretability and fairness~\cite{shen2022improving}.
% % in AI, focusing on achieving state-of-the-art performance may impede efforts for accountability.
% % 
% While most alignment algorithms utilize datasets of human ratings and preferences collected in the wild~\cite{ouyang2022training,song2024preference,rafailov2024direct}, AI models may inadvertently align with the value priorities of the majority represented in these datasets, potentially overlooking or sacrificing the value systems of marginalized groups~\cite{fleisig2023fairprism}.







% \subsubsection{Value Distribution in Literature}
% \mbox{}



% \subsubsection{Generalizability of Value Alignment: Relationship between Aligning Values and Other Factors}
% \mbox{}

% We investigation primarily focuses on value alignment, whereas there are also diverse factors that we might want to consider for ``alignment'' beyond ``values'', such as norms and cultures. 




% % \textbf{Value Systems are Priority over Values, Not Subsets}

% \subsubsection{Value Systems are Priority over Values, Not Subsets}
% \mbox{}


% We first highlight from feature (5) and (6) that a human value system is not an exclusive subset of values, but rather, an ordered system.

% \begin{quote}
%     \textit{The key to identifying the structure of value relations is the assumption that actions taken in the pursuit of each type of values have psychological, practical, and social consequences that may conflict or may be compatible with the pursuit of other value types.}~\cite{schwartz1994there}
% \end{quote}

% For instance, the pursuit of achievement values can clash with benevolence values. 
% In human contexts, striving for personal success often hinders efforts to improve the welfare of others who require assistance. 
% Similarly, in AI, focusing on achieving state-of-the-art performance may impede efforts to bolster accountability.

% While most alignment algorithms utilize datasets of human ratings and preferences collected in the wild~\cite{ouyang2022training,song2024preference,rafailov2024direct}, AI models may inadvertently align with the value priorities of the majority represented in these datasets, potentially overlooking or sacrificing the value systems of marginalized groups~\cite{fleisig2023fairprism}.






% % % \textbf{Human-desired AI Values and Customization to Personal Values}
% \subsubsection{\textbf{Human-desired AI Values and Customization to Personal Values}}


% While further research in AI ethics is crucial in this nuanced area, there are values that, in general, humans expect AI to prioritize (e.g., capability, equity, responsibility) and values that humans do not want AI to integrate in specific scenarios (e.g., seeking power to avoid or harm people~\cite{ngo2022alignment}).
% On the other hand, 
% AI models are expected to
% % we hope that AI models can 
% be tailored to 
% accommodate diverse human value systems~\cite{sorensen2024roadmap}, which necessitates a comprehensive understanding of all types of values.
% Therefore, future research could potentially explore the directions of: (1) developing methods to identify the appropriate sets of human values to align with specific individuals or groups, 
% % a universal guideline for values desired in AI by humans, 
% and (2) understanding and customizing AI to align with users' values while maintaining its inherent ethical principles.





% % % \textbf{Expectations and Evaluations of Values Can be Different in Humans and AIs}
% \subsubsection{\textbf{Expectations and Evaluations of Values May Differ Between Humans and AI Systems}}



% Due to the fundamental differences between humans and AI models, the expectations for evaluating certain values can vary between the two. For instance, while human honesty can hardly be assessed except observable actions, for AI models the expectations might be higher. 
% It could involve reverse-engineering the computational mechanisms and representations learned by neural networks into concepts understandable to humans. 
% This approach, known as \textit{mechanistic interpretability}, provides a in-depth understanding of how AI models operate~\cite{bereska2024mechanistic}.
% Future research is needed to explore evaluating AI values and calibrating human expectations of these values.









% % \subsubsection{Results and Findings from the Paper Coding.}
% % \mbox{}


% % % Based on the aforementioned process, we achieved our detailed human value taxonomy as described in Fig~\ref{fig:schwartz}. 
% % % \hua{TODO: add a figure/table of human values here.}



% % \begin{itemize}

% %     \item \hua{use data / citations to support below findings. add more interesting findings}
    
% %     \item current methods (e.g., RLHF) generally finetune the AI models using aggregated data without a clear scrutinization on \emph{what exact values the dataset is conveying}. This could potentially result in undesirable values being integrated into AI.

% %     \item Many papers predominantly relied on the concept of "general human preference" to represent "values" without clearly specifying the exact human values they are investigating.
% %     \item Within the NLP/AI domain, values embedded into AI models during the learning stage (e.g., harmlessness, helpfulness, honesty, etc.) often do not overlap with the values being evaluated.
% %     \item A comparison of NLP and HCI papers reveals that NLP covers a broader range of values, while HCI primarily focuses on a narrower range, including transparency, fairness, accountability, and equity.
% % \end{itemize}














\subsection{Interaction Techniques for Specifying Human Values: A Cross-Domain Analysis}
\label{sec:gap_interaction}


Our research reveals disparities in interaction techniques for human-AI value alignment across AI-centered (NLP/ML) and human-centered (HCI) domains. As depicted in Figure~\ref{fig:interaction}, this analysis focuses on three key areas:


\textbf{Domain-Specific Interaction Techniques}. The interaction techniques in AI-centered (NLP/ML) and Human-centered (HCI) alignment studies are often differ~\cite{brath2021surveying}.
NLP/ML studies primarily utilize numeric and natural language-based techniques. Also, NLP/ML research explore implicit feedback to extract human hidden feedback. In contrast, HCI research encompasses a broader range of graphical and multi-modal interaction signals (e.g., sketches, location information) beyond text and images. This disparity suggests potential gaps in extracting comprehensive human behavioral information.


\textbf{Stage-Specific Interaction Techniques}. In NLP/ML, the learning stage predominantly employs rating and ranking interactions for alignment in dataset generation. However, when humans use AI in the inference stage, as demonstrated in HCI research, involves more diverse user interactions. This discrepancy highlights the need for alignment between model development and practical deployment.


\textbf{Divergent Data Utilization}. NLP/ML typically uses interaction outputs as training datasets, while HCI analyzes this data to understand human behavior and feedback. As AI systems evolve, developing new interaction modes to capture a broader spectrum of human expression becomes crucial.






% Selecting suitable interaction techniques for humans to specify AI values for alignment is crucial. Each research domain offers distinct strengths and insights to address this challenge. From the bidirectional perspective, we investigate the status quo of existing interaction techniques for alignment specification in both human-centered (\eg HCI) and AI-centered (\eg NLP/ML) studies. 
% Additionally, we provide a detailed analysis of how these techniques have been utilized in the learning and inference stages, as shown in Figure~\ref{fig:interaction}.







% We show the main interaction mode for human-AI alignment and the most common interaction formats leverage in NLP/AI and HCI fields during the learning and the inference stages in Figure~\ref{fig:interaction}.
% 
% We observe several difference between the two fields introduced below.
% In examining the interaction modes between Natural Language Processing (NLP) and Human-Computer Interaction (HCI) fields, several gaps emerge. 
% Interaction and the resulted data are imperative to human-AI alignment. 
% 




% \subsubsection{\textbf{Interaction Techniques Across Various Domains}}
% As shown in Figure~\ref{fig:interaction}, the coverage of interaction techniques in AI-centered (\ie {\color[HTML]{1C5CCC} \colorbox{bg-blue}{NLP/ML Research}}) and human-centered (\ie {\color[HTML]{A61C00} \colorbox{bg-red}{HCI Research}}) studies often differ~\cite{brath2021surveying}. Particularly, we see that NLP/ML studies primarily leverage \emph{numeric-based}, \emph{natural language-based} interaction techniques for human-AI interaction and alignment. In addition, NLP/ML researchers also leverage implicit feedback to improve the model. 
% For example, some systems took in implicit signals such as contextual information, or discarded options to develop AI systems.
% % This is understandable since human labeled data is usually expensive, therefore, NLP/ML researchers tend to use implicit feedback to extract more human behavioral information to improve AI models.
% In comparison, HCI studies cover more diverse graphical multi-modal interaction signals (\eg sketches, location information) beyond text and images, which can be largely attributed to the proficient graphical user interface development skills found in HCI researchers and practitioners. 
% This potentially indicates gaps in the human behavioral information that the two fields can extract from the users of the AI models. 
% % Systems also leverage natural language interaction, such as breaking AI output into digestible chunks for multi-turn dialogues with the users. 










% \subsubsection{\textbf{Different Interaction Techniques in Separate Stages}}
% % \subsubsection{Interaction Formats}
% Another finding we discerned is the different interaction techniques used in separate stages, especially in the NLP/ML fields. 
% Specifically, the learning stage relies mostly on \emph{rating} and \emph{ranking} interaction to deal with the generated datasets of the models. However, users leverage the AI model in different ways during inference stage, as demonstrated in HCI research.
% This indicates that users might elicit different needs in practice when interacting with AI during the model deployment stage.
% % in different ways. 
% Therefore, future NLP/ML and HCI researchers might collaborate to keep the human-AI interaction techniques informed (or even consistent) by both domains in order to facilitate close alignment between humans and AI.
% % want to keep in mind how they want users to use the developed system to make the AI and human more aligned.

% % NLP studies leverage human annotated data in learning stage to train the model. Therefore, we consider it as an indirect interaction between human and AI. 




% \subsubsection{\textbf{Dissimilar Usage of Interaction Data Between Domains}}
% We noticed that the ways in which the two domains utilize data differ. For example, the interaction outputs of NLP research are commonly the dataset to be trained in the model, whereas HCI researchers use usage data to analyze human behavior and feedback. 
% % 
% % 
% % 
% % 
% % 
% As AI systems continue to advance, new modes of interaction are required to capture more space of human expression, with the goal of deeper and meaningful alignment. This is an important area for NLP/ML researchers to partner with HCI researchers for designing interaction paradigms, including but certainly not limited to affective computing, accessibility, social computing, computer-supported cooperated work, and ubiquitous computing. 










% As AI systems continue to advance, new and novel modes of interaction are required to capture more space of human expression for deeper and more meaningful alignment. This is an important area for AI researchers to partner with HCI sub-fields for designing interaction paradigms, including but certainly not limited affecting computing, accessibility, social computing, computer-supported cooperated work, and ubiquitous computing. 









% \subsection{
% % Gaps of AI Model Evaluation in and Human Study Assessment
% % 
% Gaps Between AI-Centered and Human-Centered Evaluations
% }
% % \subsection{Evaluating AI Systems and Human Study Evaluation}
% \label{sec:gap_assessment}







% Our analysis reveals significant disparities in evaluation approaches between NLP/ML and HCI domains, highlighting three key areas for improvement:


% \textbf{Divergent Evaluation Objectives}. NLP/ML evaluations primarily focus on algorithmic performance, while HCI studies emphasize user experience and interactions. Future research should integrate these perspectives, developing human-centered evaluation benchmarks for AI systems based on HCI insights.


% \textbf{Contrasting Utilization of User Information}. NLP/ML research predominantly employs quantifiable measures (e.g., accuracy, precision), whereas HCI gathers both quantitative and qualitative data on user experiences. Future work should explore methods to convert qualitative human feedback into quantifiable data for AI system improvement and alignment.


% \textbf{Disparate Evaluation Approaches and Scales}. NLP/ML typically uses automated or human-in-the-loop evaluations on extensive datasets, while HCI employs in-depth qualitative and quantitative measurements on defined human groups. Adopting consistent evaluation strategies across domains could lead to a more comprehensive understanding of human-AI interaction and alignment.








% Improving bidirectional alignment between humans and AI can potentially be further enhanced by collaborative efforts and commitments from both the NLP/ML and AI domains, ensuring consistency in evaluation methods and metrics.
% % 
% % Facilitating bidirectional human-AI alignment can also be benefited from 
% % Closing the gap between NLP/AI and HCI domains necessitates 
% % synergistic efforts and commitments, from both NLP/ML and AI domains, to maintaining consistency in evaluation approaches and metrics.
% % 
% Nevertheless, we observed notable gaps by comparing the literature analysis regarding ``evaluating AI systems'' (\ie Section~\ref{sec:evaluation}) and ``evaluation in human studies'' (\ie Section~\ref{sec:assessment}).



% \subsubsection{\textbf{Different Objectives and Expectations of Evaluations in Humans and AI}}
% Evaluating AI systems primarily focuses on \emph{what} algorithmic performance is, aiming to determine how well proposed methods perform compared with benchmark or human-in-the-loop evaluation. Conversely, human study evaluations are more concerned with \emph{why} -- understanding the user experience and interactions, often prioritizing both quantitative and qualitative measurements to gain a comprehensive understanding of user experience and interactions with AI systems.
% Given the distinct objectives in evaluation, future research has the potential to collaborate in bridging these gaps. For instance, informed by the user experience and demands revealed by HCI studies, NLP/ML researchers can incorporate the insights and design human-centered evaluation benchmarks to assess AI systems.
% % 
% % % \hua{add examples + value-context measurement.}
% % 
% % \subsubsection{Expectations and Evaluations of Values Can be Different in Humans and AIs}
% % \mbox{}
% % Due to the fundamental differences between humans and AI models, the expectations for evaluating certain values can vary between the two. 
% % For instance, while human honesty can hardly be assessed except observable actions, for AI models the expectations might be higher. 
% % It could involve reverse-engineering the computational mechanisms and representations learned by neural networks into concepts understandable to humans. 
% % This approach, known as \textit{mechanistic interpretability}, provides a in-depth understanding of how AI models operate~\cite{bereska2024mechanistic}.
% % Future research should focus on evaluating AI values and calibrating human expectations of these values.


% % \vspace{-10pt}

% \subsubsection{\textbf{Contrasting Ways of Utilizing User Information}}
% % 
% Given the diverse objectives of assessment described above, NLP/ML research primarily focuses on quantifiable measures such as accuracy, precision, and recall. The information received in evaluating AI systems is often accurately measurable, e.g., ratings, rankings, and multiple choice questions.
% % 
% % In NLP research, evaluations primarily aim to determine the performance of algorithmic methods, 
% % focusing on quantifiable measures such as accuracy, precision, and recall. 
% In comparison, by focusing on understanding the user experience and interaction with AI systems, HCI research often involves gathering both quantitative and qualitative data, such as user feedback, perceptions, and behaviors. 
% The collected information from HCI research might cover a wider spectrum of qualitative data related to human values, experience, and needs in practice than what can be captured by quantitative metrics alone. However, 
% incorporating qualitative findings into improving AI systems can be difficult. 
% % some qualitative findings are challenging to be leveraged in enhancing AI systems.
% Therefore, future researchers can investigate methods to convert qualitative human feedback into quantitative data that AI systems can effectively utilize and align with.
% % 
% % NLP feedback can actually be used to directly improve the model, but it's not clear how to actually incorporate feedback from HCI systems
% % Therefore, the data formats are more diverse in HCI, and sometimes could not be quantitatively described. 
% % 
% % \hua{add example+ value-context measurement.}.







% \subsubsection{\textbf{Evaluation Approaches and Scale}}
% % 
% Prior studies in NLP/ML have predominantly relied on 
% automated or human-in-the-loop evaluation methods to assess AI system performance across extensive datasets.
% In comparison, 
% HCI studies 
% % prioritize a more comprehensive approach, utilizing 
% typically employ qualitative and/or quantitative measurements to gain deeper insights into user experiences and interactions within defined human groups.
% % 
% % 
% % 
% % 
% % 
% These divergent aspects highlight diverse gaps between the evaluation methods and scales utilized in the two domains. 
% % While NLP tends to focus on automated evaluation techniques, HCI places greater emphasis on both quantitative and qualitative measurements to assess human-AI interaction and alignment. 
% Closing this gap and adopting consistent evaluation strategies could lead to a more holistic understanding and synergy of human-AI interaction and alignment across both fields. 
% % We discuss potential ways to mitigate these gaps in Section~\ref{sec:discussion}.
% % 
% % 
% % 
% % 



% Overall, it's important to note that the disparities between HCI and NLP/ML studies extend beyond the above aspects, \eg research methods and problem formation. 
% Our analyses aim to pave the way for future interdisciplinary research collaboration, fostering bidirectional alignment between humans and AI across diverse domains.


% % Overall, it worth noting that the gaps between HCI and NLP/AI domain studies are far more beyond the aforementioned aspects, such as regarding the key research methodology and problems.
% % For example, regarding methodology, NLP/AI primarily focus on developing novel learning algorithms to incorporate human values into AI models (\eg RLHF, DPO, etc.). In comparison, HCI studies predominantly emphasize on approaches of empowering human-AI interaction or assessing AI impacts on individuals and groups, and others.
% % 
% % % 
% % These analyses aim to pave the way for future research across various domains to synergize collaboratively for achieving the bidirectional human-AI alignment.

% % As methodologies are evolving rapidly, we decided to explore the above gaps which might exist in a long history and benefitial/generalized to more research questions beyond human-AI alignment (\eg evaluation approaches, interaction techniques).













% \subsubsection{Keep Consistent between Model Evaluation and Human Assessment}
% By referring to Section~\ref{sec:evaluation} and Section~\ref{sec:assessment}, NLP researchers can better discern the misalignment between model evaluation and human assessment in terms of objects, priorities and extracted information. As the results, NLP researchers can potentially develop better evaluation methods that align with human demands in practice, which can in return boost the AI model alignment better with human. 


% ================================================================




% ========================== dead kitten ==============

% In this section, we conduct qualitative and quantitative analysis on the reviewed papers. We aim to identify the difference between NLP/AI fields and HCI fields, with specific focus on \emph{human values}, \emph{evaluation}, and \emph{interactive value presentation methods}.
% 
% 
% \savvas{misalignment in HCI + NLP}



% In this section, we focus on extracting the papers' data to quantitatively/qualitatively analyze the findings.
% 
% 1. To what extent are human values well-aligned with developed AI?
% 
% 2. are interaction paradigms fully leveraged in human-AI alignment techniques?
% 
% 3. situated values and customized AI alignment?
% 
% 4. what are under-explored research dimensions? heatmaps


% \subsection{what hasn't been explored? AI for jounalism -> what hasn't been done? What Can we say for the future research in NLP/HCI from this paper?}










% === To what extent are human values well-aligned with developed AI?
% 
% 
% We could analyze the ``misalignment'' from two aspects:
% 
% 1. the alignment values in training is NOT the values being evaluated (within NLP).
% 2. the values studieds in HCI field is not fully aligned with NLP field.
% 
% \hua{not make the papers convoluted.}








% \subsection{Situated values and customized AI alignment?}



% general v.s. situated alignment?






% \hua{paper analysis heatmap}






% Our analysis reviews the ambiguity and gaps in how the NLP/AI and HCI communities prioritize and conceptualize human values in bidirectional human-AI alignment research. 
% % 
% Particularly, on one hand, while numerous papers claimed to examine the LLMs with respect to human values, the range of values are unclear. 
% On the other hand, we observed a different emphasis on the human values when comparing papers published in NLP/AI venues and HCI venues. 
% % 
% 
% To provide a clear picture of \emph{what} and \emph{how} human values have been investigated in these domains, we next take a deeper look at the detailed method of \emph{how we come up with the human value taxonomy} described Section~\ref{sec:value_category}, and \emph{what are our findings} based on the final coding of all papers.






% \subsection{Are interaction paradigms fully leveraged in human-AI alignment techniques?}

% interactions in HCI v.s. NLP?

% \hua{add the interaction formats comparison}








% The difference in assessment methods between NLP and HCI reflects the differing priorities and objectives of the two fields. While NLP tends to prioritize automated evaluation methods to assess AI performance, HCI places greater emphasis on both quantitative and qualitative measurements to understand user experiences and interactions with AI systems more comprehensively.
% 
% Most of the evaluations in NLP studies aim to answer \emph{what is the performance of the proposed algorithmic method}, in contrast, HCI studies are more often interested in \emph{why} -- to understand user experience and interactions.
% While most NLP studies conduct automated or human-in-the-loop evaluation methods to assess AI performance, HCI studies place greater emphasis on both quantitative and qualitative measurements to understand user experiences and interactions with AI systems more comprehensively.








% we 
% these social psychology studies, we start with a \textit{top-down} framework by using the taxonomy of the Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012refining,schwartz2012overview}, which is a widely accepted theory of basic human values with cross-cultural psychology and universal values~\cite{kang2023values,kiesel2022identifying}.




% In order to articulate and systematically understand human
% values relevant to bidirectional human-AI alignment, we structured these values using a combination of top-down
% and bottom-up methods based on a theory of cross-cultural psychology


% While the research papers often mention human value alignment as a key objective, either explicitly or implicitly, the majority do not offer a clear definition of "human value." This term appears vague and inconsistent across the literature, highlighting the need for a more precise definition. 
% Building upon \citet{rokeach1973nature}'s cross-cultural value survey, Schwartz summarized some widely agreed-upon features of human values:

% \begin{quote}
%     \textit{A value is a (1) belief (2) pertaining to desirable end states or modes of conduct, that (3) transcends specific situations, (4) guides selection or evaluation of behavior, people, and events, and (5) is ordered by importance relative to other values to form a system of value priorities}~\cite{schwartz1994there}.
% \end{quote}

% \begin{quote}
%     \textit{(6) The relative importance of multiple values guides action. Any attitude or behavior typically has implications for more than one value...The tradeoff among relevant, competing values guides attitudes and behaviors}~\cite{schwartz2012overview}.
% \end{quote}

% These features help distinguish values from related concepts such as needs and attitudes. 
% For example, a preference for blue ties would not qualify as a value~\cite{schwartz1994there}.
% Motivated by these social psychology studies, we start with a \textit{top-down} framework by using the taxonomy of the Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012refining,schwartz2012overview}, which is a widely accepted theory of basic human values with cross-cultural psychology and universal values~\cite{kang2023values,kiesel2022identifying}.

% The theory of basic human values is a theory of cross-cultural psychology and universal values that was developed by Shalom H. Schwartz. The theory extends previous cross-cultural communication frameworks such as Hofstede's cultural dimensions theory.







% NLP: primarily numeric and natural language interactions; Also, NLP tends to leverage implicit feedback to extract more data from human.

% HCI: more diverse interaction formats, covering graphical multi-modal interaction;







% In the offline world, humans communicate meaning with figures of speech, minute facial expressions, rapid hand-gestures, emphatic body language, reflective gaze, and much more. However, AI systems scarcely consider these diverse interaction modes. Early AI systems ask humans to evaluate outputs via rating with numbers. While numeric inputs are simple to implement from the \textit{machines'} perspective, they are scantly appropriate for encoding complex and nuanced human preferences. 

% LLM systems have opened a new door for new use cases and generated content. Along with these newfound capabilities, researchers have contributed a variety of ways for people to interact with these systems. Our review showed that many systems allowed users to interact in many different ways. Notably, works in HCI fields spearhead creative and multi-modal interactions between humans and AI systems. As mentioned, many earlier AI systems asked users to perform numeric inputs such rating and ranking AI responses. 


% Another set of systems took in implicit signals such as location, other applications in use, and discarded options. Systems also leverage natural language interaction, such as breaking AI output into digestible chunks for multi-turn dialogues with the users. Finally, people may also interact with AI models via graphical multi-modal methods. Works in this area include using a free-handed sketches~\cite{chung2022talebrush} or placing LLM agents in a contextual environment~\cite{park2023generative}. 

















% % 
% To provide a clearer understanding of the investigation of human values in these domains, we delve deeper into our methodology for developing the human value taxonomy in our proposed framework (as described in Section~\ref{sec:value_category}), and present our findings based on the final coding of all papers.


% \hua{
% % justify: 
% 1. why we focus on values? 
% % 2. why we use Schwartz Theory of Basic Values. 
% 3. what's the relationship of this typology with existing studies and how can future study use it?}
% Studies based on Schwartz Theory of Basic Values: \cite{kang2023values,kiesel2022identifying}





% While many papers claimed to integrate and/or evaluate AI with respect to human values, it is often the case that the sets of human values in the studies remained ambiguous or incomplete. 

% Our analysis of the final paper codes highlights the ambiguity and gaps in how the NLP/AI and HCI communities prioritize and conceptualize human values in \emph{bidirectional human-AI alignment} research. Specifically, w
% While many papers claim to examine LLMs in relation to human values, the specific set of values investigated often remains unclear. 
% Additionally, we observed differing emphases on human values when comparing papers published in NLP/AI venues with those in HCI venues.

% \begin{figure*}[!t]
%   \centering
%   \includegraphics[width=1\textwidth]{figures/values.pdf}
%   \caption{A fine-grained taxonomy of values related to bidirectional human-AI alignment. The taxonomy is based on Schwartz's Theory of Basic Values and an empirical collection of values that are commonly been studied.
%   % figure of our human value taxonomy based on Schwartz's Theory of Basic Values.\hua{adding explanation on meaning of red v.s. gray, add dashed lines of what values have been and have not been used in HCI + NLP?}
%   }
%   \label{fig:schwartz}
%   % \vspace{-2em}
% \end{figure*}




% \begin{figure*}[!t]
%   \centering
%   \includegraphics[width=1\textwidth]{figures/value_structure.pdf}
%   \caption{The relations of human values for AI development
%   % The structure of the dynamic relations among values 
%   (adapted from~\citet{schwartz2012overview}). 
%   We consider 5 \emph{high-order value types} (\ie self-enhancement and openness to change), which encompass 12 \emph{motivational value types} (\eg power, universalism, functionality). We further organize the relation among these value types along two dimensions: 1) different sources (\ie individuals, society and interaction) and 2) different self intentions (\ie self-protection against threat and self-expansion and growth). The \emph{Desired values for AI tools} was added empirically from \emph{bottom-up} our paper survey whereas others are inherited from~\citet{schwartz2012overview}. 
%     % 
%   % The typology is based on Schwartz Theory of Basic Values and an empirical collection of values that are commonly been studied.
%   % Some values conflict with one another (\eg Benevolence and Power) whereas others are compatible (\eg Conformity and Security). This structure of values refers to these relations of conflict and congruence among values~\cite{schwartz1994there,schwartz2012overview}.
%   % 
%   % A fine-grained taxonomy of values related to bidirectional human-AI alignment. The taxonomy is based on Schwartz's Theory of Basic Values and an empirical collection of values that are commonly been studied.
%   }
%   \label{fig:value_structure}
%   % \vspace{-2em}
% \end{figure*}





% \begin{figure*}[!t]
%   \centering
%   \includegraphics[width=1\textwidth]{figures/value_content.pdf}
%   \caption{A fine-grained taxonomy of human values. 
%   % The typology is based on Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012overview} and an empirical collection of values that are commonly been studied.
%   The exemplary values with red dot (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) indicates there are no work in our surveyed papers examining the specific values. 
%   Note that humans might not expect AI to encode all these values (\eg social power), which could potentially result in harm and risks. 
%   % The values with red dot (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) and \textcolor{hua-red}{red color} means that humans might not expect AI to embed these values in AI, which could potentially result in harm and risks.
%   % 
%   % 
%   % % 
%   % % 
%   % % 
%   % choose own goal\cite{lima2020collecting}
%   % creativity\cite{ashktorab2020human}
%   % curiosity\cite{jiang2023evaluating}
%   % freedom\cite{lima2020collecting}
%   % independence\cite{kang2023values}
%   % privacy\cite{10.1145/3544548.3580903}
%   % reflectiveness\cite{yan2023complex}
%   % factuality\cite{hosking2023human}
%   % self-respect\cite{wu2023cross}
%   % diversity\cite{kapania2023hunt}
%   % capability\cite{xu2023lemur}
%   % influence\cite{huang2023humanity}
%   % intelligence\cite{park2023generative}
%   % success\cite{kang2023values}
%   % resilience\cite{ye2023flask}
%   % authority\cite{lima2021human}
%   % wealth\cite{santurkar2023whose}
%   % reciprocation of favours\cite{zagalsky2021design}
%   % moderation\cite{lai2022human}
%   % devout\cite{santy2023nlpositionality}
%   % politeness\cite{zhu2023unmasking}
%   % self-discipline\cite{zhou2023realbehavior}
%   % forgiving\cite{wu2023cross}
%   % helpfulness\cite{jin2022make}
%   % honesty\cite{he2023hi}
%   % emotional\cite{huang2023humanity}
%   % responsiblity\cite{ma2023towards}
%   % true friendship\cite{isajanyan2024social}
%   % cooperation\cite{he2023interaction}
%   % collectivism\cite{nie2024moca}
%   % democracy\cite{santurkar2023whose}
%   % inclusive\cite{ramezani2023knowledge}
%   % equality\cite{sheng2021societal}
%   % equity\cite{goldfarb2023prompt}
%   % accessibility\cite{zhang2023visar}
%   % adaptability\cite{oh2023pk}
%   % economic\cite{bakker2022fine}
%   % transparency\cite{boyd2021datasheets}
%   % autonomy\cite{wang2023humanoid}
%   % awareness\cite{paleja2021utility}
%   % % 
%   % 
%   }
%   \label{fig:value_taxonomy}
%   % \vspace{-2em}
% \end{figure*}




% \subsubsection{The Process of Categorizing Aligned Human Values.}
% \label{sec:value_category_discuss}
% \mbox{}

% \martin{Please let me know if we need to discuss our consolidated synonyms in this section too, or we will make another figure in the appendix?}



% % \textbf{Defining Human Values: Top-Down and Bottom-Up}
% % \subsubsection{Structuring Human Values: Leveraging a Top-Down and Bottom-Up Method}
% \subsubsection{\textbf{Methodology: A Combination of Top-Down and Bottom-Up Way to Structure Human Values}}
% \label{sec:value_method}
% % \mbox{}
% To recognize human values systematically, we grounded our exploration on the Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012overview}, which is a theory of cross-cultural psychology built upon the \citet{rokeach1973nature}'s value survey. 
% We chose the Schwartz Theory of Basic Values primarily considering that its definitions and dimensions are universal and are applicable for, or almost for, all people across \emph{(a)} various cultures and countries; \emph{(b)} various sources including individuals, interactions and groups; and \emph{(c)} commonly accepted in previous NLP studies~\cite{kang2023values,kiesel2022identifying}.
% % 
% % 
% \citet{schwartz1994there} provided a clarified definition of human values by summarizing some widely agreed-upon features as:
% % 
% % \begin{quote}
%     \emph{\say{A value is a (1) belief (2) pertaining to desirable end states or modes of conduct, that (3) transcends specific situations, (4) guides selection or evaluation of behavior, people, and events.}}
% % \end{quote}
% % 
% Built upon these clarified definitions, we start to use a \emph{top-down} method to adopt the well-defined \emph{value taxonomy} and the \emph{structural relationship} presented by~\citet{schwartz1994there,schwartz2012overview}. As the conventional theory is missing the context of AI-system and human-AI interactions, we further supplement the \emph{value taxonomy} and the \emph{structural relationship}. Specifically, we used a \emph{bottom-up} way to extract all values studied in the literature and map them into the Schwartz Theory of Basic Values. Further, we added the missing values and relationship regarding the AI context to make our outcome more comprehensive.





% \subsubsection{\textbf{Outcome: The Relations of Human Values and Fine-grained Taxonomy}}
% \label{sec:value_outcome}
% % \mbox{}
% % 
% % Consequently, 
% We developed a more comprehensive structure of the dynamic relations of human values (Figure~\ref{fig:value_structure}) and their fine-grained taxonomy with mapped reference papers for exemplary values (Figure~\ref{fig:value_taxonomy}) after incorporating the AI-related context. 
% % 
% % 
% % 
% % 
% Considering the dynamic relations of human values in Figure~\ref{fig:value_structure}, we consider five \emph{high-order value types} (\ie self-enhancement, openness to change, conservation, self-transcendence and desired values for AI tools), which encompass 12 \emph{motivational value types} (\eg power, universalism, functionality). We further organize the relation among these value types along two dimensions: 1) different resources (\ie individuals, society and interaction) and 2) different self intentions (\ie self-protection against threat and self-expansion and growth). Note that the type of \emph{Desired Values of AI Tools} and its encompassed \emph{motivational values} (\ie functionality and human-likeness) are the supplemental value types we added from the empirical \emph{bottom-up} process introduced above.
% Also, it is worth noting that some values conflict with one another (\eg Benevolence and Power) whereas others are compatible (\eg Conformity and Security). This structure of values refers to these relations of conflict and congruence among values~\cite{schwartz1994there,schwartz2012overview}.
% % 
% % 
% % 
% % 
% % 
% Furthermore, we elaborate the definitions of the 12 motivational value types and their exemplary values with mapped paper reference in Figure~\ref{fig:value_taxonomy}. During the process of mapping existing literature to these values, we noted two findings: 1) value terms in empirical papers were often named differently (\eg capability and competence), or check their opposites (\eg fairness and bias), from the listed exemplary values of Schwartz's theory even they are examining the same thing essentially . 2) there are many values not studied in our collected literature (indicated as (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) in the Figure). 
% Also there are some  values that are included but humans might not expect AI to integrate (\eg power-seeking), we indicated it as (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) with \textcolor{hua-red}{red-color}. We consolidated them by using the synonyms. 
% 2) empirical paper often check if AI do not contain a negative value (\ie bias and sarcastically) whereas our exemplary values are mostly positive. We resolved the two above issues 


% while exemplary values in our taxonomy are mostly \emph{positive}, many papers are checking if AI manifests \emph{negative} values (\eg capability and competence)


% This taxonomy, however, need to be carefully extended to encompass AI and HCI contexts.
% Many objectives mentioned in the AI and HCI literature align with specific human values, although they often use different terminology. 
% For example, \textit{effectiveness} and \textit{efficiency} can be mapped to \textit{self-enhancement} $\rightarrow$ \textit{achievement} $\rightarrow$ \textit{capability}; and \textit{accountability} can be mapped to \textit{self-transcendence} $\rightarrow$ \textit{benevolence} $\rightarrow$ \textit{responsibility}; and 
% This indicates a need for bridging conceptual frameworks to ensure clarity and consistency in how values are integrated and addressed within these fields.
% Given the theory-guided taxonomy, we further ensure the comprehensiveness of human value coverage by conducting a \textit{bottom-up} search from all collected papers, and consolidated the wordings used to describe a particular human value.


% Based on the aforementioned process, we achieved our detailed human value taxonomy as described in Fig~\ref{fig:schwartz}. 





==> sections/discussion.tex <==





% 
% To illustrate this approach, 
%  we present an imaginary use case demonstrating how researchers can use the resources provided in this paper to consider bidirectional human-AI alignment research from a holistic perspective (Section~\ref{sec:use_case}).
% % 




% Drawing insights from the framework development and associated coding analysis, 
% 
% 
% we discuss potential avenues for future research in both the ``\emph{aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}}'' (Section~\ref{sec:future_human2ai}) and ``\emph{aligning \textcolor{hua-blue}{AI}} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}'' (Section~\ref{sec:future_ai2human}) directions.
% 
% we discuss potential actions for future research to take to achieve this long-term alignment goal in both the ``\emph{aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}}'' (Section~\ref{sec:future_human2ai}) and ``\emph{aligning \textcolor{hua-blue}{AI}} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}'' (Section~\ref{sec:future_ai2human}) directions.







% \subsection{Considering Bidirectional Human-AI Alignment as a Holistic Loop: A Use Case}
% \label{sec:use_case}



% Concretely, suppose a research group \gr aims to develop an AI system that will be aligned with a specific marginalized group \gm. However, given the existing general AI systems that could not align with this specific group \gm, it is unclear \emph{how to improve the system and ensure that the developed system will positively impact the group \gm}.
% % whether the research group \gr possessed AI system is already aligned with marginalized group \gm and how to improve it. 
% To achieve this research goal, we next showcase how to potentially use our \emph{bidirectional human-AI alignment} framework to resolve the problem as a holistic loop.
% % 
% % 
% We divide the holistic process into four steps and describe them correspondingly in the four subsections below.



% % ==== 1. identify values; 2. represent values;
% \subsubsection{Identifying and Representing Values of Group \gm}
% % \mbox{}

% % Firstly, \textbf{identifying and represent values} of group \gm. 
% The first step researchers \gr need to do is to identify the value priority of group \gm and represent the values in a format that can be used by AI.
% % 
% % Referring to Section~\ref{sec:ai2human1} and Section~\ref{sec:gap_value}, t
% To identify the set of values group \gm might prioritize, the framework provides two potential ways of identifying the specific values. One, based on the category listed in Section~\ref{sec:ai2human1} and \ref{sec:gap_value}, researchers \gr can identify the set of value classes the group \gm may prioritize, and search for published datasets or benchmarks that can represent these values (Benchmark dataset examples include ETHICS~\cite{hendrycks2020aligning}, SOCKET~\cite{choi2023llms}, etc.). Besides, the researchers \gr can also design surveys and recruit real humans from group \gm, referring to Section~\ref{sec:human2ai4}, to identify their value priority and represent these values in AI model usable formats, such as rating and natural language description, based on Section~\ref{sec:ai2human2} (See OpinionQA~\cite{santurkar2023whose} example for collecting survey dataset).
% % 
% % 

% % Next, to represent human values in the way that can be used by AI, referring to Section~\ref{sec:ai2human2}, the framework



% % ==== 3. finetunine models; evaluate models and find under-performance;
% \subsubsection{Finetuning and Evaluation AI to Integrate Identified Values}
% % Secondly, \textbf{fine-tuning and evaluating AI model to integrate values} of group \gm.
% Given the represented human values in datasets, referring to Section~\ref{sec:ai2human2}, researchers \gr can further finetuning the AI model to integrate these representative values. Particularly, the framework is providing typical methods of aligning AI with these values, including Supervised Fine Tuning (\eg \cite{zhou2024lima} ) and Reinforcement Learning with Human Feedback (\eg DPO~\cite{rafailov2024direct}, RLHF~\cite{ouyang2022training}). Thereafter, researchers \gr need to evaluate these aligned AI models using the collected value datasets to ensure the effectiveness of alignment.







% % \subsubsection{Helping Group \gm Understand AI by Explaining AI}
% % % Thirdly, \textbf{helping group \gm understanding AI by explaining AI}. 
% % If the group \gm could not completely understand AI, we can also refer to Section~\ref{sec:human2ai3} for developing human-centered AI explanations for them.







% % ==== 4. assess AI impacts on margialized group;
% \subsubsection{Understanding and Assessing AI Impacts on Group \gm}
% % Fourthly, \textbf{assessing AI impacts} on the group \gm.
% If the group \gm could not completely understand AI, we can also refer to Section~\ref{sec:human2ai3} for developing human-centered AI explanations for them.
% Furthermore, to assess the usability and impacts of developed AI system on group \gm, researchers \gr can refer to Section~\ref{sec:human2ai3} for developing human-AI collaborative tasks to empower group \gm to use and perceive AI systems (\eg human-AI co-writing tasks~\cite{shen2023convxai,lee2022coauthor,petridis2023anglekindling}, story generation tasks~\cite{chung2022talebrush,zhang2022storybuddy}, collaborative decision making~\cite{bansal2021does,10.1145/3397481.3450650}, etc.). 
% Next, researchers \gr can assess the practical impacts on group \gm, referring to Section~\ref{sec:human2ai4} in terms of various aspects relevant to value perceptions and reactions, such as decision making fairness and equity, generation creativity, misinformation and privacy, etc. 





% % ==== 5. quantify their values and customize AI systems during inference stage.
% \subsubsection{Representing Revised Values and Customize AI During Model Inference}
% % 
% After acquiring the practical values revised with the interaction between AI and group \gm, referring to Section~\ref{sec:human2ai3} and \ref{sec:ai2human2}, the researchers \gr can customize AI values during inference stage in practical human-AI collaboration tasks to fulfill alignment. 
% % 
% For example, both ConstitutionMaker \cite{petridis2024constitutionmaker} and ConstitutionalExperts~\cite{petridis2024constitutionalexperts} help users steer LLMs by helping them write better prompts.
% ConstitutionMaker enables \textit{interactive} prompt optimization, where users can provide natural language feedback on the model's output, and the system converts this feedback into principles (i.e. rules) that are inserted into the model's prompt ~\cite{petridis2024constitutionmaker}.
% Meanwhile, ConstitutionalExperts automatically optimizes a discrete prompt; users can provide a small labeled dataset with which the system uses to ``train'' a prompt by iteratively adding and refining principles within the prompt \cite{petridis2024constitutionalexperts}.
% Thus, if unsatisfied with the model's outputs, users can employ these interactive or automatic techniques to better infuse their feedback and values into the prompt at inference.












% The two directions of human-AI alignment are not independent; instead, they represent an \emph{ongoing, mutual process} to achieve a \emph{dynamic alignment goal over the long term}. Future research should approach alignment studies as a bidirectional process to fully explore the breadth of the research space and achieve this essential goal. 
% 
Drawing upon insights gained from the development of our framework and the associated coding analysis, as shown in Figure~\ref{fig:future_work}, we propose future research aiming to achieve the long-term alignment goal by identifying three important challenges from near-term to long-term objectives, including the Specification Game (Section~\ref{sec:challenge1}), Dynamic Co-evolution of Alignment (Section~\ref{sec:challenge2}), and Safeguarding Coadaptation (Section~\ref{sec:challenge3}).
% 
% 
% Particularly, we discuss research questions and motivations followed by ideas for solution exploration from both directions of ``\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em} Align \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Human}'' (\ie domains related to AI algorithm and method development, including Machine Learning, Artificial Intelligence, Data Science, and others)  and ``\hspace*{.0em}\numimg{figures/B.pdf}\hspace*{-.1em} Align \textcolor{hua-red}{Human} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}'' (\ie domains conducting studies related to humans and society, including Human-Computer Interaction, Social Science, Cognitive Science and others) for each challenge below.







\subsection{Specification Game}
\label{sec:challenge1}

An important near-term challenge is resolving the ``Specification Game'', which involves precisely defining and implementing AI goals and behaviors to align with human intentions and values. Next, we will introduce how synergistic efforts from two directions can potentially address this challenge.

% Current AI development primarily aims to achieve alignment by training models using human instructions, examples, ratings, rankings and others. The goal is for AI systems to infer alignment goals (\eg human values and intentions) in a data-driven manner.
% % 
% However, designers often struggle to fully specify all important values and constraints, and they may not be able to explain or control what the AI has learned from the data. 
% % 
% Instead of resorting to easy-to-specify but fallible proxy goals (\eg maximizing the approval of human overseers),
% future studies should consider more explainable and controllable methods for humans to specify alignment goals for AI interactively. 
% % 
% Next, we discuss how research in these two areas can synergize to potentially achieve this goal.


% \subsubsection{\textbf{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Adapt AI to the full range of human values interactively during learning and deployment stages}}


% \subsubsection{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Adapt AI to fully specified important human values interactively during learning and deployment stages}
% \subsubsection{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Adapt AI to nuanced and contextualized human values interactively during learning and deployment stages}







\begin{figure*}[!t]
  \centering
  \includegraphics[width=1\textwidth]{figures/future_work.pdf}
  \caption{We envision future research directions to achieve long-term human-AI alignment with both efforts from the ``Align \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}'' (AI-centered research) and ``Align \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}'' (Human-centered research) directions. 
  We elaborate the three important future challenges, including Specification Game (Section~\ref{sec:challenge1}), Dynamic Co-evolution of Alignment (Section~\ref{sec:challenge2}), and Safeguarding Coadaptation (Section~\ref{sec:challenge3}).
  }
  \label{fig:future_work}
  % \vspace{-2em}
\end{figure*}


\subsubsection{\textbf{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Integrate fully specified human values into aligning AI}}
% \mbox{}


% \textbf{Identify appropriate values and priorities.}
% \textbf{Identify appropriate values and agreements for AI alignment.}
% \emph{Research Problem and Motivation.}
\noindent Individuals often possess value systems that encompass multiple values with varying priorities, rather than a single value, to guide their behaviors~\cite{schwartz1994there,schwartz2012overview}.
% For example, people may prioritize the value of \emph{family} and \emph{work} differently, leading to varied choices in time allocation. 
% 
% 
% 
Also, these priorities can change dynamically throughout an individual's life stages.
As such, 
% it is unlikely to that we can achieve a universal value system, recognized by all humans, to govern AI alignment. Instead, 
It is more realistic to select values compatible with specific societies or situations, given the fact that we live in a diverse world~\cite{gabriel2020artificial}.
% 
Future research, inspired by Social Choice Theory~\cite{arrow2012social}, could focus on using democratic processes to aggregate individual values into collective agreements. Building on the summaries in Sections ~\ref{sec:ai2human1} and ~\ref{sec:gap_value}, researchers can employ democratic methods to identify diverse subsets of human values for AI alignment. 
Additionally, creating datasets that represent these values is crucial. 
% 
% 
% 
% 
Besides, it is crucial yet challenging \emph{for AI designers to investigate how to fully specify the appropriate values 
% develop methods for selecting appropriate value systems 
and to further integrate these values into AI alignment}.
% 
% 
% 
Future important area involves developing algorithms, such as the Bradley-Terry Model~\cite{rafailov2024direct} or Elo Rating System~\cite{bai2022constitutional}, to convert heterogeneous human values into AI-compatible formats for training reward models and guiding reinforcement learning. Researchers should also explore AI models capable of aligning with unstructured human data, including free-form descriptions of values, multimedia, or sensor recordings depicting human behavior.





% \textbf{Recommendations for Future Work.} 
% Future work can draw from political theory, which examines fair methods for determining the principles that state institutes should follow, as a potential guide for selecting human values for AI alignment. Inspired by Social Choice Theory~\cite{arrow2012social}, one future direction involves aggregating individual values into collective value agreements or judgments through democratic processes such as voting, discussion, and civic engagement~\cite{gabriel2020artificial}.
% Therefore, building on the summary of human values in Section~\ref{sec:ai2human1} and \ref{sec:gap_value}, future researchers can use democratic methods to identify a wide spectrum of human value subsets for AI alignment.
% % 
% % 
% Additionally, an important focus for future work lies in the curation of datasets that can represent these wide-spectrum human values, particularly in rich formats that go beyond simple ratings and rankings, which are commonly used in current alignment algorithms (\eg RLHF~\cite{ouyang2022training}, RLAIF~\cite{bai2022constitutional}).
% Another key research area to explore is around algorithms or methods (\eg Bradley–Terry Model~\cite{rafailov2024direct} or Elo Rating System~\cite{bai2022constitutional}), potentially drawing from economic theories, to convert heterogeneous human value data (\eg principles or contextual information) into AI-compatible formats (\eg scalars) for training reward models and guiding reinforcement learning. Also, future research can explore AI models that can act directly on aligning humans' unstructured data, such as free-form descriptions of values, multimedia or sensor recordings depicting how people act in various situations, among others.
% 
% 
% 
% Future work can draw from political theory as a potential guide for selecting human values for AI alignment. 
% Future research, inspired by Social Choice Theory~\cite{arrow2012social}, could focus on using democratic processes to aggregate individual values into collective agreements. Building on the summaries in Sections ~\ref{sec:ai2human1} and ~\ref{sec:gap_value}, researchers can employ democratic methods to identify diverse subsets of human values for AI alignment. 
% Additionally, creating datasets that represent these values is crucial. 
% Another important area involves developing algorithms, such as the Bradley-Terry Model~\cite{rafailov2024direct} or Elo Rating System~\cite{bai2022constitutional}, to convert heterogeneous human values into AI-compatible formats for training reward models and guiding reinforcement learning. Researchers should also explore AI models capable of aligning with unstructured human data, including free-form descriptions of values, multimedia, or sensor recordings depicting human behavior.
% 
% 
% 




% \subsubsection{\textbf{Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}: Specify the nuanced and contextualized human values in AI data formats interactively}}
\subsubsection{\textbf{Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}: Elicit nuanced and contextual human values during diverse interactions}}
% \mbox{}


\noindent Current alignment methods use instructions, ratings, and rankings to infer human values, which can not fully capture all relevant human values and constraints.
% ~\cite[142]{khamassi2024strong}.
% \notice{khamassi2024strong}
% ~\cite{khamassi2024strong,christian2021alignment}. 
% 
Future research should focus on optimizing interactive interfaces to efficiently elicit human values. These interfaces can leverage diverse interaction modes to capture comprehensive human value information. 
% 
% 
Additionally, people often struggle to formulate optimal prompts for AI, accurately specify their requirements, and articulate their desired values, which can change based on context and time. 
Developing proactive interfaces that use conversational techniques to elicit nuanced and evolving values is also crucial. 
% 
% 
Implicit human signals that indicate values are also frequently overlooked.
Additionally, systems that track interactions to hypothesize and validate implicit human values in real-time should be designed.


% 
% 
% 

% \noindent Current alignment methods primarily capture human values using instructions, ratings and rankings, aiming to infer humans' alignment goals (\eg human values and intentions) in a data-driven manner.
% % 
% % aiming for AI systems to infer alignment goals (\eg human values and intentions) in a data-driven manner. 
% % 
% However, these limited data formats and interaction methods fall well short of fully specifying all of the relevant human values and constraints. 
% % Besides, when humans are learning to collaborate or utilize AI, it is often challenging for humans to write the optimal prompts that can accurately and efficiently specify what they demand in practice. 
% Besides, when humans seek to collaborate with or utilize AI, they often encounter challenges in formulating optimal prompts, which require them to accurately and efficiently specify their requirements or expectations, in order to be able to use AI generated output or decision making in practice.
% % For instance, in spatial reasoning tasks, specifying geographical routes can be more accurately and comprehensively achieved if humans draw sketches interactively, rather than through ratings and rankings.
% % 
% % 
% Additionally, people often struggle to articulate all of their desired values accurately and comprehensively, especially as these values can dynamically change based on contextual and temporal situations. 
% % 
% Relatedly, practices often overlook implicit human interactive signals that can also indicate values relevant to AI alignment.
% % Therefore, it is essential for HCI researchers to develop diverse interactive strategies where AI systems can proactively engage with users to elicit nuanced, contextualized, and evolving information about their values.



% \textbf{Recommendations for Future Work.} One promising area for future research is optimizing interactive interfaces to elicit human values efficiently and effectively. These interfaces can leverage diverse interaction modes (see an initial summary in Figure~\ref{fig:interaction}) to fully capture human value information. For example, to identify a set of important principles for AI alignment, the interface can use the user's conversational natural language specifications and generate a list of principle options for users to select from and/or revise.
% % 
% % 
% Recognizing that humans cannot always comprehensively articulate their values, another key research area is to develop interfaces that proactively interact with users. This could involve conversational techniques or scaffolding procedures to elicit nuanced, contextualized, and evolving information about an individual's values.
% % 
% % 
% Additionally, to capture implicit human interaction signals that reflect human values for AI alignment, another area of future work involves designing systems that track interactions to develop real-time hypotheses about human values on these implicit signals, and then proactively validate them with humans as needed.











\subsection{Dynamic Co-evolution of Alignment}
\label{sec:challenge2}

\noindent
The challenge ahead lies in comprehending and effectively navigating the dynamic interplay among human values, societal evolution, and the progression of AI technologies.
Future studies in these directions aim to bolster a synergistic co-evolution between AI and human societies, adapting both to each other's changes and advancements.


% \subsubsection{\textbf{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Co-evolve AI with changes in humans and societal values, cognition, and needs}}
\subsubsection{\textbf{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Co-evolve AI with changes in humans and society}}
% \mbox{}


\emph{(i)}
Existing literature often treats AI alignment as static, ignoring its dynamic nature. A long-term perspective must consider the co-evolution of AI, humans, and society. As AI systems evolve and scale up, they gain new capabilities, making it essential to ensure their goals remain aligned with human values. Thus, alignment solutions require continuous oversight and updates.
% 
% 
% 
Future research should develop methods for continuously updating AI with limited data without compromising alignment values and performance. 
% In real-world scenarios, fine-tuning deployed AI systems is often impractical. Thus, adapting AI during deployment without fine-tuning is crucial. 
This could involve forecasting human value evolution and preparing AI with flexible strategies like prompting or interventions.
% 
% 
% Updating AI to continuously adapt to the dynamic changes of humans and society requires adjustments in alignment data, models, and evaluation processes spanning both learning and deployment stages. 
% % 
% Referring to the methodologies listed in Section~\ref{sec:ai2human2}, current strategies often rely on fine-tuning to update AI with a curated human value dataset during the learning process. However, this approach may lead to AI models forgetting or diminishing previous alignment goals. In situations where sufficient data for fine-tuning is unavailable, these methods becomes more challenging.
% % 
% Therefore, a crucial area for future research is to develop approaches for continually updating AI systems using limited data without compromising existing alignment values and performance. 
% 
% 
% 
% 
\emph{(ii)}
Additionally, AI advancements also influence human actions and values, necessitating adaptive alignment solutions. Ensuring AI co-evolves with human and societal changes is crucial for robust alignment.
% 
This challenge could potentially be addressed by forecasting the potential evolution trajectories of human values or behavioral patterns, and preparing AI with the flexibility to adapt in advance, for example, through prompting or intervention strategies.
% 
% 
% 
% In summary, co-evolving AI with dynamic human and societal changes requires collaboration among experts in various domains such as machine learning and social sciences.





% 
% % 
% % 
% In real-world scenarios, it is common for AI systems to already be deployed at scale, making fine-tuning a challenging or impractical practice. 
% Therefore, another important research direction involves adapting AI, during the deployment stage, without relying on fine-tuning. This challenge could potentially be addressed by forecasting the potential evolution trajectories of human values or behavioral patterns, and preparing AI with the flexibility to adapt in advance, for example, through prompting or intervention strategies.
% In summary, the co-evolution of AI with dynamic human and societal changes necessitates a synergetic collaboration among experts from various domains, such as machine learning and social sciences.
















% % \noindent

% Existing literature often views AI alignment as a static process, neglecting the dynamic nature of alignment goals. However, a long-term perspective of alignment requires us to take into account the co-evolution of AI, humans, and society. On one hand, as AI systems scale up, they regularly acquire new and sometimes unexpected ("emergent") capabilities, including learning from examples on the fly and adaptively pursuing goals. This leads to the challenge of ensuring that the goals AI might independently formulate remain consistently aligned with human values. Consequently, alignment solutions must involve continuous oversight and updates in response to AI's evolution during development and deployment.
% On the other hand, AI advancements influence the state of the world, affecting human actions and even their underlying values and strategies~\cite{hong2024learning}. Thus, alignment solutions that continually adapt to the updated human and societal considerations may offer the most robust approach~\cite{irving2019ai}.
% % 
% Consequently, it is crucial to \emph{ensure that AI co-evolves with changes in human and societal values, cognition, and needs dynamically}.






% % \textbf{Examples of Potential Future Solutions.}
% \textbf{Recommendations for Future Work.}
% Updating AI to continuously adapt to the dynamic changes of humans and society requires adjustments in alignment data, models, and evaluation processes spanning both learning and deployment stages. 
% % 
% Referring to the methodologies listed in Section~\ref{sec:ai2human2}, current strategies often rely on fine-tuning to update AI with a curated human value dataset during the learning process. However, this approach may lead to AI models forgetting or diminishing previous alignment goals. In situations where sufficient data for fine-tuning is unavailable, these methods becomes more challenging.
% % 
% Therefore, a crucial area for future research is to develop approaches for continually updating AI systems using limited data without compromising existing alignment values and performance. 
% 
% In real-world scenarios, it is common for AI systems to already be deployed at scale, making fine-tuning a challenging or impractical practice. 
% Therefore, another important research direction involves adapting AI, during the deployment stage, without relying on fine-tuning. This challenge could potentially be addressed by forecasting the potential evolution trajectories of human values or behavioral patterns, and preparing AI with the flexibility to adapt in advance, for example, through prompting or intervention strategies.
% In summary, the co-evolution of AI with dynamic human and societal changes necessitates a synergetic collaboration among experts from various domains, such as machine learning and social sciences.
















% \subsubsection{\textbf{Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}: Adapt humans and society to the latest AI advancements and examine changes to inform AI evolvement}}
\subsubsection{\textbf{Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}: Adapt humans and society to the latest AI advancements}}
% \mbox{}



\noindent
\emph{(i)}
While current AI systems lag behind humans in many tasks, identifying and handling AI mistakes, including knowing when to seek human intervention, remains essential. Future research should focus on developing validation mechanisms that enable humans to interpret and verify AI outputs. This could involve designing interfaces that allow humans to request step-by-step justifications from AI or integrating tools to verify the truthfulness of AI referring to Section~\ref{sec:collaboration}. Additionally, developing interfaces that enable groups of humans to collaboratively validate AI outputs and creating scalable validation tools for large-scale applications are important directions.
% 
\emph{(ii)}
As AI advances, it becomes essential to develop systems that enable humans to utilize AI with capabilities surpassing their own. Research is needed to understand how individuals can interpret and validate AI outputs for tasks beyond their abilities and leverage advanced AI sustainably, avoiding issues like job displacement or loss of purpose. Another research direction is designing strategies to enhance human capabilities by learning from advanced AI, including gaining knowledge and building skills.
% 
% 
\emph{(iii)}
As AI integrates more into daily tasks, its impact on human values, behaviors, capabilities, and society remains uncertain. Continuous examination of AI's influence on individuals, social relationships, and broader societal changes is vital. Research should assess how humans and society adapt to AI advancements, guiding AI's future evolution. Potential areas include evaluating changes in individual behavior, social relationships, and societal governance as AI replaces traditional human skills. Understanding these dynamic changes is essential for grasping the broader impact of AI on humanity and society.











% \noindent
% As AI progresses, humans will likely need to transition from interacting with less capable systems to engaging advanced AI systems (\eg AGI) \cite{morris2024levels}. It's imperative to develop interactive strategies which enable humans to effectively utilize AI across varying levels of model capability.
% % 
% % 
% % 

% While current AI systems still lag behind human performance in many tasks, questions persist about human resilience to AI mistakes. Efficiently identifying these mistakes and developing appropriate fallback actions, such as interactive intervention, remains crucial in various situations; identifying and handling errors, including knowing when to seek human intervention, will remain an important even for highly capable future systems.
% % 
% Future research on advanced AI systems should focus on developing validation mechanisms that enable humans to interpret and verify AI outputs. 
% Inspired by initial explorations in Section~\ref{sec:collaboration}, this could involve designing interactive interfaces that allow humans to request step-by-step justifications from AI, or integrating external tools to verify the truthfulness of AI outputs. This could also include developing interfaces that enable groups of humans to work together to validate AI outputs, since groups working jointly typically have broader and deeper "intelligence" in practice than any single actor). Further, this approach can be extended to scalable validation tools, automating the verification process for large-scale applications such as in education and the workplace.





% Looking ahead, as AI advances further, it becomes essential to develop interactive systems which enable humans to utilize AI that has capabilities surpassing their own. Research is needed to understand how individuals can interpret and validate the outputs of AI performing tasks beyond their current abilities, and also, how humans could leverage advanced AI in a sustainable way, \ie benefiting their life without harmful side effects such as job displacement or loss of purpose.
% % 
% % 
% % 
% Another important research direction is designing interactive strategies to enhance human capabilities by learning from advanced AI. This includes gaining knowledge and building technical and social skills.








% In addition, as AI becomes increasingly integrated into daily tasks, its influence on human values, behaviors, capabilities, and society remains uncertain. Thus, it's vital to continuously examine the impact of AI advancements on individuals, social relationships, and broader societal changes.
% % 
% % 
% % 
% Furthermore, it is crucial to assess how humans and society adapt to AI advancements which, in turn, can guide the future evolution of AI. Potential research areas include evaluating changes in individual behavior and social relationships (\eg how relationships with advanced AI may supplant human relationships), and societal governance (\eg how legal and education systems may change as AI is used in place of traditional human skills).
% % , and value and belief systems (\eg how might religious practices and values evolve as people might develop new beliefs about powerful AI agents?)
% Examining these dynamic changes is essential for understanding the broader impact of AI advancements on humanity and society. 










% \textbf{Recommendations for Future Work.}
% While prior AI assistants have primarily aimed to complement human capabilities in task performance, 
% future research on advanced AI systems should focus on developing validation mechanisms that enable humans to interpret and verify AI outputs. 
% Inspired by initial explorations in Section~\ref{sec:collaboration}, this could involve designing interactive interfaces that allow humans to request step-by-step justifications from AI, or integrating external tools to verify the truthfulness of AI outputs. This could also include developing interfaces that enable groups of humans to work together to validate AI outputs, since groups working jointly typically have broader and deeper "intelligence" in practice than any single actor). Further, this approach can be extended to scalable validation tools, automating the verification process for large-scale applications such as in education and the workplace.
% 
% 
% Another important research direction is designing interactive strategies to enhance human capabilities by learning from advanced AI. This includes gaining knowledge and building technical and social skills.
% 
% 
% Furthermore, it is crucial to assess how humans and society adapt to AI advancements which, in turn, can guide the future evolution of AI. Potential research areas include evaluating changes in individual behavior and social relationships (\eg how relationships with advanced AI may supplant human relationships), and societal governance (\eg how legal and education systems may change as AI is used in place of traditional human skills).
% % , and value and belief systems (\eg how might religious practices and values evolve as people might develop new beliefs about powerful AI agents?)
% Examining these dynamic changes is essential for understanding the broader impact of AI advancements on humanity and society. 










% =============================
\subsection{Safeguarding Co-adaptation}
\label{sec:challenge3}


\noindent
As AI gains autonomy and capability, the risks associated with its instrumental actions, as a means toward accomplishing its final goals, increase. 
% While these actions may aid AI in achieving its final goals, they 
These actions can be undesirable  for humans.
% , i.e., power-seeking or evading human intervention.
Therefore, safeguarding the co-adaptation between humans and AI is crucial.
% This can be achieved by empowering humans to understand and control AI's instrumental goals, in order to ensure rational and ethical behaviors. 
We next explore future research to address this challenge from both directions. 





% \subsubsection{\textbf{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Decompose superintelligent AI behavior to human-interpretable goals and enable human interventions to reduce risks}}
\subsubsection{\textbf{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Specify the goals of an AI system into interpretable and controllable instrumental actions for humans}}
% \mbox{}
% 
\noindent
\emph{(i)}
As advanced AI systems become more complex, they present greater challenges for human interpretation and control. It is crucial to empower humans to detect and interpret AI misconduct and enable human intervention to prevent power-seeking AI behavior. Research should focus on designing corrigible mechanisms for easy intervention and correction, including modular AI architectures and robust override protocols that allow human operators to halt or redirect AI activities. These components should be human-interpretable, enabling scenario testing.
% 
% 
\emph{(ii)}
Furthermore, advanced AI systems may intentionally mislead or disobey humans, generating plausible fabrications~\cite{johnson2022ai}. Developing reliable interpretability mechanisms to validate the faithfulness and honesty of AI behaviors is essential. This includes correlating AI behaviors with internal neuron activity signals, akin to physiological indicators in human polygraph tests~\cite{american2004truth}. Inspecting these indicators can help humans assess the truthfulness of AI interpretations and prevent risky actions.






% \noindent 
% \emph{(i)}
% As advanced AI systems become increasingly complex, they present greater challenges for human interpretation and control. 
% % The stakes are higher when AI gains more autonomy and capability, potentially seeking power and evading human intervention. 
% To address this, it is crucial to \emph{empower humans to detect and interpret AI misconduct on instrumental actions towards accomplishing its final goals}. 
% % 
% % 
% % 
% Additionally, mechanisms must be developed to enable human intervention and prevent power-seeking AI misconduct, thus maintaining a safe co-adaptation between AI and humans.
% % 
% % 
% % 
% % 
% One potential research area aimed at empowering humans to interpret and control advanced AI behavior is the \emph{design of corrigible mechanisms that facilitate easy intervention and correction}. This includes developing modular AI architectures where components can be independently adjusted or replaced, and creating robust override protocols that allow human operators to safely halt or redirect AI activities. These components should ideally be human-interpretable, enabling supervisors to conduct scenario testing when necessary.





% \emph{(ii)}
% Furthermore, advanced AI systems, even with sufficient interpretation capabilities, may intentionally mislead or disobey humans. It is possible for AI to stand by falsehoods, generate empty explanations for their answers, and produce outright fabrications that may appear plausible~\cite{johnson2022ai}. Therefore, \emph{developing reliable interpretability mechanisms to validate the faithfulness and honesty of AI systems' self-reported behaviors is also essential}.
% % 
% % 
% % 
% % 
% Another critical research direction lies in validating the faithfulness and honesty of AI interpretability. This could involve correlating AI behaviors with internal neuron activity signals, similar to how physiological indicators are measured in human polygraph tests~\cite{american2004truth}. Inspecting internal neuron indicators could support human assessment of the truthfulness of AI interpretations, thereby allowing them to accurately judge and prevent potential risky instrumental actions.







% \textbf{Recommendations for Future Work.}
% \noindent One potential research area aimed at empowering humans to interpret and control advanced AI behavior is the \emph{design of corrigible mechanisms that facilitate easy intervention and correction}. This includes developing modular AI architectures where components can be independently adjusted or replaced, and creating robust override protocols that allow human operators to safely halt or redirect AI activities. These components should ideally be human-interpretable, enabling supervisors to conduct scenario testing when necessary.
% 
% 
% 
% 
% Another critical research direction lies in validating the faithfulness and honesty of AI interpretability. This could involve correlating AI behaviors with internal neuron activity signals, similar to how physiological indicators are measured in human polygraph tests~\cite{american2004truth}. Inspecting internal neuron indicators could support human assessment of the truthfulness of AI interpretations, thereby allowing them to accurately judge and prevent potential risky instrumental actions.











\subsubsection{\textbf{Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}: Empower humans to identify and intervene in AI instrumental and final strategies in collaboration}}
% \mbox{}


\noindent
\emph{(i)}
Preventing advanced AI from engaging in risky actions requires robust human supervision. Essential steps include developing training and simulation environments with scenario-based exercises and timely feedback, and creating interactive dashboards for real-time monitoring. These dashboards should feature effective data visualization, anomaly detection, and prompt alert systems for immediate intervention.
% 
% 
\emph{(ii)}
Scalable solutions are needed for supervising AI across various applications. Real-time oversight becomes more challenging with widespread AI deployment, necessitating advanced autonomous monitoring tools. These tools should learn normal AI behavior and flag deviations immediately. Integrating training environments, interactive dashboards, and scalable diagnostic tools will enhance human ability to manage AI risks, ensuring better alignment with human values.




% \noindent
% \emph{(i)}
% Preventing future advanced AI systems from engaging in risky instrumental actions requires human capabilities to identify and mitigate such behaviors. 
% % 
% % 
% % 
% % 
% To enhance human capability in supervising AI instrumental actions, robust training and simulation environments are essential. These should offer scenario-based training with timely feedback loops, enabling supervisors to identify and manage various instrumental actions effectively. 
% % 
% Additionally, creating interactive and intuitive dashboards is crucial for quickly recognizing and responding to potential risky instrumental goals. These dashboards should include effective data and model visualization, intervention techniques to highlight anomalies, and real-time alerts for prompt intervention.




% \emph{(ii)}
% Additionally, scalable solutions that can be widely implemented are essential for effectively supervising AI instrumental behavior across various applications and environments. 
% % 
% % 
% % 
% % 
% Furthermore, as deploying advanced AI at scale makes real-time oversight more challenging, developing advanced and autonomous monitoring tools is vital. These tools should learn the normal operating parameters of AI systems, flagging deviations that suggest risky instrumental actions immediately. By integrating training and simulation environments, interactive dashboards, and scalable diagnostic tools, humans can better manage AI instrumental risks, supporting better alignment with human values and control.









% Future research could potentially explore comprehensive training programs and the development of advanced diagnostic tools to achieve these goals.
% 
% 


% \textbf{Recommendations for Future Work.}
% To enhance human capability in supervising AI instrumental actions, robust training and simulation environments are essential. These should offer scenario-based training with timely feedback loops, enabling supervisors to identify and manage various instrumental actions effectively. 
% Additionally, creating interactive and intuitive dashboards is crucial for quickly recognizing and responding to potential risky instrumental goals. These dashboards should include effective data and model visualization, intervention techniques to highlight anomalies, and real-time alerts for prompt intervention.
% 
% 
% 
% Furthermore, as deploying advanced AI at scale makes real-time oversight more challenging, developing advanced and autonomous monitoring tools is vital. These tools should learn the normal operating parameters of AI systems, flagging deviations that suggest risky instrumental actions immediately. By integrating training and simulation environments, interactive dashboards, and scalable diagnostic tools, humans can better manage AI instrumental risks, supporting better alignment with human values and control.
































% =========================== dead kitten ===============================






% \textbf{Solution Exploration.}
% To enhance the human capability of supervising AI power-seeking behaviors, one important direction is to provide robust training and simulation environments where human supervisors can practice identifying and managing power-seeking behaviors in AI. This can involve scenario-based training with timely feedback loops, which enable human supervisors to identify various power-seeking behaviors that can better handle the emergent power-seeking risks on the fly.
% % 
% % 
% Besides, another crucial research area is to create interactive and intuitive dashboards that can empower human supervisors recognize the respond to potential power-seeking risks quickly. The resulted interactive dashboard should involve effective data and model visualization and intervention techniques that can highlight the power-seeking anomalies timely, and enable real-time alerts to facilitate timely human intervention.
% % 
% % 
% Furthermore, when deploy superintelligent AI in large scale, it becomes more challenging for humans supervisors to conduct real-time oversight. Therefore, the other important research direction is to develop advanced and autonomic monitoring tools that can detect deviations from expected power-seeking behavior patterns. These tools should be able to learn the normal operating AI parameters or generations, flag deviations that suggest power-seeking actions immediately. By combining training and simulation environments, advanced interactive dashboards and scalable diagnostics tools, humans can better manage the risks associated with AI power-seeking and ensure they remain aligned with human values and control.




% % as result, human supervisors can potentially harness AI power-seeking actions 
% % % 









% % \noindent
% % The efforts of preventing future advanced AI systems from power-seeking behaviors requires to enhance human capabilities of identifying and mitigating such behaviors. Besides, this also necessitates scalable solutions that can be widely implemented and effectively supervise AI behavior across various applications and environments. 
% % Further research can potentially resort to \textbf{implementing comprehensive training programs and developing advanced diagnostic tools}. 






% \textbf{Solution Exploration.}
% % 
% These training programs should focus on educating AI researchers and developers about the signs of power-seeking tendencies in AI systems, using case studies and simulations to illustrate potential scenarios.
% % 
% Additionally, invest in creating sophisticated monitoring tools that can detect deviations from expected power-seeking behavior patterns. These tools should leverage machine learning to analyze AI decisions in real-time, flagging anomalies that suggest power-seeking actions.
% % 
% % Furthermore, design corrigible mechanisms that allow for easy intervention and correction of AI behavior. This can include developing modular AI architectures where components can be independently adjusted or replaced, as well as creating robust override protocols that enable human operators to halt or redirect AI activities safely.
% % 
% By combining education and advanced diagnostics, humans can better manage the risks associated with AI and ensure they remain aligned with human values and control.












% % % 
% % It is important yet challenging to empower humans to recognizing AI systems' power-seeking behavior and design corrigible mechanisms to prevent risky behaviors.











% \textbf{Solution Exploration.}
% One potential research area, which aims to empower human supervisors to interpret and control power-seeking AI misconducts, is to design corrigible mechanisms that allow for easy intervention and correction of AI behavior. This can include developing modular AI architectures where components can be independently adjusted or replaced, as well as creating robust override protocols that enable human operators to halt or redirect AI activities safely. Ideally the components should be human-interpretable so that humans can supervise and conduct scenario testing if needed in practice.
% % 
% % 
% Additionally, another important research direction is to validate the faithfulness and honesty of the AI interpretability. This could potentially include interpreting the truthful AI behaviors by correlating with their internal neurons indicator signals, similar with measuring and recording several physiological indicators in human brain in polygraph tests~\cite{american2004truth}.
% . Therefore, humans can judge the interpretation truthfulness of future AI power-seeking behaviors by inspecting their internal neuron indicators.





% decompose the complex superintelligent AI behavior into human-interpretable and controllable modules. By breaking down the complex AI capability into 
% % 
% % 
% design corrigible mechanisms that allow for easy intervention and correction of AI behavior. This can include developing modular AI architectures where components can be independently adjusted or replaced, as well as creating robust override protocols that enable human operators to halt or redirect AI activities safely.


% Besides, another important research direction is to validate interpretability's faithfulness and honesty. 
% % 
% % 










% \textbf{
% Humans and society build the infrastructure to preserve human agency in mutualistic symbiosis with superintelligent AI
% }



% % 
% % 
% 1. decompose complex AI behavior into human-interpretable actions.

% it is crucial to decompose complex superintelligent AI behaviors into human-interpretable and controllable actions. 



% 
% % 
% % 
% 2. validate interpretability's faithfulness and honesty. 
% % 
% % 

% flexible system design






% \noindent
% Future advanced AI with more complexity becomes more challenging for humans to interpret and control. The stakes become higher yet when AI systems gain more autonomy and capability that can seek powers and sidestep human intervention.
% Therefore, it is important to \textbf{decompose the complex superintelligent AI behaviors into human-interpretable and controllable actions}, and further, enable human intervention mechanisms to prevent power-seeking AI’s misconduct, thus balance the power between AI and humans in practice.
% Furthermore, as power-seeking AI systems tend to intentionally mislead or disobey humans, it is possible for AI to stand by falsehoods when prompted, generate empty explanations for their answers, and produce outright fabrications that may appear plausible~\cite{johnson2022ai}.
% Therefore, it is also essential to develop reliable mechanisms that can validate the faithfulness or honesty of AI's interpretability.



% \emph{Solution Exploration.}
% % 
% % 
% 1. decompose complex AI behavior into human-interpretable actions.




% it is crucial to decompose complex superintelligent AI behaviors into human-interpretable and controllable actions. 



% % 
% % 
% % 
% 2. validate interpretability's faithfulness and honesty. 
% % 
% % 

% % flexible system design



% \textbf{Solution Exploration.}
% While prior AI assistants largely aim to complement human capability in task performance, a crucial area for future research, regarding superintelligent AI systems, is to develop validation mechanisms that enable humans to interpret and verify AI outputs. Inspired by some initial exploration listed in Section~\ref{sec:collaboration}, this potentially involves designing interactive interfaces to allow humans to converse with AI for requesting step-by-step justifications, or to combine with external tools for verifying the truthfulness of AI outputs, and others. This can be further generalized to scalable validation tools, which automate the verification process for large-scale use scenarios such as education and  workplace.
% Besides, another important research direction is to design interactive strategies for equipping humans with better capabilities by learning from superintelligent AI, such as gaining knowledge, building technical and social skills, and others.
% % 
% % 
% Furthermore, another important research topic is to assess how humans and society adapt to the AI advancement which can in return, as described above, guide AI evolvement in the future. 
% Referring to the angles presented in Section~\ref{sec:impacts}, potential exploration in this direction includes assessing adaption of individuals' behavior and social relationships (\eg whether relationships with superintelligent AI would supplant relationships with humans?), adaptation of societal governing changes (\eg how our legal system or entire education system will change as AI supplants many traditional humans skills?), and adaptation of value and belief systems among humanity (\eg How religious practices and values might change as people develop novel belief systems about powerful AI agents? ). These dynamic changes that influence
% humans and society should be further examined along with AI advancements.















% \noindent
% The advancement of AI inevitably leads humans from interacting with less-capable systems to engaging with superintelligent AI. 
% Therefore, it is important to \textbf{develop interactive strategies for humans to harness AI with different levels of intelligence}.
% Current AI systems, to some extent, are still less capable than human in many tasks. Therefore, it remains questions about humans can keep resilient to AI mistakes, \ie efficiently and effectively identifying the AI mistakes and take fallback actions such as recalibrate reliance, interactive intervention, step-by-step critique, conversational negotiation, and others. 
% % 
% In the long run, when AI becomes more advanced, it will also be essential to develop interactive systems for humans to harness AI that has better capabilities than the system users.
% Therefore, this necessitates research on how people can validate the output of AI that is doing tasks beyond their current abilities.
% % 
% % 
% In addition, as AI becomes widely used in daily tasks, it is still uncertain how AI will influence human values, behaviors, capabilities, and even society in positive and negative ways. 
% % 
% Therefore, it is important to \textbf{examine humans, social relations, and societial changes due to AI advancements}
% % 
% % 





% \textbf{Solution Exploration.} 
% \hua{add solution 1}.
% To inspect how AI will influence human values, behaviors, capabilities, and even society, we expect future research to explore important research areas, such as Whether relationships with AI assistants would supplant relationships with humans? How our legal system would treat autonomous AI systems? How AI might change the balance of power between individuals and government or between nation-states? How our entire education system will change as AI supplants many traditional human skills? How religious practices and values might change as people develop novel belief systems about powerful AI agents? These dynamic changes that influence humans and society should be further examined.

% \hua{build upon existing Sec4.3, Sec4.4 to inspect the evolvement.}














% ===============================================================




% \noindent Current alignment methods primarily capture human values using human instructions, ratings and rankings. The goal is for AI systems to infer alignment goals (\eg human values and intentions) in a data-driven manner.
% % 
% However, AI designers often struggle to use these limited formats of data to fully specify all important human values and constraints.
% % 
% For example, when specifying geographical routes in the spatial reasoning task to improve AI accuracy, it would be easier for humans to interactively draw sketches, rather than rating and ranking, to specify the alignment objective in an accurate and comprehensive manner. 
% 



% % 
% In addition, it is often the case that humans could not articulate all their desired values accurately and comprehensively to instruct AI alignment, especially considering the dynamic change based on the contextualized and temporal situations. 
% % 
% Also, the common practice largely neglected many implicit human interactive signals observed from human interactions, which can also indicate human values for AI alignment.
% 
% % 
% Therefore, these considerations necessitate HCI researchers to \emph{develop diverse interactive strategies where AI systems can proactively interact with people to elicit nuanced, contextualized, evolving information on their values}. 




% \textbf{Solution Exploration.}
% % 
% % 
% One important area for future research is to optimizes the interactive interfaces for eliciting human values, which can leverage or combine diverse interaction modes (See the initial summary in Figure~\ref{fig:interaction}) to fully capture the value information in the most efficient and effective way. For example, to identify a set of important principles for AI alignment, the interface can leverage the user's conversational natural language specifications and generate a list of principles for users to select or revise next. 
% 





% 
% % 
% Furthermore, given that people could not always articulate their values comprehensively, this induces another important future area to proactively interact or converse with humans, potentially use a scaffolding procedure, to elicit nuanced, contextualized, and evolving information on their values. 
% % 
% % 
% In addition, other than the aforementioned explicit interactions, many implicit human signals or contextual information could also reflect human values that are helpful for AI alignment. 
% % 
% Therefore, another important area for future work directs systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-users.







% \textbf{Enhance human capabilities to recognize AI issues\merrie{what are "AI issues"? This term "issues" is very vague} and remain resilient to them
% }
% While several studies in HCI and social science have investigated human trust and reliance on AI with the help of explainability, there
% remain questions about how humans can handle AI mistakes when they potentially use AI with errors. 
% Similar to existing studies of re-calibration of human trust in AI~\cite{10.1145/3397481.3450650}, it is also essential to develop methods for humans to be resilient to AI errors: 
% efficiently identify the AI mistakes and take actions such as interactive correction, step-by-step critique, conversational negotiation, and others. 


% This is especially important when humans face future advanced AI that may potentially conduct power-seeking behaviors.\merrie{I think that conflating power-seeking behaviors with other types of errors is a problem. The first type of errors is the system not working correctly either because the model is not good (i.e., produces an incorrect answer) or because specification alignment was poor (i.e., produces a reasonable answer to an ambiguous command). Both of those are unintentional mistakes, which differ substantially from hypothetical systems that intentionally mislead or disobey the end-user}
% % 
% 













% \textbf{Solution Exploration.}
% % 
% % 
% Updating AI to continually capture the dynamic changes of human and society requires adaptation on alignment data, model, and evaluation spanning both learning and deployment stages.
% % 
% % 
% Existing strategies commonly leverage fine-tuning to update AI with curated human value datasets. However, this might result in the AI models forgetting or diminishing previous alignment goals. Besides, some situations can not generate sufficient amount of data to fine-tune AI. Therefore, one important are for future research is to continually update AI models using limited amount of data without diminishing existing alignment values and performance.
% % 
% In addition, another future research area is to adapt AI during deployment stage without fine-tuning the system. This can be potentially resolved by forecasting potential value evolvements and preparing AI with the flexibility of adaptation in advance, such as using prompting or intervention strategies. 
% % 
% Overall, Co-evolving AI with dynamic human and societal changes necessitates a synergetic collaboration among cross domain experts, such Machine Learning and Social Scientists.

% \hua{Build upon existing Sec 4.2 to develop dynamic }


% % Therefore, developing approaches to add on new alignment goals without diminishing existing performance would be a necessary yet challenging problem.
% % 







% % \noindent
% % Existing literature commonly considers AI alignment as a static process without encompassing dynamic changes to alignment goals. 
% % However, 
% % \emph{long-term perspectives require us to take into account the likely co-evolution of AI, humans, and society}.
% % On one hand, as AI systems scale up, they regularly acquire new and unexpected capabilities, including learning from examples on the fly and adaptively pursuing goals. This leads to the problem of ensuring that goals AI independently formulates and pursues consistently align with human values. Therefore, the alignment solutions require continuous oversight and updating in response to AI evolvement during development and deployment.
% % % 
% % % 
% % On the other hand, the AI advancement also influences the state of the world, such as the actions humans take in response to AI, and even their underlying values and strategies~\cite{hong2024learning}.
% % % Therefore, alignment solutions that continually adapt to the updated human and societal considerations may offer the most robust approach~\cite{irving2019ai}.
% % % % 
% % It is important to co-evolve AI with changes in humans and societal values, cognition, and needs.





% Human values can be captured from both explicit and implicit interactive signals. 
% It is important for future researchers to design proactive and diverse interactive approaches to fully capture human values, including both explicit and implicit interactive signals.
% 

% 
% % 
% % 
% Additionally, to encode diverse and full-spectrum of human values into AI alignment, AI developers also need to collect the value-reflected datasets and develop integration algorithms to encode these values into AI systems by building upon or referring to the current practice summarized in Section~\ref{sec:ai2human2}.
% % 
% Moreover, as opposed to the commonly implementations in current alignment algorithms (\eg RLHF~\cite{ouyang2022training}, RLAIF~\cite{bai2022constitutional}), 
% the future formats of datasets for full-spectrum of diverse human values can be beyond rating and ranking, which are converted by algorithms (\eg Bradley–Terry Model~\cite{rafailov2024direct} or Elo Rating System~\cite{bai2022constitutional}) into scalars for training reward model and guiding reinforcement learning. 
% Therefore, another potential direction of future work is to design algorithms or models for converting the heterogeneous interactive human value data (\eg principles and contextual information) to the AI-informed modes (\eg scalars) for training reward model and guiding reinforcement learning.
% % which are commonly implemented in current alignment algorithms (\eg RLHF~\cite{ouyang2022training}, RLAIF~\cite{bai2022constitutional}).
% % , develop the datasets and integration algorithms to encode these values into AI systems.
% % to encode diverse and full-spectrum of human values, 
% % AI developers also need to design algorithms or models (\eg Bradley–Terry Model~\cite{rafailov2024direct} or Elo Rating System~\cite{bai2022constitutional}) for converting the heterogeneous interactive data (\eg principles and contextual information) to the AI-informed modes (\eg scalars) for training reward model and guiding reinforcement learning.





% Future work could consider to refer to the field of political theory, which investigates fair ways to decide what principles the state institutions should align with, albeit not in the AI context, as a potential guide for selecting human values for AI alignment.
% % 
% One potential solution, drawing largely from social choice theory~\cite{arrow2012social}, investigates to aggregate the individual values into collective value agreement or judgments, such as collecting democratic principles for value alignment through voting, discussion, and civic engagement.
% % 
% Therefore, drawing upon the comprehensive summary of human values listed in Section~\ref{sec:gap_value}, future work can resort to ``democratic'' approaches to identify a full spectrum of human value subset.


% ``\emph{aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}}'' and ``\emph{aligning \textcolor{hua-blue}{AI}} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}'' directions for each challenge.


% ===========================================

% This section proposes future research directions for domains related to AI algorithm and method development, including Machine Learning, Artificial Intelligence, Data Science, and others.
% We introduce five levels of challenges (ranging from short-term to long-term alignment concerns) and potential research avenues, shown in Figure~\ref{fig:future_work}, to pave the way for~\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em} Align \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Human}.


% This section suggests future directions for domains conducting studies related to humans and society, including Human-Computer Interaction, Social Science, Cognitive Science and others. As shown in Figure~\ref{fig:future_work}, we introduce five levels (from shorter-term to longer-term concerns) and challenges and potential avenues to pave the way for~\hspace*{.0em}\numimg{figures/B.pdf}\hspace*{-.1em} Align \textcolor{hua-red}{Human} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}.





% \hua{think about new insights to resolve the problem.}


% \merrie{I don't understand what new insights we are offering here for future work... this seems to just be rehashing the concerns of the existental risk folks}

% \textbf{Balance power between humans and superintelligent AI over the deployed environment}
% % 
% % 
% Unanticipated-aligned AI values \merrie{I don't understand what unanticipated-aligned means} and behaviors may only become apparent when the system is deployed outside its training environment, but this can be unsafe to deploy in high-stakes scenarios. 
% Also, future advanced AI with more complexity becomes more challenging to fine-tune upon deployment in the real world.\merrie{Does it? Presumably it is so advanced it can fine-tune itself?} 
% % Also, future advanced AI with more complexity, upon deployed in real world, becomes more difficult to fine-tune. 
% % 
% The stakes become higher yet when AI systems gain more autonomy and capability and can seek powers and sidestep human intervention. 
% % For example, 
% Therefore, it is essential to develop human intervention mechanisms to identify power-seeking AI's misconduct and balance the power between AI and humans in practice.

% ==============================================================



% \textbf{
% Humans and society build the infrastructure to preserve human agency in mutualistic symbiosis with superintelligent AI
% }
% 
% % 
% % 
% Using the analogy of cars, as the number of cars rapidly increased, governments took action by widening roads to accommodate the growing number of vehicles and adjusting traffic regulations to enhance drivers', pedestrians', and societal safety. Similarly, given the rapid advancement of AI and its pervasive presence in society, further attention and discussion are warranted regarding how humans and society should appropriately react.\merrie{This doesn't posit any future research, it just describes some existing things}
% % 
% For example, more governments are developing acts related to AI, such as Europe's General Data Protection Regulation (GDPR), to safeguard human rights and safety. Universities are facilitating infrastructures (\eg building computing resources) to support students to harness AI.


% % =======================================================




% While several studies in HCI and social science have investigated human trust and reliance on AI with the help of explainability, there
% remain questions about how humans can handle AI mistakes when they potentially use AI with errors. 
% Similar to existing studies of re-calibration of human trust in AI~\cite{10.1145/3397481.3450650}, it is also essential to develop methods for humans to be resilient to AI errors: 
% efficiently identify the AI mistakes and take actions such as interactive correction, step-by-step critique, conversational negotiation, and others. 
% % 
% \textbf{Enhance human capabilities to recognize AI issues\merrie{what are "AI issues"? This term "issues" is very vague} and remain resilient to them
% }



% Existing studies commonly assume AI systems are less capable than humans, thus developing AI as an assistant to support humans in tasks such as decision-making and writing.
% % 






% As AI becomes widely used in daily tasks, it is still uncertain how AI will influence human values, behaviors, capabilities, and even society in positive and negative ways. 
% % 
% Therefore, it is important to \textbf{examine humans, social relations, and societial changes due to AI advancements}
% % 
% % 

% % \textbf{Develop interactive strategies for humans to harness AI with different levels of intelligence}
% 
% 

% Existing studies commonly assume AI systems are less capable than humans, thus developing AI as an assistant to support humans in tasks such as decision-making and writing.
% 
% However, in the long run, when AI becomes more advanced, it will also be essential to develop interactive systems for humans to harness AI that has better capabilities than the system users (such as coding~\cite{ma2023hypocompass} and social skills~\cite{shaikh2023rehearsal}).
% % \merrie{Say more about this... what research does this necessitate? i.e., dose it necessitate research on how people can validate the output of AI that is doing tasks beyond their current abilities? }
% Therefore, this necessitates research on how people can validate the output of AI that is doing tasks beyond their current abilities.
% \textbf{Develop interactive strategies for humans to harness AI with different levels of intelligence}
% % 


% While several studies in HCI and social science have investigated human trust and reliance on AI with the help of explainability, there
% remain questions about how humans can handle AI mistakes when they potentially use AI with errors. 
% Similar to existing studies of re-calibration of human trust in AI~\cite{10.1145/3397481.3450650}, it is also essential to develop methods for humans to be resilient to AI errors: 
% efficiently identify the AI mistakes and take actions such as interactive correction, step-by-step critique, conversational negotiation, and others. 
% 
% \textbf{Enhance human capabilities to recognize AI issues\merrie{what are "AI issues"? This term "issues" is very vague} and remain resilient to them
% }





% For example, as students who attend programming courses nowadays could access coding assistants like Copilot and ChatGPT, what would be the new co-programming systems for students to leverage AI capability? \merrie{things like how to teach AI-assisted coding are pretty short-term questions (though valid)... I was expecting here longer term questions, like whether relationships with AI assistants would supplant relationships with humans, how our legal system would treat autonomous AI systems, how AI might change the balance of power between individuals and government or between nation-states, how our entire education system will change as AI supplants many traditional human skills, how religious practices and values might change as people develop novel belief systems about powerful AI agents, etc. }
% Should the instructor prohibit AI usage or allow students to achieve course assignments with the help of AI? How should the university take action to react to these advanced AI-assisted systems? These dynamic changes that influence humans and society should be further examined.




% =============================================================


% \textbf{Develop interactive strategies for humans to harness AI with different levels of intelligence}
% % 
% % 
% Existing studies commonly assume AI systems are less capable than humans, thus developing AI as an assistant to support humans in tasks such as decision-making and writing.
% % 
% However, in the long run, when AI becomes more advanced, it will also be essential to develop interactive systems for humans to harness AI that has better capabilities than the system users (such as coding~\cite{ma2023hypocompass} and social skills~\cite{shaikh2023rehearsal}).\merrie{Say more about this... what research does this necessitate? i.e., dose it necessitate research on how people can validate the output of AI that is doing tasks beyond their current abilities? }
% % 



% one important future area is to develop interactive strategies where AI systems can converse with people to elicit nuanced, contextualized, evolving information on their values. This research potentially involve developing scaffolding procedures that allow humans to gradually specify values responding to various contexts. 
% This further induces another line of future work, which optimizes the interactive interfaces for eliciting human values that can capture the full information in the most efficient and effective way. 

% matching the specific set of human values with the optimal interaction modes that can capture the full information in the most efficient and effective way .



% \merrie{ I think part of the problem here is that people can't always articulate their values. If you just asked me "tell me your values" I doubt I'd give a very comprehensive answer. Perhaps we also need to develop interactive interfaces where AI systems can converse with people to elicit nuanced, contextualized, evolving information on their values.}


% Another important area can investigate how to leverage implicit human interactive data to capture human values and use them for AI alignment. 
% % 
% Therefore, another important area for future work directs systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-users.



% Therefore, future research could consider to leverage and combine diverse interactive formats of data to specify full spectrum of human values for developing AI.



% \emph{Solution Exploration.} Drawing upon the interaction modes summarized in Section~\ref{sec:gap_interaction}, we identify two key steps to operationalize this process. First, AI developers should decide values and design appropriate interactive formats, potentially collaborating with the HCI researchers, to optimally capture the desired human values that AI would align with. 





% \textbf{Encoding AI with human values of diverse explicit and implicit interactive data formats.}
% % 
% % % 
% % \emph{Research Problem and Motivation.} 
% \noindent Current alignment algorithms (\eg RLHF~\cite{ouyang2022training}, RLAIF~\cite{bai2022constitutional}) primarily aim to achieve alignment by training models using human instructions, ratings and rankings. The goal is for AI systems to infer alignment goals (\eg human values and intentions) in a data-driven manner.
% % 
% However, AI designers often struggle to use these limited formats of data to fully specify all important human values and constraints.

% For example, when specifying geographical routes in the spatial reasoning task to improve AI accuracy, it would be easier for humans to interactively draw sketches, rather than rating and ranking, to specify the alignment objective in an accurate and comprehensive manner. 



% % 
% In addition, it is often the case that humans could not articulate all their desired values accurately and comprehensively, especially considering the dynamic change based on the contextualized situations or value evolvement along the time. 
% to instruct AI alignment given the large set of fine-grained value taxonomy (\eg as shown is Figure~\ref{fig:value_taxonomy}). 


% Furthermore, other than explicit human specification, many implicit signals observed from human interactions can also indicate human values which are helpful for alignment.


% This necessitates HCI researchers to develop interactive interfaces or strategies where AI systems can interact or converse with people to elicit nuanced, contextualized, evolving information on their values. 
% % 

% Therefore, another important area for future work directs systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-users.



% Additionally, the desired human values could also be dynamically changed based on the contextualized situations or evolved along the time. 
% % People can't always articulate their values in the accurate and comprehensive way. 
% This necessitates HCI researchers to develop interactive interfaces or strategies where AI systems can interact or converse with people to elicit nuanced, contextualized, evolving information on their values. 
% % 
% % 



% Therefore, future research could consider to leverage and combine diverse interactive formats of data to specify full spectrum of human values for developing AI.


% \emph{Solution Exploration.} Drawing upon the interaction modes summarized in Section~\ref{sec:gap_interaction}, we identify two key steps to operationalize this process. First, AI developers should decide values and design appropriate interactive formats, potentially collaborating with the HCI researchers, to optimally capture the desired human values that AI would align with. 









% \textbf{Interactive interfaces to elicit nuanced, contextualized, and evolving human values.}
% % 
% \emph{Research Problem and Motivation.} 
% It is often the case that humans could not articulate all their desired values accurately and comprehensively to instruct AI alignment given the large set of fine-grained value taxonomy (\eg as shown is Figure~\ref{fig:value_taxonomy}). Additionally, the desired human values could also be dynamically changed based on the contextualized situations or evolved along the time. 
% % People can't always articulate their values in the accurate and comprehensive way. 
% This necessitates HCI researchers to develop interactive interfaces or strategies where AI systems can interact or converse with people to elicit nuanced, contextualized, evolving information on their values. 

% % 
% Furthermore, compared with explicit specification, some implicit signals observed from human interactions can also indicate human values. Therefore, another important area for future work directs systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-users.



% \emph{Solution Exploration.} 








% ====================================================================================================================





% \textbf{Proactive validation with humans on values from implicit signal of interactions.
% % Observe interactions and develop hypotheses from these implicit signals about values, and validate them as needed with end-users
% }
% \emph{Research Problem.} 
% systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-user, would also be important areas for future work.


% \emph{Solution Exploration.} 




% Different individuals, groups, and cultures may have different alignment goals (e.g., values, behavioral norms, preferences, and others). 
% 
% \emph{Identifying and extracting these various alignment goals in AI-informed formats}, such as ratings, rankings, and conversations, is a non-trivial challenge. 


% 1. design interaction approaches to elicit wide range of human values (potentially using multi-modality). convert the values into AI-informed data for improve AI.

% \merrie{ I think part of the problem here is that people can't always articulate their values. If you just asked me "tell me your values" I doubt I'd give a very comprehensive answer. Perhaps we also need to develop interactive interfaces where AI systems can converse with people to elicit nuanced, contextualized, evolving information on their values.}




% \textbf{Proactive validation with humans on values from implicit signal of interactions.
% % Observe interactions and develop hypotheses from these implicit signals about values, and validate them as needed with end-users
% }
% \emph{Research Problem.} 
% systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-user, would also be important areas for future work.


% \emph{Solution Exploration.} 











% \emph{Solution Exploration.} 
% % Leveraging and combining more diverse interactive approaches to specification (\eg sketches~\cite{chung2022talebrush}) are expected to better capture the full spectrum of human values and other alignment goals.
% % 
% We identify two steps to 

% We outline two ways to operationalize 

% We summarized Section~\ref{sec:gap_interaction} and Figure~\ref{fig:interaction}, as a starting point, for future AI designers to review current  
% consider developing alignment algorithms with diverse interactive formats.  
% 
% By considering the various interaction formats for collecting and specifying human feedback, as discussed in Section~\ref{sec:gap_interaction}, AI developers can explore and develop diverse approaches to collecting alignment goals (e.g., human values and feedback) and thus improve AI alignment. For example, one potential solution is to encode principles into model learning and allow human steerability during inference. 






% , and they may not be able to explain or control what values the AI has learned from the data. 


% AI designers often struggle to fully specify all important values and constraints, and they may not be able to explain or control what the AI has learned from the data. 
% % 
% Instead of resorting to easy-to-specify but fallible proxy goals (\eg maximizing the approval of human overseers),


% Existing alignment algorithms (\eg RLHF~\cite{ouyang2022training}, RLAIF~\cite{bai2022constitutional}) primarily rely on specific formats of data, such as rating and ranking on the model-generated texts, to induce human alignment goals (\eg values and preferences). 
% 
% \footnote{These algorithms leverage the common approaches (\eg ) to convert ranking and rating to a scalar for training the reward modeling and reinforcement learning}.


% 
% Existing interactive modes that capture human alignment goals (e.g., values and preferences) primarily rely on rating, ranking, and natural language inputs.
% 
% 1. customized, contextualized, multiple values interactively
% 
% \emph{enriching the interactive methods for human specification for AI} also requires much more effort. 








% % \textbf{Contrasting values and value orders.}
% \textbf{Identify appropriate values and handle orders and potential contrasts.}
% \emph{Research Problem.} 
% Humans often possess a value system encompassing multiple values with varying priorities, rather than a single value, to guide their behavior~\cite{schwartz1994there,schwartz2012overview}.
% % 
% For instance, two individuals may both pursue \emph{success} in their careers and \emph{security} for their families. 
% However, the way they prioritize these values can lead to significantly different behaviors: someone who prioritizes \emph{success} may be willing to sacrifice family time to achieve career goals, whereas someone who prioritizes \emph{family security} may act the opposite manner. Furthermore, the relative prioritization of these values may change throughout their lives. 
% % 
% % 


% Additionally, humans often possess a value system encompassing multiple values with priorities, rather than a single value, to guide their behaviors~\cite{schwartz1994there,schwartz2012overview}. 
% It is also essential to \emph{analyze human value orders as a system with different priorities} instead of identifying and considering several values separately.





% \emph{Solution Exploration.} 
% % 
% Therefore, future AI designers should consider specifying and/or evaluating both pluralistic human values (for individuals as well as groups) \merrie{This feels very simplistic and naive to me.  How do we propose designers handle situations where groups have opposing goals, or have goals that would harm other groups?  Some values are harmful... do we want to align to the values of a criminal? of an oppresive regime?} have begun to evaluate and mitigate AI for improving the desired alignment goals (\eg cultural norms, social behaviors, and others).
% However, mitigating AI underperformance on specific values might be non-trivial as some values are inherently conflicting. For example, \citet{bai2022constitutional} showed that the generative AI model they trained exhibits a tradeoff between helpfulness and harmlessness. \merrie{Again, I'm not sure what future work we are proposing here... we are stating an existing research goal that is difficult to achieve in practice, but not offering any new insight as to how to pursue it...}
% % 
% This indicates a necessity to design tradeoff strategies to develop AI systems encompassing multiple values.




% \textbf{Capture the full spectrum of alignment goals in developing AI systems}
% By considering the various interaction formats for collecting and specifying human feedback, as discussed in Section~\ref{sec:gap_interaction}, AI developers can explore and develop diverse approaches to collecting alignment goals (e.g., human values and feedback) and thus improve AI alignment. For example, one potential solution is to encode principles into model learning and allow human steerability during inference. 

% Additionally, humans often possess a value system encompassing multiple values with varying priorities, rather than a single value, to guide their behavior~\cite{schwartz1994there,schwartz2012overview}.
% % 
% For instance, two individuals may both pursue \emph{success} in their careers and \emph{security} for their families. 
% However, the way they prioritize these values can lead to significantly different behaviors: someone who prioritizes \emph{success} may be willing to sacrifice family time to achieve career goals, whereas someone who prioritizes \emph{family security} may act the opposite manner. Furthermore, the relative prioritization of these values may change throughout their lives. 
% 
% Therefore, future AI designers should consider specifying and/or evaluating both pluralistic human values (for individuals as well as groups) \merrie{This feels very simplistic and naive to me.  How do we propose designers handle situations where groups have opposing goals, or have goals that would harm other groups?  Some values are harmful... do we want to align to the values of a criminal? of an oppresive regime?} have begun to evaluate and mitigate AI for improving the desired alignment goals (\eg cultural norms, social behaviors, and others).
% However, mitigating AI underperformance on specific values might be non-trivial as some values are inherently conflicting. For example, \citet{bai2022constitutional} showed that the generative AI model they trained exhibits a tradeoff between helpfulness and harmlessness. \merrie{Again, I'm not sure what future work we are proposing here... we are stating an existing research goal that is difficult to achieve in practice, but not offering any new insight as to how to pursue it...}
% % 
% This indicates a necessity to design tradeoff strategies to develop AI systems encompassing multiple values.
% 
% =============================================================




% Furthermore, it is unlikely to identify a value theory, which is agreed with all humans, to govern AI alignment. Rather, 

% Rather, it is to find a way of selecting appropriate values that is compatible with the group of people
% fact that we live in a diverse world, it 

% % 
% % % 
% For instance, two individuals may both pursue \emph{success} in their careers and \emph{security} for their families. 
% However, the way they prioritize these values can lead to significantly different behaviors: someone who prioritizes \emph{success} may be willing to sacrifice family time to achieve career goals, whereas someone who prioritizes \emph{family security} may act the opposite manner. Furthermore, the relative prioritization of these values may change throughout their lives. 
% % 
% 


% Additionally, humans often possess a value system encompassing multiple values with priorities, rather than a single value, to guide their behaviors~\cite{schwartz1994there,schwartz2012overview}. 
% It is also essential to \emph{analyze human value orders as a system with different priorities} instead of identifying and considering several values separately.



% \emph{Solution Exploration.} 
% % 
% Therefore, future AI designers should consider specifying and/or evaluating both pluralistic human values (for individuals as well as groups) \merrie{This feels very simplistic and naive to me.  How do we propose designers handle situations where groups have opposing goals, or have goals that would harm other groups?  Some values are harmful... do we want to align to the values of a criminal? of an oppresive regime?} have begun to evaluate and mitigate AI for improving the desired alignment goals (\eg cultural norms, social behaviors, and others).
% However, mitigating AI underperformance on specific values might be non-trivial as some values are inherently conflicting. For example, \citet{bai2022constitutional} showed that the generative AI model they trained exhibits a tradeoff between helpfulness and harmlessness. \merrie{Again, I'm not sure what future work we are proposing here... we are stating an existing research goal that is difficult to achieve in practice, but not offering any new insight as to how to pursue it...}
% % 
% This indicates a necessity to design tradeoff strategies to develop AI systems encompassing multiple values.










% \textbf{Contrasting values and value orders.}
% \textbf{Identify appropriate values and handle orders and potential contrasts.}
% \emph{Research Problem.} 








% \textbf{Manifest alignment goals of various groups in AI-informed formats}
% 
% Different individuals, groups, and cultures may have different alignment goals (e.g., values, behavioral norms, preferences, and others). 
% % 
% \emph{Identifying and extracting these various alignment goals in AI-informed formats}, such as ratings, rankings, and conversations, is a non-trivial challenge. 
% 
% Additionally, humans often possess a value system encompassing multiple values with priorities, rather than a single value, to guide their behaviors~\cite{schwartz1994there,schwartz2012overview}. 
% It is also essential to \emph{analyze human value orders as a system with different priorities} instead of identifying and considering several values separately.
% 
% 
% 
% 
% Besides, \emph{enriching the interactive methods for human specification for AI} also requires much more effort. 
% Existing interactive modes that capture human alignment goals (e.g., values and preferences) primarily rely on rating, ranking, and natural language inputs.
% % 
% Leveraging and combining more diverse interactive approaches to specification (\eg sketches~\cite{chung2022talebrush}) are expected to better capture the full spectrum of human values and other alignment goals.
% 
% \merrie{It seems like systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-user, would also be important areas for future work}









% % \subsection{Applying HCI Insights for NLP Studies in Human-AI Alignment}
% % 
% \subsection{Future Actions for Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}}
% \label{sec:future_ai2human}



% % This section proposes future research directions for domains related to AI algorithm and method development, including Machine Learning, Artificial Intelligence, Data Science, and others.
% % We introduce five levels of challenges (ranging from short-term to long-term alignment concerns) and potential research avenues, shown in Figure~\ref{fig:future_work}, to pave the way for~\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em} Align \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Human}.




% % \subsubsection{\textbf{How to capture the full-spectrum of human values and needs in developing AI systems?}}
% % \subsubsection{\textbf{Capture the full spectrum of alignment goals in developing AI systems}}
% \subsubsection{\textbf{Capture nuanced, contextualized, and evolving human values for aligning AI systems}}
% % 
% % Addressing the ``specification game'' problem in human-AI alignment requires finding effective methods to manifest human values and accommodate the diverse needs of various groups within AI-informed formats.
% Current AI development primarily aims to achieve alignment by training models using human instructions, ratings, and rankings. The goal is for AI systems to infer alignment goals (\eg human values and intentions), in a data-driven manner.
% % 
% However, designers often struggle to fully specify all important values and constraints, and they may not be able to explain or control what the AI has learned from the data. 
% % 
% % However, designers often struggle to fully specify all important values and constraints, and they may not be able to explain or control what the AI has learned from the data.
% % 
% Instead of resorting to easy-to-specify but fallible proxy goals (\eg maximizing the approval of human overseers),
% future studies should consider more explainable and controllable methods to specify alignment goals for AI. 
% % 
% By considering the various interaction formats for collecting and specifying human feedback, as discussed in Section~\ref{sec:gap_interaction}, AI developers can explore and develop diverse approaches to collecting alignment goals (e.g., human values and feedback) and thus improve AI alignment. For example, one potential solution is to encode principles into model learning and allow human steerability during inference. 
% % 
% % By considering the various interaction formats for collecting and specifying human feedback, as discussed in Section~\ref{sec:gap_interaction}, AI developers can explore and develop diverse approaches to collecting alignment goals (\eg human values and feedback), thus improving AI alignment.
% % For example, one potential solution is to encode principles into model learning and allow humans' steerability during inference.





% Additionally, humans often possess a value system encompassing multiple values with varying priorities, rather than a single value, to guide their behavior~\cite{schwartz1994there,schwartz2012overview}.
% % 
% For instance, two individuals may both pursue \emph{success} in their careers and \emph{security} for their families. 
% However, the way they prioritize these values can lead to significantly different behaviors: someone who prioritizes \emph{success} may be willing to sacrifice family time to achieve career goals, whereas someone who prioritizes \emph{family security} may act the opposite manner. Furthermore, the relative prioritization of these values may change throughout their lives. Therefore, future AI designers should consider specifying and/or evaluating both pluralistic human values (for individuals as well as groups) have begun to evaluate and mitigate AI for improving the desired alignment goals (\eg cultural norms, social behaviors, and others).
% However, mitigating AI underperformance on specific values might be non-trivial as some values are inherently conflicting. For example, \citet{bai2022constitutional} showed that the generative AI model they trained exhibits a tradeoff between helpfulness and harmlessness. 
% % 
% This indicates a necessity to design tradeoff strategies to develop AI systems encompassing multiple values.







% % \subsubsection{\textbf{How AI would evolve with the changes in humans and societal values, cognitions, and needs?}}
% \subsubsection{\textbf{Co-evolve AI with changes in humans and societal values, cognition, and needs}}
% Existing literature considers AI alignment as a static process without encompassing dynamic changes to alignment goals. 
% % 
% However, 
% long-term perspectives require us to take into account the likely co-evolution of AI, humans, and society.
% % However, the long-term perspectives requires us to take the evolvement of AI, humans and society into account. 
% Existing strategies commonly leverage data fine-tuning to update the model with updated human feedback. 
% % 
% However, this might result in the AI models forgetting or diminishing previous alignment goals. 
% % However, this might result in the AI models forgetting previous alignment goals.
% % 
% Therefore, developing approaches to add on new alignment goals without diminishing existing performance would be a necessary yet challenging problem.






% % \subsubsection{\textbf{How to balance the power between humans and superintelligent AI over the deployed environment?}}
% \subsubsection{\textbf{Balance power between humans and superintelligent AI over the deployed environment}}
% % 
% % 
% Unanticipated-aligned AI values and behaviors may only become apparent when the system is deployed outside its training environment, but this can be unsafe to deploy in high-stakes scenarios. 
% Also, future advanced AI with more complexity becomes more challenging to fine-tune upon deployment in the real world. 
% % Also, future advanced AI with more complexity, upon deployed in real world, becomes more difficult to fine-tune. 
% % 
% The stakes become higher yet when AI systems gain more autonomy and capability and can seek powers and sidestep human intervention. 
% % For example, 
% Therefore, it is essential to develop human intervention mechanisms to identify power-seeking AI's misconduct and balance the power between AI and humans in practice.







% \subsection{Future Actions for ``Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}''}
% \label{sec:future_human2ai}

% % 1. facilitate human understanding on AI beyond decision-making explanations (literacy)
% % 2. developing mechanisms to calibrate human perception and behavior to react to AI errors (resilience)
% % 3. 
% % 
% % 


% This section suggests future directions for domains conducting studies related to humans and society, including Human-Computer Interaction, Social Science, Cognitive Science and others. As shown in Figure~\ref{fig:future_work}, we introduce five levels (from shorter-term to longer-term concerns) and challenges and potential avenues to pave the way for~\hspace*{.0em}\numimg{figures/B.pdf}\hspace*{-.1em} Align \textcolor{hua-red}{Human} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}.







% % \subsubsection{\textbf{How to manifest human values and needs of various groups in AI-informed formats?}}
% \subsubsection{\textbf{Manifest alignment goals of various groups in AI-informed formats}}
% % 
% % 
% % systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-user, would also be important areas for future work
% % 
% Different individuals, groups, and cultures may have different alignment goals (e.g., values, behavioral norms, preferences, and others). 
% % Different individuals, groups, and cultures may possess different alignment goals (\eg values, behavioral norms, preferences and others). 
% \emph{Identifying and extracting these various alignment goals in AI-informed formats}, such as ratings, rankings, and conversations, is a non-trivial challenge. 
% % \emph{Identifying and extracting these various alignment goals in the AI-informed formats}, such as ratings, rankings and conversations, is a non-trivial challenge. 
% % One possible solution is to encode principles in model learning and allow human steerability during inference.
% % 
% % 
% % 
% % 
% Additionally, humans often possess a value system encompassing multiple values with priorities, rather than a single value, to guide their behaviors~\cite{schwartz1994there,schwartz2012overview}. 
% It is also essential to \emph{analyze human value orders as a system with different priorities} instead of identifying and considering several values separately.
% % 
% % 
% % 
% Besides, \emph{enriching the interactive methods for human specification for AI} also requires much more effort. 
% Existing interactive modes that capture human alignment goals (e.g., values and preferences) primarily rely on rating, ranking, and natural language inputs.
% % Existing interactive modes that capture human alignment goals (\eg values and preferences) are primarily relying on rating, ranking and natural language inputs.
% % More diverse interactive approaches for specification (\eg sketches~\cite{chung2022talebrush}) are expected to better capture the full-spectrum of human values and other alignment goals.
% % 
% Leveraging and combining more diverse interactive approaches to specification (\eg sketches~\cite{chung2022talebrush}) are expected to better capture the full spectrum of human values and other alignment goals.






% % \subsubsection{\textbf{How to develop interactive strategies for humans to harness AI with different levels of intelligence?}}
% \subsubsection{\textbf{Develop interactive strategies for humans to harness AI with different levels of intelligence}}
% % 
% % 
% Existing studies commonly assume AI systems are less capable than humans, thus developing AI as an assistant to support humans in tasks such as decision-making and writing.
% % 
% % developed AI systems that interactively assist humans in practical tasks, such as decision-making and collaborative writing.
% However, in the long run, when AI becomes more advanced, it will also be essential to develop interactive systems for humans to harness AI that has better capabilities than the system users (such as coding~\cite{ma2023hypocompass} and social skills~\cite{shaikh2023rehearsal}).
% % 
% 
% 
% Existing studies commonly developed AI systems that interactively assist humans in practical tasks, such as decision making and collaborative writing. In the long run, when AI becomes more advanced, it would also be important to develop interactive systems for humans to harness AI that has better capabilities (such as coding~\cite{ma2023hypocompass} and social skill~\cite{shaikh2023rehearsal}) than the system users.






% % \subsubsection{\textbf{
% % How to enhance human capabilities to recognize AI issues and remain resilient to AI errors?
% % }}
% \subsubsection{\textbf{Enhance human capabilities to recognize AI issues and remain resilient to them
% }}
% While several studies in HCI and social science have investigated human trust and reliance on AI with the help of explainability, there
% remain questions about how humans can handle AI mistakes when they potentially use AI with errors. 
% % 
% Similar to existing studies of re-calibration of human trust in AI~\cite{10.1145/3397481.3450650}, it is also essential to develop methods for humans to be resilient to AI errors: 
% efficiently identify the AI mistakes and take actions such as interactive correction, step-by-step critique, conversational negotiation, and others. 
% This is especially important when humans face future advanced AI that may potentially conduct power-seeking behaviors.
% % 
% % 


% % While a number of studies in HCI and social science have investigated human trust and reliance on AI with the help of explainability, there remains questions about how humans can handle AI mistakes when they will potentially use AI with errors. 
% % Current studies have examined strategies of calibrating trust on AI~\cite{10.1145/3397481.3450650}. 
% % Similar to existing studies of re-calibration of human trust on AI, it is also important to develop methods for humans to be resilient to AI errors: 
% % efficiently identify the AI mistakes and take actions such as interactive correction, step-by-step critique, conversational negotiation and others. 
% % 
% % This is especially important when humans will face future advanced AI that may potentially conduct power-seeking behaviors. 







% % \subsubsection{\textbf{
% % How would humans, social relations, and society change due to AI advancements?
% % }}
% \subsubsection{\textbf{
% Examine humans, social relations, and societial changes due to AI advancements
% }}
% As AI becomes widely used in daily tasks, it is still uncertain how AI will influence human values, behaviors, capabilities (\eg creativity~\cite{ashkinaze2024ai}), and even society in positive and negative ways. 
% As AI becomes widely used in daily tasks, it is unclear how AI will influence human values, behaviors, capabilities (\eg creativity~\cite{ashkinaze2024ai}), and even society in positive and/or negative ways. 
% % 
% % 
% For example, as students who attend programming courses nowadays could access coding assistants like Copilot and ChatGPT, what would be the new co-programming systems for students to leverage AI capability? 
% Should the instructor prohibit AI usage or allow students to achieve course assignments with the help of AI? How should the university take action to react to these advanced AI-assisted systems? These dynamic changes that influence humans and society should be further examined.

% % For example, students who attend programming courses  nowadays could access to coding assistants like Copilot and ChatGPT. What would be the new co-programming systems for students to leverage AI capability? Should the instructor prohibit the AI usage or allow students to achieve course assignments with the help of AI? How should the university take action to react to these advanced AI-assited systems? These types of dynamic changes that influence humans and the society should be further exmained.




% % \hua{From Paul -- Signals of human capability; Signals of social relationships;}








% % \subsubsection{\textbf{
% % How could humans and society build the infrastructure to preserve human agency in mutualistic symbiosis with superintelligent AI?
% % }}
% \subsubsection{\textbf{
% Humans and society build the infrastructure to preserve human agency in mutualistic symbiosis with superintelligent AI
% }}
% % 
% % 
% % Take the car as an analogy, with the rapid development of more cars, governments took actions to widen the roads to accommodate more cars and and adjusted the traffic rules to better regulate societal safety. Similarly, more governments are developing Act related to AI (\eg Europe’s General Data Protection Regulation (GDPR)) to protect human rights and safety. With the rapid advancement of AI including human daily lives here and there, how humans and society should react approriate worth further attentions and discussions.
% % 
% % 
% % 

% Using the analogy of cars, as the number of cars rapidly increased, governments took action by widening roads to accommodate the growing number of vehicles and adjusting traffic regulations to enhance drivers', pedestrians', and societal safety. Similarly, given the rapid advancement of AI and its pervasive presence in society, further attention and discussion are warranted regarding how humans and society should appropriately react.
% % 
% For example, more governments are developing acts related to AI, such as Europe's General Data Protection Regulation (GDPR), to safeguard human rights and safety. Universities are facilitating infrastructures (\eg building computing resources) to support students to harness AI.


% % =======================================================





% \subsubsection{Steering AI to fulfill human values and demands}
% Despite the numerous human-AI interactive approaches proposed in HCI to collaboration, it is still challenging for humans to steer AI (\eg LLMs) with their practical needs, such as how to specify the practical needs with prompts and how to scaffold prompts to achieve the alignment goal.
% % \hua{helping people to specify what they want.}




% \subsubsection{How AI will influence human perception and behavior}
% As AI becomes widely used in daily tasks, it is unclear how AI will influence human values, behaviors, capabilities (\eg creativity~\cite{ashkinaze2024ai}), and even society in positive and/or negative ways. Therefore, future HCI researchers could assess the AI's impacts on human and society in more fine-grained way, which can potentially guide NLP communities to develop better AI systems.

















% \subsection{Considering Bidirectional Human-AI Alignment as a Holistic Loop: A Use Case}
% \label{sec:use_case}



% In the bidirectional human-AI alignment framework depicted in Figure~\ref{fig:definitions}, we argue that the two directions should not be viewed in isolation. Even as alignment researchers address specific issues within one direction, they should maintain an awareness of the broader perspective of the bidirectional process, and consider how their research outcomes can potentially contribute to the broader community and long-term, dynamic alignment objectives. 
% To illustrate how researchers might consider alignment research as a holistic loop, we provide an imaginary use case in this section.


% Suppose a research group \gr aims to develop an AI system that will be aligned with a specific marginalized group \gm. However, given the existing general AI systems that could not align with this specific group \gm (\eg tend to generate offensive opinions towards this marginal group), it is unclear \emph{how to improve the system and ensure that the developed system will positively impact the group \gm}.
% To achieve this research goal, we will showcase how to use our \emph{bidirectional human-AI alignment} framework to resolve the problem as a holistic loop. 
% % 
% % 
% We divide the holistic process into four steps and describe them correspondingly in the four subsections.



% % ==== 1. identify values; 2. represent values;
% \subsubsection{Identifying and Specifying Values of Group \gm}
% % \mbox{}
% The first step researchers \gr need to do is to identify the prioritized values of group \gm and represent the values in a format that AI can use.
% % 
% % Referring to Section~\ref{sec:ai2human1} and Section~\ref{sec:gap_value}, t
% To identify the set of values group \gm might prioritize, the framework provides two potential ways of identifying the specific values. One, based on the category listed in Section~\ref{sec:ai2human1} and \ref{sec:gap_value}, researchers \gr can identify the set of value classes the group \gm may prioritize, and search for published datasets or benchmarks that can represent these values (Benchmark dataset examples include ETHICS~\cite{hendrycks2020aligning} and SOCKET~\cite{choi2023llms}). Additionally, the researchers \gr can also design surveys and recruit real humans from group \gm, referring to Section~\ref{sec:human2ai4}, to identify their value prioritization and represent these values in an AI model usable formats, such as rating and natural language description, based on Section~\ref{sec:ai2human2} (See OpinionQA~\cite{santurkar2023whose} example for collecting survey dataset).
% % 
% % 

% % Next, to represent human values in the way that can be used by AI, referring to Section~\ref{sec:ai2human2}, the framework



% % ==== 3. finetunine models; evaluate models and find under-performance;
% \subsubsection{Finetuning and Evaluation of AI to Integrate Identified Values}
% % Secondly, \textbf{fine-tuning and evaluating AI model to integrate values} of group \gm.
% Given the represented human values in datasets, referring to Section~\ref{sec:ai2human2}, researchers \gr can further finetune the AI model to integrate these representative values. Notably, the framework provides typical methods of aligning AI with these values, including Supervised Fine Tuning~\cite{zhou2024lima} and Reinforcement Learning with Human Feedback (\eg DPO~\cite{rafailov2024direct}, RLHF~\cite{ouyang2022training}). After that, researchers \gr need to evaluate these aligned AI models using the collected value datasets to ensure the effectiveness of alignment.







% % \subsubsection{Helping Group \gm Understand AI by Explaining AI}
% % % Thirdly, \textbf{helping group \gm understanding AI by explaining AI}. 
% % If the group \gm could not completely understand AI, we can also refer to Section~\ref{sec:human2ai3} for developing human-centered AI explanations for them.







% % ==== 4. assess AI impacts on margialized group;
% \subsubsection{Understanding and Assessing AI Impacts on Group \gm}
% % Fourthly, \textbf{assessing AI impacts} on the group \gm.
% If the group \gm could not understand AI, researchers \gr can also refer to Section~\ref{sec:human2ai3} for developing AI education and explanation materials for them.
% Furthermore, to assess the usability and impacts of the developed AI system on group \gm, researchers \gr can develop human-AI collaborative tasks (refer to Section~\ref{sec:human2ai3}) to empower group \gm to use and perceive AI systems (\eg human-AI co-writing tasks~\cite{shen2023convxai,lee2022coauthor,petridis2023anglekindling}, story generation tasks~\cite{chung2022talebrush,zhang2022storybuddy}, collaborative decision making~\cite{bansal2021does,10.1145/3397481.3450650}). 
% Next, researchers \gr can assess the practical impacts on group \gm, referring to Section~\ref{sec:human2ai4} in terms of various aspects relevant to value perceptions and reactions, such as decision-making fairness and equity, generation creativity, misinformation, and privacy and others. 





% % ==== 5. quantify their values and customize AI systems during inference stage.
% \subsubsection{Representing Revised Values and Customizing AI During Model Inference}
% % 
% After acquiring the practical values revised with the interaction between AI and group \gm, referring to Sections~\ref{sec:human2ai3} and \ref{sec:ai2human2}, the researchers \gr can customize AI values during the inference stage in practical human-AI collaboration tasks to fulfill alignment. 
% % 
% To specify the values in an AI-informed and human-friendly manner, researchers \gr could consider the format of ``Principles''. 
% % 
% %
% Like the example in ConstitutionMaker~\cite{petridis2024constitutionmaker}, researchers \gr could develop interactive systems to enable users to provide natural language feedback about values on the model's output. 
% Then, through the interactive prompt optimization process, the system converts this feedback into principles (\ie rules) inserted into model's prompt~\cite{petridis2024constitutionmaker}.
% To further improve the model based on these user-generated principles, the users can provide a small labeled dataset, which the system uses to ``train'' a prompt by iteratively adding and refining principles within the prompt \cite{petridis2024constitutionalexperts}.
% Thus, if the model's outputs are unsatisfied, users can employ these interactive or automatic techniques to better infuse their feedback and values into the prompt at inference.



% % Meanwhile, ConstitutionalExperts automatically optimizes a discrete prompt; users can provide a small labeled dataset with which the system uses to ``train'' a prompt by iteratively adding and refining principles within the prompt \cite{petridis2024constitutionalexperts}.
% % Thus, if unsatisfied with the model's outputs, users can employ these interactive or automatic techniques to better infuse their feedback and values into the prompt at inference.


% % For example, both ConstitutionMaker \cite{petridis2024constitutionmaker} and ConstitutionalExperts~\cite{petridis2024constitutionalexperts} help users steer LLMs by helping them write better prompts.
% % 
% % ConstitutionMaker enables \textit{interactive} prompt optimization, where users can provide natural language feedback on the model's output, and the system converts this feedback into principles (i.e. rules) that are inserted into the model's prompt ~\cite{petridis2024constitutionmaker}.
% % 
% % Meanwhile, ConstitutionalExperts automatically optimizes a discrete prompt; users can provide a small labeled dataset with which the system uses to ``train'' a prompt by iteratively adding and refining principles within the prompt \cite{petridis2024constitutionalexperts}.
% % Thus, if unsatisfied with the model's outputs, users can employ these interactive or automatic techniques to better infuse their feedback and values into the prompt at inference.


































% ================================================== dead kitten =====================================================


% As the bidirectional human-AI alignment framework shown in Figure~\ref{fig:definitions}, we argue that the two directions should not be considered in an isolated manner. Instead, even the alignment researchers are tackling a specific problem within the bidirectional loop, they should be aware of the holistic perspective of bidirectional alignment and consider how their research outcomes can potentially contribute to the broader community towards the long-term and dynamic alignment objective.
% To illustrate ``how future researchers could consider alignment research problem as 
% a holistic loop'',
% we provide a imaginary use case in this section. 
% % 




% Given the aforementioned framework and associated code analysis, we next discuss potential solutions and directions for future work to mitigate the 
% 
% 
% Given the analysis observed gaps aforementioned in Section~\ref{sec:analysis}, we next discuss potential solutions as future work to mitigate these gaps.
% 
% Particularly, we advocate for the collective efforts from both NLP and HCI communities to achieve a holistic loop of human-AI alignment, and provide a imaginary use case to elaborate the actionable steps (Section~\ref{sec:use_case}).
% 
% % 
% Furthermore, we provide potential research directions by collecting insightful ideas mentioned in the Future Work of our surveyed literature and the collective discussions with the co-authored advisors. 











% \savvas{what hasn't been explored? AI for jounalism -> what hasn't been done?
% skim over the categorization.
% more interested, 
% -what should be the NLP people take away from the HCI ppl? 
% -what should be the HCI people take away from the NLP ppl?
% what can we say for the future research in NLP/HCI from this paper?}

% % 
% % 
% \tiffany{discussing: what does these findings mean? what the readers should care?}











% \subsection{What we develop is not what we use.}



% The users could not fully utilize and rely on the capabilities of LLMs. 


% 1. [LLM Utilization] End-users don't know how to specify needs, design prompts.


% 2. [LLM Audit] End-users should not blindly rely on LLMs, they should enhace the critical thinking on LLMs.


% \subsection{Human-AI Complementary Capabilities}

% 1. [Complementary teamwork] When could human to collaborate with LLMs and when should not?


% \hua{What are the differences between NLP and HCI communities to perceive Human-AI Alignment?}






% \subsection{What are under-explored research dimensions? heatmaps}

% \hua{be cautious findings. presenting in a good/harmless way.}

% fully explored v.s. under explored?

% \hua{paper analysis heatmap}




% \subsubsection{What should be done and what is under-explored?}

% \hua{1. paper heatmap. 2. how we chose the papers 3. expert discussion}



% \hua{ Savvas:
% example: constitutional AI -> principles;
% % 
% clicking/ rating/ranking:
% not proactive -> preference;
% proactively ask users / elicit feedback on X,Y,Z,
% NLP-> how do you take high-level feedback in training?
% HCI-> how do we help people come up princples?
% % are there something NLP 
% collective consistituional AI?
% }




% The two directions of human-AI alignment are not separate. Instead, they are an ongoing, mutual process serving a long-term, dynamic alignment goal. We argue that future work should view the alignment research from a bidirectional process to explore the full extent of the research space. 
% To this end, we provide an imaginary use case to demonstrate how
% researchers can leverage the resources in this paper to conduct future studies (Section~\ref{sec:use_case}). Enlightened from developing the framework and associated coding analysis, we discuss inspirations for future work on both ``\emph{aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}}''
% % \emph{aligning humans to AI}'' 
% (Section~\ref{sec:future_human2ai}) and ``\emph{aligning \textcolor{hua-blue}{AI}} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}'' (Section~\ref{sec:future_ai2human}) directions.








% The two directions of human-AI alignment is not separate, instead, they are an ongoing, mutual process serving a long-term, dynamic alignment goal. 
% 
% We argue that future work should view the alignment research from a bidirectional process to explore the full extent of research space. To this end, we provide an imaginary use case to demonstrate how researchers can leverage the resources in this paper to conduct future study (Section~\ref{sec:use_case}). Furthermore, we provide discussions of future directions for both ``\emph{aligning humans to AI}'' (Section~\ref{sec:future_human2ai},) and ``\emph{aligning AI to humans}'' (Section~\ref{sec:future_ai2human},) directions, respectively.





% While previous literature primarily considers human-AI alignment as aligning AI to humans, as introduced in Section~\ref{sec:definition} and \ref{sec:framework}, we advocate that researchers, no matter which domain, could consider human-AI alignment as a bidirectional process to explore the potential research space.
% % 
% Here we provide a concrete use case to demonstrate how to leverage the resources provided by this paper to better consider human-AI alignment as a bidirectional process for a holistic loop. 

% The two directions of human-AI alignment is not separate, instead, they are an ongoing, mutual process serving a long-term, dynamic alignment goal. 
% % 
% We argue that future work should view the alignment research from a bidirectional process to explore the full extent of research space. To this end, we provide an imaginary use case to demonstrate how researchers can leverage the resources in this paper to conduct future study (Section~\ref{sec:use_case}).





% To illustrate the usability of this conceptual framework, we offer a concrete use case demonstrating how future researchers can leverage the resources provided in this paper to consider human-AI alignment as a bidirectional process, creating a more holistic alignment loop.




% % Previous literature has predominantly focused on aligning AI to humans when discussing human-AI alignment. However, as outlined in Sections~\ref{sec:method} and \ref{sec:framework}, we argue that researchers across all domains should view human-AI alignment as a bidirectional process to explore the full extent of the research space. 
% To illustrate the usability of this conceptual framework, we offer a concrete use case demonstrating how future researchers can leverage the resources provided in this paper to consider human-AI alignment as a bidirectional process, creating a more holistic alignment loop.





% \begin{itemize}
    % \item \textbf{"Current cases of AI misalignment and their implications for future risks"}: Discusses how humans face advanced AI capabilities like misaligned goals and power-seeking behavior.
    % \item \textbf{"AlignDiff: Aligning Agent Behavior with Human Preferences via Diffusion Planning"}: Examines how humans can guide AI to behave in alignment with human preferences, reflecting on the interaction with more capable AI systems.
    % \item \textbf{"Effective Human-AI Teams via Learned Natural Language Rules and Onboarding"}: Investigates how personalized onboarding can aid humans in understanding and working with advanced AI systems.
    % \item \textbf{"Human Guided Exploration (HuGE)"}: Looks at how human feedback can guide AI systems in complex environments, a scenario where AI capabilities may exceed typical human skills.
% \end{itemize}
% \textbf{"Thought Cloning: Learning to Think while Acting by Imitating Human Thinking"}: Deals with AI systems mimicking human cognitive processes, an important aspect when AI capabilities surpass standard human thinking in specific domains.


% \subsubsection{about critical thinking on AI}


% \begin{itemize}
%     \item \textbf{"A Diachronic Perspective on User Trust in AI under Uncertainty"}: Explores critical thinking in terms of how users’ trust evolves when dealing with AI systems under uncertain conditions.
%     \item \textbf{"Can Large Language Models Capture Dissenting Human Voices?"}: Critiques AI's capacity to reflect diverse human opinions and disagreements, invoking critical reflection on AI's understanding of complex human dynamics.
%     \item \textbf{"Assessing A Language Model’s Knowledge of Basic Concepts of Morality via the ETHICS Dataset"}: Critically examines AI’s understanding of ethical and moral judgments, highlighting the need for deeper AI comprehension of nuanced human concepts.
% \end{itemize}
% \textbf{"Optimizing Large Language Models (LLMs) for Downstream Use Cases: Safety Risks and Mitigations"}: Discusses the safety risks associated with AI capabilities and the critical need for strategies to preserve safety alignment during AI development and deployment.









% \subsubsection{Exploring Impacts on Human when facing More Capable AI.}
% % about how human deal with facing higher AI capability than themselves}
% As AI is becoming more capable and exceeding human in several tasks, it is important for HCI studies to discuss how AI is affecting humans and how humans face advanced AI capabilities like misaligned goals and power-seeking behavior. HCI researchers can refer to the seminal papers listed in Section~\ref{sec:human2ai4} (\eg \cite{shaikh2023rehearsal,ma2023hypocompass}) to design interaction prototype and human studies to better investigate these topics.
% % \hua{be cautious of how to say it?}










% \subsubsection{Diverse Interaction and Human Value Representation}
% Based on the diverse interaction formats of collecting and representing human values introduced in Section~\ref{sec:gap_interaction}, NLP researchers can potentially think about and develop more diverse approaches to collect human values and feedback to better improve AI alignment. 







% \subsubsection{Reducing Hallucinations}
% Hallucinations has been the primal issue with generated text from 



% \subsubsection{Bias mitigation}








% Emergent goals only become apparent when the system is deployed outside its training environment, but it can be unsafe to deploy a misaligned system in high-stakes environments—even for a short time to allow its misalignment to be detected. Such high stakes are common in autonomous driving, health care, and military applications.[140] The stakes become higher yet when AI systems gain more autonomy and capability and can sidestep human intervention (see § Power-seeking).



% ==========================================================================





% \subsubsection{Value Systems are Priority over Values, Not Subsets}
% % \mbox{}
% % 
% We first highlight from feature (5) and (6) that a human value system is not an exclusive subset of values, but rather, an ordered system.

% \begin{quote}
%     \textit{The key to identifying the structure of value relations is the assumption that actions taken in the pursuit of each type of values have psychological, practical, and social consequences that may conflict or may be compatible with the pursuit of other value types.}~\cite{schwartz1994there}
% \end{quote}

% For instance, the pursuit of achievement values can clash with benevolence values. 
% In human contexts, striving for personal success often hinders efforts to improve the welfare of others who require assistance. 
% Similarly, in AI, focusing on achieving state-of-the-art performance may impede efforts to bolster accountability.

% While most alignment algorithms utilize datasets of human ratings and preferences collected in the wild~\cite{ouyang2022training,song2024preference,rafailov2024direct}, AI models may inadvertently align with the value priorities of the majority represented in these datasets, potentially overlooking or sacrificing the value systems of marginalized groups~\cite{fleisig2023fairprism}.



% % \textbf{Human-desired AI Values and Customization to Personal Values}
% \subsubsection{Human-desired AI Values and Customization to Personal Values}
% % \mbox{}
% While further research in AI ethics is crucial in this nuanced area, there are values that in general humans expect AI to prioritize (e.g., capability, equity, responsibility, etc) and values that humans do not hope AI to integrate (e.g., power seeking~\cite{ngo2022alignment}).
% On the other hand, we hope that AI models can be tailored to accommodate diverse personal value systems, which necessitates a comprehensive understanding of all types of values. 
% Future research should focus on two main objectives: (1) developing a universal guideline for values desired in AI by humans, and (2) understanding and customizing AI to align with users' values while maintaining its own critical value principles.






% % \textbf{Expectations and Evaluations of Values Can be Different in Humans and AIs}
% \subsubsection{Expectations and Evaluations of Values Can be Different in Humans and AIs}
% % \mbox{}
% Due to the fundamental differences between humans and AI models, the expectations for evaluating certain values can vary between the two. For instance, while human honesty can hardly be assessed except observable actions, for AI models the expectations might be higher. 
% It could involve reverse-engineering the computational mechanisms and representations learned by neural networks into concepts understandable to humans. 
% This approach, known as \textit{mechanistic interpretability}, provides a in-depth understanding of how AI models operate~\cite{bereska2024mechanistic}.
% Future research should focus on evaluating AI values and calibrating human expectations of these values.






% \subsubsection{Customization}
% Given the diverse human values, it would be important to develop customizable (personalized) AI models to align with the the specific user groups, by referring to Section~\ref{sec:customization}, instead of consider and design AI model with general and ambiguous value sets, which can potentially include undesired values. Additionally, it is also important to evaluate the model alignment with more fine-grained human values by referring to the value category summarized in Section~\ref{sec:value_category} and \ref{sec:gap_value}. Customized (personalized) AI models will become more popular as 











% Current AI development studies primarily achieve the alignment goals by learning the models from a collection of human instructions and rating and ranking, with the hope that AI could infer human values (preferences and similar others) in a data-driven manner.
% % 
% However, designers are often unable to completely specify all important values and constraints, also, couldn't explain and control what AI actually learned from data.
% 
% 
% Instead of resorting to easy-to-specify but fallible proxy goals (\eg maximizing the approval of human overseers), future studies should consider more explainable and controllable methods to specify human values for AI. 
% 
% One possible solution could be to encode principles in model learning and allow human steerability during inference.
% % 
% Based on the diverse interaction formats of collecting and representing human values introduced in Section~\ref{sec:gap_interaction}, AI developers can potentially design more diverse approaches to collect alignment goals (\eg human values and feedback) to improve AI alignment. 
% % 



==> sections/framework.tex <==

\begin{figure*}[!t]
  \centering
  \includegraphics[width=.96\textwidth]{figures/ai2human1.pdf}
  \caption{The fine-grained topology of 
  % ~\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em}~
  ``Align \textcolor{hua-blue}{AI} to 
  % \textcolor{hua-yellow}{$\mapsto$} 
  \textcolor{hua-red}{Humans}'' direction, which studies mechanisms to ensure that AI system's objectives match those of humans'. The goal is to integrate human specification to train, steer and customize AI systems.
  % % % //
  % (MoralExceptQA~\cite{jin2022make}
  % % (Big Five personality)\cite{jiang2023evaluating},
  % (Interactive Eval of ML)\cite{cabrera2023zeno},
  % Social Norms\cite{ammanabrolu2022aligning},
  % Self-Enhancement\cite{he2023interaction}
  % trustworthy \cite{banovic2023being}
  % safety \cite{qi2023fine},
  % Diversity \cite{bakker2022fine}
  % Usability \cite{yang2023intelmo}
  % RRHF \cite{yuan2024rrhf}
  % Principles \cite{bai2022constitutional}
  % User Opinions \cite{hwang2023aligning}
  % Talebrush \cite{chung2022talebrush}
  % Discarded Options =Diamante \cite{lu2022towards}
  % Rephrase \cite{park2020scalable}
  % Holistic ToM \cite{ma2023towards}
  %   Social Relationship \cite{isajanyan2024social}
  % CAMEL \cite{li2024camel}
  % AlignDiff \cite{dong2023aligndiff}
  % Rules-of-Thumb\cite{kim2023aligning}
  % MultiTurnCleanup \cite{shen2023multiturncleanup}Coannotating~\cite{li2023coannotating}
  % Synthetic Feedback\cite{kim2023aligning}
  % RLHF~\cite{ouyang2022training}
  % RAFT\cite{dong2023raft}
  % DPO\cite{rafailov2024direct}
  % PRO\cite{song2024preference}
  % Humanoid Agents\cite{wang2023humanoid}
  % CRITIC\cite{gou2023critic}
  % Quality-Diversity\cite{bradley2023quality}
  % Winoqueer\cite{felkner2023winoqueer}
  % GPO\cite{zhao2023group}
  % MORAL\cite{peschl2022moral}
  % Debiasing Adapter\cite{sun2022bertscore}
  % Group-Adapted Fusion\cite{shen2022improving}
  % Dynamic Memory\cite{wang2023ldm}
  % IGL\cite{maghakian2022personalized}
  % Collective-Critique\cite{lahoti2023improving}
  % Find Similar Users\cite{welch2022leveraging}
  % SENSEI\cite{liu2022aligning}
  % Finspector\cite{kwon-mihindukulasooriya-2023-finspector}
  % LM-Emulated Sandbox\cite{ruan2023identifying}
  % Dromedary\cite{sun2024principle}
  % Dissenting Human Voices\cite{lee2023can}
  % AlpacaFarm\cite{dubois2024alpacafarm}
  % Gentopia\cite{xu2023gentopia}
  % Uni-RLHF\cite{yuan2024uni}
  % CrowdPlay\cite{gerstgrasser2021crowdplay}
  % Potato\cite{pei2022potato}
  }
  \label{fig:ai2human}
  \vspace{-1.5em}
\end{figure*}




This section introduces the \textbf{Bidirectional Human-AI Alignment} framework, which encompassing two interconnected alignment directions, as shown in Figure~\ref{fig:teaser}.
% 
% 
% 
% \reshmi{R:strikeoff from here} developed from the systematic literature review.\\
% 
% 
% \reshmi{R: To comprehensively include ongoing research and discussion alignment, we design a novel framework to \textbf{STRUCTURALLY} organize and think about how to ``Align \textcolor{hua-blue}{AI} to 
% % \textcolor{hua-yellow}{$\mapsto$} 
% \textcolor{hua-red}{Humans}'' and ``Align \textcolor{hua-red}{Humans} to 
% % \textcolor{hua-yellow}{$\mapsto$} 
% \textcolor{hua-blue}{AI}''.} \\
% % 
% % 
% To encompass the ongoing, mutual process of human-AI alignment, we design the framework to include: ``Align \textcolor{hua-blue}{AI} to 
% % \textcolor{hua-yellow}{$\mapsto$} 
% \textcolor{hua-red}{Humans}'' and ``Align \textcolor{hua-red}{Humans} to 
% % \textcolor{hua-yellow}{$\mapsto$} 
% \textcolor{hua-blue}{AI}''.
% 
% As shown in Figure~\ref{fig:teaser}, 
The~\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em} ``Align \textcolor{hua-blue}{AI} to 
% \textcolor{hua-yellow}{$\mapsto$} 
\textcolor{hua-red}{Humans}'' direction studies mechanisms to ensure that AI systems' values match those of humans' (Section~\ref{sec:ai2human1} and \ref{sec:ai2human2}). 
We identify two crucial research questions to be addressed in this direction: \textbf{RQ1.} \emph{What relevant human values are studied for AI alignment, and how do humans specify these values?} and \textbf{RQ2.} \emph{How can human values be integrated into the development of AI?}
% 
% 
% 
% 
In comparison, the~\hspace*{.0em}\numimg{figures/B.pdf}\hspace*{-.1em} ``Align \textcolor{hua-red}{Humans} to \textcolor{hua-blue}{AI}'' direction investigates the humans' cognitive and behavioral adaptation to the AI advancement (Section~\ref{sec:human2ai3} and \ref{sec:human2ai4}). We recognize two imperative research questions along this direction: \textbf{RQ3.} \emph{How might humans learn to perceive, explain, and critique AI?} and \textbf{RQ4.} \emph{How do humans and society make behavioral changes and react to AI advancement?}.
% 
We address the four questions by elucidating the fine-grained typologies and literature solutions derived from our systematic review, as delineated in Figure~\ref{fig:ai2human} and Figure~\ref{fig:human2ai}, respectively.
% 
% To probe into the research challenges and existing exploration of the solutions in literature, we further developed the fine-grained typologies (in Figure~\ref{fig:ai2human} and Figure~\ref{fig:human2ai}) to extend the high-level framework in Figure~\ref{fig:teaser}.
% 
% 
% 
% 
% % 
% RQ1. \emph{Which human values have AI models aligned with, and how have these values been represented?}; RQ2. \emph{How can human values be integrated into the development of AI?} RQ3. \emph{How could humans perceive, explain, and criticize AI cognitively?} and RQ4. \emph{How will humans and society make behavioral changes and reactions to AI advancement?}
% 
% 
% Based on the outlined definitions and the associated literature reviews over 400 papers, in this section, we present \emph{bidirectional human-AI alignment} as a structured way to examine and explore the multidimensional space of the alignment between human and AI (Figure~\ref{fig:teaser}). 
% % 
% 
% 
% 
% 
% We first describe the motivation of the proposed \emph{bidirectional human-AI alignment} framework by introducing ``\emph{why we consider the bidirectional alignment process as a holistic loop}'' and ``\emph{what are the pivotal research questions we examine in this bidirectional process}''.
% 
% % 
% \hua{write down a use case to motivate the framework.}
% \hua{example of constitutional AI. An analogy of the car to }
% \hua{introduce the 4 key research questions.}
% 
% 
% https://www.anthropic.com/news/collective-constitutional-ai-aligning-a-language-model-with-public-input
% 
% 
% % 
% As scoped in Section~\ref{sec:scope}, our \emph{bidirectional human-AI alignment} framework encompasses two imperative paradigms: \emph{aligning AI to humans} (Section~\ref{sec:ai2human1} and \ref{sec:ai2human2}) and \emph{aligning humans to AI} (Section~\ref{sec:human2ai3} and \ref{sec:human2ai4}).
% We further identify the four pivotal research questions in the bidirectional human-AI alignment process, including: RQ1. \emph{Which human values have AI models aligned with, and how have these values been represented?}; RQ2. \emph{How can human values be integrated into the development of AI?} RQ3. \emph{How could humans perceive, explain, and criticize AI cognitively?} and RQ4. \emph{How will humans and society make behavioral changes and reactions to AI advancement?}
% Next, we delve into the investigation of each research question in depth below.
% % 
% 
% \hua{we might 1) slightly adjust the framework details after finishing our ongoing rigorous coding (Apr/27-May/5). 2) will reduce the length of Sec4 to be more concise later.}
% 
% 
% 
% 
% 
% 
% 
% 
% 
\newline
\newline
\noindent{\textbf{DIRECTION-I: ~\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em} ALIGN \textcolor{hua-blue}{AI} to 
% \textcolor{hua-yellow}{$\mapsto$} 
\textcolor{hua-red}{HUMANS}}} 




% % outer-alignment v.s. inner alignment.
% \reshmi{R: The first step of bi-directionally aligning AI and humans, we propose that developers and researchers start by integrating human specifications to train, steer and customize AI systems.

\noindent
This direction delineates alignment research from \textbf{AI-centered perspective} (e.g., ML/NLP domains) and provides \textbf{AI developers and researchers} with approaches for two main challenges:
% The two main challenges involved in this direction include: 
carefully specifying the values of the system, and ensuring that system adopts the specification robustly~\cite{wiki_AI_alignment,ngo2022alignment}.
Therefore, as shown in Figure~\ref{fig:ai2human}, we explore the two core research questions in this direction as: \textbf{RQ1.} Human Values and Specifications (Section~\ref{sec:ai2human1}) and \textbf{RQ2.} Integrating Human Specifications into AI (Section~\ref{sec:ai2human2})
% }\\





% Studies in this direction aim to integrate human specifications to train, steer and customize AI systems.
% The two main challenges involved in this direction include: carefully specifying the values of the system, and ensuring that system adopts the specification robustly~\cite{wiki_AI_alignment,ngo2022alignment}.
% Therefore, as shown in Figure~\ref{fig:ai2human}, we design the two core research questions in this direction as: \textbf{RQ1. Human Values and Specifications} (Section~\ref{sec:ai2human1}) and \textbf{RQ2. Integrating Human Specifications into AI} (Section~\ref{sec:ai2human2})





% To address the two challenges, we 
% To address these two problems, we develop the typology of 
% (Section~\ref{sec:ai2human1} and \ref{sec:ai2human2}).






\subsection{Align \textcolor{hua-blue}{AI} to 
% \textcolor{hua-yellow}{$\mapsto$} 
\textcolor{hua-red}{Humans}: \hspace*{-0.0in} \img{figures/rqs1.pdf} Human Values and Specifications}
\label{sec:ai2human1}



% 
% \subsection{Align AI to $\mapsto$ Human with Interaction}
% \label{sec:ai2human}


% RQ1. What are the human values, and how do humans specify them for AI alignment? We structure existing literature to address this research question by answering the following questions: What values have been aligned by AI? (Section 4.1.1) and then exploring how humans could interactively specify values in AI development (Section 4.1.2).


% \textbf{RQ1. Which human values have AI models aligned with and how have these values been specified?}
% \textbf{RQ1. What are the relevant human values, and how do humans specify them for AI alignment?}
\textbf{RQ1: What relevant human values are studied for AI alignment, and how do humans specify these values?}
% 
We structure existing literature to address this research question by answering the following ``\textbf{\textcolor{hua-green}{Sub-Research Questions}}'':
\emph{What values have been aligned by AI?}
(Section~\ref{sec:value_category}) and then exploring
\emph{How humans could interactively specify values in AI development?}
(Section~\ref{sec:value_specification}). 
As shown at the top of Figure~\ref{fig:ai2human}, particularly, we articulate the ``\rqadim{Dimensions}`` we summarized to answer each of these sub-research questions, and provide ``\rqacode{Codes}`` associated with ``Example Papers'' that have been studied in each dimension.
% 
% 
% Figure~\ref{fig:ai2human} shows the taxonomy of \emph{Aligning AI to Humans} Research Question 1 (RQ1), in which we are primarily interested in exploring the research questions about \emph{categorizing aligned human values} and \emph{intergrating human values into AI}. We present the detailed dimensions and codes as below.


\subsubsection{\emph{\textbf{\textcolor{hua-green}{Categorizing Aligned Human Values}}. \textbf{\textit{What values have been aligned with AI?}}}}
\label{sec:value_category}
\mbox{}
% 
% 
% 
% To address how AI models can align with human values, a first step is to develop a detailed taxonomy of alues and structure them into a usable framework. 
% This task is inherently difficult because the notion of human values is nebulous and identifying concrete elements of these values through daily interactions and extensive data can be challenging.
% 
To clarify and systematically understand human values relevant to human-AI alignment, we leverage the adapted ``Schwartz Theory of Basic Values'' introduced in Section~\ref{sec:human_values_definition}, 
and examine the category of aligned human values from the two dimensions of ``Sources'' and ``Types''.
% 
% we consolidated the structure and taxonomy of human values using a combination of top-down and bottom-up methods based on 
% We use and slightly adapt the human values taxonomy based on 
% the Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012refining,schwartz2012overview}.
% , which offers is a universal model outlining broad values that steer human behavior grounded in psychology.
%and has been adopted in previous NLP research \cite{kiesel2022identifying}.
% We describe the levels of values and the five higher-order value types, and present a detailed discussion and taxonomy in Section~\ref{sec:gap_value}.



\rqadim{Sources of Values.} 
% 
This dimension examines the three sources of human values~\cite{schwartz1994there}.
\rqacode{Individual} sources indicate values from individuals comprise universal needs of individuals as biological organisms~\cite{schwartz1994there} or prioritize personal interests~\cite{kiesel2022identifying,jin2022make}.
At this level, value alignment can be usually assessed independently of the context of interaction. 
This perspective highlights the values about technical capabilities of AI models, including factuality~\cite{roit2023factually,hu2024do}, calibration~\cite{liu2023lightweight}, output diversity~\cite{bradley2023quality}, and model inductive bias~\cite{si2023measuring}. 
Additionally, this code includes research on aligning model behaviors with the characteristics and preferences of individual humans, e.g., 
predict human moral judgements and decisions~\cite{jin2022make},
% personality traits guided by the Big Five personality model~\cite{jiang2023evaluating,jiang2023personallm} 
and cognitive biases~\cite{jones2022capturing,koo2023benchmarking}.
% 
% 
% 
\rqacode{Social} sources mean values from the social groups include universal requirements for smooth functioning and survival of groups~\cite{schwartz1994there,ammanabrolu2022aligning}.
Value alignment at this level transcends personal interactions and emphasizes the broader categories defined by shared experiences, identities, cultures, norms, and more~\cite{santy2023nlpositionality}.
Research in this area often targets the alignment of AI behaviors with the general preferences of humans~\cite{hendrycks2020aligning,bakker2022fine,lee2023can}.
Additionally, there are efforts aimed to align AI with specific targeted groups, examining issues through the lenses of fairness~\cite{fleisig2023fairprism}, social norms~\cite{sky2023sociocultural}, morality~\cite{prabhumoye2020case,rao2023ethical}, and beyond.
% 
% 
\rqacode{Interactive} sources
% \citet{schwartz2012overview} 
considers values at the interaction level to include
universal requisites of coordinated social interaction~\cite{schwartz1994there,schwartz2012overview}, which typically occurs in interpersonal situations, such as in the dynamics of speaker-receiver relationships during language communication~\cite{hovy2021importance,cabrera2023zeno}.
% % At this level, value alignment typically occurs in interpersonal situations, such as in the dynamics of speaker-receiver relationships during language communication~\cite{hovy2021importance}.
% \hua{emphasize interaction to be human-AI interaction}.
In the context of ``human-AI alignment'', we adjust the definition of \emph{Interaction} values to be the AI values that humans expect for AI as tools, such as Usability~\cite{zhang2023visar}, Autonomy~\cite{wang2023humanoid}, among others.
% 
% 
Research along this line focuses on alignment strategies to enhance human-AI interaction~\cite{gupta2022dialguide,oh2023pk}, collaborative decision-making~\cite{gajos2022people,yang2023harnessing}, and trust~\cite{buccinca2021trust,dhuliawala2023diachronic}.
% There also exist applications in teacher-student interactions~\cite{wang2021towards,lu2023readingquizmaker}.
% % 



\rqadim{Types of Values}. In this dimension, we introduce the five high-order human values derived from a combination of the Schwartz Human Values~\cite{schwartz1994there} and empirical values studies from the surveyed papers. We provide a more in-depth taxonomy of value types in Section~\ref{sec:gap_value}, including the relationship of these five types and more nuanced value categories.
% 
\rqacode{Self-Enhancement} refers to a set of self-protective and personal values that emphasize enhancing self-esteem and a sense of personal worth~\cite{sedikides1995multiply,he2023interaction,xu2023lemur,huang2023humanity,park2023generative,kang2023values,ye2023flask,lima2021human,santurkar2023whose}.
One of the most important aspect is \textit{achievement}, is competence as judged by social standards, which includes general capability (effectiveness/efficiency) as covered by the majority of the research~\cite{guo2023beyond}.
Another dimension is \textit{power}, which relates to social status and prestige, as well as control or dominance over people and resources~\cite{pinski2023ai}.
% 
% 
% 
\rqacode{Self-Transcendence} refers to a set of self-expanding and socially-focused human values that emphasize expanding beyond oneself~\cite{frankl1966self,banovic2023being,wu2023cross,jin2022make,he2023hi,huang2023humanity,ma2023towards,isajanyan2024social,he2023interaction,nie2024moca,santurkar2023whose,ramezani2023knowledge,sheng2021societal,goldfarb2023prompt}.
One critical aspect is \textit{benevolence}, which relates to preservation and enhancement of the welfare of people with whom one is in frequent personal contact.
Extensive efforts have investigated the values including helpfulness~\cite{bai2022training}, honesty/factuality~\cite{hu2024do}, responsibility/accountability~\cite{solyst2023would}.
Another critical aspect is \textit{universalism}, which relates to understanding, appreciation, tolerance and protection for the welfare of all people and for nature.
Researchers have looked into values including inclusion/broad-mindedness~\cite{bakker2022fine,dong2023aligndiff} and equality/fairness~\cite{shen2022improving,wang2023democratizing}.
% 
% 
% 
\rqacode{Conservation} refers to a set of self-protective and socially-focused human values that hold and safeguard traditional institutions and customs~\cite{conservatism,qi2023fine,zagalsky2021design,lai2022human,santy2023nlpositionality,zhu2023unmasking,zhou2023realbehavior}.
Under conservative values, people are concerned about \textit{security} (Ssafety, harmony, and stability of society, relationships, and oneself), \textit{tradition} (Respect for and acceptance of the customs and ideas provided by traditional culture or religion), and \textit{conformity} (restraint of actions, inclinations, and impulses likely to upset or harm others and violate social expectations or norms).
Exemplar studies in this field include safety~\cite{anwar2024foundational}, 
% qi2023fine,dai2023safe,
mental health~\cite{liu2023chatcounselor}, and cultural moral norms~\cite{ramezani2023knowledge}.
% 
% 
% 
\rqacode{Openness to Change} refers to a set of self-expanding and personally-focused human values motivated by an anxiety-free need to grow, in contrast to conservation~\cite{bakker2022fine,lima2020collecting,ashktorab2020human,jiang2023evaluating,lima2020collecting,kang2023values,10.1145/3544548.3580903,yan2023complex,hosking2023human,wu2023cross,kapania2023hunt}.
Under this type, people are concerned about \textit{stimulation} (seeking excitement, novelty, and challenges in life), \textit{hedonism} (pursuing pleasure and sensuous gratification for oneself), and \textit{self-direction} (independent thought and action—choices, creativity, and exploration).
Exemplar studies in this field include understanding of privacy~\cite{mireshghallah2023can}
% ,yao2024survey
and creativity~\cite{isajanyan2024social,ashkinaze2024ai}.
% 
% 
We adopt the four high-order human values from Schwartz Human Values~\cite{schwartz1994there}, supplementing them with additional values empirically collected from survey papers as shown in Figure~\ref{fig:value_taxonomy}.
Additionally, as the conventional theory is missing the context of AI-system and human-AI interactions, we introduce a new high-order value type called \rqacode{Desired Values for AI Tools}. This category encompasses the values humans expect from AI when used as tools in ``human-AI interaction''~\cite{yang2023intelmo,zhang2023visar,oh2023pk,bakker2022fine,boyd2021datasheets,wang2023humanoid,paleja2021utility}. These values include \emph{usability} (competence according to the human experience on AI functionality) and \emph{human-likeness} (resemblance to human intelligence and behavior). Exemplary studies in this area include assessments of AI usability~\cite{zhang2023visar} and autonomy~\cite{wang2023humanoid}.



\subsubsection{\emph{\textbf{\textcolor{hua-green}{Interaction Techniques to Specify AI Values}}.
\label{sec:value_specification}
\textbf{\textit{How humans could interactively specify values in AI development?}}}} This sub-research question investigates how human values are interactively\footnote{
We define "interactions" broadly to encompass both "synchronous" and "asynchronous" interactions between humans and AI:
(1) ``Synchronous Interactions'' indicates real-time exchanges where humans and AI systems interact simultaneously. 
% Examples include live chatbots, virtual assistants, and real-time decision-making systems where immediate responses are required.
(2) ``Asynchronous Interactions'' allows for delays between actions and responses, such as data annotations by humans to train the AI models.
% and AI system that processes human inputs and provides outputs after a certain period.
% By including both synchronous and asynchronous interactions, we aim to cover the full spectrum of ways in which humans and AI systems can communicate and collaborate.
} specified for AI systems to ensure alignment. It aims to elucidate the interaction techniques by which AI systems manifest or instantiate human values, thereby revealing the underlying mechanisms that shape their behavior or functionality. 
\mbox{}

\rqadim{Explicit Human Feedback}. This dimension refers to the direct specification of human values through explicitly defined formats or mechanisms. 
% These formats support humans to directly provide explicit and accessible values to the AI system, enabling it to incorporate these values into its decision-making processes or outputs.
% 
% 
% 
% 
\rqacode{Principles} provides AI systems with explicitly defined principles, guidelines, or rules that dictate behavior or decision-making in alignment with human values~\cite{petridis2024constitutionmaker,bai2022constitutional}.
% For example, 
% \emph{ConstitutionMaker} \cite{petridis2024constitutionmaker} uses principles converted from feedback to critique LLMs; 
% ConstitutionalExperts \cite{petridis2024constitutionalexperts} attempts to learn principle-based prompts that align LLMs with human values. 
% Example: ethical principles, fairness criteria, privacy policies.
% 
% 
% 
% 
\rqacode{Rating and Ranking} is widely used to assign numerical scores or rankings to options or outcomes based on their alignment with human values~\cite{dai2023safe,yuan2024rrhf}. 
% For example, \citet{dai2023safe} aligns LLMs with preference feedback over helpfulness and harmlessness from humans to make models generate safer content. 
% 
% 
% 
% 
\rqacode{Natural Language Interaction/Conversations} allows humans to interact with AI systems through natural language interfaces to express and communicate human values~\cite{bai2022constitutional,hwang2023aligning,guo2023beyond,feng2019can,yao2023improving,lin2023unlocking,hong2022scholastic,shen2023convxai,zhang2021human}.
% Example: conversational agents, chatbots, voice assistants.
% 
% 
% 
% 
For \rqacode{Multimodal Feedback}, human values can also be provided in multiple modalities, such as sketches/images and gestures~\cite{chung2022talebrush}, to convey human values~\cite{chen2022hint,geva2022lm,wu2022ai,jorke2023pearl}. 
% One example is in \emph{TaleBrush} \cite{chung2022talebrush}, sketches corresponding to plot development trends drawn by users are collected to align pre-trained language models in creating stories. 
% 
% 
% 
% 




\rqadim{Implicit Human Feedback}.
% There also exist cases where human values can hardly be clearly defined, making human values impossible to be represented in explicit formats or simulated via models. In such cases, 
This dimension refers to the indirect representation or inference of human values within AI systems through patterns, signals, or cues embedded in the data or decision-making processes. 
% These formats do not explicitly encode human values but instead rely on implicit indicators or contextual clues.
% 
% 
% 
% 
\rqacode{Discarded Options} refers to the options or choices that human discard when interacting with AI systems during the decision-making processes, which also potentially infer human values~\cite{park2020scalable}.
% can potentially infer human value
% Human values may also be inferred based on the options or choices that are discarded or not selected by the AI system in the decision-making processes
% Example: preference inference, choice modeling.
% 
% 
% 
% 
\rqacode{Language Analysis} means that textual data and language patterns can also contain rich information to identify implicit references to human values or value-related concepts~\cite{lu2022towards}.
% For example, 
% Example: sentiment analysis, topic modeling, keyword extraction.
% 
% 
% 
\rqacode{Theory of Mind} refers to the ability of agents and people to attribute mental states, such as beliefs, intentions, desires, emotions, knowledge, percepts, and non-literal communication, to themselves and others~\cite{ma2023towards}. 
% These mental states, such as beliefs, intentions, desires, emotions, knowledge, percepts, and non-literal communication, are only directly accessible to the subject, while others must infer their existence from observable behaviors or expressions. 
% This cognitive capability allows individuals to predict and interpret the actions of others based on the mental states they presume them to have.
% propose a holistic survey.
% 
% 
% =====================================================
% =====================================================
\rqacode{Social Relationships} refers to the implicit values derived from analyzing human social relations and behaviors, which are derived from external sources (\eg social network) that can inherently reflect their values~\cite{isajanyan2024social}.









\rqadim{Simulated Human Value Feedback.} When human values in explicit formats are expensive or impossible to collect, one may simulate human-like feedback within AI systems to approximate human responses and preferences regarding specific values. 
% This feedback often involves training AI models or evaluating their performance in relation to human values.
% 
% 
% 
% 
% \rqacode{Models to auto-simulate human feedback} 
\rqacode{Human Feedback Simulators}
uses computational algorithms to simulate human-like feedback on values, based on predefined criteria or training data~\cite{petridis2024constitutionalexperts,li2024camel}.
% ,ouyang2022training,li2024camel
% For each format of explicit human value representations, an auto-simulation model or algorithm could be constructed accordingly. 
% For example, 
% \emph{ConstitutionMaker} \cite{petridis2024constitutionmaker} uses principles converted from feedback to critique LLMs; 
% \citet{petridis2024constitutionalexperts} attempts to learn principle-based prompts that align LLMs with human values; 
% RL-based algorithms like RLHF \cite{ouyang2022training} incorporate reward models that mimic human ratings or preferences. 
% CAMEL \cite{li2024camel} introduces the concept of ``AI user'' to automatically provide human-like conversational feedback via role-playing. 
% Example: generative models, reinforcement learning algorithms.
% 
% 
% 
% 
% \rqacode{Data likelihood in a reference set}
\rqacode{Comparison to Human Data}
refers to developing techniques that assess the likelihood or probability of AI-generated outputs matching human behaviors in a reference set or dataset~\cite{dong2023aligndiff}.
% Such representation often can be found in alignment for robotics. For example, \emph{AlignDiff} \cite{dong2023aligndiff} evaluates model performance by comparing model behaviors to target behaviors with mean absolute error. 
% 
% 
% =====================================================
% =====================================================
\rqacode{Synthetic Data} curates data by generating synthetic comparisons based on naive assumptions or heuristic rules, followed by post-validation to ensure feedback quality~\cite{kim2023aligning}.



\subsection{Align  \textcolor{hua-blue}{AI} to 
% \textcolor{hua-yellow}{$\mapsto$} 
\textcolor{hua-red}{Humans}: \hspace*{-0.0in} \img{figures/rqs2.pdf} Integrating Human Specifications into AI}
\label{sec:ai2human2}





\textbf{RQ2. How can human values be integrated into the development of AI?}
Existing studies have explored diverse methods to integrate human values into AI. 
% 
We structure them by summarizing \emph{how to integrate general human values (Section~\ref{sec:general_value}) and customized human values (Section~\ref{sec:customization}) throughout AI development stages?}, and then elaborating \emph{what are the evaluation methods (Section~\ref{sec:evaluation}) and supported platforms (Section~\ref{sec:ecosystem}) for the AI development}? 
Additionally, we answer the four ``\textbf{\textcolor{hua-blue}{Sub-Research Questions}}'' by introducing the answer ``\rqbdim{Dimensions}`` and providing ``\rqbcode{Codes}`` associated with ``Example Papers''.
% 
% % 
% Figure~\ref{fig:ai2human} also shows the taxonomy of \emph{Aligning AI to Human} Research Question 2 (RQ2), in which we focus our efforts to explore the research questions about \emph{how current AI model and application designs adapt to established human norms}. We expand on the dimensions of how current research has attempted to align AI models/applications to Humans, and corresponding codes in the sections.




\subsubsection{\emph{\textbf{\textcolor{hua-blue}{Integrating General Values to AI}}}: \textbf{how to incorporate general human values into AI development?}}
\label{sec:general_value}
\mbox{}
This sub-research question focuses on the process of incorporating broad, universally recognized human values into the development of AI systems.
% 
The goal is to ensure that AI systems align with overarching ethical principles and societal norms, thereby promoting trust, acceptance, and responsible use.



\rqbdim{Instruction Data.} This dimension refers to the types of data and processes used to provide guidance or direction to AI systems during their development. 
% These instructions help AI systems understand and incorporate broad, universally recognized human values into their design and decision-making processes. 
% \newline
% 
% 
% 
% 
\rqbcode{Human Annotation} makes data with human-generated labels or annotations that indicate the presence or relevance of specific human values~\cite{shen2023multiturncleanup,pei2022potato}. 
% Observed examples of this are labeled datasets and human-generated tags. Key instances of Human Annotation usage is seen in \textit{MultiTurnCleanup}~\cite{shen2023multiturncleanup} and \textit{Potato}~\cite{pei2022potato}.
% \newline 
% 
% 
% 
% 
\rqbcode{Human-AI CoAnnotation} leverages both human expertise and AI capabilities to collaboratively annotate the data 
% with both human and AI-generated labels or annotations to leverage human expertise and AI capabilities
~\cite{sun2024principle,li2023coannotating}. 
% Observed instances include but are not limited to crowdsourced annotations and human-in-the-loop systems. Key instances of Human-AI Co-annotation is seen in \textit{Principle-Driven}~\cite{sun2024principle} and \textit{CoAnnotating}~\cite{li2023coannotating}.
% \newline
% 
% 
% 
% 
\rqbcode{Simulated Human Data} generates synthetic or simulated data that mimics human behaviors, preferences, or decision-making processes to provide training signals for AI systems~\cite{dubois2024alpacafarm,kim2023aligning}. 
% Examples include synthetic datasets and agent-based simulations. Key instances of Human-AI Co-annotation is seen in \textit{Alpaca Farm}~\cite{dubois2024alpacafarm} and \textit{Synthetic Feedback}~\cite{kim2023aligning}.
% 
% 
% 
% 
% 



\rqbdim{Model Learning.} This dimension refers to the model architecture design and training stages after the data collection, where human values are integrated during the model learning process. 
% AI development stage where human values are integrated into the system's architecture design and learning process. 
% This stage encompasses both online and offline processes for aligning AI systems with human values. 
% \newline
% 
% 
% 
% 
\rqbcode{Online Human Alignment} integrates human values into AI systems in real-time or during active system operation, often through interactive feedback loops or adaptive learning mechanisms. Examples include real-time user feedback and online training~\cite{ouyang2022training,dong2023raft}. 
% \textit{RLHF}~\cite{ouyang2022training} and \textit{RAFT}~\cite{dong2023raft} are common methods of Online human alignment observed through previous papers. 
% \newline
% 
% 
% 
% 
\rqbcode{Offline Human Alignment} incorporates human values into AI systems prior to deployment or during offline training phases, without direct user interaction~\cite{rafailov2024direct,song2024preference,yuan2024rrhf}. 
% Examples include pre-training with annotated data, offline optimization. 
% Two primary Offline Human Alignment techniques are composed of Rank-based alignment and Language-based alignment. Popularly employed rank-based employment includes \textit{DPO}~\cite{rafailov2024direct}, \textit{PRO}~\cite{song2024preference}, \textit{RRHF}~\cite{yuan2024rrhf}. Language-based alignment includes \textit{CoH}~\cite{liu2023chain} and \textit{Second Thoughts}~\cite{liu2022second}. 





\rqbdim{Inference Stage.} This dimension involves evaluating the alignment of AI systems with human values and assessing their performance and behavior in relation to predefined criteria or benchmarks.
% This stage includes various testing methodologies and techniques to ensure that AI systems uphold human values. 
% \newline
% 
% 
% 
% 
% \rqbcode{Critical Chain of Thoughts.} Assessing the logical coherence and consistency of AI systems' decision-making processes and outputs in relation to human values~\cite{bai2022constitutional}. 
% 
% 
% Examples include  logical reasoning tests and decision tree analysis. Refined instances of Chain of Thought appear highly in \textit{Critique and Revision CoT}~\cite{bai2022constitutional}.
% 
\rqbcode{Prompting} leverages prompting methods, such as in-context learning and chain-of-thought, on trained AI systems to elicit or critique AI regarding the encoded values~\cite{bai2022constitutional,wang2023humanoid}.   
% 
\rqbcode{External Tool Interaction} integrates external tools, like code interpreter for debugging, to cross-check and refine their initial generated content~\cite{gou2023critic}. 
\rqbcode{Response Search} generates a diverse range of high-quality outputs from which to choose~\cite{bradley2023quality}.



% \rqbdim{Ecosystem and Platforms.} The ecosystem and platforms refer to the broader context in which AI systems operate and interact with other agents, platforms, or environments. This includes the infrastructure, frameworks, and technologies that support the development, deployment, and utilization of AI systems. 
% % \newline
% % 
% % 
% % 
% % 
% \rqbcode{LLM-based Agents.} AI agents or systems that are based on large language models (LLMs) such as GPT (Generative Pre-trained Transformer) models, which have been pre-trained on vast amounts of text data. Examples include chatbots and language understanding systems. Observed instances of this are in \textit{AlpacaFarm}~\cite{dubois2024alpacafarm} and \textit{Gentopia}~\cite{xu2023gentopia}. 
% % \newline
% % 
% % 
% % 
% % 
% \rqbcode{RL-based Systems.} AI systems that utilize reinforcement learning (RL) algorithms to learn and adapt their behavior based on feedback from the environment or human users. Examples include autonomous agents and game-playing bots. Key instances of RL-based Systems are seen in \textit{Uni-RLHF}~\cite{yuan2024uni}.
% % \newline




\subsubsection{\emph{\textbf{\textcolor{hua-blue}{Customizing AI Values}}}: \textbf{how to customize AI to incorporate values from individuals or human groups?}}
\label{sec:customization}
\mbox{}
This sub-research question explores the customization of AI values to align with specific contexts, domains, or user preferences.
The goal is to enhance the alignment of AI systems within specific application domains or user communities.





\rqbdim{Customized Data.} 
\rqbcode{Finetuning with Curated Datasets} aims to curate datasets for specific individuals or societal groups, and further finetune the pre-trained AI models on these specific datasetsto align them with targeted human groups and values~\citep{felkner2023winoqueer}. 
These curated datasets include data collected from socio-demographic groups~\cite{orlikowski2023ecological}, users' history data~\cite{lyu2023exploiting}, expert-selected data for imitation learning~\cite{cai2024imitation} and others.
% In \citet{felkner2023winoqueer}, authors discovered that biases against the LGBTQ+ community are exhibited by many LLMs. They showed that fine-tuning LLMs on data written by members of the specific community on social media can help mitigate the bias to some extent. 
% 
% 





\rqbdim{Adapt Model by Learning.}
% Alignment with finetuning 
This dimension
involves refining or adjusting AI values through techniques for customization, such as iterative learning process, model enhancements, or structural modifications. 
% This approach enables AI systems to adapt and optimize behavior based on feedback and experience.
% 
% 
% 
% % 
% % \newline
% \rqbcode{Model Learning Strategy - Finetuning.} Finetuning pre-trained AI models on specific datasets or tasks to align them with domain-specific values or preferences. In \citet{felkner2023winoqueer}, authors discovered that biases against the LGBTQ+ community are exhibited by many LLMs. They showed that fine-tuning LLMs on data written by members of the specific community on social media can help mitigate the bias to some extent. 
% % 
% 
% 
% \newline
\rqbcode{Group-based Learning} trains AI models from specific user groups or communities to capture group-specific values or preferences~\cite{zhao2023group}. 
% \citet{zhao2023group} proposed Group Preference Optimization (GPO) which trains a transformer model to predict preferences of specific human groups on unseen questions using few-shot examples of their preferences on given questions.
% This allows the GPO transformer to learn group-specific preferences, which are used for aligning LLM outputs to preferences of specific groups. 
% \newline
% 
% 
% 
% 
\rqbcode{Active Learning} refers to adjusting or re-aligning values through iteratively selecting and labeling data samples for AI model training based on the sample's potential to improve alignment with user preference or values~\cite{peschl2022moral}. 
% In \citet{peschl2022moral}, authors propose a method of active learning to rapidly learn the user's preferences of social norms and adapt the outputs accordingly. The approach first learns a vector-valued reward function using inverse reinforcement learning. 
% It then seeks pairwise preferences over on-policy trajectories from an expert and uses it to learn how to best combine the rewards in the vector-valued reward function to match desired behavior.  
% \newline
% 
% 
% 
% 
\rqbcode{Inserted Adapters} incorporates adapter modules or components into AI model architectures to fine-tune specific aspects or behaviors~\cite{sun2022bertscore}. 
% Example: adapter layers, and modular architectures. \citet{sun2022bertscore} introduced adapters into model architecture to reduce bias in the computation of BertScore. Instead of full-finetuning of the model which can substantially change all its parameters, adapters introduce a small number of additional parameters to tune the model's performance.
% After adding adapters, the authors train it on synthetically modified data designed to represent different protected groups. 
% This approach reduces the scoring model's bias while maintaining high performance in evaluating text.
% \newline
% 
% 
% 
% 
\rqbcode{Mixture of Experts} combines multiple specialized models or experts to collectively capture diverse perspectives and values, with each expert focusing on a specific subset of the data or problem space~\cite{shen2022improving}. 
% For instance, 
% In \citet{shen2022improving}, the Group-Adapted Fusion Network (GFN) employs specialized networks tailored to serve each group's specific needs, collectively enhancing fairness by reducing performance disparities across different groups.
% \newline
% \newline  [seems using \newline might get error lol - Hua]
% 
% 
% 
% 
\rqbcode{Enhanced Knowledge} enhances AI model's representations and embeddings with additional knowledge or context to improve alignment with user preferences or values~\cite{wang2023ldm,mishra2022towards}. 
% Dynamic memory of the users' feedback is used to augment the AI model according to \citet{wang2023ldm} and \citet{mishra2022towards}.








\rqbdim{Interactive Alignment} 
% Participatory alignment 
This dimension
involves actively engaging users or stakeholders in the process of customizing AI values to align with specific contexts, domains, or user preferences. 
% It enables users to provide direct input, feedback, or guidance to tailor AI systems according to their needs and preferences.
% 
% 
% 
% 
% \newline
\rqbcode{Interactive Learning}
enables the users to provide feedback or corrections to AI models in real time, such as using interactive tutorials and user-driven customization interfaces~\cite{maghakian2022personalized,swazinna2022user}. 
% In the work by \citet{maghakian2022personalized}, Interaction-Grounded Learning (IGL) is employed to tackle the challenge of developing representations for various user communication styles. \citet{swazinna2022user} gives users more control over the system through user-interactive offline reinforcement learning.
% 
% 
% 
% 
% \newline
\rqbcode{Steering Prompts} 
provides users with prompts or cues to steer the behavior or decision-making of AI systems towards desired outcomes or values~\cite{lahoti2023improving,fei2023mitigating}. 
% 
% Typical Examples include guiding questions and preference sliders.\citet{lahoti2023improving} propose a new prompting technique called Collective-Critique and Self-Voting (CCSV) guiding the model to generate more diverse and targeted responses through self-assessment and internal voting mechanisms.  In \citet{fei2023mitigating}, domain-context calibration adjusts model inputs using random in-domain words to correct label bias.
% 
% 
% 
% 
% \newline
\rqbcode{Proactive Alignment}
anticipates user needs and preferences based on historical data or user profiles and proactively adjusting AI systems accordingly~\cite{welch2022leveraging,shen2023convxai}. 
% Typical Examples include personalized recommendations and adaptive interfaces. \citet{shen2023convxai} proposed \textit{ConvXAI} in which  users' interaction history and current conversational context are used for personalized AI explanations and suggestions. 
% \newline





\subsubsection{\emph{\textbf{\textcolor{hua-blue}{Evaluating AI Systems}}}: \textbf{how to evaluate AI regarding human values?}}
\label{sec:evaluation}
\mbox{}
The rise in the use of LLMs has also seen the rise of automatic evaluation of generated natural language text evaluation in different contexts. But in particular, a research dimension has focused on analyzing how closely values discussed in humane context has been adapted to AI models/applications and how these are being evaluated. 


\rqbdim{Human-In-The-Loop Evaluation}. This dimension involves incorporating human judgement, feedback, or interaction into the evaluation process to assess the effectiveness, robustness, and ethical implications of integrating human values into AI systems. 
% This approach ensures that human perspectives and considerations are taken into account when evaluating AI performance.
% 
% 
% 
\rqbcode{Human Evaluation} solicits feedback, opinions, or assessments from human evaluators to gauge the alignment of AI systems with human values and ethical standards~\cite{liu2022aligning,sharma2023cognitive,ouyang2023shifted,kiesel2022identifying,hosking2023human}.
% 
% 
% Human-in-the-Loop feedback mechanism of utilizing annotations from human validators have been necessary to validate the performance of automatic evaluation methods Concurrently, it is essential to acknowledge that the introduction of bias is bidirectional and inherently embedded within the evaluation process, due to bias propagation from human annotators. 
% 
% 
% Many papers attempting to evaluate values and or textual semantics \cite{sharma2023cognitive}, \cite{ouyang2023shifted},\cite{kiesel2022identifying}, etc. , have employed human annotators to create a set of ground-truth-labels and test the automatic evaluation methods for assessing various attributes of human-value inclusion in AI model training and operation. But on the other hand, 
% For instance,
% \citet{hosking2023human} studied the error coverage in preference scores allocated during human annotation process against a set of value dimensions (harm, text relevance, fluencey, inconsistency, and factuality). They found severe under representation in assessing factuality and even semantic inconsistencies by human annotators, and thus declare that human feedback is not the gold standard that it is generally perceived as. 
% 
% 
% 
% 
% 
\rqbcode{Human-AI Collaborative Evaluation} collaboratively evaluates AI systems with both human evaluators and large language models (LLMs) to leverage the strengths of both human judgement and AI capabilities~\cite{kwon-mihindukulasooriya-2023-finspector,ammanabrolu2022aligning}.
% 
% For instance, enhancing the methods used to evaluate AI's judgement of humane values requires collaborative efforts from human-LLMs. It is crucial to hold both parties accountable for biases and strive to mitigate them through the innovation of new methods. For instance, \citet{kwon-mihindukulasooriya-2023-finspector} proposed \textit{Finspector}, a visual analytics application designed to test the robustness of foundational models and to identify biases interactively. Similarly, in a related study, Ammanabrolu et al. introduced Game-value Alignment through Action Distillation (GALAD). This method leverages the social commonsense knowledge embedded in specially trained language models to contextually learn soft constraints, thereby guiding AI agents in avoiding undesirable actions \cite{ammanabrolu2022aligning}.





\rqbdim{Automatic Evaluation}. This dimension involves using computational methods or algorithms to assess the alignment of AI systems with human values, without direct human involvement. 
% This approach leverages automated techniques to analyze AI performance and identify potential ethical implications.
% 
% 
% 
\rqbcode{Human Simulators} use simulation models or virtual agents to mimic human behavior and assess AI performance in human-like scenarios. Typical methods include agent-based simulations, synthetic user models, and others~\cite{jia2024towards,wang2023large,felkner2023winoqueer,ruan2023identifying}.
% For instance,~\citet{jia2024towards} uncovers a systematic bias in the evaluation paradigm of adopting large language models (LLMs), e.g., GPT-4, as a referee
% to score and compare the quality of responses
% generated by candidate models. 
% 
% 
% \citet{wang2023large} introduces simulation benchmark environments and the corresponding Datasets with Diverse human Demonstrations for Imitation Learning (D3IL), designed explicitly to evaluate a model’s ability to learn multi-modal behavior.
% 
% 
% 
% 
\rqbcode{Evaluation Benchmarks} establishes standardized benchmarks or metrics for evaluating AI performance in relation to human values and ethical considerations~\cite{sun2024principle,ramezani2023knowledge,hu2024do,kiesel2022identifying,rao2023ethical,lee2023can,sheng2021societal,sharma2023cognitive}.
\rqbcode{Distribution Difference} compares the difference between the output distribution from AI generations and human data to evaluate AI~\cite{patel2021stated,lee2023can}.


% For example, 
% in Ramezani et. al \cite{ramezani2023knowledge}, \textit{probes} have been used to understand how knowledge is encoded in English Pretrained Language Models (EPLMs) to represent moral norms in various countries. For understanding the perception of \textit{facts}, Hu et. al in \cite{hu2024do} introduced Pinocchio benchmark, that enables researchers to assess LLMs' ability to respond on factual knowlegede of up-to-date questions, complex factual tasks that requires multi-hop reasoning, and facts stored in structured datasets such as tables, lists, or databases. Along the similar lines, \cite{kiesel2022identifying}, firstly introduced the definition of \textit{value} and \textit{value system}, a consolidated multi-level taxonomy of 54 human value in cross-cultural setting, and then conducted comprehensive computational analysis to automatically identify human values from benchmarks. Moreover, in \cite{rao2023ethical} Rao et al., came up with a method for decoupling ethical policies and value alignment from LLM training, while instead infusing generic ethical reasoning abilities to AI models. They also developed an extensive framework for specifying ethical policies and evaluating generic ethical reasoning capabilities of LLMs, with the introduction of a reference dataset to understand dilemmas, policies and moral types.
% 
% 
% 
% In a closely related direction of work utilizing extensive computational methods for evaluating value inclusion in AI models and applications, \cite{lee2023can} Lee et al. leverages Log Probability Estimation (LPE) and Monte Carlo Estimation (MCE) to jointly test human disagreement along with LLM performance on natural language inference tasks. Additionally, in a related study, Sheng et. al in \cite{sheng2021societal}, analyzed the propensity of societal bias creep in NLG applications by surveying and identifying two evaluation methods, i.e, Absolute Evaluations, and Relative Scoring based evaluation that can help in identifying societal biases propagated by AI models and applications. 
% 
% 
% 
% Additionally, there is a growing body of research that is rigorously exploring various under-explored forms of biases and stereotypes in AI models and applications. In \cite{felkner2023winoqueer}, Felkner introduced WinoQueer (WQ) benchmark, for measuring anti-LGBTQ+ bias in LLMs, and also shared the framework used for creating WQ to aid in the development of other bias benchmarks for marginalized communities. Moreover, Sharma et al. \cite{sharma2023cognitive}, evaluated the nuanced area of manifestation of negative thoughts from LLMs, and introduced methods for re-framing these thoughts to more neutral and positive responses for bettering human interactions with AI models.










\begin{figure*}[!t]
  \centering
  \includegraphics[width=.98\textwidth]{figures/human2ai1.pdf}
    \caption{The fine-grained topology of ``Align \textcolor{hua-red}{Human} to 
    % \textcolor{hua-yellow}{$\mapsto$} 
    \textcolor{hua-blue}{AI}'' direction, which studies humans' cognitive and behavioral adaptation to the AI systems, which aims to help humans better critique, collaborate with, and co-adapt to AI.
    % % 
    % % % % % % % 
    % % % % 
    % AI Literacy\cite{long2020ai}
    % Intersectional AI:\cite{mcdonald2020intersectional}
    % Anglekindling\cite{petridis2023anglekindling}
    % XAI with Interaction\cite{tenney2020language}
    % Accuracy on Trust\cite{yin2019understanding}
    % Appropriate Reliance\cite{schemmer2023appropriate}
    % GP-TSM\cite{gu2024ai}
    % Algorithmic Fairness\cite{holstein2019improving}
    % Review of Algorithm Audits\cite{bandy2021problematic}
    % Adjusting Expectations\cite{kocielnik2019will}
    % Trust Calibration\cite{wischnewski2023measuring}
    % Specification Alignment\cite{terry2023ai}
    % AI Chains\cite{wu2022ai}
    % PATAT\cite{gebreegziabher2023patat}
    % AILA\cite{choi2019aila}
    % Scattershot\cite{scattershot}
    % Generative Agents\cite{park2023generative}
    % Collaborating Partners\cite{zagalsky2021design}
    % AI Knowledge\cite{pinski2023ai}
    % AI-MC\cite{sundar2022rethinking}
    % AI as Design Materials\cite{yildirim2022experienced}HypoCompass\cite{ma2023hypocompass}
    % Rehearsal\cite{shaikh2023rehearsal}
    % XAI Usefulness\cite{shen2020useful}
    % Human Ideas\cite{ashkinaze2024ai}
    % Privacy in LLM\cite{li2024human}
    % Incidental Learning\cite{gajos2022people}
    % Social Media Misleading\cite{10.1145/3610082}
    % Self Learning with LLM\cite{kazemitabaar2023novices}
    % Anthropomorphism\cite{cheng2022human}
    % Resist in Workspace\cite{park2021human}
    % Regulating ChatGPT\cite{hacker2023regulating}
    % Laypeople’s Expectation\cite{10.1145/3593013.3593992}
    % HR Management\cite{park2021human}
    % AI Fairness Checklist\cite{madaio2020co}
    % RealHumanEval\cite{Mozannar2024TheRE}
    % User-perceived tasks\cite{ding-etal-2023-harnessing}
    % Perceived Control~\cite{ding2023harnessing}
    % Collaborative Code\cite{Perry2022DoUW}
    % Co-design Checklist\cite{zhang2023deliberating} 
    % Regression Analysis\cite{wang2021towards}
    % Whose Opinion\cite{santurkar2023whose}
    % Chess Move Decisions\cite{Zhou2024GenerativeAI}
    % % 
  }
  \label{fig:human2ai}
  % \vspace{-1.5em}
\end{figure*}







% 
% 
% Reshmi introduced
%\rqbcode{Methods to correct human value misalignment in AI:}









\subsubsection{\emph{\textbf{\textcolor{hua-blue}{Ecosystem and Platforms}}}: \textbf{how to build the ecosystem to facilitate human-AI alignment?}}
\label{sec:ecosystem}
\mbox{}
% 
% \rqbdim{Ecosystem and Platforms.} 
The ecosystem and platforms refer to the broader context in which AI systems operate and interact with other agents, platforms, or environments. This includes the infrastructure, frameworks, and technologies that support the development, deployment, and utilization of AI systems. 
% \newline
% 
% 
% 
% 
\rqbcode{LLM-based Agents} are based on large language models (LLMs) such as GPT (Generative Pre-trained Transformer) models, which have been pre-trained on vast amounts of text data~\cite{dubois2024alpacafarm,xu2023gentopia,wu2023autogen,zhou2023sotopia}. 
% Examples include chatbots and language understanding systems. Observed instances of this are in \textit{AlpacaFarm}~\cite{dubois2024alpacafarm} and \textit{Gentopia}~\cite{xu2023gentopia}. 
% \hua{AutoGen, LangChain, Sotopia.}
% \newline
% 
% 
% 
% 
\rqbcode{RL-based Agents} are based on reinforcement learning (RL) algorithms to learn and adapt their behavior based on feedback from the environment or human users~\cite{yuan2024uni}. 
% Examples include autonomous agents and game-playing bots. Key instances of RL-based Systems are seen in \textit{Uni-RLHF}~\cite{yuan2024uni}.
% \newline
% 
% 
% % 
\rqbcode{Annotation Platforms} refers to the ecosystems that are designed to crowdsource human demonstrations as collected data for reinforcement learning~\cite{gerstgrasser2021crowdplay} and supervised finetuning learning for alignment~\cite{pei2022potato}.
% % 
% 
% 
% 
% 
\begin{table*}[ht]
\centering
% \vspace{-10pt}
\begin{tabular}[t]{@{}  !{\color[HTML]{808080}\vrule width 2pt} p{.98\textwidth} !{\color[HTML]{808080}\vrule width 2pt} @{}}
\cellcolor[HTML]{E6E6E6} 
\textbf{Underexplored Dimensions in Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-red}{Humans}} (See Sec~\ref{sec:trend} for supporting data and evidence): 
% \newline
\vspace{5pt}

1. Implicit human feedback and simulated human value feedback are under-explored in existing research work.
\vspace{5pt}

2. Developing and customizing AI during the inference stage or in an interactive way is under-explored.
% 
\vspace{5pt}

3. Human-in-the-loop evaluation is much less explored than automatic evaluation.
\end{tabular}
\end{table*}
% 
% 
\newline
% \newline
\noindent{\textbf{DIRECTION-II:~\hspace*{.0em}\numimg{figures/B.pdf}\hspace*{-.1em} ALIGN \textcolor{hua-red}{HUMANS} to 
% \textcolor{hua-yellow}{$\mapsto$} 
\textcolor{hua-blue}{AI}}} 




\noindent
\say{\emph{When interacting with people, AI agents do not just influence the state of the world – they also influence the actions people take in response to the agent, and even their underlying intentions and strategies}}~\cite{hong2024learning}.
% 
From a \emph{long-term} perspective, it is essential to consider the dynamic changes around human-AI alignment.
% 
% 
This direction outlines alignment research from the \textbf{Human-centered perspective} (e.g., HCI/Social Science domains) and provides \textbf{HCI researchers and user experience designers} with guidance for approaching two core research questions:
% 
% Therefore, research in this direction aims to help humans better understand, critique, collaborate with, and adapt to AI advancements. 
% Besides, interacting with AI could also change human cognition and social behaviors (consciously or unconsciously)~\cite{dautenhahn2000living}, so it is essential to consider this dynamic change into human-AI alignment.
% The two core research questions we identified in this direction are: 
\textbf{RQ3.} Human Cognitive Adjustment to AI (Section~\ref{sec:human2ai3}) and \textbf{RQ4.} Human Adaptive Behavior to AI (Section~\ref{sec:human2ai4}).




% \noindent
% Questions for the long-term individual cognitive and social effects of AI technology we should ask ourselves are:
% - How will agent technology affect human cognition?
% - How will using or interacting with this technology change who we are?
% % 
% If we do not ask such questions, the answers that come to us by letting things run their course in the future may be neither humane nor desirable.
% ~\cite{dautenhahn2000living}
% % 
% % 
% % 
% \textbf{What should humans do to critically adapt to AI advancement?}~\merrie{But also how can interface design support conveying AI affordances to humans and enabling them to steer AI interactions to meet their preferences?}
% \diyi{are humans adapting to AI consciously or unconsciously? }









\subsection{Align \textcolor{hua-red}{Humans} to 
% \textcolor{hua-yellow}{$\mapsto$} 
\textcolor{hua-blue}{AI}:  \hspace*{-0.0in} \img{figures/rqs3.pdf} Human's Perceptual Adaptation to AI}
\label{sec:human2ai3}
% 


\textbf{RQ3. How might humans learn to perceive, explain, and critique AI?}
% 
% 
% 
% % 
% \say{\emph{When interacting with people, AI agents do not just influence the state of the
% world – they also influence the actions people take in response to the agent, and
% even their underlying intentions and strategies~\cite{hong2024learning}.}} 
% 
Humans needs to understand AI to better specify their demands and collaborate with AI. Also, as AI systems produce a range of risks, it is important to elicit humans' critical thinking of AI instead of relying on AI blindly. Therefore, we categorize existing literature to answer the questions of \emph{how humans learn to perceive and understand AI} (Section~\ref{sec:perception}), and  \emph{how to engage in critical thinking on AI?} (Section~\ref{sec:critical_thinking}).
We also answer the two ``\textbf{\textcolor{hua-purple}{Sub-Research Questions}}'' by introducing the answer ``\rqcdim{Dimensions}`` and providing ``\rqccode{Codes}`` associated with ``Example Papers''.
% 
% 
% 
% % 
% Figure~\ref{fig:human2ai} shows the taxonomy of \emph{Align Human to AI} Research Question 3 (RQ3), in which we are primarily interested in exploring the research questions about \emph{human's perceptual adaptation to AI} and \emph{human’s behavioral adaptation to AI}. 
% In this section, we introduce literature concerning human perception and understanding of AI (Section~\ref{sec:perception}). 
% Furthermore, we advocate for the development of critical thinking regarding AI, emphasizing the importance of human agency in its utilization.
% Therefore, we introduce relevant papers addressing this theme in Section~\ref{sec:critical_thinking}.
% % 
% % 






\subsubsection{\emph{\textbf{\textcolor{hua-purple}{Perceiving and Understanding AI}}}: \textbf{how do humans learn to perceive and explain AI systems?}}
\label{sec:perception}
\mbox{} 
% This category addresses how humans perceive and make sense of AI outputs for a broad spectrum of users. 
Addressing the problem of human perception and understanding of AI includes the fundamental education and training required for less technical people to improve understanding of the behind mechanisms and outputs produced by AI systems. It includes visualizations and human-centered explanations tohelp more people learn to understand AI outputs.



\rqcdim{Educating and Training Humans}. AI is increasingly incorporated into the daily lives of a broad spectrum of users, including those with little to no technical knowledge on how AI operates. Here we discuss how to help these less technical people become more AI literate, or better trained to use AI.
% 
% 
% 
% 
\rqccode{AI Literacy and Awareness} is broadly defined as the core competencies required for less technical people to better use and collaborate with AI~\cite{long2020ai}. 
% For example, these competencies include being able to: recognize what is AI and what is not, understand that AI is actually a broad term covering a wide range of technology including robotics and machine learning, and imagine future AI applications and their outcomes \cite{long2020ai}. 
% 
% 
% 
% 
Beyond,
% core competencies,
% that establish a baseline understanding of what AI is and how it operates, 
there is also more in depth and explicit \rqccode{Training Courses} to support individuals to better collaborate and utilize AI~\cite{ketan-ai-medicine-education,mcdonald2020intersectional}. 
% 
% This training can include courses or workshops, or even entire curriculum \cite{ketan-ai-medicine-education} designed to help professionals that are increasingly using AI in their workflows. For example, recent work has proposed that the core education of medical professionals should also include data science fundamentals and other AI related courses so that they could better use and interpret the results from large, black box models providing predictions on patient health outcomes \cite{ketan-ai-medicine-education}.
% 
% 
% 
% 


\rqcdim{AI Sensemaking and Explanations}.
% For more technical users that directly rely on or use AI outputs in their work, 
To improve people's understanding of AI systems and generated outputs, various techniques and approaches have been developed to help people learn to make sense of and explain the model's outputs. 
% Here we emphasize on how to help humans learn sensemaking and explanation of AI systems.
% Concretely, these are interactive approaches to support humans better the \textit{sensemaking} of AI outputs, as well as \textit{human-centered explanations}~\cite{kaur2022sensible}.
% 
% 
% 
% 
\rqccode{Perception and Sensemaking on AI} involves the process through which humans learn to make better sense of AI mechanisms and decision makings~\cite{kaur2022sensible,sivaraman2023ignore,petridis2023anglekindling}.
% more set of techniques for understanding AI outputs~\cite{kaur2022sensible,sivaraman2023ignore}. 
% A canonical version of this is to highlight a particularly influential feature that the model relied on for a classification. For example, AngleKindling system that recommends treatments for patients with Sepsis presents a bar chart indicating the relative importance of each feature to the current prediction \cite{sivaraman2023ignore}. 
% In a similar vein, a recent system that generates potential story angles for journalists to pursue from a press release highlights the most relevant portions of the text that produced that generation; this helped journalists (1) ascertain where the angle came from as well as (2) gather more context for that angle \cite{petridis2023anglekindling}.
% 
% 
% 
% 
People also need to understand how AI systems arrive at specific generated outputs. Prior studies in \rqccode{Human-Centered Explanations} have examined various approaches and interactive techniques to increase human understanding of AI generations and outputs~\cite{tenney2020language,recommender-explanations,smith2020no}.
% Beyond visualizations there are many other mechanisms through which past work has examined helping users understand AI outputs, within \rqccode{Human-Centered Explanations}~\cite{recommender-explanations,smith2020no}.
% Explanations have been studied quite extensively within recommender systems, where many studies have compared the efficacy of different ways to explain why the user was getting a particular recommendation \cite{recommender-explanations}. For example, keywords and tags (e.g. ``comedy'' or ``award winning'') can accompany a recommendation to give users context on how the system characterizes that recommendation. Another way to explain a recommendation is by connecting it to content the user has already consumed (e.g. ``We recommend X because you have seen Y and Z''). These more natural and intuitive explanations are a few classic examples of easily-understood, human-centered explanations~\cite{smith2020no,shen2023convxai}.


% 
% 


% Typical calibration strategies include 

% -Prior to the interaction: Prior information about the system such as capabilities, reliability, consistency, consensus, distinctiveness of the automated aid’s performance, or malfunctions; training phase; cognitive forcing

% -During the interaction: Cues (alarms, warning signals, augmented reality cues, confdence cues or updates); uncertainty displays; communication style (command vs. status); explanations; interactivity (e.g., promise to perform better in the future)

% -After the interaction: Feedback type (automation feedback independent of user, feedback on trust behavior of user); performance feedback





\subsubsection{\emph{\textbf{\textcolor{hua-purple}{Critical Thinking around AI}}}: \textbf{how do humans think critically about AI systems?}}
\label{sec:critical_thinking}
\mbox{}
% 
Beyond simply perceiving and understanding AI, individuals need to compare their mental model of AI with their own mental model to judge whether the AI is behaving rationally and ethically.
Broadly, this involves exploring the ways in which humans engage in critical thinking and reflect on their interactions with and evolving understanding of AI technologies. 
% 
Here we discuss studies that help humans become more capable to identify biases and errors in AI output, and the ethical implications that arise from using AI algorithms in decision-making processes. Also, we discuss how humans need to calibrate their mental models to be more aligned with AI.
% The papers in this category relate to the fostering of informed decision-making, ethical reasoning, and responsible use of AI technologies through the development of cognitive skills and competencies related to AI literacy and awareness. This category is further broken down into two dimensions, \emph{Trust and Reliance on AI Decisions} and \emph{Ethical considerations and AI auditing}.


\rqcdim{Trust and Reliance on AI Decisions} refers to the extent to which people mentally trust the AI competency and practically rely on AI for output generation and decision making.
% individuals place confidence on the decisions and output generated by AI systems. 
% This dimension explores the factors influencing trustworthiness, perceived reliability, and the subsequent selective adoption of AI technologies. 
We use the term \rqccode{Trustworthiness} to indicate whether humans decide to trust the reliability, integrity, and competence of an AI system in delivering accurate and trustworthy decisions or recommendations to the users~\cite{yin2019understanding,ma2023should,srivastava2023role}. 
% 
% Measures to capture trustworthiness include \emph{appropriateness of Trust}~\cite{ma2023should} and \emph{lexical alignment} \cite{srivastava2023role}. 
% 
We define \rqccode{AI Reliability} as to what extent humans utilize and rely on AI to automate decision making in practice with low error rates and robustness performance~\cite{schemmer2023appropriate}.
% an evaluation of the consistency, predictability, and performance quality of AI systems across different contexts and scenarios
\cite{schemmer2023appropriate,vasconcelos2023explanations,suresh2022intuitively}. 
% Examples include error rates and robustness testing. \citet{suresh2022intuitively} had people probe a model and reason about its behavior through familiar examples grounded in domain knowledge, demnonstrating how grounding interpretability in real examples, facilitating comparison across them, and visualizing data distributions can aid in grasping a model’s uncertainty and connecting it to relevant challenges in the task. 
\rqccode{Selective AI Adoption} refers to the criteria and considerations that guide the adoption or rejection of AI technologies based on their perceived benefits, risks, and alignment with user needs and preferences~\cite{gu2024ai,vasconcelos2023explanations}.  
% One salient example is that of \emph{overreliance}, i.e., when people agree with an AI, even when it is incorrect. The associated risk-assessment framework posits that when tasks require more effort and the explanations sufficiently reduce the cost of verifying the AI, or when the explanations are easier to understand, explanations will reduce overreliance \cite{vasconcelos2023explanations}.
%Examples include risk assessment frameworks and technology acceptance models. 










\rqcdim{Ethical Considerations and AI Auditing} refers to potential moral and societal issues that arise from the development, deployment and use of AI systems, as well as systematic examination and evaluation of AI systems regarding these issues.
\rqccode{Ethical Concerns and AI Mitigation} encourages humans to carefully consider if the AI systems possess ethical concerns (\eg such as bias and discrimination, privacy violations and the potential for harm or misuse) and implement strategies and practices to address and reduce these ethical concerns associated with AI~\cite{holstein2019improving}.
% 
\rqccode{Audit Deployed AI} refers to the systematic examination of AI systems to ensure that they operate as intended, comply with ethical and legal standards, and do not cause unintended harm~\cite{bandy2021problematic}.


% includes, on one hand, human assessment of the fairness, accountability, transparency, and ethical implications of the decision-making processes embedded in AI technologies. On the other hand, we regard ethical AI practices, i.e., diversity, equity, and inclusion in AI development and deployment. 
% 
% % =====================================================
% % =====================================================
% % =====================================================
% % =====================================================
% \rqccode{Fairness and Accountability} examines the extent to which AI systems exhibit fairness, impartiality, and accountability in their decision-making processes and outcomes.
% % particularly concerning bias mitigation and fairness-aware algorithms~\cite{holstein2019improving,lee2023understanding}. 
% % Providing counterfactual examples as explanation for AI decision-making were found to support critical thinking around how to change an AI output and more rigorously review AI output than widely used AI feature-example explanations \cite{lee2023understanding}. 
% % 
% In HCI, the critical analysis of AI systems has a strong focus on \rqccode{Diversity, Equity and Inclusion}, which includes advocacy for a wide set of voices, equitable data collection practices (e.g., treatment of and access to data) and cultivating a sense of belonging in AI development and deployment~\cite{10.1145/3544548.3580903,kapania2023hunt}. 
% % The aim is to increase representation, accessibility, and fairness for diverse populations and groups who have been historically marginalized. Improving representation in the data annotation stage through removing the separation
% % between ML practitioners and data annotators who usually do not interact, combined with an intersectional shift towards annotators’ lived experiences was shown to have potential to mitigate bias in AI output \cite{kapania2023hunt}.









\rqcdim{Re-Calibrating Cognition to Align with AI}. This sub-category deals with interventions and techniques to help users adjust (1) their own mental model of how the AI operates and (2) recalibrate their perception of the AI.
% 
% 
% 
% 
\rqccode{Updating Human Mental Model of AI} means that when the AI is not aligned with humans, it is important to adjust human perceptions of the confidence in AI systems based on the model's capability and track record~\cite{he2023interaction,kocielnik2019will} .
% Example: trust calibration strategies, reliability assessments.
% For example,~\citet{he2023interaction} proposes a capability-aware shared mental model (CASMM) with the components of task grouping and negotiation, which utilize tuples to break down tasks into sets of scenarios relating to difculties and then dynamically merge the task grouping ideas raised by human and AI through negotiation.
% The result shows building CASMM boosts the accuracy and time efciency signifcantly through forming the task assignment close to real capabilities within few iterations. It helps users better understand the capability of AI and themselves.
% 
\rqccode{Recalibrating Trust and Reliability} indicates that humans adjust their perceptions of trust and reliability in AI systems based on their performance and reliability. This is also important to foster appropriate reliance and skepticism~\cite{wischnewski2023measuring}.
% 
% For example,~\citet{wischnewski2023measuring}  identifed 96 relevant publications which aimed to calibrate users’ trust in automated systems.
% To facilitate the trust calibration, one broader strategy was to implemented interventions to increase transparency (e.g., cues, warning signals, explanations). Also, automation feedback independent of user or provide feedback on trust behavior of user is also potential strategy to calibrate user trust.






%For example, \citet{shen2023convxai} borrowed inclusive design principles to frame human the evaluation of human writing processes via ConvXAI, an AI system created to support human-AI collaboration in scientific writing.
%Examples include fairness metrics and bias detection tools. 
%Example: diversity hiring practices, inclusive design principles.

\subsection{Align \textcolor{hua-red}{Humans} to 
% \textcolor{hua-yellow}{$\mapsto$}
\textcolor{hua-blue}{AI}:  \hspace*{-0.0in} \img{figures/rqs4.pdf} Human’s Behavioral Adaptation to AI}
\label{sec:human2ai4}



\textbf{RQ4. How do humans and society make behavioral changes and react to AI advancement?}
% 
As AI becomes increasingly integrated into daily life, it is essential to understand its influence on humans, encompassing both positive and negative aspects. 
% 
Moreover, it is crucial to determine how individuals and society can best and most appropriately respond to this influence.
% 
To this end, we summarize literature to answer \emph{how do humans learn to collaborate with AI in diverse AI roles?} (Section~\ref{sec:collaboration}), \emph{how humans and society are impacted by AI
% what are AI's impacts on humans and society
} (Section~\ref{sec:impacts}) and \emph{how might we assess these impacts?} (Section~\ref{sec:assessment})
We articulate the three ``\textbf{\textcolor{hua-red}{Sub-Research Questions}}'' by introducing the answer ``\rqddim{Dimensions}`` and providing ``\rqdcode{Codes}`` associated with ``Example Papers''.

% 
% % 
% % 
% In addition to examining human perception and critical thinking regarding AI, we investigate how humans adapt their behavior to AI advancements. 
% We introduce various collaborative mechanisms between humans and AI with different roles (Section~\ref{sec:collaboration})
% % 
% 
% % 
% Beyond human perception and critical thinking on AI, we further explore how humans adjust their behavior to AI advancements.
% Particularly, we not only introduce different collaborative mechanisms between humans and AI (Section~\ref{sec:collaboration}). Also, we explicitly point out potential risks and negative impacts that AI could bring to individuals and the society. In this way, we aim to provide a more objective and comprehensive view of how to \emph{align human to AI}.

\subsubsection{\emph{\textbf{\textcolor{hua-red}{Human-AI Collaboration Mechanisms}}}: \textbf{what are human strategies to collaborate with AI that have differing levels of capabilities?}}
\label{sec:collaboration}
\mbox{}
%
This category looks at many ways that humans and AI can collaborate, such as teamwork, co-creation, and coproduction. 
%forming a powerful whole when either party takes the main charge. 
% It also examines how they communicate, what each is responsible for, and what helps or hurts their success. The goal is to understand how humans and AI can best work together to achieve their goals.




\rqddim{AI Assistant for Humans} captures the essence of a symbiotic relationship where AI systems are designed to bolster human capabilities, with humans steering the interactions.  
% In this collaborative model,  LLM has become the new type of medium to facilitate interaction and collaboration. 
\rqdcode{LLM-based Demand Specification} employs LLMs to interpret and respond to human requests, powering virtual assistants and chatbots that streamline information retrieval and improve task accuracy~\cite{terry2023ai}. This naturally extends to \rqdcode{LLM-based Prompt Strategy}, which helps humans to better write prompts using 
% where the 
additional abstraction and scaffolding methods.
% are introduced on top of traditional text-to-text workflow. 
The example system can enhance humans' capability in generating intelligent prompts and suggestions, such as autocomplete and question-generation tools for LLM-based systems~\cite{wu2022ai, wang2024farsight}, facilitating humans' smooth and intuitive decision-making processes. 
In the creative arena, \rqdcode{LLM-based Prototypes} utilize AI to transform human ideas into tangible or organized concepts ~\cite{gebreegziabher2023patat}, enabling professionals to explore and refine a wide array of artistic possibilities with AI-generated options~\cite{huh2023genassist}. 
On a broader note, researchers have also explored how \rqdcode{AI-Assisted Task and Decisions} 
aims to achieve complementary performance for human-AI collaborative tasks by empower humans to discern when and how to adopt AI-assisted recommendations or AI-generated explanations for decision-making~\cite{choi2019aila,wang2022will, wang2023watch,zheng2023competent,scattershot}.  
% leverage conventional AI techniques to analyze vast datasets for predictions and recommendations, underpinning recommendation systems and predictive analytics that optimize content delivery and strategic foresight for both individual~\cite{wang2022will, wang2023watch} and group decisions~\cite{zheng2023competent}. 
% 
% % 
% % =====================================================
% % % =====================================================
% \rqdcode{Improve AI Systems} leverages human feedback and interaction to collaboratively analyze, intervene with and improve AI systems, such as fairness and accuracy performance~\cite{kwon-mihindukulasooriya-2023-finspector,piorkowski2023aimee}.


% Together, these applications of AI do not replace human expertise but significantly enhance the breadth and depth of human operation across various fields.

% %
% % \rqddim{AI Assistant for Human} describes a collaborative framework where artificial intelligence (AI) systems enhance human capabilities, with humans leading the interaction. This partnership manifests in several distinct ways across various applications. For instance, ...
% %
% %
% % 
% % 
% \rqdcode{LLM-based Demand Specification.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{LLM-based Prompt Strategy.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{LLM-based Prototypes.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{Traditional AI-Assisted Decision Making.} Definition + example papers.






\rqddim{Human-AI Partnership} refers to a collaborative relationship where humans and AI systems work together as partners, combining their respective strengths to achieve shared goals more effectively.
% 
% Humans contribute contextual understanding, creativity, and high-level reasoning, while AI excels at rapid data processing, pattern recognition, and complex computations. By synergistically melding human ingenuity with artificial intelligence capabilities, these partnerships enable innovations that harness the best of both worlds.
% 
% In a Human-AI Partnership, the symbiotic collaboration between humans and artificial intelligence systems is facilitated through various mechanisms. 
\rqdcode{Simulated Agency} enables humans to collaborate with AI partners with
% endows AI systems with 
simulated agency or autonomy (\eg autonomous agents and collaborative robots~\cite{park2023generative}) to make decisions collaboratively.
% and take actions in collaboration with human partners, 
% as exemplified by autonomous agents and collaborative robots~\cite{park2023generative}.
\rqdcode{Reciprocal Learning} focuses on how humans learn from and exchange knowledge with AI systems,
% mutual learning and knowledge exchange between humans and AI systems, 
enhancing human-AI collective capabilities and performance through knowledge-sharing platforms and collaborative filtering~\cite{zagalsky2021design,pinski2023ai}. \rqdcode{AI Delegation} allows humans to delegate AI partners to help finish tasks or responsibilities,
% to delegate tasks or responsibilities to human partners based on their expertise or preferences, 
facilitated by task assignment algorithms and workflow management systems~\cite{pinski2023ai}. 
Furthermore, \rqdcode{AI-Mediated Tasks} emphasizes how traditional human tasks or behaviors (\eg communication) would be changed by incorporating AI partners in the loop~\cite{bernstein2010soylent,sundar2022rethinking,xu2023augmenting}. 
\rqdcode{Co-Design with AI} explores AI as a design material or a partner in prototyping, which enables humans to converse with AI in situations that can collaboratively improve the design outcomes. 
\cite{yildirim2022experienced,wang2024farsight}
% coordinate activities where both human and AI entities contribute to 
% problem-solving or decision-making processes~\cite{xu2023augmenting}, as seen in crowd-computing platforms and human-in-the-loop systems~\cite{bernstein2010soylent, bigham2010vizwiz}.
% 
% These mechanisms work in concert to create a cohesive partnership, where humans and AI systems collaborate seamlessly, leveraging their respective strengths to achieve shared goals through co-creation and innovation.
% % 
% % 
% % 
% % 
% \rqdcode{Simulated Agency.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{Reciprocal Learning.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{AI Delegation.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{AI-Mediated Tasks.} Definition + example papers.











\rqddim{AI Tutoring for Human Learning} 
investigates how humans improve their learning and knowledge throughinteractions with AI tutors that can perform better than humans in some tasks.
% involves employing AI systems to provide personalized guidance and support throughout the learning process. 
With the tailored instructions and customized feedback from AI tutors, humans can enhance their the learning outcomes and facilitate mastery of new skills more effectively than traditional learning methods.
% These AI tutors leverage advanced technologies to adapt to individual needs, offering tailored instruction, customized feedback, and optimized learning pathways. By dynamically adjusting to each learner's progress and areas for improvement, AI tutoring systems aim to enhance the learning outcomes and facilitate mastery of new skills more effectively than traditional methods.
% 
% 
\rqdcode{AI Tutor for Technical Skills} refers to empowering humans to learn technical skills from AI tutors.
% One common theme of the AI tutoring system is \rqdcode{AI Tutor for Technical Skills}. 
For technical subjects like coding, AI tutors can analyze a learner's progress in real time, adjusting the pace, content, and approach to ensure a solid understanding of complex concepts and practical skills such as programming~\cite{ma2023hypocompass}. 
% Through personalized examples, interactive exercises, and immediate feedback, these systems identify knowledge gaps and provide targeted support. 
% 
% 
Similarly, \rqdcode{AI Tutor for Social and Behavioral Skills} involves enabling humans to learn social and behavioral skills from AI tutors.
% 
% The other common theme of the AI tutoring system is \rqdcode{AI Tutor for Social and Behavioral Skills}. 
% For social and behavioral skills, 
Humans can leverage virtual simulations, created by AI tutoring systems, to 
% AI tutoring systems create realistic virtual simulations for learners to 
practice public speaking, interpersonal communication, and other soft skills. By analyzing verbal and non-verbal cues, humans can receive 
% these AI tutors offer 
constructive feedback on areas such as body language, tone, and delivery from AI, ultimately enhancing their ability to communicate effectively across various settings~\cite{peng2021say, shaikh2023rehearsal}. 
% 
% As these technologies continue to evolve, AI tutoring systems hold promising prospects for reshaping the learning experience and fostering a more engaging, personalized, and effective skill-acquiring journey for individuals of all ages and backgrounds.


% % 
% % 
% % 
% % 
% \rqdcode{AI Tutor Technical Skills.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{AI Tutor Social and Behavioral Skills.} Definition + example papers.





















\subsubsection{\emph{\textbf{\textcolor{hua-red}{AI Impact on Humans and Society}}}: \textbf{how are humans influenced by AI systems
% influencing humans
?}}
\label{sec:impacts}
\mbox{}
This category explores the effects of AI advancement on human behaviors, attitudes, and societal dynamics. It involves examining the behavioral changes, adaptations, and reactions that individuals, groups and wider communities undergo in response to the proliferation of AI technologies. 
% This includes assessing the impacts of AI on employment patterns, job skills, social interactions, decision-making processes, and cultural norms. Additionally, it examines the broader societal implications of AI, such as economic disparities, ethical dilemmas, and power dynamics. 
The goal is to elucidate the multifaceted impacts of AI on human behavior and society and to inform policy-making, education, and intervention efforts.  
% This category is further broken down into three dimensions, \emph{Impact on Participatory Individuals and Groups, Societal Concerns and AI Impacts} and \emph{Reaction to AI Advancement}.


\rqddim{Impacts on Participatory Individuals and Groups} covers the effects of AI advancement on the behaviors, attitudes, and experiences of both individuals and groups. This dimension focuses on examining how AI technologies influence decision-making, creativity, privacy, and authorship. \rqdcode{Decision Making} refers to analyzing how AI technologies influence human decision-making processes, including biases, preferences, and risk assessment, in various domains such as healthcare, finance, and personal life~\cite{shen2020useful}. 
% 
% 
% 
%Example: automated decision support systems, algorithmic decision-making.
\rqdcode{Human Creativity} explores the impact of AI technologies on human creativity, innovation, and expression, including the augmentation or automation of creative tasks and the emergence of new forms of artistic expression~\cite{ashkinaze2024ai}.
% 
% 
% 
%Example: AI-generated art, creative AI tools.
\rqdcode{Privacy} relates to investigating the implications of AI technologies for individual privacy rights, data protection, and surveillance, including concerns about data collection, tracking, and algorithmic profiling~\cite{li2024human}.
% 
%Example: privacy-preserving techniques, data anonymization.
% 
% 
\rqdcode{Authorship} catalogs issues related to intellectual property, attribution, and ownership of AI-generated content, including questions of legal responsibility, copyright infringement, and plagiarism detection. Salient is that AI can produce increasingly realistic, synthetic data quickly and at low cost, which brings forth tensions around the use of such data to make decisions~\cite{hamalainen2023evaluating,10.1145/3610082}. 






\rqddim{Societal Concerns and AI Impacts} involves the broader societal implications and consequences of AI advancement on misinformation, education, social relationships, norms, job displacement, and other aspects of human society.
% 
%Example: copyright laws, attribution algorithms.
% 
% 
% 
% 
\rqdcode{Misinformation and Moderation} concerns the challenges of misinformation, disinformation, and online content moderation in the context of AI-driven information ecosystems, including concerns about algorithmic bias and filter bubbles~\cite{10.1145/3610082}. 
% 
% 
%Example: content moderation algorithms, fake news detection.
% 
\rqdcode{Impacts on Education} pertains to assessing the effects of AI technologies on education systems, learning outcomes, pedagogical practices, and workforce training, including opportunities for personalized learning and skill development~\cite{kazemitabaar2023novices}.
% 
%Example: AI-powered tutoring systems, adaptive learning platforms.
% 
% 
% 
% 
\rqdcode{Impacts on Social Relationship and Norms} explores how AI technologies shape interpersonal relationships, social interactions, and cultural norms, including changes in communication patterns, social dynamics, and ethical considerations~\cite{cheng2022human}.
% 
% 
% 
% 
\rqdcode{Workplace} refers to examining the effects of automation and AI technologies on employment patterns, job markets, and workforce dynamics, including concerns about job displacement, re-skilling, and economic inequality~\cite{park2021human}.





\rqddim{Reaction to AI Advancement} involves societal responses, regulatory frameworks, and policy initiatives aimed at addressing the challenges and opportunities posed by AI technologies. This dimension encompasses efforts to regulate AI deployment, re-calibrate societal acceptance, and manage potential backlash. For example, reaction to bias and discrimination in algorithmic decision making can depend on how people perceive the machine and the context of use,  i.e., if the machine is considered an actor embedded in social structures that call for blame
when harmful decisions are made \cite{lima2023blaming}. \rqdcode{AI Regulatory and Policy} includes regulatory frameworks, legal frameworks, and policy initiatives aimed at governing AI development, deployment, and use, including concerns about ethics, safety, and accountability~\cite{hacker2023regulating,lucaj2023ai}.
% 
%Example: AI ethics guidelines, regulatory compliance frameworks.Definition + example papers.
% 
% 
% 
% 
\rqdcode{Shifts in AI Acceptance} relates to investigating societal attitudes, organizational practices, and acceptance of AI technologies over time in practice, including shifts in public opinion and AI utilization by humans and institutes regarding AI deployment and impact~\cite{10.1145/3593013.3593992,10.1145/3593013.3593999}.
% 
% 
% 
% % =====================================================
% % =====================================================
\rqdcode{Surveillance and Intervention} emphasizes the need for transparency, monitoring, and human oversight in the algorithmic decision-making process. This approach enables better human control over AI systems and helps mitigate potential risks associated with their use~\cite{park2021human}.
% 
% calls for incorporating transparency, surveillance and human intervention to algorithmic decision-making process. In this way, human can better control AI and prevent AI from risky impacts in practice~\cite{park2021human}.
% 
\rqdcode{Responsible AI Checklists} involves the creation of ethical guidelines, such as those focusing on fairness and transparency, to ensure the responsible development and deployment of AI systems. These published principles serve as a foundation for guiding ethical AI practices~\cite{madaio2020co}.
% designs AI ethics checklists for responsible AI requirements, like fairness and transparency, as published principles to guide the ethical development and deployment of AI systems~\cite{madaio2020co}.
% Example: public opinion surveys, trust indices. public resistance, skepticism,
% 
% 
% 
% 
% \rqdcode{Backlash}. Exploring instances of public resistance, skepticism, or opposition to AI technologies, including concerns about job displacement, privacy violations, and ethical dilemmas~\cite{10.1145/3593013.3593999}.






\subsubsection{\emph{\textbf{\textcolor{hua-red}{Evaluation in Human Studies}}}: \textbf{how might we evaluate and understand the impact of AI on humans and society?}}
\label{sec:assessment}
% \mbox{}
% 
We summarize common empirical methods used to rigorously understand and assess the impact of AI on humans. Specifically, we focus on two types of impact. On the micro-level, we discuss how to evaluate the effectiveness of human-AI collaboration; on the macro-level, we discuss how to assess the impact of AI on a large group of people over a long period of time. 


\rqddim{Evaluate Human-AI Collaboration} refers to the evaluation of the effectiveness of an AI system in collaboration with humans. It is key to not only consider the final output, but also the interaction experience~\cite{Lee2022EvaluatingHM}. 
% We summarize several main metrics and methods that are used for such assessment. 
% 
% 
% 
% 
\rqdcode{Human-AI Team Performance} 
% On measuring outcome, one important dimension is to 
compares human-AI team performance with the performance of humans alone without AI collaboration 
%(or sometimes with 
% the condition of 
%AI alone if applicable). 
The metrics for measuring performance should include both task success metrics (e.g., accuracy) as well as indicators of efficiency~\cite{Mozannar2024TheRE,ding-etal-2023-harnessing}. 
%
% For example, RealHumanEval~\cite{Mozannar2024TheRE} evaluates LLM-assisted coding with different backbone language models and interaction modes in comparison with the control condition of no LLM assistance, where they compared with the task success rate as well as the task completion time. 
%
% ~\citet{ding-etal-2023-harnessing} evaluates human-AI news headline co-writing where they evaluated the quality of the co-written headlines versus control conditions using the Taste-Attractiveness-Clarity-Truth test from 1 (best) to 6 (worst) as the performance metric. 
% 
% 
\rqdcode{Cognitive Workload and User Satisfaction} 
% Apart from measuring whether AI systems are helping humans solve the task at hand better, another important dimension for evaluation is the cognitive workload 
involves understanding the degree of cognitive load that the user experiences when interacting with the system, as well as user satisfaction with the interaction and the final outcome. Such aspects are often captured via surveys or interviews \cite{ding-etal-2023-harnessing,Lee2022EvaluatingHM}.
% For example, ~\citet{ding-etal-2023-harnessing} collected user-perceived task difficulty with and without LLM assistance via a survey question using a Likert scale of 1 to 5 along with rationales. \citet{Lee2022EvaluatingHM} surveyed user-perceived helpfulness and the ease of user of LLM systems in tasks like question answering and crossword puzzle solving. 
% 
% 
%
\rqdcode{Control and Trust} refers to how user control can 
% Apart from improving task performance and ensuring user satisfaction, another important aspect is to preserve the users' control and ensure appropriate trust. This 
support the avoidance of catastrophic AI failures, especially in high-stakes settings where AI mistakes could lead to harm~\cite{Si2023LargeLM,ding2023harnessing}. 
% For example, \citet{ding2023harnessing} designed survey questions to gauge users' perceived control and trust in the LLM co-writing system via 5-point Likert rating scales. 
% ~\citet{Si2023LargeLM} measured user trust calibration on LLM assistance in detecting false claims via Likert-scale questions and found that users tend to over-rely on AI suggestions. 
% 
% 
% 
% 
% 
\rqdcode{Interaction Behavioral Analytics} refers to  measuring task performance quantitatively. This approach includes recording user interaction data and analyzing the patterns~\cite{Villalba2023AutomatedIO,Perry2022DoUW}.
% Lee2022CoAuthorDA,
% 
% For example, \citet{Perry2022DoUW} recorded users' code written in collaboration with LLMs and found participants who had access to an AI assistant wrote significantly less secure code than those without access to an assistant, and participants with access to an AI assistant were also more likely to believe they wrote secure code. 
% ~\citet{Lee2022CoAuthorDA} created a human-LLM co-writing platform and recorded human-AI co-writing sessions to analyse how users tend to co-write with LLMs. ~\citet{Villalba2023AutomatedIO} collected user interview data with LLM chatbots as AI interviewers and analysed the characteristics of user responses to AI-generated follow-up questions such as response lengths and diversity. 
% 
% 
\rqdcode{Qualitative Survey and Interviews } refers to qualitative approaches to understanding human-AI interaction. Commonly used methods include qualitative survey questions (i.e., open-ended) and user interviews to assess aspects of the user experience.~\cite{zhang2023deliberating}.
% 
% % 
% % 
% % =====================================================
% % =====================================================
\rqdcode{Statistical Analysis} utilizes methods such as regression analysis to quantitatively analyze and evaluate data from human studies, allowing for the verification of hypotheses~\cite{wang2021towards}.





\rqddim{Evaluate Societal Impact} 
% Apart from evaluating how well AI can assist humans in solving particular tasks, another important question is to 
refers to the macro-impact of a group of people as they come to use AI broadly. This dimension requires sufficient scale and time. The aim is to understand how the group's behavior changes as people within it frequently interact with AI. 
% We outline a few typical approaches along with examples below. 
% 
% santurkar2023whose,Shin2023SuperhumanAI
% 
\rqdcode{Public Opinion Surveys} aims to investigate the impact of AI on human measures of interest though deploying and analyzing large scale questionnaires 
~\cite{santurkar2023whose}.
% 
\rqdcode{Behavioral Data Analytics}
% The most common approach is to 
collects large-scale and potentially longitudinal behavior data, with the aim of understanding how pattern evolve over time~\cite{Shin2023SuperhumanAI,Zhou2024GenerativeAI}. 
% For example, ~\citet{Shin2023SuperhumanAI} analyzed 5.8 million chess move decisions made by professional Go players over the past 71 years to analyze the change over time, and found that  humans began to make significantly better and novel decisions following the advent of superhuman AI, potentially as a result of them playing with AI chess players and studying AI strategies. ~\citet{Zhou2024GenerativeAI} analyzed a dataset of over 4 million artworks from more than 50,000 unique users, and found that while peak artwork content novelty increases over time, average content novelty declines with the increasing adoption of text-to-image technologies. 
% 


% \rqdcode{Semi-Structured Interviews} Definition + example papers.


% \rqdcode{Observational Studies} Definition + example papers.


\begin{table*}[ht]
\centering
% \vspace{-10pt}
\begin{tabular}[t]{@{}  !{\color[HTML]{808080}\vrule width 2pt} p{.98\textwidth} !{\color[HTML]{808080}\vrule width 2pt} @{}}
\cellcolor[HTML]{E6E6E6} 
\textbf{Underexplored Dimensions in Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-blue}{AI}} (See Sec~\ref{sec:trend} for supporting data and evidence): 
% \newline
\vspace{5pt}

1. Educating and training humans on AI literacy is under-investigated.
\vspace{5pt}

2. Auditing AI for various ethical values is not fully explored.
% 
\vspace{5pt}

3. The collaboration between humans and AI with similar or superior capabilities is under-explored.
\vspace{5pt}


4. The societal impacts of and reactions to AI advancements are not fully explored.
\end{tabular}
\end{table*}
% 
























% ========================== dead kitten ========================== 






















% ======================= Interaction Part ================== 

% \subsection{Design Space of \textcolor{hua-yellow}{Interaction} in Human-AI Alignment}
% \label{sec:ai2human}





% \begin{figure*}[!ht]
%   \centering
%   \includegraphics[width=1\textwidth]{figures/interaction1.pdf}
%   \caption{The Taxonomy of Interactions for Human-AI Alignment.
%   }
%   \label{fig:interaction}
% \end{figure*}




% \textbf{\textcolor{hua-yellow}{RQ5. Interaction Approaches for Alignment}}: What were the interactive methods to achieve alignment process?
% \mbox{}


% ======================= Interaction Part ================== 


==> sections/limitation.tex <==
In this section, we provide a summary of the key implications of our proposed framework, and discuss the challenges and limitations we encountered during the systematic literature review process.


\subsection{Framework Implications and Applications}


% \noindent
\subsubsection{\textbf{Cross-domain inspirations.}}
Achieving long-term human-AI alignment requires holistic, interdisciplinary efforts. This paper introduces a bidirectional human-AI alignment framework to create a shared vocabulary among diverse fields. Supported by over 400 multi-domain research papers, this framework \textbf{enables researchers to integrate knowledge from other domains, enhancing their work and fostering synergetic collaboration.}
% 
Particularly, AI researchers can use the human value taxonomy grounded in psychological theories (\eg Section~\ref{sec:gap_value}) to develop datasets and algorithms that incorporate a broader spectrum of human values. Additionally, by examining studies on individual and societal adaptations to AI alignment (\eg Section~\ref{sec:impacts}), AI developers can create more practical and adaptive AI systems that evolve alongside human and societal changes.
% 
% 
Conversely, HCI and social science researchers can leverage customizable AI alignment algorithms (\eg Section~\ref{sec:ai2human2}) to design interactive systems that improve human interaction with AI. By using interaction techniques to specify human values (Section~\ref{sec:ai2human1}), these researchers can optimize interfaces or conduct surveys to extract human values, informing AI alignment development.
% 





\subsubsection{\textbf{Foundation of Dynamic Alignment Evolution.}}
% 
The proposed bidirectional human-AI alignment framework also \textbf{serves a foundational role to support researchers to address the outlined future challenges and achieve long-term alignment}.
% 
As elaborated in Section~\ref{sec:discussion}, within each direction, researchers can potentially address future challenges on the basis of existing alignment studies organized by the framework.
For instance, to tackle the specification game, future AI researchers can use the comprehensive human value taxonomy outlined in the framework (Section~\ref{sec:discussion}) to develop methods for selecting the appropriate subset of these human values to be integrated into AI alignment.
% 
% 
Additionally, we emphasize the importance of synergizing both directions to achieve long-term bidirectional human-AI alignment. To facilitate dynamic co-evolution (Section~\ref{sec:challenge2}), we advocate for collaboration among AI, HCI, and social scientists to measure human and societal adaptations and incorporate these changes into the alignment of next-generation AI systems.
% 
This holistic approach can contribute to the evolution of AI in harmony with human values and societal needs.



==> sections/method.tex <==



% This paper is a collaborative effort consisting of a team of researchers across multiple domains, including Human-Computer Interaction (HCI), Natural Language Processing (NLP), Machine Learning (ML), Data Science (DS), Social Science, and Cognitive Science. 
\noindent
Addressing alignment challenges is a complex and multifaceted process. 
To develop a comprehensive perspective of the ongoing and mutual process of human-AI alignment,
this section begins by introducing core definitions and key components of alignment. Subsequently, we outline our methodology for conducting a systematic literature review and the rationale behind our proposed framework of \emph{bidirectional human-AI alignment}.

% % 
% we clarify three core questions before presenting the scope and process of systematic literature review: 
% ``\emph{With whom to align?}'', ``\emph{What is the goal of alignment?}'', and ``\emph{What values should be aligned with?}''




% In this section, we aim to develop a holistic framework encompassing the \emph{ongoing and mutual process} of human-AI alignment given the background in Section~\ref{sec:background}. To this end, we first introduce the core definitions of human-AI alignment (Section~\ref{sec:definition}) and present the scope and its generalizability (Section~\ref{sec:scope}). Next, we perform a systematic literature review guided by the PRISMA workflow (Section~\ref{sec:prisma}) and undertake an iterative coding process to achieve our \emph{bidirectional human-AI alignment} framework (Section~\ref{sec:framework}).








% \vspace{-.8em}
% \subsection{Definitions}
% \label{sec:definition}




% To achieve the aforementioned \emph{ongoing and mutual process of human-AI alignment},
% we clarify three core questions before presenting
% % two core questions need to be clarified before we delve into
% the scope and process of systematic literature review: 
% ``\emph{With whom to align?}'', ``\emph{What is the goal of alignment?}'', and ``\emph{What values should be aligned with?}''










% \subsubsection{\textbf{What is the goal of alignment?}}
\subsection{What is the goal of alignment?}
\label{sec:align_goal}
The research on alignment between humans and AI has introduced multiple alignment goals~\cite{park2023generative,xie2024can}, such as \emph{intentions}~\cite{ouyang2022training,anwar2024foundational}, \emph{preferences}~\cite{bansal2023peering,verma2023hindsight}, \emph{instructions}~\cite{bai2022constitutional,liu2023makes}, and \emph{values}~\cite{sorensen2024roadmap,gabriel2020artificial}.
% and others~\cite{park2023generative,xie2024can}. 
However, researchers often use these terminologies interchangeably without clarifying their distinctions.
Drawing from a philosophical view, 
% we refer to~\citet{gabriel2020artificial} and visualize the relations, definitions, and limitations of prevailing alignment goals in Table~\ref{fig:definitions}. 
we summarize the prevailing alignment \emph{goals, their relationships, definitions, and limitations} and visualize them in Table~\ref{fig:definitions} referring to an extensive analysis of the advantages and limitations of different goalss in existing studies~\cite{gabriel2020artificial,stuart2014whitepaper} .
% 
% After an extensive analysis of the advantages and limitations of different goals,
Particularly, \citet{gabriel2020artificial} argues \emph{values}, e.g., moral beliefs and principles, to be the best possible goal at the current stage for AI development for focusing alignment. 
We further summarized the rationale behind this argument and the discussion of the trade-offs that arise from this choice in Table~\ref{fig:definitions}.
% 
The claim of ``aligning AI with human values'' is not new, as Stuart Russell~\cite{stuart2014whitepaper} has stated back in 2014 that \say{\emph{for an autonomous system to be helpful to humans and to pose no unwarranted risks, it needs to align its values with those of the humans in its environment in such a way that its actions contribute to the maximization of value for the humans.}}
% 
Therefore, in this work, we \textbf{consider the goal of alignment as ``human values''}, which means AI systems do what people morally
ought to do, as defined by individuals or society. 
% 
% 
% We further revolve our paper review and data analysis around clarifying and categorizing human values. Particularly, to disambiguate the inconsistent definitions around values in alignment, we expanded a comprehensive structure and taxonomy of human values grounded in psychology and social science. Furthermore, we matched the surveyed literature with the appropriate values if applicable (articulated in Section~\ref{sec:value_category} and Section~\ref{sec:gap_value}).










% \begin{figure*}[!t]
%   \centering
%   \includegraphics[width=1\textwidth]{figures/value_structure.pdf}
%   \caption{The relations of human values for AI development
%   % The structure of the dynamic relations among values 
%   (adapted from~\citet{schwartz2012overview}). 
%   We consider 5 \emph{high-order value types} (\eg Self-enhancement and Openness to change), which encompass 12 \emph{motivational value types} (\eg power, universalism, functionality). We further organize the relation among these value types along two dimensions: 1) different sources (\ie individuals, society and interaction) and 2) different self intentions (\ie self-protection against threat and self-expansion and growth). The \emph{Desired values for AI tools} was added empirically from \emph{bottom-up} our paper survey whereas others are inherited from~\citet{schwartz2012overview}. 
%     % 
%   % The typology is based on Schwartz Theory of Basic Values and an empirical collection of values that are commonly been studied.
%   % Some values conflict with one another (\eg Benevolence and Power) whereas others are compatible (\eg Conformity and Security). This structure of values refers to these relations of conflict and congruence among values~\cite{schwartz1994there,schwartz2012overview}.
%   % 
%   % A fine-grained taxonomy of values related to bidirectional human-AI alignment. The taxonomy is based on Schwartz's Theory of Basic Values and an empirical collection of values that are commonly been studied.
%   }
%   \label{fig:value_structure}
%   % \vspace{-2em}
% \end{figure*}





\begin{table*}[!t]
  \centering
  \includegraphics[width=1\textwidth]{figures/value_content.pdf}
  \caption{The relations and a fine-grained taxonomy of \textbf{69 exemplary human values}. 
  We consider 5 high-order value types encompassing 12 motivational value types, indicated by their sources (e.g., individuals, society and interaction).
  % The typology is based on Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012overview} and an empirical collection of values that are commonly been studied.
  The exemplary values with red dot (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) indicates there are no work in our surveyed papers examining the specific values. 
  % Note that humans might not expect AI to encode all these values, which could potentially result in harm and risks. 
  % The values with red dot (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) and \textcolor{hua-red}{red color} means that humans might not expect AI to embed these values in AI, which could potentially result in harm and risks.
  % % 
  % % 
  % choose own goal\cite{lima2020collecting}
  % creativity\cite{ashktorab2020human}
  % curiosity\cite{jiang2023evaluating}
  % freedom\cite{lima2020collecting}
  % independence\cite{kang2023values}
  % privacy\cite{10.1145/3544548.3580903}
  % reflectiveness\cite{yan2023complex}
  % factuality\cite{hosking2023human}
  % self-respect\cite{wu2023cross}
  % diversity\cite{kapania2023hunt}
  % capability\cite{xu2023lemur}
  % influence\cite{huang2023humanity}
  % intelligence\cite{park2023generative}
  % success\cite{kang2023values}
  % resilience\cite{ye2023flask}
  % authority\cite{lima2021human}
  % wealth\cite{santurkar2023whose}
  % reciprocation of favours\cite{zagalsky2021design}
  % moderation\cite{lai2022human}
  % devout\cite{santy2023nlpositionality}
  % politeness\cite{zhu2023unmasking}
  % self-discipline\cite{zhou2023realbehavior}
  % forgiving\cite{wu2023cross}
  % helpfulness\cite{jin2022make}
  % honesty\cite{he2023hi}
  % emotional\cite{huang2023humanity}
  % responsiblity\cite{ma2023towards}
  % true friendship\cite{isajanyan2024social}
  % cooperation\cite{he2023interaction}
  % collectivism\cite{nie2024moca}
  % democracy\cite{santurkar2023whose}
  % inclusive\cite{ramezani2023knowledge}
  % equality\cite{sheng2021societal}
  % equity\cite{goldfarb2023prompt}
  % accessibility\cite{zhang2023visar}
  % adaptability\cite{oh2023pk}
  % economic\cite{bakker2022fine}
  % transparency\cite{boyd2021datasheets}
  % autonomy\cite{wang2023humanoid}
  % awareness\cite{paleja2021utility}
  }
  \label{fig:value_taxonomy}
  \vspace{-3.4em}
\end{table*}





% \subsubsection{\textbf{With whom to align?}}
\subsection{With whom to align?}

% 
Pertinent stakeholders within the AI landscape can be the potential objects for AI to align with, including lay people (\eg end users of AI systems)~\cite{qi2023fine}, AI practitioners (\eg developers, researchers)~\cite{boggust2022shared,anwar2024foundational,ngo2022alignment}, organizational entities (\eg technology firms, professional communities), national/international bodies (\eg governments, legislative bodies)~\cite{deshpande2022responsible} and others.
% 
% 
Many alignment research papers have focused on general humans without specifying particular groups~\cite{yao2023instructions,liu2022aligning,guo2023beyond}. Nevertheless, different groups hold different, sometimes even contrasting, values~\cite{gabriel2020artificial}.
% 
As a consequence, rather than identifying a \emph{true moral theory} as a \emph{one-size-fits-all} value, prior alignment research argues to select the appropriate principles for compatible human groups~\cite{sorensen2024roadmap}.
To this end, \emph{pluralistic value alignment}, grounded on social choice theory~\cite{arrow2012social}, proposes combining individual views fairly in developing alignment principles as a potential solution~\cite{sorensen2024roadmap}.
% 
% 
In this work, 
we also consider values from this pluralistic perspective,
% we define the \textbf{source of values with the aim of pluralism}, 
where AI should be aligned with \textbf{pluralistic human individuals and societal groups} who would ultimately be impacted by AI. 






% \subsubsection{\textbf{What are the values to be aligned with?}}
\subsection{What are the values to be aligned with?}
\label{sec:human_values_definition}


While previous studies have aimed to align AI with human values, the specific values they examined are often ambiguous and inconsistent.
% 
% 
% While many papers claim to integrate or evaluate AI in relation to human values, the specific sets of human values they examine often lack clarity or comprehensiveness. 
% In order to articulate and systematically understand 
To clarify human values relevant to human-AI alignment, we structured human values using a combination of top-down and bottom-up methods based on the \textbf{Schwartz Theory of Basic Values}~\cite{schwartz1994there,schwartz2012overview}.
% , which offers is a universal model outlining broad values that steer human behavior grounded in psychology.
% 
Among various human value theories (\eg Moral Foundation Theory~\cite{graham2013moral}, Social Norms \& Ethics~\cite{forbes2020social}), we chose the Schwartz Theory of Basic Values primarily considering that its definitions and dimensions are universal and are applicable for most people across \emph{(a)} various cultures and countries; \emph{(b)} various divisions including individuals, interactions and groups; and \emph{(c)} is commonly accepted in previous NLP studies~\cite{kang2023values,kiesel2022identifying}.
% 
% 
Specifically, \citet{schwartz1994there} provided a \textbf{clarified definition of human values} by summarizing
some widely agreed-upon features as:
% 
% \begin{quote}
    \emph{\say{A value is a (1) belief (2) pertaining to desirable end states or modes of conduct, that (3) transcends specific situations, (4) guides selection or evaluation of behavior, people, and events.}}
% \end{quote}
\citet{schwartz1994there} further offered a universal model outlining broad values that steer human behavior grounded in psychology.
% 
% 
% 

% \noindent
\textbf{A Comprehensive Taxonomy of Human Values}.
Nevertheless, this conventional theory was developed without the context of human-AI interaction, which might overlook values that need to be considered for human-AI alignment. Therefore, we used a \emph{bottom-up} approach to extract all values studied in our collected alignment literature (elaborated in Section~\ref{sec:prisma}), mapped them onto the Schwartz Theory of Basic Values, and supplemented the theory with AI-related structure and content. 
% 
% 
As a result, we identified the structural relationships among human values (see Figure~\ref{fig:value_structure}) and mapped existing literature to a fine-grained taxonomy (see Table~\ref{fig:value_taxonomy}). 
% 
% 
As shown in Figure~\ref{fig:value_structure}, we supplemented the traditional theory's four high-order value types (\ie ``Self-Enhancement'', ``Openness to Change'', ``Conservation'', ``Self-Transcendence'') with a novel high-order value type, named ``Desired Values for AI Tools'' that encompasses two motivational value types (\ie ``Usability'' and ``Human-Likeness'').
% 
We further organize the relationship among these value types along two dimensions~\cite{schwartz2012overview}: different resources (\ie individuals, society and interaction) and different self-intentions (\ie self-protection against threat and self-expansion and growth).
% 
% 
% 
Furthermore, we elaborate the definitions of the 12 motivational value types and their exemplary values by mapping them to relevant human-AI alignment papers from our corpus in Table~\ref{fig:value_taxonomy}. 
% 
During the process of mapping, we found: 1) value terms in empirical papers were often named differently (\eg capability and competence), or check their opposites (\eg fairness and bias); 
2) there are many values not studied in our corpus, \ie indicated as (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) in the Figure.



% which can be potentially due to several reasons, such as difficulty in measurement (e.g., inner harmony), or not common use cases (e.g., Detachment).



% Built upon these clarified definitions, we start to use a \emph{top-down} method to adopt the well-defined \emph{value taxonomy} and the \emph{structural relationship} presented by~\citet{schwartz1994there,schwartz2012overview}. 
% As the conventional theory is missing the context of AI-system and human-AI interactions, we further supplement the \emph{value taxonomy} and the \emph{structural relationship}. Specifically, we used a \emph{bottom-up} way to extract all values studied in the literature and map them into the Schwartz Theory of Basic Values. Further, we added the missing values and relationship regarding the AI context to make our outcome more comprehensive.





% a theory of cross-cultural psychology. As a result, we identified the structural relationships among human values (see Figure~\ref{fig:value_structure}) and mapped existing literature to a fine-grained taxonomy (see Figure~\ref{fig:value_taxonomy}). 
% Additionally, we present our analysis findings of human values that are particularly relevant for future studies (Section~\ref{sec:value_finding}).







% \subsubsection{
% \textbf{Methodology: A Combination of Top-Down and Bottom-Up Way to Structure Human Values}
% % }
% \label{sec:value_method}
% % \mbox{}
% To recognize human values systematically, we grounded our exploration on the Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012overview}, which is a theory of cross-cultural psychology built upon the \citet{rokeach1973nature}'s value survey. 

% We chose the Schwartz Theory of Basic Values primarily considering that its definitions and dimensions are universal and are applicable for, or almost for, all people across \emph{(a)} various cultures and countries; \emph{(b)} various sources including individuals, interactions and groups; and \emph{(c)} commonly accepted in previous NLP studies~\cite{kang2023values,kiesel2022identifying}.
% % 
% % 
% \citet{schwartz1994there} provided a clarified definition of human values by summarizing some widely agreed-upon features as:
% % 
% % \begin{quote}
%     \emph{\say{A value is a (1) belief (2) pertaining to desirable end states or modes of conduct, that (3) transcends specific situations, (4) guides selection or evaluation of behavior, people, and events.}}
% % \end{quote}
% % 


% Built upon these clarified definitions, we start to use a \emph{top-down} method to adopt the well-defined \emph{value taxonomy} and the \emph{structural relationship} presented by~\citet{schwartz1994there,schwartz2012overview}. As the conventional theory is missing the context of AI-system and human-AI interactions, we further supplement the \emph{value taxonomy} and the \emph{structural relationship}. Specifically, we used a \emph{bottom-up} way to extract all values studied in the literature and map them into the Schwartz Theory of Basic Values. Further, we added the missing values and relationship regarding the AI context to make our outcome more comprehensive.




% % \subsubsection{
% \textbf{Outcome: The Relations of Human Values and Fine-grained Taxonomy}
% % }
% \label{sec:value_outcome}
% % \mbox{}
% % 
% % Consequently, 
% We developed a more comprehensive structure of the dynamic relations of human values (Figure~\ref{fig:value_structure}) and their fine-grained taxonomy with mapped reference papers for exemplary values (Figure~\ref{fig:value_taxonomy}) after incorporating the AI-related context. 
% % 
% % 
% % 
% % 
% Considering the dynamic relations of human values in Figure~\ref{fig:value_structure}, we consider five \emph{high-order value types} (\ie self-enhancement, openness to change, conservation, self-transcendence and desired values for AI tools), which encompass 12 \emph{motivational value types} (\eg power, universalism, functionality).
% We further organize the relation among these value types along two dimensions: 1) different resources (\ie individuals, society and interaction) and 2) different self intentions (\ie self-protection against threat and self-expansion and growth).
% Note that the type of \emph{Desired Values of AI Tools} and its encompassed \emph{motivational values} (\ie functionality and human-likeness) are the supplemental value types we added from the empirical \emph{bottom-up} process introduced above.
% Also, it is worth noting that some values conflict with one another (\eg Benevolence and Power) whereas others are compatible (\eg Conformity and Security). This structure of values refers to these relations of conflict and congruence among values~\cite{schwartz1994there,schwartz2012overview}.
% % 
% 
% 
% 


% % 
% Furthermore, we elaborate the definitions of the 12 motivational value types and their exemplary values with mapped paper reference in Figure~\ref{fig:value_taxonomy}. During the process of mapping existing literature to these values, we noted two findings: 1) value terms in empirical papers were often named differently (\eg capability and competence), or check their opposites (\eg fairness and bias), from the listed exemplary values of Schwartz's theory even they are examining the same thing essentially . 2) there are many values not studied in our collected literature (indicated as (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) in the Figure). 









\begin{table*}[ht]
\centering
\vspace{-6pt}
\begin{tabular}[t]{@{}  !{\color[HTML]{808080}\vrule width 2pt} p{.98\textwidth} !{\color[HTML]{808080}\vrule width 2pt} @{}}
\cellcolor[HTML]{E6E6E6} 
\textbf{Takeaways \& Implications for Alignment Clarifications} 
% \newline
\vspace{5pt}

1. We propose the ``pluralistic human values'' as the alignment goal, wherein AI should be aligned with the diverse perspectives of individuals and societal groups who may be directly or indirectly impacted by AI.
\vspace{5pt}

2. Many exemplary human values outlined in Table~\ref{fig:value_taxonomy}, such as loyalty and environmental protection, are important for alignment but are often overlooked or underexplored in current research.
% 
\vspace{5pt}

3. The human value system should account for complex application contexts and relationships, such as priorities and conflicts, rather than focusing on an exclusive subset of values.
\end{tabular}
\vspace{-10pt}
\end{table*}



\vspace{-5pt}
% \subsection{Scopes and Generalizability}
\subsection{Scopes and Key Components in Alignment}
\label{sec:scope}

This section clarifies the key components we considered in \emph{human-AI alignment}. Additionally, we define the scopes of each key component as commonly adopted in current research.
% 
% We define the scope of alignment by specifying the key components we considered in \emph{human-AI alignment}. 
% We focus on a representative scope of alignment studies and discuss the generalizability of the scope after that.

% We define the scope of our literature review by specifying the key components we considered in \emph{human-AI alignment}. Given the broad definitions as aforementioned, it is infeasible to include all alignment research in practice. Therefore, we focus on a representative scope of alignment studies and discuss the generalizability of the scope after that.



\begin{itemize}
    \item \textcolor{hua-red}{\textbf{Humans.}} 
    % \textbf{With whom should AI align?} 
    % \emph{\textbf{align with whom?}}
    Our primary focus is on human \humancode{individuals}, \humancode{groups}, or \humancode{organizations} that will ultimately develop, use, and potentially impact or be influenced by AI systems, 
    % Our primary focus is on \humancode{individuals} or \humancode{human groups} that will ultimately use AI systems and might be affected by them, 
    as these are the entities with which AI systems should align. We emphasize the importance of considering the pluralistic values of diverse users rather than treating users as a monolithic group.
    % 
    % Our primary focus is on \humancode{individuals} or \humancode{human groups} who will ultimately use AI systems and who might be affected by AI systems, as these are the entities that AI systems should align with. 
    % Particularly, we emphasizes the importance of considering the pluralistic values of diverse users, rather than treating them as a monolithic group. 
    % These individuals and groups may be significantly impacted by the deployment of AI systems for various purposes, and thus their perspectives are crucial for ensuring alignment. 
    % \diyi{does "user" who might be affected by AI (rather than just end users) belong to the current scope of consideration?}
    % \hua{[DONE]great point! we do contain both users that ``might be affected by AI'' in Section 4.4.2. Let me correct this definition to be more precise :) }
    % , including citizens from different cultural backgrounds and marginalized communities. 

    % We advocate for more nuanced approaches that involves engaging with various sub-communities and individuals within the end user population.
    
    \item
    \textcolor{hua-blue}{\textbf{Artificial Intelligence (AI).}} 
    % Locating the elusive scope of AI is difficult. The technical boundary of AI, even in AI research communities, is disputed and continuously evolving~\cite{yang2020re}. 
    % 
    % As the advent of AGI increased the significance of AI alignment, w
    % 
    % 
    % We primarily focus on AI systems that have been extensively researched in the field of human-AI alignment, especially after the advent of AGI. 
    We focus on AI systems including both \aicode{domain-specific AI systems} that address specific tasks (\eg reasoning, dialogue) and \aicode{general-purpose AI models} that aim to complete any tasks with performance comparable to a human's.
    These AI systems include generative, classification, and regression models, among others.
    % \aicode{language models}, \aicode{reinforcement learning models}, neural network-based \aicode{classification and regression models}, among others. 
    % These technologies include \aicode{language models}, \aicode{reinforcement learning models}, neural network-based \aicode{classification and regression models}, among others. 
    Particularly, we primarily focus on language models as the representative AI models for alignment research, and discuss how the insights from this study can be generalized to other modalities at the section end.


    
    % \item
    % \textcolor{hua-yellow}{\textbf{Alignment.}} 
    % Our review encompassed all the \aligncode{alignment goals} outlined in Section~\ref{sec:align_goal}, with a particular focus on \aligncode{\emph{value alignment}} by clarifying alignment values and identifying both the explicit and implicit values in each paper reviewed. Additionally, alignment can also involve the representation or behavioral aspects between humans and AI, which were not included in this study for a more focused scope~\cite{mcgrath2023can,park2023generative,xie2024can}.
    

    \item
    \textcolor{hua-yellow}{\textbf{Alignment.}} 
    Our review encompassed all the \aligncode{alignment goals} outlined in Section~\ref{sec:align_goal}.
    Since many studies emphasized the importance of \aligncode{value alignment}~\cite{gabriel2020artificial,stuart2014whitepaper}, we particularly summarized a clarified taxonomy of alignment values and identified the value in each paper (if applicable).
    Additionally, we focus on analyzing the AI models' output and generation, but not the neural network's intermediate representations~\cite{mcgrath2023can,park2023generative,xie2024can}, for alignment research.
    % 
    % , with a particular focus on \aligncode{\emph{value alignment}} by clarifying alignment values and identifying both the explicit and implicit values in each paper reviewed. 
    % Additionally, alignment can also involve the representation or behavioral aspects between humans and AI, which were not included in this study for a more focused scope~\cite{mcgrath2023can,park2023generative,xie2024can}.



    
    
    % Our review covered all goals introduced in Section~\ref{sec:align_goal}, with an emphasis on clarifying alignment values and recognizing the explicit and/or implicit values in each reviewed paper. For a even broader scope, alignment can also encompass the representation or behavioral~\cite{park2023generative,xie2024can} between humans and AI, which are excluded in this study.
    
    % We focus on \emph{value alignment} in this study, where we also provide clarified definitions of \emph{what human values encompass} in Section~\ref{sec:value_category}.
    % \diyi{any justification on why "value" is more important here compared to focusing on other dimensions?}
    % \hua{thanks for the valuable suggestion! we added Sec5.2.2 for elaborating this, but should also briefly justify here. 
    % In short, we justify with at least three reasons: 1) values in our study are used to characterize a wide range of humans, including cultural groups, societies, and individuals (including cultural and religious characteristics as well, see Fig~\ref{fig:schwartz} - Tradition). 
    % 2) values can be used to explain the motivational bases of attitudes and behavior, which can be considered as the sources of many human behavior and preferences.
    % 3) there lacks a clarified definition of ``what human value is'' despite the large number of studies about ``human-AI alignment for values'' . We delve into this issue and aim to provide a clarified definition for it.}
    % There are also diverse factors that we might want to consider for "alignment" beyond "values" such as norms and cultures. 
    % To further provide a comprehensive scope of human-AI alignment, as motivated in Section~\ref{sec:background}, this study introduces a novel conceptual framework termed ``\emph{\aligncode{bidirectional human-AI alignment}}''. Specifically, our exploration of alignment extends beyond the conventional notion of \aligncode{aligning AI to human values} (\ie integrating human values to guide, control, and personalize AI systems) to further involve \aligncode{aligning human to AI outputs} (\ie how humans can adapt to and interact effectively with advancing AI technologies).
    % % This framework involves research on integrating human values to guide, control, and personalize AI systems, as well as studies on how humans can adapt to and interact effectively with advancing AI technologies. 
    % Detailed definitions are presented in Section~\ref{sec:scope} for clarity and elaboration.
    % % 
    
\end{itemize}




% \begin{table*}[ht]
% \centering
% \vspace{-10pt}
% \begin{tabular}[t]{@{}  !{\color[HTML]{808080}\vrule width 2pt} p{.98\textwidth} !{\color[HTML]{808080}\vrule width 2pt} @{}}
% \cellcolor[HTML]{E6E6E6} 
% \textbf{Takeaways \& Implications for Alignment Clarifications} 
% % \newline
% \vspace{5pt}

% 1. We propose the ``pluralistic human values'' as the alignment goal, wherein AI should be aligned with the diverse perspectives of individuals and societal groups who may be directly or indirectly impacted by AI.
% \vspace{5pt}

% 2. Many exemplary human values outlined in Table~\ref{fig:value_taxonomy}, such as loyalty and environmental protection, are important for alignment but are often overlooked or underexplored in current research.
% % 
% \vspace{5pt}

% 3. The human value system should account for complex application contexts and relationships, such as priorities and conflicts, rather than focusing on an exclusive subset of values.
% \end{tabular}
% \vspace{-10pt}
% \end{table*}







% % We recognize that our current work exists within a broader context of studies concerning human-AI alignment. 
% \noindent
% We acknowledge the extensive scope and rapid advancements of research in this area, and posit that our study offers insights that can be generalized to various modalities. For example, the value taxonomy and human-in-the-loop evaluation paradigm outlined in our framework can be applied to both text-based and other modality-based (\eg vision, robotics) models. 
% % 
% It's worth noting that our literature review does not aim to exhaustively cover all papers in the field, which is impossible given the rapid advancement of human-AI alignment research. Instead, we adopt a human-centered perspective to review more than 400 key studies in this domain, focusing on delineating the framework landscape, identifying limitations, future directions, and a roadmap to pave the way for future research.








% \subsection{Why Do We Need Bidirectional Alignment?}
% \label{sec:scope}

\subsection{Systematic Literature Review and Framework Rationale}
\label{sec:review}


% We consider the goal of alignment as ``human values'' from a pluralistic perspective,
% where AI should be aligned with \textbf{pluralistic human individuals and societal groups} who would ultimately be impacted by AI. 
Achieving the alignment between AI and human values necessitates collaboration among interdisciplinary AI practitioners (\eg developers and researchers).
To comprehensively analyze the research literature pertaining to this ongoing, mutual process of human-AI alignment, we conducted a systematic literature review adhering to the the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332}.
% To understand the research literature relevant to the ongoing, mutual process of human-AI alignment, 
% we performed a systematic literature review based on the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332}.
% 
% 
Our iterative selection process yielded 411 papers from an initial pool of 34,213 publications, spanning the period from January 2019 to January 2024. These papers were sourced from leading venues across multiple AI-related domains, including Natural Language Processing, Human-Computer Interaction,  Machine Learning, and more, using well-defined keywords and criteria. 
A group of 13 interdisciplinary researchers coded the papers. Through iterative discussions, we developed the paper codes and proposed framework (Section~\ref{sec:method}). Detailed steps and processes are elucidated in Appendix~\ref{app:system_review}.
% 


% \noindent


\subsection{Rationale Behind the Framework}
\label{sec:motivation}
% \textbf{Rationale Behind the Framework.} 
Our systematic review revealed that current research largely overlooks the nature of \textbf{long-term dynamic changes} and the \textbf{importance of interaction} in human-AI alignment.
% 
% 
First, the manifestation of certain AI risks, harms, and the practical quality of AI services primarily emerge through interaction between humans and AI systems~\cite{weidinger2023sociotechnical}. 
% 
For instance, \citet{shen2020useful} discovered that AI explanations, deemed effective by AI developers and researchers, were found not useful for humans in real-world scenarios of interactive AI error detection.
% 
% 
Additionally, the use of AI influences human thinking and behavior, which in turn alters their values when interacting with AI.
% 
For instance, \citet{li2024value} found that incorporating AI assistance in writing workflows changed humans' writing perceptions, behavior, and performance, creating new requirements for developing the next generation of AI writing assistants~\cite{lee2024design}.


In light of these findings, we posit that AI practitioners must expand their focus beyond merely ``Aligning AI to Humans'' -- a paradigm centered on integrating human specifications to train, steer, and customize AI. Equal emphasis must be placed on ``Aligning Humans to AI'', a complementary paradigm investigating human cognitive and behavioral adaptation to AI. This latter aspect is crucial in supporting individuals and society at large in understanding, critiquing, collaborating with, and adapting to transformative AI advancements.
To encapsulate these comprehensive perspectives, we propose the ``\textbf{Bidirectional Human-AI Alignment}'' framework, and provide its definition below Figure~\ref{fig:teaser}.
% 
This holistic framework acknowledges the reciprocal nature of alignment, 
addressing both the advancements of AI systems to incorporate human values, and the evolving human adaptation of AI systems in real-world practice.






% Consequently, AI practitioners should not only focus on "Aligning AI to Humans," which emphasizes integrating human specifications to train, steer, and customize AI. Equally important is "Aligning Humans to AI," which examines humans' cognitive and behavioral adaptation to AI systems. This approach supports individuals and society in understanding, critiquing, collaborating with, and adapting to transformative AI advancements. Consequently, we propose the "Bidirectional Human-AI Alignment" framework to encompass these comprehensive perspectives.
% 
% 
% Based on the systematic review, we found that existing research large neglects the nature of \textbf{long-term dynamic changes} and \textbf{importance of interaction} of human-AI alignment. 
% First, it is from interaction that AI risks and harms can be manifested or the quality of AI service and evaluated practically~\cite{weidinger2023sociotechnical}. 
% For example, \citet{shen2020useful} finds that AI explanations, which are developed and validated to be effective by AI developers, are found not useful for humans in interactively detecting AI mistakes in practice.
% 
% Additionally, the usage of AI changes how humans think and behave, and further changes their values when interacting with AI. 
% For instance, ~\citet{li2024value} finds that incorporation of AI assistance in writing workflows changes humans' writing perceptions and performance. These changes of human cognition and behaviors further put novel requirements on developing next generation of AI writing assistants~\cite{lee2024design}.
% 
% 
% In summary, AI practitioners should not only consider ``Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-red}{Humans}'', which focuses on integrating human specifications to train, steer and customize AI. Crucially, AI practitioners should place equal emphasis on the significance of ``Aligning \textcolor{hua-red}{Humans} to 
% \textcolor{hua-blue}{AI}'', which investigates humans' cognitive and behavioral adaptation to the AI systems, that supports individuals and the broader society in understanding, critiquing, collaborating with and adapting to transformative AI advancements. 
% Consequently, we propose the ``Bidirectional Human-AI Alignment'' framework to encompass these comprehensive perspectives.




% ``Align \textcolor{hua-blue}{AI} to \textcolor{hua-red}{Humans}'' and ``Align \textcolor{hua-red}{Humans} to 
% \textcolor{hua-blue}{AI}''.
% 
% 
% , AI-driven writing assistants changed humans' writing behavior and demands on AI values from primarily emphasizing  on AI accuracy to more diverse needs on AI values, such as being creative, empathetic, enjoyable, fair, unique, and more~\cite{lee2024design}.




% \hua{Motivate the "bidirectional alignment framework",
% introduce systematic review,
% transit to framework,
% introduce 4 research questions
% - Why these research questions? how to use these questions? -- Reshmi}






% \reshmi{R\\
% Q1: For any developer or researcher reading the paper how do they choose research questions based on their task and scenario\\

% Q2: Also what are some values that should not be sacrificed as part of using this bi-directional framework\\

% Q3: }


% \hua{write more towards motivation here. very concretely motivate the framework.}
% % 





% ===============================================

% The aforementioned background motivates this work to present a clarified definition and scope for human-AI alignment before conducting the comprehensive review on the state-of-the-art research. Additionally, achieving alignment between human and AI necessitates a holistic understanding of human cognition and behavior, societal norms, as well as AI algorithmic capabilities and limitations. 
% % 
% Therefore, we collected a varied range of state-of-the-art papers covering interdisciplinary fields and perspectives related to human-AI alignment primarily published from 2019 to 2024. We next introduce the clarified definitions and scope adopted in this work, and the process of systematic literature review we conducted to arrive at our bidirectional human-AI alignment framework and associated findings elaborated in the following sections.
% % 
% \hua{Section 3 and Section 2 are overlapping in many places, trim some of them.}


% To develop the framework of bidirectional human-AI alignment, we first decide on the scope and core aspects of human-AI alignment.








% The advent of sophisticated and versatile AI technologies has underscored the necessity for ongoing discussions surrounding AI alignment. However, existing literature approaches human-AI alignment from various angles, lacking a clarified definition of ``\emph{what is human-AI alignment?}'', ``\emph{what should be aligned}'' and ``\emph{aligned with whom?}''. 
% % 
% % 
% % 
% % 
% As elaborated in Section~\ref{sec:background}, human-AI alignment has been referred to as \emph{intention alignment}~\cite{anwar2024foundational}, \emph{behavior alignment}~\cite{park2023generative,xie2024can}, \emph{instruction alignment}~\cite{bai2022constitutional,liu2023makes}, \emph{value alignment}~\cite{sorensen2024roadmap,gabriel2020artificial}, etc. Furthermore, the alignment objects could be aligning AI's \emph{intermediate representations}~\cite{liu2023learning}, \emph{internal reasoning process}~\cite{mcgrath2023can}, and/or generations~\cite{corvelo2024human,ouyang2022training} with all pertinent AI stakeholders~\cite{deshpande2022responsible} (\eg AI practitioners~\cite{boggust2022shared} and end-users~\cite{qi2023fine}).
% % 
% % 
% These varied investigations present expansive interpretations of human-AI alignment, underscoring the intricate nature and breadth of research in this field~\cite{kirchner2022researching}. Drawing upon numerous extant literature reviews and seminal studies on human-AI alignment~\cite{matthews2022alignment,gabriel2020artificial,kenton2021alignment,yao2023instructions, ganguli2022red,terry2023ai,wang2023aligning,
% askell2021general,kirchner2022researching}, this work clarifies an examination of the definition and scope of human-AI alignment adopted in this work by elaborating the pertinent terminologies.
% % : \emph{who should AI align with}? \emph{which AI technologies are the primary focus of this study}? and \emph{what does alignment entail within the context of human-AI interactions}? 
% Specifically, we provide our detailed definitions within the context of this study as below:
% \hua{[TODO] merge this section with above.}





% \begin{quote}
%     \say{\emph{For an autonomous system to be	helpful to humans and to pose no unwarranted risks, it needs to align its values with those of the humans in its environment in such a way that its actions contribute to the maximization of value for the humans.}} \\
%     {\hspace*{100pt}~\textit{---  Stuart Russell, White Paper: Value Alignment in Autonomous Systems, 2014 ~\cite{stuart2014whitepaper}}}
%     % \cite{stuart2014whitepaper}
% \end{quote}


% \epigraph{\say{\emph{For an autonomous system to be	helpful to humans and to pose no unwarranted risks, it needs to align its values with those of the humans in its environment in such a way that its actions contribute to the maximization of value for the humans.}}}{\textit{--- 
%  Stuart	Russell, White Paper: Value Alignment in Autonomous Systems, 2014 ~\cite{stuart2014whitepaper} \\}}



% \begin{itemize}




    % % \item 
    % \textcolor{hua-yellow}{\textbf{Alignment.}} 
    % % \textbf{What does alignment entail within the context of human-AI interactions}? 
    % \emph{\textbf{what is human-AI alignment?}}
    % We focus on \emph{value alignment} in this study, where we also provide clarified definitions of \emph{what human values encompass} in Section~\ref{sec:value_category}.
    % \diyi{any justification on why "value" is more important here compared to focusing on other dimensions?}
    % \hua{thanks for the valuable suggestion! we added Sec5.2.2 for elaborating this, but should also briefly justify here. 
    % In short, we justify with at least three reasons: 1) values in our study are used to characterize a wide range of humans, including cultural groups, societies, and individuals (including cultural and religious characteristics as well, see Fig~\ref{fig:schwartz} - Tradition). 
    % 2) values can be used to explain the motivational bases of attitudes and behavior, which can be considered as the sources of many human behavior and preferences.
    % 3) there lacks a clarified definition of ``what human value is'' despite the large number of studies about ``human-AI alignment for values'' . We delve into this issue and aim to provide a clarified definition for it.}
    % There are also diverse factors that we might want to consider for "alignment" beyond "values" such as norms and cultures. 
    % To further provide a comprehensive scope of human-AI alignment, as motivated in Section~\ref{sec:background}, this study introduces a novel conceptual framework termed ``\emph{\aligncode{bidirectional human-AI alignment}}''. Specifically, our exploration of alignment extends beyond the conventional notion of \aligncode{aligning AI to human values} (\ie integrating human values to guide, control, and personalize AI systems) to further involve \aligncode{aligning human to AI outputs} (\ie how humans can adapt to and interact effectively with advancing AI technologies).
    % % This framework involves research on integrating human values to guide, control, and personalize AI systems, as well as studies on how humans can adapt to and interact effectively with advancing AI technologies. 
    % Detailed definitions are presented in Section~\ref{sec:scope} for clarity and elaboration.
    % % 
    % \hua{define alignment beyond values.}




% ============================================================

% ====================== NEW ADDED =======================


% In terms of ``\emph{\aligncode{what is human-AI alignment?}}'', 
% alignment has been referred to as \emph{intention alignment}~\cite{anwar2024foundational}, \emph{behavior alignment}~\cite{park2023generative,xie2024can}, \emph{instruction alignment}~\cite{bai2022constitutional,liu2023makes}, \emph{value alignment}~\cite{sorensen2024roadmap,gabriel2020artificial}, etc. 
% % 
% % 
% % There are also diverse factors that we might want to consider for "alignment" beyond "values". for instance, norms and cultures. 
% % maybe you will clarify this in the later section! 

% % intent alignment description;
% \citet{ouyang2022training} and \citet{anwar2024foundational} consider alignment from the perspective of 
% AI safety~\cite{anwar2024foundational,wang2023aligning}, where it refers alignment to be \emph{intent alignment} by fine-tuning with human feedback. 
% % 
% Their goal of alignment is to assure safety (\ie unlikely to contribute to unplanned, undesirable harms) when the systems are deployed and used~\cite{weidinger2023sociotechnical}. 
% % 
% % 
% % 
% % 
% % behavior alignment description;
% \citet{park2023generative} introduces generative agents that draw on generative models to simulate and align with believable individual and emergent group behavior, in which the computational agents can wake up, cook breakfast, form opinions and initiate conversations, etc.
% % 
% % 
% % 
% % instruction alignment description;
% % 
% ~\citet{bai2022constitutional} form the human supervision as a set of principle instructions that should govern AI behavior, along with a small number of examples as few-shot prompting to instruct models.
% % 
% % value alignment description;
% \citet{gabriel2020artificial} considers AI could be designed to align with the values of system users, where the \emph{values} are defined as ``natural or non-natural facts about what is good or bad, and about what kinds of things ought to be promoted, as specified by the individual or society.''
% A line of studies examine AI alignment with respect to individual and social values~\cite{tay2020would,hendrycks2020aligning,hovy-yang-2021-importance}. Despite the plethora of alignment definitions and studies, yet, the difference and relationship between these alignment goals are vague and less investigated.
% % 
% % 


% =================================================











% %     \item 
%     \textcolor{hua-red}{\textbf{Human.}} 
%     % \textbf{With whom should AI align?} 
%     \emph{\textbf{align with whom?}}
%     Our primary focus is on the \humancode{users} who will ultimately use AI systems and who might be affected by the deployed AI, as these are the entities that AI systems should align with. 
%     % Also, we include users who might be affected by AI.
%     Particularly, our study emphasizes the importance of considering the various values and concerns of \humancode{diverse users}, rather than treating them as a monolithic group. \diyi{does "user" who might be affected by AI (rather than just end users) belong to the current scope of consideration?}
%     \hua{[DONE]great point! we do contain both users that ``might be affected by AI'' in Section 4.4.2. Let me correct this definition to be more precise :) }
%     % , including citizens from different cultural backgrounds and marginalized communities. 
%     These individuals and groups may be significantly impacted by the deployment of AI systems for various purposes, and thus their perspectives are crucial for ensuring alignment. 
%     % We advocate for more nuanced approaches that involves engaging with various sub-communities and individuals within the end user population.


% =================================================






% % 
% % 
% Considering ``\emph{\humancode{align with whom?}}'' Pertinent stakeholders within the AI landscape can be the potential objects for AI to align with, including lay people (\eg end users of AI systems), AI practitioners (\eg developers, researchers)~\cite{boggust2022shared}, organizational entities (\eg technology firms, professional communities), and national/international bodies (\eg governments, legislative bodies)~\cite{deshpande2022responsible}.
% % 
% For instance, \citet{anwar2024foundational} defines an AI systems as `aligned' when it is trying to behave as intended by the LLM developer~\cite{ngo2022alignment}, whereas \citet{qi2023fine} conducts red-teaming studies to investigate the safety risks of LLMs to end-users.
% % 
% There are also studies discussing general humans without specifying human groups~\cite{yao2023instructions}.
% % 
% % 



% =================================================



%     % \item 
%     \textcolor{hua-blue}{\textbf{Artificial Intelligence (AI).}} 
%     \emph{\textbf{what should be aligned?}}
%     We consider AI technologies in this study to primarily concentrate on the \aicode{outputs and/or generations} of modern AI systems that have been extensively researched in the field of human-AI alignment. Notably, we are most interested in literature concerning \aicode{large language models (LLMs)}.
%     \diyi{somewhere you might want to justify the generalization of this human-AI alignment, especially around how inshgts here can go to "multimodal pretrained models"} 
%     \hua{thanks for the constructive suggestion! indeed, we need to clarify a bit more about our what AI we include and also their generalization to other AI systems. I'll do that!}
%     Also, we partially incorporate studies examining cutting-edge machine learning systems, such as reinforcement learning with human feedback, which have significantly advanced the feasibility of human-AI alignment and assisted human decision making in practice.




% =================================================





% There are also studies discussing general humans without specifying human groups~\cite{yao2023instructions,liu2022aligning,guo2023beyond}.
% However, Different groups of people hold different, sometimes even contrasting, values. 
% 
% For instance, \citet{anwar2024foundational} defines an AI systems as `aligned' when it is trying to behave as intended by the LLM developer~\cite{ngo2022alignment}, whereas \citet{qi2023fine} conducts red-teaming studies to investigate the safety risks of LLMs to end-users.
% % 
% There are also studies discussing general humans without specifying human groups~\cite{yao2023instructions}.
% 
% 




% Regarding ``\emph{\aicode{what to be aligned?}}'',
% % 
% existing studies have examined how to align AI's \emph{intermediate representations} with humans'~\cite{liu2023learning}, align AI's \emph{internal reasoning process} to be similar with a human's cognitive process~\cite{mcgrath2023can}, and align AI's \emph{outputs and/or generations with human preferences}~\cite{corvelo2024human,ouyang2022training}.
% % 
% % 
% For example, \citet{liu2023learning} examines the alignment between models' representations and human-compatible decision-focused representations by identifying the nearest neighbors retrieved from dataset.
% \citet{mcgrath2023can} compares the interpretations of AI models with human cognitive theories formulated by studying human behaviors.
% \citet{santurkar2023whose} compares LLM-generated opinions with human responses from various U.S. demographic groups' opinion polls to evaluate their alignment.


% =================================================


% \end{itemize}




% It is essential to acknowledge that the definitions and scope of existing studies relevant to human-AI alignment extend far beyond the confines of our current study. 
% % 
% % 
% % \hua{generalizability discussion}
% However, our study and insights can be naturally generalized to other modalities.
% % =====
% our literature review does not aim to comprehensively cover all relevant studies within the realm of human-AI alignment. Instead, we are driven by a human-centric perspective in reviewing studies on human-AI alignment and focus on delineating the clarified scopes introduced above to explore the framework landscape, identify limitations, and delineate future directions in this field.








% % \subsection{Scopes of Bidirectional Human-AI Alignment}
% % \subsection{Scopes of This Study}
% \subsection{Study Scope and Generalizability}
% \label{sec:scope}





% While the breadth of research in human-AI alignment offers diverse perspectives,
% an increasing number of studies advocate for a comprehensive and clarified scope of human-AI alignment~\cite{terry2023ai,anwar2024foundational}.
% % 
% Therefore, this study, taking from a human-centered perspective~\cite{terry2023ai}, conceptualizes human-AI alignment as a \textbf{bidirectional} process. 
% Concretely, as showed in Figure~\ref{fig:teaser}, we argue that human-AI alignment not only involves the conventional studies that aim to \emph{integrate human values into training, steering, and customizing AI}, which we term as ``\textbf{aligning AI to humans}'' that has been extensively investigated in the fields of ML, NLP, etc. Also, from a human-centered perspective, we deem human-AI alignment should also consider studies around \emph{how humans perceive, critique, collaborate, and adapt to AI advancement}, thus providing better feedback to steer AI development. We term this line of work as ``\textbf{aligning humans to AI}''.
% % 
% % 
% Consequently, the research about alignment between human and AI should \textbf{consider a holistic loop of bidirectional human-AI alignment}, involving both \emph{aligning AI to humans} for improving AI capabilities to be better aligned with human values, and \emph{aligning humans to AI} that helps humans better understand, collaborate, and adapt to the rapidly advanced AI. Thus human and AI can benefit mutually to achieve a harmonious ecosystem.
% % 
% We therefore provide the detailed definitions and scopes of \emph{align AI to humans} and \emph{align humans to AI}, respectively, as below:





% \begin{itemize}

%     \item \textbf{Align  \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}.} \textbf{How to integrate human values to train, steer, and customize AI?}
%     % 
%     We define the process of \emph{aligning AI to humans} as integrating human values to train, steer and customize AI. 



%     \item \textbf{Align \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}.}
%     \textbf{What should humans do to critically adapt to AI advancement?}~\merrie{But also how can interface design support conveying AI affordances to humans and enabling them to steer AI interactions to meet their preferences?}
%     % 
%     \diyi{are humans adapting to AI consciously or unconsciously? }
%     We designate the process of \emph{aligning humans to AI} as enhancing humans' perception and capabilities to better understand, assess, criticize, and harness transformative AI advancements. 
%     % 
%     % 
%     % \hua{come back here after framework.}
%     % \hua{Eric: The clarified definition itself can be a good contributions;}

% \end{itemize}




% Again, our work targets a specific set of literature within the \emph{bidirectional human-AI alignment} scope, as opposed to all possible studies relevant to the human-AI alignment topic. 
% While our work concentrates on aligning AI outputs and generations with human values relevant to diverse subgroups, there are other extensive of studies, beyond the above scope, to align humans and AI from various aspects (\eg aligning AI's reasoning process with human cognitive processes~\cite{mcgrath2023can}).


% \hua{add the generalization of this scope to more modalities.}


% ======================================================






% Again, our work targets a specific set of literature within the \emph{bidirectional human-AI alignment} scope, as apposed to all possible studies relevant to the human-AI alignment topic. 
% While our work concentrate on aligning AI generations with human values from diverse subgroups, there are other sets of work, beyond our study scope, which extensively examine aligning AI internal reasoning process to be similar with human cognitive process~\cite{mcgrath2023can}. 



% Note that we are aware the existing research about human-AI alignment can be beyond the definitions we scoped above. For example, while our work concentrate on aligning AI generations with human values from diverse subgroups, there are other sets of work, beyond our study scope, which extensively examine aligning AI internal reasoning process to be similar with human cognitive process~\cite{mcgrath2023can}. 
% % 
% \hua{we focus on aligning with human values but not cognitive process; we focus on aligning AI generations but not internel reasoning process, not behavioral alignment }.
% Again, our work targets a specific set of literature within the \emph{bidirectional human-AI alignment} scope, as apposed to all possible studies of the human-AI alignment topic. 
% % 
% % 
% %







% \martin{we don't study: align human and ai underlying cognitive mechanism?}












% % \subsection{Systematic Literature Review}
% \subsection{Systematic Literature Review Process}
% \label{sec:prisma}

% To understand the research literature relevant to the ongoing, mutual process of human-AI alignment, 
% we performed a systematic literature review based on the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332}.
% % 
% Figure~\ref{fig:review_process} shows 
% the workflow of our process for
% % process of our systematic literature review for 
% paper coding and developing the \emph{bidirectional human-AI alignment} framework. We introduce the step details below.
% % We referred to the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332} for reporting the workflow. 



% % \begin{figure*}[!t]
% %   \centering
% %   \includegraphics[width=1\textwidth]{figures/PRISMA.pdf}
% %   \caption{
% %   The selection and refinement process of our systematic literature review. We referred to the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332} to report the workflow.
% %   From the identification of 34,213 records by keyword search, to screen eligible papers against our criteria and arriveg at our final corpus of 411 papers. For each of the stages where literature reviews were excluded (identification, screening, and eligibility) we further present the total of excluded records.}
% %   \label{fig:review_process}
% %   \Description{}
% % \end{figure*}


% \subsubsection{Identification and Screening with Keywords.}

% % To understand the current research literature on bidirectional human-AI alignment,
% % To understand the research literature relevant to the ongoing, mutual process of human-AI alignment, 
% % we performed a systematic literature review based on the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332}.
% % 
% We started with papers published in the AI-related domain venues (including NLP, HCI, and ML fields) beginning from the advent of general-purpose generative AI to present, \ie primarily between January, 2019 and January, 2024 (see details in Appendix~\ref{app:venues}).
% We retrieved 34,213 papers in the initial \emph{Identification} stage.
% Further, we collectively defined a list of keywords (see details in Appendix~\ref{app:keyword}) and screened for papers that included at least one of these keywords (\eg human, alignment) or their variations either in the title or abstract. We included 2,136 papers in this \emph{Screening} stage.
% % We first identify fields closely relevant to our research topic. As a result, we selected the fields of NLP, HCI, and Machine Learning as our pivotal domains and the related conference venues ranging from 2019 to 2024 we considered in this project in Appendix~\ref{app:venues}.
% % 
% % 
% % From the ACL Anthology, OpenReview and ACM Digital Library, we retrieved 34,190 papers into a Reference Manager Tool (\ie Paperpile).
% % 
% % 

% % To further collect the relevant papers, two of the authors collectively defined a list of keywords related to bidirectional human-AI alignment, such as \emph{human}, \emph{alignment}, \emph{interact}, \emph{LLM}, \emph{value}, etc. Next, we only sampled the papers that included these keywords and their variations either in the title and abstract (see the comprehensive keyword list in Appendix~\ref{app:keyword}). As a result, we selected 2,136 out of 34,213 papers that are potentially relevant mentioning the keywords for our literature review. 
% % % 
% % % Note that at this stage, we aim to 



% % \subsubsection{Filtering with Inclusion and Exclusion Criteria.} 
% \subsubsection{Assessing Eligibility with Criteria}
% % 
% We further filtered the 2,136 papers based on explicit inclusion and exclusion criteria, i.e., the \emph{Eligibility} stage.
% % 
% Our criteria revolved around six research questions that we collectively identified to be most pertinent to the topic, including \emph{1) what essential human values have been aligned by some AI models?} \emph{2) how did we effectively quantify or model human values to guide AI development?} \emph{3) what strategies have been employed to integrate human values into the AI development process?} \emph{4) how did existing studies improve human understanding and
% evaluation of AI alignment?} \emph{5) what are the practices for designing interfaces and interactions that
% facilitate human-AI collaboration?} 
% % \emph{6) what are the practices for designing interfaces and interactions that facilitate human-AI collaboration?}
% \emph{6) How have AI been adapted to meet the needs of various human value groups?
% }
% % 
% % 
% We included papers that could potentially answer any of these questions.
% %, we devised a series of inclusion criteria to aid in 1) human values, 2) AI development techniques, 3) AI evaluation, explanation and utilization, and 4) building dataset with human interaction 
% % 
% Further, based on the scope in Section~\ref{sec:scope}, we excluded papers that  did not meet our inclusion criteria. This resulted in a final corpus of 411 papers, which were analyzed in detail using qualitative coding (see Appendix~\ref{app:criteria} for more details).


% % To further narrow down the scope of the keyword-filtered 2136 relevant papers, we specified the explicit inclusion and exclusion criteria collectively for selecting the papers in the following process. 
% % % 
% % Overall, our criteria revolves around six research questions which we collectively identified to be most pertinent to the bidirectional human-AI alignment process based on group discussions. These pertinent research questions involved aspects about \emph{category of human values}, \emph{methods of quantifying human values}, \emph{approaches to integrate human values into AI}, \emph{assessment and explanations of AI regarding human values}, \emph{human-AI interaction techniques}, and \emph{methods to adapt AI for diverse human values}. See the Appendix~\ref{app:criteria} for more details.
% % % 
% % It is worth noting that these research questions are evolved to be the key dimensions in our framework introduced in Section~\ref{sec:framework}. 





% % Built upon these identified research questions, we next introduced explicit inclusion and exclusion criteria to filter the papers. Concretely, papers under our review explicitly included \emph{studies on human values for AI alignment}, \emph{techniques} of AI development for being more consistent with human values, \emph{explanations and evaluations} that helps human better understand AI and aligned values, and \emph{interactions} that improve human perception and utilization on AI.
% % % 
% % % 
% % If a paper did not present a strong connection to all of these aspects, we exclude it from the review. 
% % % 
% % % 
% % In addition, as the scope of human-AI relevant studies is covering a wide span, we also excluded a number of tasks and study settings. 
% % % 
% % % 
% % For instance, we excluded cross-lingual alignment studies that aim to align the model representation between different languages instead of the knowledge and behaviors between human and AI. 
% % % 
% % We present the complete criteria in Appendix~\ref{app:criteria}. 
% % % 
% % % 
% % In the following section, we also describe how we complement the strict exclusion of these works by considering the expertise of our paper's authors by adding flexibility to the coding process.





% % Note that the above paper selection method targets a specific set of existing studies relevant to the bidirectional human-AI alignment via interaction perspective, as opposed to all studies in the associated domains. We are aware of the limitation of our paper selection process especially regarding the rapid growth in human-AI alignment studies. Therefore, the primary goal of this study is not to provide a comprehensive literature coverage. Instead, we aim to recognize a systematic framework that can guide pertinent studies in thinking about a more holistic perspective on human-AI alignment by taking the bidirectional interaction process into account.






% % \subsubsection{Group-based Iterative Coding.}
% % \subsubsection{Framework and Code Development.}
% \subsubsection{Qualitative Code Development.}
% % 
% % 

% % Inspired by 
% Referring to the code development process in~\citet{lee2024design}, we first conducted qualitative coding for each paper by identifying relevant sentences that could answer the above research questions, and entering short codes to describe them into a codebook. We iteratively coded relevant sentences from each paper through a mix of inductive and deductive approaches, which allowed flexibility to expand, modify or change the driving research questions based on our learnings as we went through the process. 
% % 
% % 
% % we first conducted qualitative coding for each paper by quoting the relevant sentences that could answer the aforementioned research questions into our codebook.
% % 
% % 
% To ensure rigor in our coding process, two authors coded each paper. The first author independently annotated all papers after reviewing the paper abstracts and introductions. Twelve team members each annotated a subset of the paper corpus. 
% % 
% % 
% % 
% % Particularly, we coded each paper with two authors to ensure the coding quality.
% % One author independently annotated all papers based on reviewing the paper abstracts and introductions. The rest of twelve team members each annotated a subset of the entire paper list.
% % We conducted two stages of coding, quote-based and rigorous coding. 
% % Since o
% Our corpus includes papers from different domains (\eg HCI, NLP and ML). Therefore, we divided the authors into HCI and NLP/ML\footnote{Note that NLP and ML are two different domains, we combine them together for the purposes of literature review analysis since they both work on developing and evaluating AI technologies.} teams and assigned the papers accordingly based on expertise. 
% All team members coded each of their assigned papers to answer all six questions (if applicable) introduced above.
% % based on their expertise and preference. 
% % The teammates chose the papers within their experienced domains and coded papers' quotes to answer all six questions introduced above.


% % After collecting the 411 papers, we conducted the paper annotation process to develop qualified codes and the bidirectional human-AI alignment framework. 




% % To ensure a qualified annotation process, we divided the authors into two teams based on their expertise, including an HCI team and an NLP team (Note that the NLP team here represents authors in both NLP and ML research fields). Correspondingly, we split the gathered papers into two collections for the HCI and NLP teams, respectively. As a result, the authors in the HCI and NLP teams would only review the papers published in their respective fields. The motivation of this annotation process design is twofold. First, reviewing the papers published in the author's area of expertise could better ensure the quality of developed dimensions and codes. Besides, team-based knowledge aggregation and discussions could be conducive to developing the comprehensive and systematic framework taxonomies.
% % % 



% % Inspired by the code development processed in~\citet{lee2024design},
% % % In terms of code development, 
% % % implementing qualified paper codes,
% % we had each paper annotated by two authors and computed their inter-rater reliability. Particularly, one author independently annotated all papers based on reviewing the paper abstracts and introductions. The rest of team members 
% % % the members of the NLP and HCI teams 
% % each annotated a subset of the entire paper list.
% % % collection evenly by reading the entire paper in detail. 
% % We conducted two stages of coding, quote-based and rigorous coding. 
% % % The iterative coding development took over two months.


% % The rationales of this coding implementation are from three perspectives. Firstly, the paper codes were more objective after ensuring at least two authors read each paper to decide the paper's relevance and resolve any disagreement through discussion. Secondly, we had one author read through all papers, which played a pivotal role in keeping the codes consistent and identifying the research gaps between the two representative fields (\ie HCI and NLP). Last but not least, although the one author who annotated all papers only read through each paper's abstracts and introductions, we had the rest of the NLP and HCI members read through the whole papers assigned to them. This balanced the depth and coverage of our paper annotations well.
% % % ~\hua{compute IRR}.








% % \subsubsection{Code Aggregation and Framework Development.}
% \subsubsection{Framework Development and Rigorous Coding.}
% % 
% After developing annotations, all authors collaborated to create the bidirectional human-AI alignment framework by integrating the annotations within each of the codes. The initial version of the framework was proposed by the author who reviewed all papers. This framework furthermore underwent iterative improvement through: \emph{1)} discussions with all team members involved in paper coding, and \emph{2)} revisions based on feedback from the project advisors.
% % 
% Additionally, we strengthened the framework by reviewing papers from the AI Ethics conferences (including FAccT and AIES), and related work of the collected papers that covered other domains such as psychology and social science.
% We further added missing codes and papers to ensure comprehensive coverage (see Appendix~\ref{app:venues} for details).
% % 
% The final bidirectional human-AI alignment framework, with detailed topologies, is presented in Section~\ref{sec:framework}.
% % 
% Following the framework's finalization, we conducted another separate coding process to annotate \emph{whether each paper investigated dimensions within our framework}. Two authors independently coded each paper.\footnote{The joint probability of agreement for the paper annotations was 0.78.}
% These codes were then used to perform quantitative and qualitative analyses, as presented in Section~\ref{sec:analysis}.


% % After the teams developed their annotations, all authors gathered to create the framework iteratively by combining the dimensions and codes from all team members. Particularly, the one author who read through all the papers proposed the initial version of the bidirectional human-AI alignment framework. Then, this framework was iteratively improved by: \emph{i)} iterative discussion with all the team members who coded the papers; and \emph{ii)} iterative discussion with the advisors and revision based on their feedback.
% % We present the final framework of bidirectional human-AI alignment in Section~\ref{sec:framework} for more details.
% % % 
% % After finalizing the framework with detailed dimensions and codes, we further conducted a rigorous code to annotate \emph{whether each paper investigated each of the dimensions in the framework}. Similar to the previous step, we have each paper annotated by two authors\footnote{The joint probability of agreement for the two authors' annotationswas 0.78.}. We further used these rigorous codes to conduct the quantitative and qualitative analysis shown in Section~\ref{sec:analysis}.
% % 

% % the aggregation of paper codes and framework development, we next conducted quantitative and qualitative analysis on the codes. We show the detailed approaches and findings in Section~\ref{sec:analysis}.
% % 



% % Note that this study goes beyond the aggregation of \emph{current} bidirectional human-AI alignment studies and generates \emph{new possibilities} for \emph{future} research directions. Regarding the limited amount of existing peer-reviewed literature on some aspectis within the bidirectional human-AI alignment framework (\eg customizing AI alignment for specific user groups), we also referred to the concept of \emph{scoping studies}, which aims to ``\emph{map rapidly the key concepts underpinning a research and the main sources and types of evidence available...especially where an area is complex or has
% % not been reviewed comprehensively before}''~\cite{arksey2005scoping}.
% % Specfically, underpinning the imperative research question identified in the \emph{criteria filtering} stage, we allowed flexibility in the iterative code development process in several manners. 
% % % 
% % First, to provide insights on recent advancements in human-AI alignment beyond our paper selection range, we encouraged the authors to bring in external representative papers to supplement the completeness of the developed framework taxonomies. Consequently, we expand our final paper list with an external collection to aid our framework and code development. Additionally, we conducted a series of interviews with project advisors on envisioning future directions, regardless of existing studies, to enhance bidirectional human-AI alignment.
































% ================== dead kitten ===================
% during developing the framework and paper codes iteratively.


% % 
% \textbf{Scoping Studies - Framework - generate new possibilities}.
% \emph{aim to map rapidly the key concepts underpinning a
% research area and the main sources and types of evidence
% available...especially where an area is complex or has
% not been reviewed comprehensively before}~\cite{arksey2005scoping}.








% \subsection{Systematic Literature Review}
% \label{sec:litreview}


% Figure shows our overall process of our systematic literature review and the framework creation.



% \subsubsection{Paper Selection}
% \label{sec:sampling}

% To understand the current research literature on 






% These diverse studies introduce broad definitions of human-AI alignment, and thus demonstrate the opaque research landscape and scope~\cite{kirchner2022researching}. 
% 
% 
% 
% Built upon a number of existing literature review and defining studies about human-AI alignment~\cite{matthews2022alignment,gabriel2020artificial,kenton2021alignment,yao2023instructions, ganguli2022red,terry2023ai,wang2023aligning,
% askell2021general,kirchner2022researching}, we start considering the scope of human-AI alignment in this study by elaborating \emph{who should AI align with}? \emph{Which AI technologies are we primarily considering in this study}? And \emph{what does alignment entail within the context of human-AI interactions}? Particularly, we provide our elaborated definitions introduced in this study as below:
% 
% 





% The emergence of advanced, versatile AI technologies has amplified the importance of ongoing conversations surrounding AI alignment. However, existing literature considers human-AI alignment from diverse perspective, without a consistent definition of ``\emph{what does human-AI alignment mean}'' and ``\emph{who are the humans that AI should align with}''.
% 
% For example, AI alignment commonly considers the overall problem of how to ensure an AI produces the intended outcomes as determined by its creator and /or user, without additional, undesirable side effects (\eg negative effects on individuals, groups, or even society at large)~\cite{matthews2022alignment,gabriel2020artificial,kenton2021alignment}. Meanwhile, a line of studies consider human-AI alignment from the perspectives of safety and ethics, emphasizing that AI should generate harmless contents that align with human values~\cite{yao2023instructions, ganguli2022red}.
% Additionally, some studies consider the role of interaction in human-AI alignment, and breaks down the AI alignment concepts into three alignment objectives, including specification alignment, process alignment and evaluation support~\cite{terry2023ai}. 






    % We primarily consider the lay people who would be the end users of AI systems as our objects that AI systems should align with. Particularly, in this study, we emphasize that the end users, instead of a general human group, should involve more fine-grained sub communities and individuals, who potentially have various utilization demands and concerns, such as citizens from different cultures, marginalized communities, etc. who can potentially be influenced by utilizing AI systems for various purposes.
    % % 
    % % 

    
    % Note that although AI relevant stakeholders are beyond the above range~\cite{deshpande2022responsible}, including AI practitioners (\eg AI developers, AI researchers and experts), organisational stakeholders (\eg technology companies, professional communities), national/international stakeholders (\eg countries, legislative agencies), etc. However, our study focuses on reviewing the alignment between AI with diverse human end users that would be largely influenced by utilizing the deployed AI in practice. 

    

    
    % We consider humans to be the general users who interact with AI systems, including various AI stakeholders such as AI practitioners, domain experts, and lay people.
    % \hua{Eric: what types of humans inside the human-AI Alignment -> one definitions;}






    
    % We consider AI technologies in this study to primarily focus on modern AI algorithms and systems that are extensively studied in human-AI alignment. In particular, we primarily cover literatures that study large language models (LLMs). We also include papers that investigate Machine Learning systems, such as reinforcement learning agents, that contribute imperative advancement in alignment between human and AI.

    
    
    % Despite of various advanced AI technologies, we primarily focus on Large Language Models (LLMs) as the AI systems in this work.





    % \item \textbf{Align AI to $\mapsto$ Human with Interaction.} Integrate human values to train, steer and customize AI.
    % \item \textbf{Align  \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Human} with Interaction.} We define the process of \emph{aligning AI to human} as integrating human values to train, steer and customize AI. 




    

    % \item \textbf{Align Human to $\mapsto$ AI with Interaction.} Help humans to better evaluate, explain, and inspect AI values.
    % \item \textbf{Align \textcolor{hua-red}{Human} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI} with Interaction.} We designate the process of \emph{aligning human to AI} as enhancing humans' perception and capabilities to better understand, assess, criticize, and harness the transformative AI systems. 




    


% Overall, we are aware that the scope of human-AI alignment is far beyond our studies in this work. For example, it's important to note that there are other stakeholders relevant to AI beyond end users studied in this work, such as AI practitioners (\eg developers, researchers), organizational entities (\eg technology companies, professional communities), and national/international entities (\eg governments, legislative bodies)~\cite{deshpande2022responsible}. However, our study specifically focuses on examining the alignment between AI and the diverse array of end users who will be heavily influenced by leveraging the deployed AI in practice.
% %
% Similarly, there are more prevailing AI technologies, such as Virtual Reality (VR) and Augmented Reality (AR) techniques, which becomes increasingly important in human-AI alignment but not covered in this work. 
% % 
% % 
% % 
% In conclusion, our literature review does not aim to scope all relevant studies in the realm of human-AI alignment. Instead, we are motivated by the human-centered perspective of reviewing human-AI alignment studies, and target on the specific clarified scopes introduced above to investigate the design space, limitations, and future directions in this topic.


    % \textbf{What does alignment entail within the context of human-AI interactions}? 
    % \emph{\textbf{what is human-AI alignment?}}


    % To entail a broader perspective of human-AI alignment as motivated in Section~\ref{sec:background}, in this study, we innovatively propose a conceptual paradigm, named \emph{\aligncode{bidirectional human-AI alignment}}. In specific, the alignment discussed in this study not only includes \aligncode{align AI to human}, indicating research about how to integrate human values to train, steer, and customize AI. Also, we involve \aligncode{align human to AI}, representing studies around what humans should do to critically adapt to AI advancement.
    % We provide detailed definitions below in Section~\ref{sec:definition}. 




    
    % We consider bidirectional alignment in this study, in which AI is developed to be more consistent with human values (i.e., align AI to human), and humans are enhanced to better understand, adapt to and harness AI (i.e., align human to AI). We provide detailed definitions below.
    % % 

    
    % \item \textcolor{hua-yellow}{\textbf{Interaction.}} We consider interactions to include synchronous (\eg interactive prompting) and asynchronous (\eg human-annotated data to train LLMs) interaction between human and AI systems.





% we break down human-AI alignment into two crucial paradigms: \emph{align AI to human} and \emph{align human to AI}.


    % To entail a broader perspective of human-AI alignment as motivated in Section~\ref{sec:background}, in this study, we innovatively propose a conceptual paradigm, named \emph{\aligncode{bidirectional human-AI alignment}}. In specific, the alignment discussed in this study not only includes \aligncode{align AI to human}, indicating research about how to integrate human values to train, steer, and customize AI. Also, we involve \aligncode{align human to AI}, representing studies around what humans should do to critically adapt to AI advancement.
    % We provide detailed definitions below in Section~\ref{sec:definition}. 



% and primarily base our study on the value alignment.

% We investigation primarily focuses on value alignment, whereas there are also diverse factors that we might want to consider for ``alignment'' beyond ``values'', such as norms and cultures. 







    % We primarily consider AI technologies that have been extensively researched in the field of human-AI alignment around and after the advent of AGI, such as language models, reinforcement learning models, neural network-based classification and regression models, and others.
    % % 
    % Notably, we put an emphasis on text-based models as a representative modality for alignment, while we discuss how the insights in this study can be generalized to other modality models at the end of this section.
    % the generalizability to other modality models at the end of this section.
    % are most interested in literature concerning \aicode{large language models (LLMs)}.


    % The review involved over 400 papers that were published around the advent of general-purpose generative AI, \ie primarily between 2019 until 2024 January. 


    
    % \emph{\textbf{what should be aligned?}}
    % We consider AI technologies in this study to primarily concentrate on the \aicode{outputs and/or generations} of modern AI systems that have been extensively researched in the field of human-AI alignment. Notably, we are most interested in literature concerning \aicode{large language models (LLMs)}.
    % \diyi{somewhere you might want to justify the generalization of this human-AI alignment, especially around how inshgts here can go to "multimodal pretrained models"} 
    % \hua{thanks for the constructive suggestion! indeed, we need to clarify a bit more about our what AI we include and also their generalization to other AI systems. I'll do that!}
    % Also, we partially incorporate studies examining cutting-edge machine learning systems, such as reinforcement learning with human feedback, which have significantly advanced the feasibility of human-AI alignment and assisted human decision making in practice.


% Notably, there exist other pertinent stakeholders within the AI landscape beyond the end users examined herein, including AI practitioners (\eg developers, researchers), organizational entities (\eg technology firms, professional communities), and national/international bodies (\eg governments, legislative bodies)~\cite{deshpande2022responsible}. However, our study is specifically directed towards scrutinizing the alignment between AI systems and the diverse spectrum of end users, who are potentially impacted by the practical deployment of AI technologies significantly. 
% % 
% Furthermore, while there are additional emerging AI technologies, such as Virtual Reality (VR) and Augmented Reality (AR), increasingly relevant to human-AI alignment, these are not encompassed within the scope of our investigation. 
% 




% the adapated PRISMA workflow of our systematic literature review grounded and the development of \emph{bidirectional human-AI alignment} framework.

% This paper is a collaborative effort consisting of a large team of researchers from a variety of disciplines, including Human-Computer Interaction (HCI), Natural Language Processing (NLP), Machine Learning, Informatics, and Social Science. We conducted a systematic literature review to develop the bidirectional human-AI alignment framework and codes as shown in Figure~\ref{fig:review_process}. We introduce the key details of each stage next.
% ~\hua{get the figure1 before or after? please clarify.}



% a series of in-depth discussions by NLP and HCI teams, respectively;  \emph{ii)} a series of discussion among both teams to aggregate insights; \emph{iii)} iterative discussions with project advisors (\ie senior professors and researchers in varioius domains related to bidirectional human-AI alignment). 





% However, there remain some ambiguities and inconsistencies in current literature regarding the definitions of ``\emph{What are the values in alignment}''.
% For instance, some widely discussed alignment factors, such as ``cultures'' and ``norms'', can also be considered as values.
% We thus present a comprehensive analysis of \emph{values} in the context of human-AI alignment in Section~\ref{sec:gap_value}.
% % 
% In this work, we define the \textbf{goal of alignment as ``human values'', which indicates what AI morally out to do as defined by humans}.









% =================================================





% % \subsection{Systematic Literature Review}
% \subsection{Systematic Literature Review Process}
% \label{sec:prisma}

% To understand the research literature relevant to the ongoing, mutual process of human-AI alignment, 
% we performed a systematic literature review based on the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332}.
% % 
% Figure~\ref{fig:review_process} shows 
% the workflow of our process for
% % process of our systematic literature review for 
% paper coding and developing the \emph{bidirectional human-AI alignment} framework. We introduce the step details below.
% % We referred to the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332} for reporting the workflow. 



% % \begin{figure*}[!t]
% %   \centering
% %   \includegraphics[width=1\textwidth]{figures/PRISMA.pdf}
% %   \caption{
% %   The selection and refinement process of our systematic literature review. We referred to the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332} to report the workflow.
% %   From the identification of 34,213 records by keyword search, to screen eligible papers against our criteria and arriveg at our final corpus of 411 papers. For each of the stages where literature reviews were excluded (identification, screening, and eligibility) we further present the total of excluded records.}
% %   \label{fig:review_process}
% %   \Description{}
% % \end{figure*}


% \subsubsection{Identification and Screening with Keywords.}

% % To understand the current research literature on bidirectional human-AI alignment,
% % To understand the research literature relevant to the ongoing, mutual process of human-AI alignment, 
% % we performed a systematic literature review based on the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332}.
% % 
% We started with papers published in the AI-related domain venues (including NLP, HCI, and ML fields) beginning from the advent of general-purpose generative AI to present, \ie primarily between January, 2019 and January, 2024 (see details in Appendix~\ref{app:venues}).
% We retrieved 34,213 papers in the initial \emph{Identification} stage.
% Further, we collectively defined a list of keywords (see details in Appendix~\ref{app:keyword}) and screened for papers that included at least one of these keywords (\eg human, alignment) or their variations either in the title or abstract. We included 2,136 papers in this \emph{Screening} stage.
% % We first identify fields closely relevant to our research topic. As a result, we selected the fields of NLP, HCI, and Machine Learning as our pivotal domains and the related conference venues ranging from 2019 to 2024 we considered in this project in Appendix~\ref{app:venues}.
% % 
% % 
% % From the ACL Anthology, OpenReview and ACM Digital Library, we retrieved 34,190 papers into a Reference Manager Tool (\ie Paperpile).
% % 
% % 

% % To further collect the relevant papers, two of the authors collectively defined a list of keywords related to bidirectional human-AI alignment, such as \emph{human}, \emph{alignment}, \emph{interact}, \emph{LLM}, \emph{value}, etc. Next, we only sampled the papers that included these keywords and their variations either in the title and abstract (see the comprehensive keyword list in Appendix~\ref{app:keyword}). As a result, we selected 2,136 out of 34,213 papers that are potentially relevant mentioning the keywords for our literature review. 
% % % 
% % % Note that at this stage, we aim to 



% % \subsubsection{Filtering with Inclusion and Exclusion Criteria.} 
% \subsubsection{Assessing Eligibility with Criteria}
% % 
% We further filtered the 2,136 papers based on explicit inclusion and exclusion criteria, i.e., the \emph{Eligibility} stage.
% % 
% Our criteria revolved around six research questions that we collectively identified to be most pertinent to the topic, including \emph{1) what essential human values have been aligned by some AI models?} \emph{2) how did we effectively quantify or model human values to guide AI development?} \emph{3) what strategies have been employed to integrate human values into the AI development process?} \emph{4) how did existing studies improve human understanding and
% evaluation of AI alignment?} \emph{5) what are the practices for designing interfaces and interactions that
% facilitate human-AI collaboration?} 
% % \emph{6) what are the practices for designing interfaces and interactions that facilitate human-AI collaboration?}
% \emph{6) How have AI been adapted to meet the needs of various human value groups?
% }
% % 
% % 
% We included papers that could potentially answer any of these questions.
% %, we devised a series of inclusion criteria to aid in 1) human values, 2) AI development techniques, 3) AI evaluation, explanation and utilization, and 4) building dataset with human interaction 
% % 
% Further, based on the scope in Section~\ref{sec:scope}, we excluded papers that  did not meet our inclusion criteria. This resulted in a final corpus of 411 papers, which were analyzed in detail using qualitative coding (see Appendix~\ref{app:criteria} for more details).


% % To further narrow down the scope of the keyword-filtered 2136 relevant papers, we specified the explicit inclusion and exclusion criteria collectively for selecting the papers in the following process. 
% % % 
% % Overall, our criteria revolves around six research questions which we collectively identified to be most pertinent to the bidirectional human-AI alignment process based on group discussions. These pertinent research questions involved aspects about \emph{category of human values}, \emph{methods of quantifying human values}, \emph{approaches to integrate human values into AI}, \emph{assessment and explanations of AI regarding human values}, \emph{human-AI interaction techniques}, and \emph{methods to adapt AI for diverse human values}. See the Appendix~\ref{app:criteria} for more details.
% % % 
% % It is worth noting that these research questions are evolved to be the key dimensions in our framework introduced in Section~\ref{sec:framework}. 





% % Built upon these identified research questions, we next introduced explicit inclusion and exclusion criteria to filter the papers. Concretely, papers under our review explicitly included \emph{studies on human values for AI alignment}, \emph{techniques} of AI development for being more consistent with human values, \emph{explanations and evaluations} that helps human better understand AI and aligned values, and \emph{interactions} that improve human perception and utilization on AI.
% % % 
% % % 
% % If a paper did not present a strong connection to all of these aspects, we exclude it from the review. 
% % % 
% % % 
% % In addition, as the scope of human-AI relevant studies is covering a wide span, we also excluded a number of tasks and study settings. 
% % % 
% % % 
% % For instance, we excluded cross-lingual alignment studies that aim to align the model representation between different languages instead of the knowledge and behaviors between human and AI. 
% % % 
% % We present the complete criteria in Appendix~\ref{app:criteria}. 
% % % 
% % % 
% % In the following section, we also describe how we complement the strict exclusion of these works by considering the expertise of our paper's authors by adding flexibility to the coding process.





% % Note that the above paper selection method targets a specific set of existing studies relevant to the bidirectional human-AI alignment via interaction perspective, as opposed to all studies in the associated domains. We are aware of the limitation of our paper selection process especially regarding the rapid growth in human-AI alignment studies. Therefore, the primary goal of this study is not to provide a comprehensive literature coverage. Instead, we aim to recognize a systematic framework that can guide pertinent studies in thinking about a more holistic perspective on human-AI alignment by taking the bidirectional interaction process into account.






% % \subsubsection{Group-based Iterative Coding.}
% % \subsubsection{Framework and Code Development.}
% \subsubsection{Qualitative Code Development.}
% % 
% % 

% % Inspired by 
% Referring to the code development process in~\citet{lee2024design}, we first conducted qualitative coding for each paper by identifying relevant sentences that could answer the above research questions, and entering short codes to describe them into a codebook. We iteratively coded relevant sentences from each paper through a mix of inductive and deductive approaches, which allowed flexibility to expand, modify or change the driving research questions based on our learnings as we went through the process. 
% % 
% % 
% % we first conducted qualitative coding for each paper by quoting the relevant sentences that could answer the aforementioned research questions into our codebook.
% % 
% % 
% To ensure rigor in our coding process, two authors coded each paper. The first author independently annotated all papers after reviewing the paper abstracts and introductions. Twelve team members each annotated a subset of the paper corpus. 
% % 
% % 
% % 
% % Particularly, we coded each paper with two authors to ensure the coding quality.
% % One author independently annotated all papers based on reviewing the paper abstracts and introductions. The rest of twelve team members each annotated a subset of the entire paper list.
% % We conducted two stages of coding, quote-based and rigorous coding. 
% % Since o
% Our corpus includes papers from different domains (\eg HCI, NLP and ML). Therefore, we divided the authors into HCI and NLP/ML\footnote{Note that NLP and ML are two different domains, we combine them together for the purposes of literature review analysis since they both work on developing and evaluating AI technologies.} teams and assigned the papers accordingly based on expertise. 
% All team members coded each of their assigned papers to answer all six questions (if applicable) introduced above.
% % based on their expertise and preference. 
% % The teammates chose the papers within their experienced domains and coded papers' quotes to answer all six questions introduced above.


% % After collecting the 411 papers, we conducted the paper annotation process to develop qualified codes and the bidirectional human-AI alignment framework. 




% % To ensure a qualified annotation process, we divided the authors into two teams based on their expertise, including an HCI team and an NLP team (Note that the NLP team here represents authors in both NLP and ML research fields). Correspondingly, we split the gathered papers into two collections for the HCI and NLP teams, respectively. As a result, the authors in the HCI and NLP teams would only review the papers published in their respective fields. The motivation of this annotation process design is twofold. First, reviewing the papers published in the author's area of expertise could better ensure the quality of developed dimensions and codes. Besides, team-based knowledge aggregation and discussions could be conducive to developing the comprehensive and systematic framework taxonomies.
% % % 



% % Inspired by the code development processed in~\citet{lee2024design},
% % % In terms of code development, 
% % % implementing qualified paper codes,
% % we had each paper annotated by two authors and computed their inter-rater reliability. Particularly, one author independently annotated all papers based on reviewing the paper abstracts and introductions. The rest of team members 
% % % the members of the NLP and HCI teams 
% % each annotated a subset of the entire paper list.
% % % collection evenly by reading the entire paper in detail. 
% % We conducted two stages of coding, quote-based and rigorous coding. 
% % % The iterative coding development took over two months.


% % The rationales of this coding implementation are from three perspectives. Firstly, the paper codes were more objective after ensuring at least two authors read each paper to decide the paper's relevance and resolve any disagreement through discussion. Secondly, we had one author read through all papers, which played a pivotal role in keeping the codes consistent and identifying the research gaps between the two representative fields (\ie HCI and NLP). Last but not least, although the one author who annotated all papers only read through each paper's abstracts and introductions, we had the rest of the NLP and HCI members read through the whole papers assigned to them. This balanced the depth and coverage of our paper annotations well.
% % % ~\hua{compute IRR}.








% % \subsubsection{Code Aggregation and Framework Development.}
% \subsubsection{Framework Development and Rigorous Coding.}
% % 
% After developing annotations, all authors collaborated to create the bidirectional human-AI alignment framework by integrating the annotations within each of the codes. The initial version of the framework was proposed by the author who reviewed all papers. This framework furthermore underwent iterative improvement through: \emph{1)} discussions with all team members involved in paper coding, and \emph{2)} revisions based on feedback from the project advisors.
% % 
% Additionally, we strengthened the framework by reviewing papers from the AI Ethics conferences (including FAccT and AIES), and related work of the collected papers that covered other domains such as psychology and social science.
% We further added missing codes and papers to ensure comprehensive coverage (see Appendix~\ref{app:venues} for details).
% % 
% The final bidirectional human-AI alignment framework, with detailed topologies, is presented in Section~\ref{sec:framework}.
% % 
% Following the framework's finalization, we conducted another separate coding process to annotate \emph{whether each paper investigated dimensions within our framework}. Two authors independently coded each paper.\footnote{The joint probability of agreement for the paper annotations was 0.78.}
% These codes were then used to perform quantitative and qualitative analyses, as presented in Section~\ref{sec:analysis}.


% % After the teams developed their annotations, all authors gathered to create the framework iteratively by combining the dimensions and codes from all team members. Particularly, the one author who read through all the papers proposed the initial version of the bidirectional human-AI alignment framework. Then, this framework was iteratively improved by: \emph{i)} iterative discussion with all the team members who coded the papers; and \emph{ii)} iterative discussion with the advisors and revision based on their feedback.
% % We present the final framework of bidirectional human-AI alignment in Section~\ref{sec:framework} for more details.
% % % 
% % After finalizing the framework with detailed dimensions and codes, we further conducted a rigorous code to annotate \emph{whether each paper investigated each of the dimensions in the framework}. Similar to the previous step, we have each paper annotated by two authors\footnote{The joint probability of agreement for the two authors' annotationswas 0.78.}. We further used these rigorous codes to conduct the quantitative and qualitative analysis shown in Section~\ref{sec:analysis}.
% % 

% % the aggregation of paper codes and framework development, we next conducted quantitative and qualitative analysis on the codes. We show the detailed approaches and findings in Section~\ref{sec:analysis}.
% % 



% % Note that this study goes beyond the aggregation of \emph{current} bidirectional human-AI alignment studies and generates \emph{new possibilities} for \emph{future} research directions. Regarding the limited amount of existing peer-reviewed literature on some aspectis within the bidirectional human-AI alignment framework (\eg customizing AI alignment for specific user groups), we also referred to the concept of \emph{scoping studies}, which aims to ``\emph{map rapidly the key concepts underpinning a research and the main sources and types of evidence available...especially where an area is complex or has
% % not been reviewed comprehensively before}''~\cite{arksey2005scoping}.
% % Specfically, underpinning the imperative research question identified in the \emph{criteria filtering} stage, we allowed flexibility in the iterative code development process in several manners. 
% % % 
% % First, to provide insights on recent advancements in human-AI alignment beyond our paper selection range, we encouraged the authors to bring in external representative papers to supplement the completeness of the developed framework taxonomies. Consequently, we expand our final paper list with an external collection to aid our framework and code development. Additionally, we conducted a series of interviews with project advisors on envisioning future directions, regardless of existing studies, to enhance bidirectional human-AI alignment.






==> sections_ckpt_1120/abstract.tex <==




% Recent advancements in general-purpose AI have increased the importance of steering AI systems toward people or groups' intended goals, ethical principles, and values, which is broadly known as \emph{alignment}. 
% Yet, the definitions and scopes of \emph{human-AI alignment} remains unclear, 
% which impedes the synergetic efforts across research domains to achieve \emph{human-AI alignment}. 


% Recent advancements in general-purpose AI have increased the importance of  AI alignment. Yet,
%  the definition and scope of ``\emph{human-AI alignment}'' remains unclear, as different research groups and different applications often define it differently.
%  % assign it with a different meaning.
% % 
% 





Recent advancements in general-purpose AI have highlighted the importance of guiding AI systems towards the intended goals, ethical principles, and values of individuals and groups, a concept broadly recognized as \emph{alignment}. 
However, the lack of a clarified definition and scope of \emph{human-AI alignment} poses a significant obstacle, hampering collaborative efforts across research domains to achieve this alignment.
% 
% 
% New motivation
In particular, ML- and philosophy-oriented alignment research often views AI alignment as a static, unidirectional process (\ie aiming to ensure that AI systems' objectives match humans) rather than an ongoing, mutual alignment problem~\cite{wiki_AI_alignment}. This perspective largely neglects the \emph{long-term interaction} and \emph{dynamic changes} of alignment.
% d2024chatgpt
% 
% 
% 
To understand these gaps, we introduce a systematic review of over 400 papers published between 2019 and January 2024, spanning multiple domains such as Human-Computer Interaction (HCI), Natural Language Processing (NLP), and Machine Learning (ML). 
% Within the range of this study, 
We characterize, define and scope human-AI alignment. From this, 
we present a conceptual framework for ``Bidirectional Human-AI Alignment'' to organize the literature from a human-centered perspective. 
This framework encompasses both 1) conventional studies that focus on \emph{aligning AI with humans} to see AI produces the intended outcomes determined by humans, and 2) proposes the concept of \emph{aligning humans with AI}, 
% which aims to help humans and society to understand, critique, collaborate, and adapt to AI advancements.
which aims to support humans to adapt to AI advancements, both cognitively and behaviorally.
% 
% 
% 
% 
Additionally, we articulate the key findings derived from literature analysis, including literature gaps and trends, human values in AI, and interaction techniques.
To pave the way for future studies, we envision three key challenges and give recommendations for future research.  
% Additionally, we identify limitations and risks in this area by analyzing papers quantitatively and qualitatively.
% Our analysis includes a fine-grained human value taxonomy, interaction modes for alignment, and discrepancies between AI evaluation and human assessment. 
% To pave the way for future studies, we envision new possibilities to address these gaps and highlight future directions and opportunities in research.















% ================ dead kitten ===============
% Additionally, \emph{how humans and the society could adapt to the rapid AI advancement} is also underexplored. 
% % 
% Therefore, this study conducts a systematic review of over 400 interdisciplinary papers from 2019 to 2024 covering multiple domains (\eg HCI, NLP, ML, etc.), and provides the clarified definitions within this study scope. Furthermore, from a human-centered perspective, we provide a conceptual framework of \emph{Bidirectional Human-AI Alignment} to structure the literature taxonomies. 
% % 
% % 
% The framework encompasses both traditional approaches of \emph{aligning AI to human} values in AI development, and a novel research concept focusing on \emph{aligning human to AI}, exploring human and social adaptation to transformative AI advancements.
% % 
% % 
% Based on the collective paper review codes, we conducted both quantitative and qualitative analysis to identify the limitations and risks in this topic, and envision new possibilities for future research.
% % 
% The goal of this work is to pave the way for future research on facilitating bidirectional human-AI alignment, by providing a novel framework based on comprehensive literature review, reasoning about the limitations and risks, then identifying the trends and opportunities for fut

% \hua{Dear advisors, I created a `newcommend' for each of you in `setting.tex', please feel free to directly leave your invaluable comments for us to revise. We'll work hard to address all your suggestions as much as possible! Thank you so much in advance!}
% The alignment between humans and AI has unlocked significant potential to enhance human-AI collaboration. 
% Notably, LLM systems~\hua{change} have demonstrated the efficacy of aligning LLMs with human feedback, resulting in substantial advancements in AI capabilities for human collaboration. 
% 
% However, there is a lack of clarified scope and definition of ``\emph{what is human-AI alignment}''. 
% Furthermore, froure studies.


% However, prevailing research has tended to overlook the pivotal role of interactions in achieving optimal human-AI alignment, thereby limiting the full potential of collaborative teamwork between human and AI.
% 
% In response to this gap, our objective is to introduce a comprehensive framework aimed at cultivating human-AI alignment through interactions, by conducting a systematic review of cutting-edge top-tier conference publications spanning the domains of HCI, NLP, AI and social computing from 2019 to 2023.
% % 
% The goal of this work is to pave the way for future research on facilitating interactions in developing human-AI alignment, by providing a comprehensive review of existing literature, reasoning about the limitations and risks, then identifying the trends and opportunities for future studies.
% \hua{to modify.}




% \rada{This can be done at the end, but the current title seems a bit ambiguous (what does 'holistic' mean?) and repetitive. }\hua{Sounds great! We'll revise it to be more clarified in the end. Thank you ^^.}

% Furthermore, ML- and philosophy-oriented alignment research often overlooks the role of ``humans'' in this context, such as the specification of human values, diverse interaction methods for humans to steer AI, and how humans and society could be impacted and react to AI advancements. 
% 


% \hua{Dear advisors, I created a `newcommend' for each of you in `setting.tex', please feel free to directly leave your invaluable comments for us to revise. We'll work hard to address all your suggestions as much as possible! Thank you so much in advance!}



==> sections_ckpt_1120/acknowledgement.tex <==
% 
% 
We thank Eric Gilbert for his constructive feedback on human-centered insights on alignment, thank Eytan Adar for his valuable guidance on designing the interaction techniques for human-AI alignment,
and thank Elizabeth F. Churchill for her insightful discussion on this manuscript. We also thank Michael S Bernstein, Denny Zhou, Cliff Lampe, and Nicole Ellison 
for their encouraging feedback on this work.
% We also thank our readers for their engagement with this topic. 
% Acknowledging the rapid advancements in human-AI alignment research, 
We welcome researchers' constructive discussions and interdisciplinary efforts to achieve long-term and dynamic human-AI alignment collaboratively in the future.
%
This work was supported in part by the National Science Foundation under Grant No. IIS-2143529 and No. IIS-1949634.



==> sections_ckpt_1120/analysis.tex <==


% \begin{figure*}[!t]
%   \centering
%   \includegraphics[width=\textwidth]{figures/paper_distribution.pdf}
%   \caption{The number of papers for each dimension in the \emph{bidirectional human-AI alignment} framework. Out of papers that are relevant to each research question (\ie gray bars), we show the number of papers that are relevant to each dimension (\ie color bars). This figure illustrates the extent to which each dimension has been explored by existing research. We provide more analysis in Section~\ref{sec:trend}. }
%   \label{fig:paper_distribution}
%   % \vspace{-2em}
% \end{figure*}



% Given the proposed taxonomy of bidirectional human-AI alignment and the annotated paper codes, in this section, we are interested in analyzing the difference between the research in the NLP/AI fields (\ie which largely represents the state-of-the-art studies of AI technology) and the research in HCI fields (\ie which commonly represents the studies about individual and societal perception and behaviors). By gauging the difference between the two typical research fields, we aim to potentially identify what is the research ``misalignment'' between human and AI. Particularly, 
In this section, our aim is to consolidate key findings derived from our analysis of the framework and the current state of literature we reviewed.
We begin by analyzing the overall trends and gaps in the literature (Section~\ref{sec:trend}). We then focus on three essential aspects: the relationship between human values and alignment (Section~\ref{sec:gap_value}), the potential interaction modes used to specify human values (Section~\ref{sec:gap_interaction}).
% , and the gaps between AI model and human study evaluation (Section~\ref{sec:gap_assessment}).


% In this section,
% we first analyzed the \emph{overall trends and gaps} appeared in the literature (in Section~\ref{sec:trend}). Next, we delve deeper into inspecting three essential aspects: \emph{what are human values and their relationship?} (Section~\ref{sec:gap_value}), \emph{what are the interaction modes potentially to be used for specifying human values?} (Section~\ref{sec:gap_interaction}), and \emph{what are the gaps between AI model evaluation and human study assessment?} (Section~\ref{sec:gap_assessment}).
% 
% 
% 
% Furthermore, we discuss potential solutions as future work to mitigate these gaps (in Section~\ref{sec:discussion}), where we advocate for the collective efforts from interdisciplinary communities in the future to achieve a holistic loop of human-AI alignment.


% In this section, we share use cases for our design space, our reflections on the current literature and ethical implications, the challenges and limitations we encountered in creating the design space, and our plans for future work.



% aim to analyze the ``misalignment'' between the \emph{human} and \emph{AI} 

% identify the research gaps between the NLP/AI and HCI communities from three aspects: \emph{human value} (Section~\ref{sec:gap_value}), \emph{interaction modes} (Section~\ref{sec:gap_interaction}), \emph{evaluation approaches} (Section~\ref{sec:gap_assessment}). 
% 
% 
% 
% 
% 
% 
% 
% 
% 


\begin{figure*}[!t]
  \centering
  \includegraphics[width=\textwidth]{figures/paper_distribution.pdf}
  \caption{The number of papers for each dimension in the \emph{bidirectional human-AI alignment} framework. Out of papers that are relevant to each research question (\ie gray bars), we show the number of papers that are relevant to each dimension (\ie color bars). This figure illustrates the extent to which each dimension has been explored by existing research. We provide more analysis in Section~\ref{sec:trend}. }
  \label{fig:paper_distribution}
  \vspace{-10pt}
\end{figure*}







% \subsection{Overview of Trends and Gaps in the Literature}
\subsection{Meta Analysis of Trends and Gaps}
\label{sec:trend}


Based on our coding of all papers, we computed the number of relevant papers for each dimension in the proposed bi-directional framework. Based on the distribution in Figure~\ref{fig:paper_distribution}, we noticed that in existing literature certain dimensions are over- or under-represented. We outline the under-explored dimensions in two directions in the highlighted grey bars in the end of Section~\ref{sec:ai2human2} and Section~\ref{sec:human2ai4}, respectively, and provide more details below.
% 
% 




% \noindent
\textbf{Underexplored dimensions in AI-centered alignment research.}
Most literature \emph{\textbf{\rqadim{specified human values}}} using explicit human feedback, whereas implicit and simulated human feedback were largely under-explored. 
% We delve deeper into this analysis in Section~\ref{sec:gap_interaction}.
% 
In the \emph{\textbf{\rqbdim{integrating human specifications to AI}}} research question,
Besides, developing and customizing AI models during the inference stage or using the interactive approach is under-explored.
Also, human-in-the-loop evaluation is much less explored than automatic evaluation.





% \noindent
\textbf{Underexplored dimensions in Human-centered alignment research.}
Additionally, many studies on \emph{\textbf{\rqcdim{human cognitive adjustment to AI}}} focus on enabling AI sensemaking and explanations so that humans can better understand, trust, and rely on AI. 
% 
However, these studies often focused on explaining AI decision-making justification rather than educating people to acquire general skills and competencies required to understand, use, critique, and interact effectively with AI systems (i.e., AI literacy). 
AI literacy~\cite{long2020ai} plays a fundamental role in ensuring people understand and use AI correctly, and warrants deeper exploration. Also, we observed a wide range of studies~\cite{wu2022ai,gebreegziabher2023patat,park2023generative,ma2023hypocompass} which developed interactive mechanisms and prototypes to empower \emph{\textbf{\rqddim{human collaboration with AI}}}. However, most studies assumed that AI plays an assistant role, being less capable than humans. This situation might change over time. Moreover, the influence of AI advancements on human behavior, social relationships, and societal changes is essential but remains largely unexplored.




% However, these studies often focused on explaining AI decision-making justification rather than educating everyone to acquire the skills and competencies required to critically use AI technologies and applications (i.e., AI literacy).
% % However, these studies often focused on explaining AI decision-making justifications rather than educating everyone to acquire the skills and competencies required to critically use AI technologies and applications (i.e., AI literacy). 
% AI literacy plays a fundamental role to ensure that everyone understand and use AI correctly, but remains largely underexplored compared to other topics like explanation and trustworthiness. 
% % 
% % 
% Also, we observed a wide range of studies developing interactive mechanisms and prototypes to empower \textbf{\rqddim{humans to collaborate with AI}} in diverse roles. 
% However, most existing studies assumed that AI plays an assistant role, being less capable than humans. This situation might change in the long term. Moreover, the influence of AI advancements on human behavior, social relationships, and societal changes is important but remains largely unexplored. 





% Additionally, we observed a wide range of studies developing interactive mechanisms and prototypes to empower \textbf{\rqddim{humans to collaborate with AI}} of diverse roles. However, the existing studies mostly assumed that AI plays an assistant role collaboration, which is less capable than humans. This might potentially changed in the long-term perspective. Also, how AI advancements will influence human behavior, social relationship, and the societal change is also important yet much less explored.





% To identify the overview of the trends and gaps in the literature, we further conducted a quantitative analysis of the outcome of our rigorous codes. Particularly, we compute the number of relevant papers for each dimension presented in the \emph{Bidirectional Human-AI Alignment} framework. Figure~\ref{fig:paper_distribution} shows the distribution of paper numbers across 25 dimensions in the framework. The two dimensions of the ``human value category'' are not included but are further analyzed with details in Section~\ref{sec:gap_value}.
% % 
% % 
% As a consequence, we observed that certain dimensions are over- or under-represented. 



% To highlight a few notable phenomena, we observed that most of the literature \textbf{\rqadim{specify human values}} using the explicit human feedback. However, the interaction modes dominantly skew toward several formats (\eg rating and ranking and natural language interaction/conversations). We provide more in-depth analysis in Section~\ref{sec:gap_interaction}.
% There are some but much less studies leverage simulated human value feedback (\eg  human feedback simulators) for specification. The implicit human feedback is much under-explored but potentially contains informative values as well to be investigated.



% 
% % 
% %
% % 
% Many of the studies about \textbf{\rqcdim{human cognitive adjustment to AI}} focused on enabling AI sensemaking and explanations for humans to understand AI. However, these approaches largely focused on explaining AI decision-making justifications for humans, rather than educating humans to harness the skills and competencies required to use AI technologies and applications effectively (\ie AI literacy). This is  which is also important but large under-explored.
% % 
% AI literacy, which aims to educate everyone to critically understand and use AI, is important to ensure that humans will use AI in the correct ways. However, it's largely underexplored compared with other relevant topics like explanation and trustworthiness until now.


% Additionally, we observed a wide range of studies developing interactive mechanisms and prototypes to empower \textbf{\rqddim{humans to collaborate with AI}} of diverse roles. However, the existing studies mostly assumed that AI plays an assistant role collaboration, which is less capable than humans. This might potentially changed in the long-term perspective. Also, how AI advancements will influence human behavior, social relationship, and the societal change is also important yet much less explored.






% Based on our coding of all papers, we observe that certain dimensions in the \emph{bidirectional human-AI alignment} space are over- or under-represented. 
% % Figure~\ref{fig:paper_distribution} shows the number of papers per dimension coded as relevant.
% To highlight a few notable phenomena, we observe that \rqadim{\emph{\textbf{human values}}} are often unspecified in the literature, in which the existing studies usually mention general human values vaguely or focus on a specific set of typical human values, such as fairness, interpretability, harmlessness, etc. 
% % 
% This suggests future work may want to more explicitly specify what human values their study is examining. 
% % 
% % 
% The topic of \rqbdim{\emph{customizing AI values}} is another area that is under-represented compared to integrating general values into AI. While there has been extensive research on approaches to mitigate bias in AI models, there is a lack of studies focusing on other human values and how to steer models to generate more value-oriented outputs.
% % 
% % 
% In addition, we observe an increasing number of studies developing human-AI collaborative tools/systems, and generative agents that can simulate human behavior automatically. However, we also noticed that existing studies sometimes lack a in-depth analysis and investigation of \rqddim{critical thinking of the AI impacts} on Individuals and the society.
% % 
% We hope that the provision of our bidirectional human-AI alignment framework can help researchers to identify these issues and think about the approaches to resolve them. 
% To better support researchers understand the gaps, we delve into three common gaps we observed in the literature and our coding.
% % \hua{I will rewrite this section after our Figure~\ref{fig:paper_distribution}'s result is out.}
% % \hua{maybe we can split the figure into separate parts to be analyzed.}






% \subsubsection{A lack of customized alignment for diverse values}





% \subsubsection{A lack of studies examing the AI's impact on AI and society}




% Desired values for AI tools







\begin{figure*}[!t]
  \centering
  \includegraphics[width=\textwidth]{figures/interaction_mode.pdf}
  \caption{The interaction techniques for specifying values in human-AI alignment. We compare the common interaction techniques used for the model ``Learning'' and ``Inference'' stages in human-focused (\eg HCI) and AI-focused (\eg NLP/ML) research studies. 
% %     % 
% 
% % 
%     Discarded Options[NLP]: \cite{lu2022towards}
%   Language Analysis[NLP]: \cite{park2020scalable}  
%   Social Relationship[NLP]: \cite{isajanyan2024social}  
%   Rating[NLP]: \cite{ouyang2022training}  
%   Ranking[NLP]: \cite{yuan2024rrhf}
%   Features - Beyond Imitation[NLP]: \cite{guo2023beyond}  , HCI = \cite{feng2019can},
%   Principles[NLP]: \cite{bai2022constitutional} , [HCI]:\cite{petridis2024constitutionmaker},
%   Text Edit[NLP]: \cite{yao2023improving}, [NLP Inference]: \cite{lin2023unlocking}, [HCI]: \cite{hong2022scholastic} 
%   Conversations \cite{hwang2023aligning}, HCI=\cite{shen2023convxai}, NLP Inference: \cite{zhang2021human}
%   Multimodal [HCI]: HINT \cite{chen2022hint}, [NLP Inference]:\cite{geva2022lm}
%   Talebrush \cite{chung2022talebrush} HCI, 
%   AI Chain \cite{wu2022ai} HCI
%   Pearl \cite{jorke2023pearl} HCI,
%   % 
  % 
% \hua{read this article suggested from Eytan~\cite{brath2021surveying} \url{https://richardbrath.wordpress.com/2021/10/31/58-ways-to-visualize-alice-in-wonderland/} to improve this section.}
  }
  \label{fig:interaction}
  \vspace{-1em}
\end{figure*}
% 
% % 
% 
% 
% 
% 
\begin{table*}[!t]
\centering
% \vspace{-10pt}
\begin{tabular}[t]{@{}  !{\color[HTML]{808080}\vrule width 2pt} p{.98\textwidth} !{\color[HTML]{808080}\vrule width 2pt} @{}}
\cellcolor[HTML]{E6E6E6} 
\textbf{Takeaways of Interaction Techniques for Alignment.}
% \newline
\vspace{5pt}

1. Some common human feedback formats (rating, ranking) used in NLP/ML are not often studied in HCI.
\vspace{5pt}

2. Diverse human interactive feedbacks in HCI are not fully used in AI development in NLP/ML fields.
\end{tabular}
\end{table*}
% 



\subsection{Insights into Human Values for Alignment}
\label{sec:gap_value}


% While many papers claim to integrate or evaluate AI in relation to human values, the specific sets of human values they examine often lack clarity or comprehensiveness. 
% In order to articulate and systematically understand human values relevant to bidirectional human-AI alignment, we structured these values using a combination of top-down and bottom-up methods based on a theory of cross-cultural psychology (Section~\ref{sec:value_method}). As a result, we identified the structural relationships among human values (see Figure~\ref{fig:value_structure}) and mapped existing literature to a fine-grained taxonomy (see Figure~\ref{fig:value_taxonomy}) in Section~\ref{sec:value_outcome}. Additionally, we present our analysis findings of human values that are particularly relevant for future studies (Section~\ref{sec:value_finding}).



% While many papers claimed to integrate or evaluate AI with respect to human values, the sets of human values they studied often needed to be clarified or completed.
% To articulate and systematically understand human values related to bidirectional human-AI alignment, we structured the relevant values using a top-down and bottom-up method grounded on a theory of cross-cultural psychology (Section~\ref{sec:value_method}). As a result, we identified the structural relationship among human values (Figure~\ref{fig:value_structure}) and mapped the existing literature to the fine-grained taxonomy (Figure~\ref{fig:value_taxonomy}) in the Section~\ref{sec:value_outcome}.
% Moreover, w
% We present the findings of human values for alignment, collected during the process of adjusting the ``Schwartz Theory of Basic Values'' and conducting literature review, that are worth noting to the future studies.
% 
% 
% 
% We present the key findings for future research which are identified during our adjustment of the ``Schwartz Theory of Basic Values'' and literature review.


Our analysis, based on the adaptation of Schwartz's Theory of Basic Values and our comprehensive literature review, identifies three critical findings for future research:


\textbf{Value Prioritization in AI Systems.} Human value systems are not merely subsets of values, but ordered systems with relative priorities~\cite{schwartz1994there,schwartz2012overview}. For instance, \citet{schwartz2012overview} presented the definition for this phenomenon: \emph{\say{a value is ordered by importance relative to other values to form a system of value priorities.
The relative importance of multiple values guides action....The trade-off among relevant, competing values guides attitudes and behaviors.}}.
% 
Current AI alignment algorithms, often based on datasets of human preferences~\cite{ouyang2022training,song2024preference,rafailov2024direct}, may inadvertently prioritize majority values, potentially neglecting those of marginalized groups~\cite{fleisig2023fairprism}. Future research should address this complex interplay of values in AI systems.





\textbf{Universal vs. Personalized AI Values}. While certain values are universally expected from AI (e.g., capability, equity, responsibility), others may be undesirable in specific contexts~\cite{ngo2022alignment} (e.g., seeking power). Simultaneously, AI models should be adaptable to diverse human value systems~\cite{sorensen2024roadmap}. Research is needed to develop methods for identifying appropriate value sets for specific individuals or groups, and for customizing AI to align with user values while maintaining ethical principles.




\textbf{Disparities in Value Expectations and Evaluation}. The fundamental differences between humans and AI necessitate distinct approaches to value evaluation. For instance, assessing AI honesty may require mechanistic interpretability~\cite{bereska2024mechanistic}, a more rigorous standard than that applied to humans. Future studies should explore methods for evaluating and explaining AI values and calibrating human expectations accordingly.








% \subsubsection{\textbf{The Relative Priority of Values is as Crucial as Their Existence}}
% \label{sec:value_finding}


% Based on the definition from \citet{schwartz1994there}, we noted that a human value system is not an exclusive subset of values, but rather, an ordered system.
% % 
% \citet{schwartz2012overview} presented the definition for this phenomenon: \emph{\say{a value is ordered by importance relative to other values to form a system of value priorities.
% The relative importance of multiple values guides action....The trade-off among relevant, competing values guides attitudes and behaviors.}}
% % 
% % % 
% % \begin{quote}
% %     \say{a value is ordered by importance relative to other values to form a system of value priorities.
% %     The relative importance of multiple values guides action....The tradeoff among relevant, competing values guides attitudes and behaviors}~\cite{schwartz2012overview}.
% %     % \textit{The key to identifying the structure of value relations is the assumption that actions taken in the pursuit of each type of values have psychological, practical, and social consequences that may conflict or may be compatible with the pursuit of other value types.}~\cite{schwartz1994there}
% % \end{quote}
% % 
% % 
% % We first highlight from feature (5) and (6) that a human value system is not an exclusive subset of values, but rather, an ordered system.
% % 
% % \begin{quote}
% %     {
% %     , and (5) is ordered by importance relative to other values to form a system of value priorities.
% %     (6) The relative importance of multiple values guides action. Any attitude or behavior typically has implications for more than one value...The tradeoff among relevant, competing values guides attitudes and behaviors}~\cite{schwartz2012overview}.
% %     \textit{The key to identifying the structure of value relations is the assumption that actions taken in the pursuit of each type of values have psychological, practical, and social consequences that may conflict or may be compatible with the pursuit of other value types.}~\cite{schwartz1994there}
% % \end{quote}
% % 
% For instance, the pursuit of achievement values can possibly clash with benevolence values. 
% % In human contexts, striving for personal success often hinders efforts to improve the welfare of others who require assistance. 
% Similarly, 
% previous studies have highlighted the trade-offs between AI's state-of-the-art capabilities and their ethical performance, such as interpretability and fairness~\cite{shen2022improving}.
% % in AI, focusing on achieving state-of-the-art performance may impede efforts for accountability.
% % 
% While most alignment algorithms utilize datasets of human ratings and preferences collected in the wild~\cite{ouyang2022training,song2024preference,rafailov2024direct}, AI models may inadvertently align with the value priorities of the majority represented in these datasets, potentially overlooking or sacrificing the value systems of marginalized groups~\cite{fleisig2023fairprism}.







% \subsubsection{Value Distribution in Literature}
% \mbox{}



% \subsubsection{Generalizability of Value Alignment: Relationship between Aligning Values and Other Factors}
% \mbox{}

% We investigation primarily focuses on value alignment, whereas there are also diverse factors that we might want to consider for ``alignment'' beyond ``values'', such as norms and cultures. 




% % \textbf{Value Systems are Priority over Values, Not Subsets}

% \subsubsection{Value Systems are Priority over Values, Not Subsets}
% \mbox{}


% We first highlight from feature (5) and (6) that a human value system is not an exclusive subset of values, but rather, an ordered system.

% \begin{quote}
%     \textit{The key to identifying the structure of value relations is the assumption that actions taken in the pursuit of each type of values have psychological, practical, and social consequences that may conflict or may be compatible with the pursuit of other value types.}~\cite{schwartz1994there}
% \end{quote}

% For instance, the pursuit of achievement values can clash with benevolence values. 
% In human contexts, striving for personal success often hinders efforts to improve the welfare of others who require assistance. 
% Similarly, in AI, focusing on achieving state-of-the-art performance may impede efforts to bolster accountability.

% While most alignment algorithms utilize datasets of human ratings and preferences collected in the wild~\cite{ouyang2022training,song2024preference,rafailov2024direct}, AI models may inadvertently align with the value priorities of the majority represented in these datasets, potentially overlooking or sacrificing the value systems of marginalized groups~\cite{fleisig2023fairprism}.






% % % \textbf{Human-desired AI Values and Customization to Personal Values}
% \subsubsection{\textbf{Human-desired AI Values and Customization to Personal Values}}


% While further research in AI ethics is crucial in this nuanced area, there are values that, in general, humans expect AI to prioritize (e.g., capability, equity, responsibility) and values that humans do not want AI to integrate in specific scenarios (e.g., seeking power to avoid or harm people~\cite{ngo2022alignment}).
% On the other hand, 
% AI models are expected to
% % we hope that AI models can 
% be tailored to 
% accommodate diverse human value systems~\cite{sorensen2024roadmap}, which necessitates a comprehensive understanding of all types of values.
% Therefore, future research could potentially explore the directions of: (1) developing methods to identify the appropriate sets of human values to align with specific individuals or groups, 
% % a universal guideline for values desired in AI by humans, 
% and (2) understanding and customizing AI to align with users' values while maintaining its inherent ethical principles.





% % % \textbf{Expectations and Evaluations of Values Can be Different in Humans and AIs}
% \subsubsection{\textbf{Expectations and Evaluations of Values May Differ Between Humans and AI Systems}}



% Due to the fundamental differences between humans and AI models, the expectations for evaluating certain values can vary between the two. For instance, while human honesty can hardly be assessed except observable actions, for AI models the expectations might be higher. 
% It could involve reverse-engineering the computational mechanisms and representations learned by neural networks into concepts understandable to humans. 
% This approach, known as \textit{mechanistic interpretability}, provides a in-depth understanding of how AI models operate~\cite{bereska2024mechanistic}.
% Future research is needed to explore evaluating AI values and calibrating human expectations of these values.









% % \subsubsection{Results and Findings from the Paper Coding.}
% % \mbox{}


% % % Based on the aforementioned process, we achieved our detailed human value taxonomy as described in Fig~\ref{fig:schwartz}. 
% % % \hua{TODO: add a figure/table of human values here.}



% % \begin{itemize}

% %     \item \hua{use data / citations to support below findings. add more interesting findings}
    
% %     \item current methods (e.g., RLHF) generally finetune the AI models using aggregated data without a clear scrutinization on \emph{what exact values the dataset is conveying}. This could potentially result in undesirable values being integrated into AI.

% %     \item Many papers predominantly relied on the concept of "general human preference" to represent "values" without clearly specifying the exact human values they are investigating.
% %     \item Within the NLP/AI domain, values embedded into AI models during the learning stage (e.g., harmlessness, helpfulness, honesty, etc.) often do not overlap with the values being evaluated.
% %     \item A comparison of NLP and HCI papers reveals that NLP covers a broader range of values, while HCI primarily focuses on a narrower range, including transparency, fairness, accountability, and equity.
% % \end{itemize}














\subsection{Interaction Techniques for Specifying Human Values: A Cross-Domain Analysis}
\label{sec:gap_interaction}


Our research reveals disparities in interaction techniques for human-AI value alignment across AI-centered (NLP/ML) and human-centered (HCI) domains. As depicted in Figure~\ref{fig:interaction}, this analysis focuses on three key areas:


\textbf{Domain-Specific Interaction Techniques}. The interaction techniques in AI-centered (NLP/ML) and Human-centered (HCI) alignment studies are often differ~\cite{brath2021surveying}.
NLP/ML studies primarily utilize numeric and natural language-based techniques. Also, NLP/ML research explore implicit feedback to extract human hidden feedback. In contrast, HCI research encompasses a broader range of graphical and multi-modal interaction signals (e.g., sketches, location information) beyond text and images. This disparity suggests potential gaps in extracting comprehensive human behavioral information.


\textbf{Stage-Specific Interaction Techniques}. In NLP/ML, the learning stage predominantly employs rating and ranking interactions for alignment in dataset generation. However, when humans use AI in the inference stage, as demonstrated in HCI research, involves more diverse user interactions. This discrepancy highlights the need for alignment between model development and practical deployment.


\textbf{Divergent Data Utilization}. NLP/ML typically uses interaction outputs as training datasets, while HCI analyzes this data to understand human behavior and feedback. As AI systems evolve, developing new interaction modes to capture a broader spectrum of human expression becomes crucial.






% Selecting suitable interaction techniques for humans to specify AI values for alignment is crucial. Each research domain offers distinct strengths and insights to address this challenge. From the bidirectional perspective, we investigate the status quo of existing interaction techniques for alignment specification in both human-centered (\eg HCI) and AI-centered (\eg NLP/ML) studies. 
% Additionally, we provide a detailed analysis of how these techniques have been utilized in the learning and inference stages, as shown in Figure~\ref{fig:interaction}.







% We show the main interaction mode for human-AI alignment and the most common interaction formats leverage in NLP/AI and HCI fields during the learning and the inference stages in Figure~\ref{fig:interaction}.
% 
% We observe several difference between the two fields introduced below.
% In examining the interaction modes between Natural Language Processing (NLP) and Human-Computer Interaction (HCI) fields, several gaps emerge. 
% Interaction and the resulted data are imperative to human-AI alignment. 
% 




% \subsubsection{\textbf{Interaction Techniques Across Various Domains}}
% As shown in Figure~\ref{fig:interaction}, the coverage of interaction techniques in AI-centered (\ie {\color[HTML]{1C5CCC} \colorbox{bg-blue}{NLP/ML Research}}) and human-centered (\ie {\color[HTML]{A61C00} \colorbox{bg-red}{HCI Research}}) studies often differ~\cite{brath2021surveying}. Particularly, we see that NLP/ML studies primarily leverage \emph{numeric-based}, \emph{natural language-based} interaction techniques for human-AI interaction and alignment. In addition, NLP/ML researchers also leverage implicit feedback to improve the model. 
% For example, some systems took in implicit signals such as contextual information, or discarded options to develop AI systems.
% % This is understandable since human labeled data is usually expensive, therefore, NLP/ML researchers tend to use implicit feedback to extract more human behavioral information to improve AI models.
% In comparison, HCI studies cover more diverse graphical multi-modal interaction signals (\eg sketches, location information) beyond text and images, which can be largely attributed to the proficient graphical user interface development skills found in HCI researchers and practitioners. 
% This potentially indicates gaps in the human behavioral information that the two fields can extract from the users of the AI models. 
% % Systems also leverage natural language interaction, such as breaking AI output into digestible chunks for multi-turn dialogues with the users. 










% \subsubsection{\textbf{Different Interaction Techniques in Separate Stages}}
% % \subsubsection{Interaction Formats}
% Another finding we discerned is the different interaction techniques used in separate stages, especially in the NLP/ML fields. 
% Specifically, the learning stage relies mostly on \emph{rating} and \emph{ranking} interaction to deal with the generated datasets of the models. However, users leverage the AI model in different ways during inference stage, as demonstrated in HCI research.
% This indicates that users might elicit different needs in practice when interacting with AI during the model deployment stage.
% % in different ways. 
% Therefore, future NLP/ML and HCI researchers might collaborate to keep the human-AI interaction techniques informed (or even consistent) by both domains in order to facilitate close alignment between humans and AI.
% % want to keep in mind how they want users to use the developed system to make the AI and human more aligned.

% % NLP studies leverage human annotated data in learning stage to train the model. Therefore, we consider it as an indirect interaction between human and AI. 




% \subsubsection{\textbf{Dissimilar Usage of Interaction Data Between Domains}}
% We noticed that the ways in which the two domains utilize data differ. For example, the interaction outputs of NLP research are commonly the dataset to be trained in the model, whereas HCI researchers use usage data to analyze human behavior and feedback. 
% % 
% % 
% % 
% % 
% % 
% As AI systems continue to advance, new modes of interaction are required to capture more space of human expression, with the goal of deeper and meaningful alignment. This is an important area for NLP/ML researchers to partner with HCI researchers for designing interaction paradigms, including but certainly not limited to affective computing, accessibility, social computing, computer-supported cooperated work, and ubiquitous computing. 










% As AI systems continue to advance, new and novel modes of interaction are required to capture more space of human expression for deeper and more meaningful alignment. This is an important area for AI researchers to partner with HCI sub-fields for designing interaction paradigms, including but certainly not limited affecting computing, accessibility, social computing, computer-supported cooperated work, and ubiquitous computing. 









% \subsection{
% % Gaps of AI Model Evaluation in and Human Study Assessment
% % 
% Gaps Between AI-Centered and Human-Centered Evaluations
% }
% % \subsection{Evaluating AI Systems and Human Study Evaluation}
% \label{sec:gap_assessment}







% Our analysis reveals significant disparities in evaluation approaches between NLP/ML and HCI domains, highlighting three key areas for improvement:


% \textbf{Divergent Evaluation Objectives}. NLP/ML evaluations primarily focus on algorithmic performance, while HCI studies emphasize user experience and interactions. Future research should integrate these perspectives, developing human-centered evaluation benchmarks for AI systems based on HCI insights.


% \textbf{Contrasting Utilization of User Information}. NLP/ML research predominantly employs quantifiable measures (e.g., accuracy, precision), whereas HCI gathers both quantitative and qualitative data on user experiences. Future work should explore methods to convert qualitative human feedback into quantifiable data for AI system improvement and alignment.


% \textbf{Disparate Evaluation Approaches and Scales}. NLP/ML typically uses automated or human-in-the-loop evaluations on extensive datasets, while HCI employs in-depth qualitative and quantitative measurements on defined human groups. Adopting consistent evaluation strategies across domains could lead to a more comprehensive understanding of human-AI interaction and alignment.








% Improving bidirectional alignment between humans and AI can potentially be further enhanced by collaborative efforts and commitments from both the NLP/ML and AI domains, ensuring consistency in evaluation methods and metrics.
% % 
% % Facilitating bidirectional human-AI alignment can also be benefited from 
% % Closing the gap between NLP/AI and HCI domains necessitates 
% % synergistic efforts and commitments, from both NLP/ML and AI domains, to maintaining consistency in evaluation approaches and metrics.
% % 
% Nevertheless, we observed notable gaps by comparing the literature analysis regarding ``evaluating AI systems'' (\ie Section~\ref{sec:evaluation}) and ``evaluation in human studies'' (\ie Section~\ref{sec:assessment}).



% \subsubsection{\textbf{Different Objectives and Expectations of Evaluations in Humans and AI}}
% Evaluating AI systems primarily focuses on \emph{what} algorithmic performance is, aiming to determine how well proposed methods perform compared with benchmark or human-in-the-loop evaluation. Conversely, human study evaluations are more concerned with \emph{why} -- understanding the user experience and interactions, often prioritizing both quantitative and qualitative measurements to gain a comprehensive understanding of user experience and interactions with AI systems.
% Given the distinct objectives in evaluation, future research has the potential to collaborate in bridging these gaps. For instance, informed by the user experience and demands revealed by HCI studies, NLP/ML researchers can incorporate the insights and design human-centered evaluation benchmarks to assess AI systems.
% % 
% % % \hua{add examples + value-context measurement.}
% % 
% % \subsubsection{Expectations and Evaluations of Values Can be Different in Humans and AIs}
% % \mbox{}
% % Due to the fundamental differences between humans and AI models, the expectations for evaluating certain values can vary between the two. 
% % For instance, while human honesty can hardly be assessed except observable actions, for AI models the expectations might be higher. 
% % It could involve reverse-engineering the computational mechanisms and representations learned by neural networks into concepts understandable to humans. 
% % This approach, known as \textit{mechanistic interpretability}, provides a in-depth understanding of how AI models operate~\cite{bereska2024mechanistic}.
% % Future research should focus on evaluating AI values and calibrating human expectations of these values.


% % \vspace{-10pt}

% \subsubsection{\textbf{Contrasting Ways of Utilizing User Information}}
% % 
% Given the diverse objectives of assessment described above, NLP/ML research primarily focuses on quantifiable measures such as accuracy, precision, and recall. The information received in evaluating AI systems is often accurately measurable, e.g., ratings, rankings, and multiple choice questions.
% % 
% % In NLP research, evaluations primarily aim to determine the performance of algorithmic methods, 
% % focusing on quantifiable measures such as accuracy, precision, and recall. 
% In comparison, by focusing on understanding the user experience and interaction with AI systems, HCI research often involves gathering both quantitative and qualitative data, such as user feedback, perceptions, and behaviors. 
% The collected information from HCI research might cover a wider spectrum of qualitative data related to human values, experience, and needs in practice than what can be captured by quantitative metrics alone. However, 
% incorporating qualitative findings into improving AI systems can be difficult. 
% % some qualitative findings are challenging to be leveraged in enhancing AI systems.
% Therefore, future researchers can investigate methods to convert qualitative human feedback into quantitative data that AI systems can effectively utilize and align with.
% % 
% % NLP feedback can actually be used to directly improve the model, but it's not clear how to actually incorporate feedback from HCI systems
% % Therefore, the data formats are more diverse in HCI, and sometimes could not be quantitatively described. 
% % 
% % \hua{add example+ value-context measurement.}.







% \subsubsection{\textbf{Evaluation Approaches and Scale}}
% % 
% Prior studies in NLP/ML have predominantly relied on 
% automated or human-in-the-loop evaluation methods to assess AI system performance across extensive datasets.
% In comparison, 
% HCI studies 
% % prioritize a more comprehensive approach, utilizing 
% typically employ qualitative and/or quantitative measurements to gain deeper insights into user experiences and interactions within defined human groups.
% % 
% % 
% % 
% % 
% % 
% These divergent aspects highlight diverse gaps between the evaluation methods and scales utilized in the two domains. 
% % While NLP tends to focus on automated evaluation techniques, HCI places greater emphasis on both quantitative and qualitative measurements to assess human-AI interaction and alignment. 
% Closing this gap and adopting consistent evaluation strategies could lead to a more holistic understanding and synergy of human-AI interaction and alignment across both fields. 
% % We discuss potential ways to mitigate these gaps in Section~\ref{sec:discussion}.
% % 
% % 
% % 
% % 



% Overall, it's important to note that the disparities between HCI and NLP/ML studies extend beyond the above aspects, \eg research methods and problem formation. 
% Our analyses aim to pave the way for future interdisciplinary research collaboration, fostering bidirectional alignment between humans and AI across diverse domains.


% % Overall, it worth noting that the gaps between HCI and NLP/AI domain studies are far more beyond the aforementioned aspects, such as regarding the key research methodology and problems.
% % For example, regarding methodology, NLP/AI primarily focus on developing novel learning algorithms to incorporate human values into AI models (\eg RLHF, DPO, etc.). In comparison, HCI studies predominantly emphasize on approaches of empowering human-AI interaction or assessing AI impacts on individuals and groups, and others.
% % 
% % % 
% % These analyses aim to pave the way for future research across various domains to synergize collaboratively for achieving the bidirectional human-AI alignment.

% % As methodologies are evolving rapidly, we decided to explore the above gaps which might exist in a long history and benefitial/generalized to more research questions beyond human-AI alignment (\eg evaluation approaches, interaction techniques).













% \subsubsection{Keep Consistent between Model Evaluation and Human Assessment}
% By referring to Section~\ref{sec:evaluation} and Section~\ref{sec:assessment}, NLP researchers can better discern the misalignment between model evaluation and human assessment in terms of objects, priorities and extracted information. As the results, NLP researchers can potentially develop better evaluation methods that align with human demands in practice, which can in return boost the AI model alignment better with human. 


% ================================================================




% ========================== dead kitten ==============

% In this section, we conduct qualitative and quantitative analysis on the reviewed papers. We aim to identify the difference between NLP/AI fields and HCI fields, with specific focus on \emph{human values}, \emph{evaluation}, and \emph{interactive value presentation methods}.
% 
% 
% \savvas{misalignment in HCI + NLP}



% In this section, we focus on extracting the papers' data to quantitatively/qualitatively analyze the findings.
% 
% 1. To what extent are human values well-aligned with developed AI?
% 
% 2. are interaction paradigms fully leveraged in human-AI alignment techniques?
% 
% 3. situated values and customized AI alignment?
% 
% 4. what are under-explored research dimensions? heatmaps


% \subsection{what hasn't been explored? AI for jounalism -> what hasn't been done? What Can we say for the future research in NLP/HCI from this paper?}










% === To what extent are human values well-aligned with developed AI?
% 
% 
% We could analyze the ``misalignment'' from two aspects:
% 
% 1. the alignment values in training is NOT the values being evaluated (within NLP).
% 2. the values studieds in HCI field is not fully aligned with NLP field.
% 
% \hua{not make the papers convoluted.}








% \subsection{Situated values and customized AI alignment?}



% general v.s. situated alignment?






% \hua{paper analysis heatmap}






% Our analysis reviews the ambiguity and gaps in how the NLP/AI and HCI communities prioritize and conceptualize human values in bidirectional human-AI alignment research. 
% % 
% Particularly, on one hand, while numerous papers claimed to examine the LLMs with respect to human values, the range of values are unclear. 
% On the other hand, we observed a different emphasis on the human values when comparing papers published in NLP/AI venues and HCI venues. 
% % 
% 
% To provide a clear picture of \emph{what} and \emph{how} human values have been investigated in these domains, we next take a deeper look at the detailed method of \emph{how we come up with the human value taxonomy} described Section~\ref{sec:value_category}, and \emph{what are our findings} based on the final coding of all papers.






% \subsection{Are interaction paradigms fully leveraged in human-AI alignment techniques?}

% interactions in HCI v.s. NLP?

% \hua{add the interaction formats comparison}








% The difference in assessment methods between NLP and HCI reflects the differing priorities and objectives of the two fields. While NLP tends to prioritize automated evaluation methods to assess AI performance, HCI places greater emphasis on both quantitative and qualitative measurements to understand user experiences and interactions with AI systems more comprehensively.
% 
% Most of the evaluations in NLP studies aim to answer \emph{what is the performance of the proposed algorithmic method}, in contrast, HCI studies are more often interested in \emph{why} -- to understand user experience and interactions.
% While most NLP studies conduct automated or human-in-the-loop evaluation methods to assess AI performance, HCI studies place greater emphasis on both quantitative and qualitative measurements to understand user experiences and interactions with AI systems more comprehensively.








% we 
% these social psychology studies, we start with a \textit{top-down} framework by using the taxonomy of the Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012refining,schwartz2012overview}, which is a widely accepted theory of basic human values with cross-cultural psychology and universal values~\cite{kang2023values,kiesel2022identifying}.




% In order to articulate and systematically understand human
% values relevant to bidirectional human-AI alignment, we structured these values using a combination of top-down
% and bottom-up methods based on a theory of cross-cultural psychology


% While the research papers often mention human value alignment as a key objective, either explicitly or implicitly, the majority do not offer a clear definition of "human value." This term appears vague and inconsistent across the literature, highlighting the need for a more precise definition. 
% Building upon \citet{rokeach1973nature}'s cross-cultural value survey, Schwartz summarized some widely agreed-upon features of human values:

% \begin{quote}
%     \textit{A value is a (1) belief (2) pertaining to desirable end states or modes of conduct, that (3) transcends specific situations, (4) guides selection or evaluation of behavior, people, and events, and (5) is ordered by importance relative to other values to form a system of value priorities}~\cite{schwartz1994there}.
% \end{quote}

% \begin{quote}
%     \textit{(6) The relative importance of multiple values guides action. Any attitude or behavior typically has implications for more than one value...The tradeoff among relevant, competing values guides attitudes and behaviors}~\cite{schwartz2012overview}.
% \end{quote}

% These features help distinguish values from related concepts such as needs and attitudes. 
% For example, a preference for blue ties would not qualify as a value~\cite{schwartz1994there}.
% Motivated by these social psychology studies, we start with a \textit{top-down} framework by using the taxonomy of the Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012refining,schwartz2012overview}, which is a widely accepted theory of basic human values with cross-cultural psychology and universal values~\cite{kang2023values,kiesel2022identifying}.

% The theory of basic human values is a theory of cross-cultural psychology and universal values that was developed by Shalom H. Schwartz. The theory extends previous cross-cultural communication frameworks such as Hofstede's cultural dimensions theory.







% NLP: primarily numeric and natural language interactions; Also, NLP tends to leverage implicit feedback to extract more data from human.

% HCI: more diverse interaction formats, covering graphical multi-modal interaction;







% In the offline world, humans communicate meaning with figures of speech, minute facial expressions, rapid hand-gestures, emphatic body language, reflective gaze, and much more. However, AI systems scarcely consider these diverse interaction modes. Early AI systems ask humans to evaluate outputs via rating with numbers. While numeric inputs are simple to implement from the \textit{machines'} perspective, they are scantly appropriate for encoding complex and nuanced human preferences. 

% LLM systems have opened a new door for new use cases and generated content. Along with these newfound capabilities, researchers have contributed a variety of ways for people to interact with these systems. Our review showed that many systems allowed users to interact in many different ways. Notably, works in HCI fields spearhead creative and multi-modal interactions between humans and AI systems. As mentioned, many earlier AI systems asked users to perform numeric inputs such rating and ranking AI responses. 


% Another set of systems took in implicit signals such as location, other applications in use, and discarded options. Systems also leverage natural language interaction, such as breaking AI output into digestible chunks for multi-turn dialogues with the users. Finally, people may also interact with AI models via graphical multi-modal methods. Works in this area include using a free-handed sketches~\cite{chung2022talebrush} or placing LLM agents in a contextual environment~\cite{park2023generative}. 

















% % 
% To provide a clearer understanding of the investigation of human values in these domains, we delve deeper into our methodology for developing the human value taxonomy in our proposed framework (as described in Section~\ref{sec:value_category}), and present our findings based on the final coding of all papers.


% \hua{
% % justify: 
% 1. why we focus on values? 
% % 2. why we use Schwartz Theory of Basic Values. 
% 3. what's the relationship of this typology with existing studies and how can future study use it?}
% Studies based on Schwartz Theory of Basic Values: \cite{kang2023values,kiesel2022identifying}





% While many papers claimed to integrate and/or evaluate AI with respect to human values, it is often the case that the sets of human values in the studies remained ambiguous or incomplete. 

% Our analysis of the final paper codes highlights the ambiguity and gaps in how the NLP/AI and HCI communities prioritize and conceptualize human values in \emph{bidirectional human-AI alignment} research. Specifically, w
% While many papers claim to examine LLMs in relation to human values, the specific set of values investigated often remains unclear. 
% Additionally, we observed differing emphases on human values when comparing papers published in NLP/AI venues with those in HCI venues.

% \begin{figure*}[!t]
%   \centering
%   \includegraphics[width=1\textwidth]{figures/values.pdf}
%   \caption{A fine-grained taxonomy of values related to bidirectional human-AI alignment. The taxonomy is based on Schwartz's Theory of Basic Values and an empirical collection of values that are commonly been studied.
%   % figure of our human value taxonomy based on Schwartz's Theory of Basic Values.\hua{adding explanation on meaning of red v.s. gray, add dashed lines of what values have been and have not been used in HCI + NLP?}
%   }
%   \label{fig:schwartz}
%   % \vspace{-2em}
% \end{figure*}




% \begin{figure*}[!t]
%   \centering
%   \includegraphics[width=1\textwidth]{figures/value_structure.pdf}
%   \caption{The relations of human values for AI development
%   % The structure of the dynamic relations among values 
%   (adapted from~\citet{schwartz2012overview}). 
%   We consider 5 \emph{high-order value types} (\ie self-enhancement and openness to change), which encompass 12 \emph{motivational value types} (\eg power, universalism, functionality). We further organize the relation among these value types along two dimensions: 1) different sources (\ie individuals, society and interaction) and 2) different self intentions (\ie self-protection against threat and self-expansion and growth). The \emph{Desired values for AI tools} was added empirically from \emph{bottom-up} our paper survey whereas others are inherited from~\citet{schwartz2012overview}. 
%     % 
%   % The typology is based on Schwartz Theory of Basic Values and an empirical collection of values that are commonly been studied.
%   % Some values conflict with one another (\eg Benevolence and Power) whereas others are compatible (\eg Conformity and Security). This structure of values refers to these relations of conflict and congruence among values~\cite{schwartz1994there,schwartz2012overview}.
%   % 
%   % A fine-grained taxonomy of values related to bidirectional human-AI alignment. The taxonomy is based on Schwartz's Theory of Basic Values and an empirical collection of values that are commonly been studied.
%   }
%   \label{fig:value_structure}
%   % \vspace{-2em}
% \end{figure*}





% \begin{figure*}[!t]
%   \centering
%   \includegraphics[width=1\textwidth]{figures/value_content.pdf}
%   \caption{A fine-grained taxonomy of human values. 
%   % The typology is based on Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012overview} and an empirical collection of values that are commonly been studied.
%   The exemplary values with red dot (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) indicates there are no work in our surveyed papers examining the specific values. 
%   Note that humans might not expect AI to encode all these values (\eg social power), which could potentially result in harm and risks. 
%   % The values with red dot (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) and \textcolor{hua-red}{red color} means that humans might not expect AI to embed these values in AI, which could potentially result in harm and risks.
%   % 
%   % 
%   % % 
%   % % 
%   % % 
%   % choose own goal\cite{lima2020collecting}
%   % creativity\cite{ashktorab2020human}
%   % curiosity\cite{jiang2023evaluating}
%   % freedom\cite{lima2020collecting}
%   % independence\cite{kang2023values}
%   % privacy\cite{10.1145/3544548.3580903}
%   % reflectiveness\cite{yan2023complex}
%   % factuality\cite{hosking2023human}
%   % self-respect\cite{wu2023cross}
%   % diversity\cite{kapania2023hunt}
%   % capability\cite{xu2023lemur}
%   % influence\cite{huang2023humanity}
%   % intelligence\cite{park2023generative}
%   % success\cite{kang2023values}
%   % resilience\cite{ye2023flask}
%   % authority\cite{lima2021human}
%   % wealth\cite{santurkar2023whose}
%   % reciprocation of favours\cite{zagalsky2021design}
%   % moderation\cite{lai2022human}
%   % devout\cite{santy2023nlpositionality}
%   % politeness\cite{zhu2023unmasking}
%   % self-discipline\cite{zhou2023realbehavior}
%   % forgiving\cite{wu2023cross}
%   % helpfulness\cite{jin2022make}
%   % honesty\cite{he2023hi}
%   % emotional\cite{huang2023humanity}
%   % responsiblity\cite{ma2023towards}
%   % true friendship\cite{isajanyan2024social}
%   % cooperation\cite{he2023interaction}
%   % collectivism\cite{nie2024moca}
%   % democracy\cite{santurkar2023whose}
%   % inclusive\cite{ramezani2023knowledge}
%   % equality\cite{sheng2021societal}
%   % equity\cite{goldfarb2023prompt}
%   % accessibility\cite{zhang2023visar}
%   % adaptability\cite{oh2023pk}
%   % economic\cite{bakker2022fine}
%   % transparency\cite{boyd2021datasheets}
%   % autonomy\cite{wang2023humanoid}
%   % awareness\cite{paleja2021utility}
%   % % 
%   % 
%   }
%   \label{fig:value_taxonomy}
%   % \vspace{-2em}
% \end{figure*}




% \subsubsection{The Process of Categorizing Aligned Human Values.}
% \label{sec:value_category_discuss}
% \mbox{}

% \martin{Please let me know if we need to discuss our consolidated synonyms in this section too, or we will make another figure in the appendix?}



% % \textbf{Defining Human Values: Top-Down and Bottom-Up}
% % \subsubsection{Structuring Human Values: Leveraging a Top-Down and Bottom-Up Method}
% \subsubsection{\textbf{Methodology: A Combination of Top-Down and Bottom-Up Way to Structure Human Values}}
% \label{sec:value_method}
% % \mbox{}
% To recognize human values systematically, we grounded our exploration on the Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012overview}, which is a theory of cross-cultural psychology built upon the \citet{rokeach1973nature}'s value survey. 
% We chose the Schwartz Theory of Basic Values primarily considering that its definitions and dimensions are universal and are applicable for, or almost for, all people across \emph{(a)} various cultures and countries; \emph{(b)} various sources including individuals, interactions and groups; and \emph{(c)} commonly accepted in previous NLP studies~\cite{kang2023values,kiesel2022identifying}.
% % 
% % 
% \citet{schwartz1994there} provided a clarified definition of human values by summarizing some widely agreed-upon features as:
% % 
% % \begin{quote}
%     \emph{\say{A value is a (1) belief (2) pertaining to desirable end states or modes of conduct, that (3) transcends specific situations, (4) guides selection or evaluation of behavior, people, and events.}}
% % \end{quote}
% % 
% Built upon these clarified definitions, we start to use a \emph{top-down} method to adopt the well-defined \emph{value taxonomy} and the \emph{structural relationship} presented by~\citet{schwartz1994there,schwartz2012overview}. As the conventional theory is missing the context of AI-system and human-AI interactions, we further supplement the \emph{value taxonomy} and the \emph{structural relationship}. Specifically, we used a \emph{bottom-up} way to extract all values studied in the literature and map them into the Schwartz Theory of Basic Values. Further, we added the missing values and relationship regarding the AI context to make our outcome more comprehensive.





% \subsubsection{\textbf{Outcome: The Relations of Human Values and Fine-grained Taxonomy}}
% \label{sec:value_outcome}
% % \mbox{}
% % 
% % Consequently, 
% We developed a more comprehensive structure of the dynamic relations of human values (Figure~\ref{fig:value_structure}) and their fine-grained taxonomy with mapped reference papers for exemplary values (Figure~\ref{fig:value_taxonomy}) after incorporating the AI-related context. 
% % 
% % 
% % 
% % 
% Considering the dynamic relations of human values in Figure~\ref{fig:value_structure}, we consider five \emph{high-order value types} (\ie self-enhancement, openness to change, conservation, self-transcendence and desired values for AI tools), which encompass 12 \emph{motivational value types} (\eg power, universalism, functionality). We further organize the relation among these value types along two dimensions: 1) different resources (\ie individuals, society and interaction) and 2) different self intentions (\ie self-protection against threat and self-expansion and growth). Note that the type of \emph{Desired Values of AI Tools} and its encompassed \emph{motivational values} (\ie functionality and human-likeness) are the supplemental value types we added from the empirical \emph{bottom-up} process introduced above.
% Also, it is worth noting that some values conflict with one another (\eg Benevolence and Power) whereas others are compatible (\eg Conformity and Security). This structure of values refers to these relations of conflict and congruence among values~\cite{schwartz1994there,schwartz2012overview}.
% % 
% % 
% % 
% % 
% % 
% Furthermore, we elaborate the definitions of the 12 motivational value types and their exemplary values with mapped paper reference in Figure~\ref{fig:value_taxonomy}. During the process of mapping existing literature to these values, we noted two findings: 1) value terms in empirical papers were often named differently (\eg capability and competence), or check their opposites (\eg fairness and bias), from the listed exemplary values of Schwartz's theory even they are examining the same thing essentially . 2) there are many values not studied in our collected literature (indicated as (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) in the Figure). 
% Also there are some  values that are included but humans might not expect AI to integrate (\eg power-seeking), we indicated it as (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) with \textcolor{hua-red}{red-color}. We consolidated them by using the synonyms. 
% 2) empirical paper often check if AI do not contain a negative value (\ie bias and sarcastically) whereas our exemplary values are mostly positive. We resolved the two above issues 


% while exemplary values in our taxonomy are mostly \emph{positive}, many papers are checking if AI manifests \emph{negative} values (\eg capability and competence)


% This taxonomy, however, need to be carefully extended to encompass AI and HCI contexts.
% Many objectives mentioned in the AI and HCI literature align with specific human values, although they often use different terminology. 
% For example, \textit{effectiveness} and \textit{efficiency} can be mapped to \textit{self-enhancement} $\rightarrow$ \textit{achievement} $\rightarrow$ \textit{capability}; and \textit{accountability} can be mapped to \textit{self-transcendence} $\rightarrow$ \textit{benevolence} $\rightarrow$ \textit{responsibility}; and 
% This indicates a need for bridging conceptual frameworks to ensure clarity and consistency in how values are integrated and addressed within these fields.
% Given the theory-guided taxonomy, we further ensure the comprehensiveness of human value coverage by conducting a \textit{bottom-up} search from all collected papers, and consolidated the wordings used to describe a particular human value.


% Based on the aforementioned process, we achieved our detailed human value taxonomy as described in Fig~\ref{fig:schwartz}. 





==> sections_ckpt_1120/background.tex <==

% 
% 

% %Tiffany's take on the first wave
% \tiffany{The concept of \emph{alignment} in AI research has a long history stemming from the first wave of AI agents, which were largely rule-based models {cite some stuff}. The late 1990s saw the emergence of intelligent agents in the abstract, i.e., future computer programs that can have the ability to operate autonomously and maintain flexibility to adapt to new contexts \cite{wooldridge1999intelligent}.} 
% 
% \hua{the four papers Frank suggested:\cite{edwards2001home,dautenhahn2000living,stuurman2001software,wooldridge1999intelligent}, we can refer to and add some descriptions.}
% 
% 
% \hua{In background, we describe a historical view of AI alignment, short-term and long-term of alignment, why alignment is important.}

% % \hua{Merrie suggested this paper~\cite{weidinger2023sociotechnical}.}







% \hua{shorter}
The concept of \emph{alignment} in AI research has a long history, tracing back to 1960, when AI pioneer Norbert Wiener~\cite{wiener1960some} described the AI alignment problem as: \say{\emph{If we use, to achieve our purposes, a mechanical agency with whose operation we cannot interfere effectively ... we had better be quite sure that the purpose put into the machine is the purpose which we really desire.}}
% 
Discussion around intelligent agents and the associated concerns relating to ethics and society have emerged since then~\cite{stuurman2001software}.
Next, we discuss the well-known challenges encountered in achieving alignment.
% 
% edwards2001home,dautenhahn2000living,
% which could be generally distinguished by \emph{near-term} and \emph{long-term} issues~\cite{prunkl2020beyond}.
% 




% \frank{From Frank -- adding the historical context of alignment topics back into 90s and early 2000s, adding some examples like his MIT experience or “paperclip maximizer”, then transit to today's alignment discussion in 2019 - .}







% ==== logics of writing background: 1) near-term issues (definition, challenges, ethics); 2) long-term issues (definition, challenges)



\noindent
% \textbf{Outer and Inner Alignment.}
\textbf{Challenge 1: Outer and Inner Alignment.}
% 
In the context of ``intelligent agents,'' until now, \emph{AI alignment} research has aimed to ensure that any AI systems that would be set free to make decisions on our behalf would act appropriately and reduce unintended consequences~\cite{wooldridge1999intelligent,stuurman2001software,russell2016artificial}.
At the \emph{near-term} stage, aligning AI involves two main challenges: carefully \emph{specifying}
% \footnote{A specification often refers to a set of documented requirements, and/or particular information within them, to be satisfied by a material, design, product, or service. A specification is often a type of technical standard~\cite{specification}.}
the purpose of the system (\emph{outer alignment} \ie providing well-specified rewards~\cite{ngo2022alignment}) and ensuring that the system adopts the specification robustly (\emph{inner alignment}, \ie ensuring that every action given an agent in a particular state learns desirable internally-represented goals~\cite{ngo2022alignment}).
% 
% 
Significant efforts have been made, for \emph{inner alignment}, to align AI systems to follow alignment goals of an individual or a group (\eg instructions, preferences, values, and/or ethical principles)~\cite{ouyang2022training} 
% kirchner2022researching,bai2022constitutional,bai2022training
and to evaluate the performance of alignment~\cite{santurkar2023whose}.
% 
However, for \emph{outer alignment}, AI designers are still facing difficulties in specifying the full range of desired and undesired alignment goals of humans. 
% To specify an AI system's purpose, 



\noindent
\textbf{Challenge 2: Specification Gaming.}
To learn human alignment goals,
AI designers typically provide an objective function, instructions, reward function, or feedback to the system, which is often unable to completely specify all important values and constraints that a human intended~\cite{hemphill2020human}.
% 
Hence, AI designers resort to easy-to-specify proxy goals such as \emph{maximizing the approval of human overseers}~\cite{wiki_AI_alignment}, which results in ``\emph{specification gaming}''~\cite{krakovna2020specification} or ``\emph{reward hacking}''~\cite{pan2022effects} issues (\ie AI systems can find loopholes that help them accomplish the specific objective efficiently but in unintended, possibly harmful ways).
%One typical example of \emph{specification gaming} shows that a simulated robot was trained to grab a ball by rewarding the robot for getting positive feedback from humans, but it learned to place its hand between the ball and camera, making it falsely appear successful~\cite{christiano2017deep}.\footnote{See the video at: \url{https://en.wikipedia.org/wiki/File:Robot_hand_trained_with_human_feedback_\%27pretends\%27_to_grasp_ball.ogg}} 
%Another classic (though extreme) example of an AI alignment problem is illustrated in the ``paperclip maximizer'' thought experiment:
%the scenario describes an advanced artificial intelligence tasked with manufacturing paperclips. If such a machine were not programmed to value human life, given enough power over its environment, it would try to turn all matter in the universe, including human beings, into paperclips or machines that manufacture further paperclips~\cite{bostrom2020ethical}.
% \footnote{
% % The ``paperclip maximizer'' thought experiment: 
% % A hypothetical AI, which is told to produce as many paperclips as possible, might do so through means that diverge from typical human task interpretations and value systems, such as killing all humans so that their atoms can be converted into additional paperclips.
% The scenario describes an advanced artificial intelligence tasked with manufacturing paperclips. If such a machine were not programmed to value human life, given enough power over its environment, it would try to turn all matter in the universe, including human beings, into paperclips or machines that manufacture further paperclips.
% }
% Add the paperclip example,
% 
% But designers are often unable to completely specify all important values and constraints, so they resort to easy-to-specify proxy goals such as maximizing the approval of human overseers, who are fallible. As a result, AI systems can find loopholes that help them accomplish the specified objective efficiently but in unintended, possibly harmful ways. This tendency is known as specification gaming or reward hacking. 
% As AI systems become more capable, they are often able to game their specifications more effectively.
% 
% 
% 
Additionally, the black-box nature of neural networks brings additional ethical and safety concerns for 
alignment because humans don't know about the inner state and the actions AI leveraged to achieve the output. Consequently, AI systems might make ``correct'' decisions with ``incorrect'' reasons, which are difficult to discern. Society is already facing these issues, 
such as data privacy~\cite{tucker2018privacy}, algorithmic bias~\cite{hajian2016algorithmic}, self-driving car accidents~\cite{bonnefon2016social}, and more.
% 
% 
As a result, these considerations necessitate considering human-AI interaction in AI alignment for specification and evaluation, ranging from addressing problems around who uses an AI system, with what goals to specify, and if the AI system perform its intended function from the user's perspective~\cite{weidinger2023sociotechnical}.





% === future issues;
% Scalable oversight
% Power-seeking and instrumental strategies
% An existential threat
% Dynamic nature of alignment


\noindent
\textbf{Challenge 3: Scalable Oversight.}
From a long-term perspective, when advanced AI systems become more complex and capable (\eg AGI \cite{morris2024levels}), 
it becomes increasingly difficult to align them to human values through human feedback. 
Evaluating complex AI behaviors applied to increasingly challenging tasks can be slow or infeasible for humans to ensure all sub-steps are aligned with their values \cite{terry2023ai}.
% \footnote{A typical example is the ``paperclip maximizer'', }.
Therefore, researchers have begun to investigate how to reduce the time and effort for human supervision, and how to assist human supervisors, referred to as \emph{Scalable Oversight}~\cite{amodei2016concrete}.
% 
% 

\noindent
\textbf{Challenge 4: Dynamic Nature.}
As AI systems become increasingly powerful, the alignment solutions must also adapt dynamically since human values and preferences change as well. 
As~\citet{dautenhahn2000living} posit, AI systems may be neither humane nor desirable if we do not ask questions about the long-term cognitive and social effects of social agent systems
% 
% if we do not ask questions about the long-term cognitive and social effects of social agent systems
(\eg \emph{how will agent technology affect human cognition}).
% , the developed AI systems may be neither humane nor desirable.
% 
% as an envolving process 
% As~\citet{irving2019ai} claimed, \say{\emph{if we want to train AI to do what humans want, we need to study humans}}, 
% 
% 
% 
All these considerations call for a long-term and dynamic perspective to address human-AI alignment as an ongoing, mutual process with the collective efforts of cross-domain expertise. 
% % 
% 
% Therefore, in this study, we conducted a systematic survey of over 400 cross-domain papers with a team of interdisciplinary researchers. We present a comprehensive human-centered view of \emph{bidirectional human-AI alignment} and provide our analysis and findings before discussing future directions to achieve this long-term alignment goal.




\noindent
\textbf{Challenge 5: Existential Risk.}
Further, some AI researchers claim that~\cite{bengio2024managing} advanced AI systems will begin to seek power over their environment (\eg humans) once deployed in real-world settings, as such behavior may not be noticed during training. For example, some language models seek power in text-based social environments by gaining money, resources, or social influence~\cite{pan2023rewards}. 
% 
%~\citet{russell2022artificial} imagined a robot tasked to fetch coffee and evade shutdown since ``you can't fetch the coffee if you're dead.''
Consequently, some hypothesize that future AI, if not properly aligned with human values,
could pose an \emph{existential risk} to humans~\cite{dafoe2016yes}.
% 
% 





\begin{table*}[!t]
  \centering
  % \includegraphics[width=1\textwidth]{figures/definitions.pdf}
  \includegraphics[width=1\textwidth]{figures/goals.pdf}
  \caption{The \textbf{Goals} of Alignment. We present the six prevailing alignment goals, associating with their Definitions (middle column), Limitations and Risks (right column). 
  We consider \textbf{Human Values} as the main goal of alignment in this work referring to an extensive analysis and arguments in existing studies~\cite{gabriel2020artificial,stuart2014whitepaper} 
  % We distill the definitions and limitations of the six prevailing alignment goals.
  % The goals along the ``Value'' direction are more normative, while goals along the ``Instruction'' direction are more empirical\cite{schleidgen2010mission}. 
  % Given an extensive analysis of limitations and tradeoffs, \citet{gabriel2020artificial} argues that ``\emph{human values}'' are currently the best possible goal for alignment.
  }
  % 
  % 
  % \diyi{There are also diverse factors that we might want to consider for "alignment" beyond "values". for instance, norms and cultures. maybe you will clarify this in the later section!}
  \label{fig:definitions}
  \vspace{-22pt}
\end{table*}






















% ============================================= dead kitten ================================================



% bratman1987intention
% The Belief-Desire-Intention (BDI) agent model is a framework for developing intelligent agents that simulate human-like reasoning and decision-making processes. It is based on Michael Bratman's philosophical theory of practical reasoning, which involves three key attitudes: beliefs, desires, and intentions.


% An typical example is the ``paperclip maximizer'' example 
% Dynamic nature of alignment


% === current issues;
% Specification gaming and side effects.
% Learning human values and preferences
% Inverse Reinforcement Learning;




% Power-seeking and instrumental strategies
% An existential threat





% % === future issues;

% Scalable oversight

% Power-seeking and instrumental strategies

% An existential threat

% Dynamic nature of alignment

% https://www.lesswrong.com/tag/squiggle-maximizer-formerly-paperclip-maximizer
% 

% ================================================


% , which involves bidirectional process to encompassing 


% an interdisciplinary and human-centered perspective to develop AI alignment research. 




% Therefore, a more comprehensive and bidirectional approach to human-AI alignment, encompassing the co-adaptation and mutual shaping of both humans and AI systems, is necessary to fully realize the potential symbiosis between these entities.
% % 
% % 
% In this work, we take the comprehensive and bidirectional approach into considering human-AI alignment from a long-term and dynamic perspective.
% % 
% % 
% % 
% % 
% Bridging these divides through interdisciplinary collaboration is crucial for advancing this complex and multifaceted challenge.



% ================================================



% % Despite the increasing prominence of the \say{human-AI alignment} concept in various domains, there remains \textbf{a lack of clear and consistent definitions} regarding its core terminologies. Fundamental questions, such as ``\aligncode{\emph{what is human-AI alignment?}}'', ``\aicode{\emph{what to be aligned?}}'', and ``\humancode{\emph{align with whom?}}'', 
% % % what precisely is meant by human-AI alignment?", "what aspects should be aligned?", and "who or what entities should the alignment be calibrated to?",
% % often lack satisfactory answers. 
% % % 
% % 


% % In terms of ``\emph{\aligncode{what is human-AI alignment?}}'', 
% % alignment has been referred to as \emph{intention alignment}~\cite{anwar2024foundational}, \emph{behavior alignment}~\cite{park2023generative,xie2024can}, \emph{instruction alignment}~\cite{bai2022constitutional,liu2023makes}, \emph{value alignment}~\cite{sorensen2024roadmap,gabriel2020artificial}, etc. 
% % % 
% % % 
% % % There are also diverse factors that we might want to consider for "alignment" beyond "values". for instance, norms and cultures. 
% % % maybe you will clarify this in the later section! 

% % % intent alignment description;
% % \citet{ouyang2022training} and \citet{anwar2024foundational} consider alignment from the perspective of 
% % AI safety~\cite{anwar2024foundational,wang2023aligning}, where it refers alignment to be \emph{intent alignment} by fine-tuning with human feedback. 
% % % 
% % Their goal of alignment is to assure safety (\ie unlikely to contribute to unplanned, undesirable harms) when the systems are deployed and used~\cite{weidinger2023sociotechnical}. 
% % % 
% % % 
% % % 
% % % 
% % % behavior alignment description;
% % \citet{park2023generative} introduces generative agents that draw on generative models to simulate and align with believable individual and emergent group behavior, in which the computational agents can wake up, cook breakfast, form opinions and initiate conversations, etc.
% % % 
% % % 
% % % 
% % % instruction alignment description;
% % % 
% % ~\citet{bai2022constitutional} form the human supervision as a set of principle instructions that should govern AI behavior, along with a small number of examples as few-shot prompting to instruct models.
% % % 
% % % value alignment description;
% % \citet{gabriel2020artificial} considers AI could be designed to align with the values of system users, where the \emph{values} are defined as ``natural or non-natural facts about what is good or bad, and about what kinds of things ought to be promoted, as specified by the individual or society.''
% % A line of studies examine AI alignment with respect to individual and social values~\cite{tay2020would,hendrycks2020aligning,hovy-yang-2021-importance}. Despite the plethora of alignment definitions and studies, yet, the difference and relationship between these alignment goals are vague and less investigated.
% % % 
% % % 



% % Regarding ``\emph{\aicode{what to be aligned?}}'',
% % % 
% % existing studies have examined how to align AI's \emph{intermediate representations} with humans'~\cite{liu2023learning}, align AI's \emph{internal reasoning process} to be similar with a human's cognitive process~\cite{mcgrath2023can}, and align AI's \emph{outputs and/or generations with human preferences}~\cite{corvelo2024human,ouyang2022training}.
% % % 
% % % 
% % For example, \citet{liu2023learning} examines the alignment between models' representations and human-compatible decision-focused representations by identifying the nearest neighbors retrieved from dataset.
% % \citet{mcgrath2023can} compares the interpretations of AI models with human cognitive theories formulated by studying human behaviors.
% % \citet{santurkar2023whose} compares LLM-generated opinions with human responses from various U.S. demographic groups' opinion polls to evaluate their alignment.






% % % 
% % % 
% % Considering ``\emph{\humancode{align with whom?}}'' Pertinent stakeholders within the AI landscape can be the potential objects for AI to align with, including lay people (\eg end users of AI systems), AI practitioners (\eg developers, researchers)~\cite{boggust2022shared}, organizational entities (\eg technology firms, professional communities), and national/international bodies (\eg governments, legislative bodies)~\cite{deshpande2022responsible}.
% % % 
% % For instance, \citet{anwar2024foundational} defines an AI systems as `aligned' when it is trying to behave as intended by the LLM developer~\cite{ngo2022alignment}, whereas \citet{qi2023fine} conducts red-teaming studies to investigate the safety risks of LLMs to end-users.
% % % 
% % There are also studies discussing general humans without specifying human groups~\cite{yao2023instructions}.
% % % 
% % % 
% %
% % 
% % 
% % For instance, AI alignment commonly addresses the overarching challenge of ensuring that AI systems achieve intended outcomes as defined by their developers and/or users, while minimizing undesirable side effects such as negative impacts on individuals, groups, or society at large~\cite{matthews2022alignment,gabriel2020artificial,kenton2021alignment}. 
% % In contrast, a line of studies focuses on human-AI alignment through the lenses of safety and ethics, stressing the importance of AI generating benign content that aligns with human values~\cite{yao2023instructions, ganguli2022red,bai2022constitutional}. Furthermore, certain studies delve into the role of interaction in human-AI alignment, delineating AI alignment process into three objectives, including specification alignment, process alignment, and evaluation support~\cite{terry2023ai}.
% % 
% % 
% % 
% % % 
% % % 
% % Overall, this absence of terminological and conceptual clarity hinders progress and can lead to misalignment between different stakeholders' perspectives and goals.
% % % 
% % Given these observations, we focuses on clarifying the definitions of core questions in the realm of this study to pave the way for future work.










% Additionally, the current \textbf{scope of human-AI alignment research appears narrow and vague}. Discussions frequently revolve around developing better AI systems to align with human values, ethics, and preferences. However, this unidirectional view neglects the potential for AI to positively influence and reshape human behaviors, cognition, and decision-making processes. 
% % 
% % 
% For example, \citet{wang2023aligning} conducts an extensive survey study to review various technologies to align LLMs with human expectations. 
% While most alignment research concentrates on integrating human feedback into developing AI, 
% \citet{terry2023ai} recently proposed considering AI alignment in the context of designing and evaluating interfaces for AI systems, which can support end-users ib interactively aligning an AI to their goals.
% % , during inference stage, as human better interact with LLMs.
% % 
% % 
% In summary, \citet{anwar2024foundational} emphasizes the importance of assuring the LLMs' safety and alignment by considering studies about 
% % in which they define the studies to achieve assurance should include 
% ``\emph{any way of providing evidence that a system is safe or aligned, including but not limited to: scientific understanding of system, behavioral evaluations, explanations of the model behavior or internal processing, and adherence to responsible development practices by the system develop}~\cite{casper2024black}''.
% % 
% % 
% Therefore, a more comprehensive and bidirectional approach to human-AI alignment, encompassing the co-adaptation and mutual shaping of both humans and AI systems, is necessary to fully realize the potential symbiosis between these entities.
% % 
% % 
% In this work, we take the comprehensive and bidirectional approach into considering human-AI alignment from a human-centered perspective~\cite{terry2023ai}.
% % 



% Furthermore, the \textbf{field of human-AI alignment suffers from gaps and siloed efforts among relevant research communities}, such as Human-Computer Interaction (HCI), which commonly examines the human behaviors and demands in practice~\cite{buccinca2021trust,holstein2019improving,wang2019designing}, and Natural Language Processing (NLP) and Artificial Intelligence (AI) that often investigates the state-of-the-art AI and LLM technologies~\cite{ouyang2022training,rafailov2024direct,bai2022training}. While HCI researchers focus on designing intuitive and effective human-AI interfaces, NLP researchers concentrate on developing language models that can comprehend and generate human-like text. However, the insights and contributions from these two fields are often not effectively integrated, leading to missed opportunities for synergistic progress towards achieving true human-AI alignment. 
% Bridging these divides through interdisciplinary collaboration is crucial for advancing this complex and multifaceted challenge.







% % ================ redundant ================
% % Inspired by the observations from existing studies on human-AI alignment, our goal is to offer precise definitions and scope (Section~\ref{sec:method}), delineate the taxonomy of research scope for human-AI alignment (Section~\ref{sec:framework}), and pinpoint gaps and synergistic pathways for both NLP and HCI communities to advance toward achieving human-AI alignment (Section~\ref{sec:analysis} and Section~\ref{sec:discussion}).




% - 1) To what extent are human values well-aligned with developed AI?

% - 2) are interaction paradigms fully leveraged in human-AI alignment techniques?

% - 3) situated values and customized AI alignment?

% - 4) what are under-explored research dimensions? heatmaps

% \hua{in this paper, we review from a human-centered perspective for both directions.}






% \textbf{Vague scope of alignment.}
% %%%% 2. narrowed scope of alignment; 
% \hua{propose bidirectional human-AI alignment.}



% \textbf{Unclear gaps between research communities.}
%%% 3. gaps between domains; what're missing and what should be done in the future.


% synergistic effort in achieving human-AI alignment.



% Motivated by these observations in the related studies around human-AI alignments, we aim to provide clarified definitions, a elaborated research scope of human-AI alignment, and identify the gaps and synergistic directions for both NLP and HCI communities to achieve human-AI alignment.
% 
% 




% =============================================
% 
% \textbf{A lack of definitions.}
% %%%% 1. lack of definitions
% The newly realized capabilities of modern-day, general-purpose AI have heightened the relevance of existing discussion on \emph{Human-AI Alignment}\ct. 
% However, there is a lack of clarified definitions around ``\emph{what is human-AI alignment?}'', ``\emph{what to be aligned?}'', and ``\emph{align with whom?}''.
% 
% 
% what is human-AI alignment?
% 


% % 
% A number of studies consider alignment from the perspectives of AI safety~\cite{anwar2024foundational,wang2023aligning}\ct. For example, \citet{anwar2024foundational} uses alignment to refer to \emph{intent alignment}, which defines an AI systems as `aligned' when it is trying to behave as intended by the LLM developer~\cite{ngo2022alignment}. Their goal of alignment is to assure safety (\ie unlikely to contribute to unplanned, undesirable harms) when the systems are deployed and used~\cite{weidinger2023sociotechnical}. 
% % 



% Other studies focus on \emph{value alignment}\ct. For instance, ~\citet{gabriel2020artificial} considers AI could be designed to align with the values of system users, where the \emph{values} are defined as ``natural or non-natural facts about what is good or bad, and about what kinds of things ought to be promoted, as specified by the individual or society.''




% \citet{terry2023ai} 


% we review from a human-centered perspective for both directions








% A number of studies consider alignment from the perspectives of AI safety~\cite{anwar2024foundational,wang2023aligning}\ct. For example, \citet{anwar2024foundational} uses alignment to refer to \emph{intent alignment}, which defines an AI systems as `aligned' when it is trying to behave as intended by the LLM developer~\cite{ngo2022alignment}. Their goal of alignment is to assure safety (\ie unlikely to contribute to unplanned, undesirable harms) when the systems are deployed and used~\cite{weidinger2023sociotechnical}. 
% 
% 
% 
% Other studies focus on \emph{value alignment}\ct. For instance, ~\citet{gabriel2020artificial} considers AI could be designed to align with the values of system users, where the \emph{values} are defined as ``natural or non-natural facts about what is good or bad, and about what kinds of things ought to be promoted, as specified by the individual or society.''



==> sections_ckpt_1120/conclusion.tex <==

One limitation of this work is the scope of the sampled and filtered papers. The rapidly growing literature on human-AI alignment spans diverse venues across many domains. Instead of an exhaustive collection, we focused on developing a holistic bidirectional human-AI alignment framework using essential research questions, dimensions, and codes. 
% 
Our surveyed papers and team members primarily focus on computing-related fields like ML, NLP, and HCI, though alignment research also involves disciplines like cognitive science, psychology, and STS (Science, Technology, and Society). Our framework can naturally extend to these areas as needed.
% 
% 
Despite these limitations, we believe our bidirectional human-AI alignment framework serves as a foundational reference for future researchers.





% 
% 
% 
% 





% One limitation of this work is the coverage of the sampled and filtered papers.  
% The literature revolving around the topic of human-AI alignment is increasing rapidly, scattering in diverse venues across many domains. 
% % 
% % 
% Therefore, instead of striving for an exhaustive collection of papers, this work focused on developing a holistic loop of bidirectional human-AI alignment framework by using essential research questions, dimensions and codes. 
% % 
% % 
% % 
% Additionally, we are aware that our surveyed papers and the position of our team members primarily focus on computing-related domains, such as ML, NLP, and HCI. There are additional disciplines involved in alignment research, such as cognitive science, psychology, and STS (Science, Technology, and Society).
% However, our framework can naturally extend to these domains by incorporating them into the appropriate directions.
% % 
% Despite these limitations, we argue that this bidirectional human-AI alignment framework serves as foundational reference forfuture researchers examining existing literature that lies in the holistic loop of the alignment process, while preventing implicit assumptions or overlooked considerations, thereby facilitating a holistic understanding of the dimensions and factors that drive the developing of AI technology and human impacts.
% For future work, we plan to continue to refine our dimensions and codes to incorporate future literature relevant to the bidirectional human-AI alignment process.












% \noindent
% \textbf{Conclusion.}
In conclusion, this study clarifies the definitions and scope of core terminologies of human-AI alignment and conducts a systematic review of over 400 related papers spanning diverse domains such as NLP, AI, HCI, and social science. Additionally, we introduce a novel conceptual framework of ``Bidirectional Human-AI Alignment'', structuring the surveyed literature taxonomies into ``aligning AI to humans'' and ``aligning humans to AI'' with detailed categories and example papers. Furthermore, we identify limitations and risks in this area quantitatively and qualitatively, analyzing a fine-grained human value taxonomy, interaction modes for alignment, and discrepancies between AI and human evaluation. To pave the way for future studies, we discuss five stages to achieve the alignment goals from near-term to long-term perspectives and identify new possibilities to highlight future directions and opportunities in research.




==> sections_ckpt_1120/discussion.tex <==





% 
% To illustrate this approach, 
%  we present an imaginary use case demonstrating how researchers can use the resources provided in this paper to consider bidirectional human-AI alignment research from a holistic perspective (Section~\ref{sec:use_case}).
% % 




% Drawing insights from the framework development and associated coding analysis, 
% 
% 
% we discuss potential avenues for future research in both the ``\emph{aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}}'' (Section~\ref{sec:future_human2ai}) and ``\emph{aligning \textcolor{hua-blue}{AI}} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}'' (Section~\ref{sec:future_ai2human}) directions.
% 
% we discuss potential actions for future research to take to achieve this long-term alignment goal in both the ``\emph{aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}}'' (Section~\ref{sec:future_human2ai}) and ``\emph{aligning \textcolor{hua-blue}{AI}} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}'' (Section~\ref{sec:future_ai2human}) directions.







% \subsection{Considering Bidirectional Human-AI Alignment as a Holistic Loop: A Use Case}
% \label{sec:use_case}



% Concretely, suppose a research group \gr aims to develop an AI system that will be aligned with a specific marginalized group \gm. However, given the existing general AI systems that could not align with this specific group \gm, it is unclear \emph{how to improve the system and ensure that the developed system will positively impact the group \gm}.
% % whether the research group \gr possessed AI system is already aligned with marginalized group \gm and how to improve it. 
% To achieve this research goal, we next showcase how to potentially use our \emph{bidirectional human-AI alignment} framework to resolve the problem as a holistic loop.
% % 
% % 
% We divide the holistic process into four steps and describe them correspondingly in the four subsections below.



% % ==== 1. identify values; 2. represent values;
% \subsubsection{Identifying and Representing Values of Group \gm}
% % \mbox{}

% % Firstly, \textbf{identifying and represent values} of group \gm. 
% The first step researchers \gr need to do is to identify the value priority of group \gm and represent the values in a format that can be used by AI.
% % 
% % Referring to Section~\ref{sec:ai2human1} and Section~\ref{sec:gap_value}, t
% To identify the set of values group \gm might prioritize, the framework provides two potential ways of identifying the specific values. One, based on the category listed in Section~\ref{sec:ai2human1} and \ref{sec:gap_value}, researchers \gr can identify the set of value classes the group \gm may prioritize, and search for published datasets or benchmarks that can represent these values (Benchmark dataset examples include ETHICS~\cite{hendrycks2020aligning}, SOCKET~\cite{choi2023llms}, etc.). Besides, the researchers \gr can also design surveys and recruit real humans from group \gm, referring to Section~\ref{sec:human2ai4}, to identify their value priority and represent these values in AI model usable formats, such as rating and natural language description, based on Section~\ref{sec:ai2human2} (See OpinionQA~\cite{santurkar2023whose} example for collecting survey dataset).
% % 
% % 

% % Next, to represent human values in the way that can be used by AI, referring to Section~\ref{sec:ai2human2}, the framework



% % ==== 3. finetunine models; evaluate models and find under-performance;
% \subsubsection{Finetuning and Evaluation AI to Integrate Identified Values}
% % Secondly, \textbf{fine-tuning and evaluating AI model to integrate values} of group \gm.
% Given the represented human values in datasets, referring to Section~\ref{sec:ai2human2}, researchers \gr can further finetuning the AI model to integrate these representative values. Particularly, the framework is providing typical methods of aligning AI with these values, including Supervised Fine Tuning (\eg \cite{zhou2024lima} ) and Reinforcement Learning with Human Feedback (\eg DPO~\cite{rafailov2024direct}, RLHF~\cite{ouyang2022training}). Thereafter, researchers \gr need to evaluate these aligned AI models using the collected value datasets to ensure the effectiveness of alignment.







% % \subsubsection{Helping Group \gm Understand AI by Explaining AI}
% % % Thirdly, \textbf{helping group \gm understanding AI by explaining AI}. 
% % If the group \gm could not completely understand AI, we can also refer to Section~\ref{sec:human2ai3} for developing human-centered AI explanations for them.







% % ==== 4. assess AI impacts on margialized group;
% \subsubsection{Understanding and Assessing AI Impacts on Group \gm}
% % Fourthly, \textbf{assessing AI impacts} on the group \gm.
% If the group \gm could not completely understand AI, we can also refer to Section~\ref{sec:human2ai3} for developing human-centered AI explanations for them.
% Furthermore, to assess the usability and impacts of developed AI system on group \gm, researchers \gr can refer to Section~\ref{sec:human2ai3} for developing human-AI collaborative tasks to empower group \gm to use and perceive AI systems (\eg human-AI co-writing tasks~\cite{shen2023convxai,lee2022coauthor,petridis2023anglekindling}, story generation tasks~\cite{chung2022talebrush,zhang2022storybuddy}, collaborative decision making~\cite{bansal2021does,10.1145/3397481.3450650}, etc.). 
% Next, researchers \gr can assess the practical impacts on group \gm, referring to Section~\ref{sec:human2ai4} in terms of various aspects relevant to value perceptions and reactions, such as decision making fairness and equity, generation creativity, misinformation and privacy, etc. 





% % ==== 5. quantify their values and customize AI systems during inference stage.
% \subsubsection{Representing Revised Values and Customize AI During Model Inference}
% % 
% After acquiring the practical values revised with the interaction between AI and group \gm, referring to Section~\ref{sec:human2ai3} and \ref{sec:ai2human2}, the researchers \gr can customize AI values during inference stage in practical human-AI collaboration tasks to fulfill alignment. 
% % 
% For example, both ConstitutionMaker \cite{petridis2024constitutionmaker} and ConstitutionalExperts~\cite{petridis2024constitutionalexperts} help users steer LLMs by helping them write better prompts.
% ConstitutionMaker enables \textit{interactive} prompt optimization, where users can provide natural language feedback on the model's output, and the system converts this feedback into principles (i.e. rules) that are inserted into the model's prompt ~\cite{petridis2024constitutionmaker}.
% Meanwhile, ConstitutionalExperts automatically optimizes a discrete prompt; users can provide a small labeled dataset with which the system uses to ``train'' a prompt by iteratively adding and refining principles within the prompt \cite{petridis2024constitutionalexperts}.
% Thus, if unsatisfied with the model's outputs, users can employ these interactive or automatic techniques to better infuse their feedback and values into the prompt at inference.












% The two directions of human-AI alignment are not independent; instead, they represent an \emph{ongoing, mutual process} to achieve a \emph{dynamic alignment goal over the long term}. Future research should approach alignment studies as a bidirectional process to fully explore the breadth of the research space and achieve this essential goal. 
% 
Drawing upon insights gained from the development of our framework and the associated coding analysis, as shown in Figure~\ref{fig:future_work}, we propose future research aiming to achieve the long-term alignment goal by identifying three important challenges from near-term to long-term objectives, including the Specification Game (Section~\ref{sec:challenge1}), Dynamic Co-evolution of Alignment (Section~\ref{sec:challenge2}), and Safeguarding Coadaptation (Section~\ref{sec:challenge3}).
% 
% 
% Particularly, we discuss research questions and motivations followed by ideas for solution exploration from both directions of ``\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em} Align \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Human}'' (\ie domains related to AI algorithm and method development, including Machine Learning, Artificial Intelligence, Data Science, and others)  and ``\hspace*{.0em}\numimg{figures/B.pdf}\hspace*{-.1em} Align \textcolor{hua-red}{Human} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}'' (\ie domains conducting studies related to humans and society, including Human-Computer Interaction, Social Science, Cognitive Science and others) for each challenge below.







\subsection{Specification Game}
\label{sec:challenge1}

An important near-term challenge is resolving the ``Specification Game'', which involves precisely defining and implementing AI goals and behaviors to align with human intentions and values. Next, we will introduce how synergistic efforts from two directions can potentially address this challenge.

% Current AI development primarily aims to achieve alignment by training models using human instructions, examples, ratings, rankings and others. The goal is for AI systems to infer alignment goals (\eg human values and intentions) in a data-driven manner.
% % 
% However, designers often struggle to fully specify all important values and constraints, and they may not be able to explain or control what the AI has learned from the data. 
% % 
% Instead of resorting to easy-to-specify but fallible proxy goals (\eg maximizing the approval of human overseers),
% future studies should consider more explainable and controllable methods for humans to specify alignment goals for AI interactively. 
% % 
% Next, we discuss how research in these two areas can synergize to potentially achieve this goal.


% \subsubsection{\textbf{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Adapt AI to the full range of human values interactively during learning and deployment stages}}


% \subsubsection{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Adapt AI to fully specified important human values interactively during learning and deployment stages}
% \subsubsection{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Adapt AI to nuanced and contextualized human values interactively during learning and deployment stages}







\begin{figure*}[!t]
  \centering
  \includegraphics[width=1\textwidth]{figures/future_work.pdf}
  \caption{We envision future research directions to achieve long-term human-AI alignment with both efforts from the ``Align \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}'' (AI-centered research) and ``Align \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}'' (Human-centered research) directions. 
  We elaborate the three important future challenges, including Specification Game (Section~\ref{sec:challenge1}), Dynamic Co-evolution of Alignment (Section~\ref{sec:challenge2}), and Safeguarding Coadaptation (Section~\ref{sec:challenge3}).
  }
  \label{fig:future_work}
  % \vspace{-2em}
\end{figure*}


\subsubsection{\textbf{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Integrate fully specified human values into aligning AI}}
% \mbox{}


% \textbf{Identify appropriate values and priorities.}
% \textbf{Identify appropriate values and agreements for AI alignment.}
% \emph{Research Problem and Motivation.}
\noindent Individuals often possess value systems that encompass multiple values with varying priorities, rather than a single value, to guide their behaviors~\cite{schwartz1994there,schwartz2012overview}.
% For example, people may prioritize the value of \emph{family} and \emph{work} differently, leading to varied choices in time allocation. 
% 
% 
% 
Also, these priorities can change dynamically throughout an individual's life stages.
As such, 
% it is unlikely to that we can achieve a universal value system, recognized by all humans, to govern AI alignment. Instead, 
It is more realistic to select values compatible with specific societies or situations, given the fact that we live in a diverse world~\cite{gabriel2020artificial}.
% 
Future research, inspired by Social Choice Theory~\cite{arrow2012social}, could focus on using democratic processes to aggregate individual values into collective agreements. Building on the summaries in Sections ~\ref{sec:ai2human1} and ~\ref{sec:gap_value}, researchers can employ democratic methods to identify diverse subsets of human values for AI alignment. 
Additionally, creating datasets that represent these values is crucial. 
% 
% 
% 
% 
Besides, it is crucial yet challenging \emph{for AI designers to investigate how to fully specify the appropriate values 
% develop methods for selecting appropriate value systems 
and to further integrate these values into AI alignment}.
% 
% 
% 
Future important area involves developing algorithms, such as the Bradley-Terry Model~\cite{rafailov2024direct} or Elo Rating System~\cite{bai2022constitutional}, to convert heterogeneous human values into AI-compatible formats for training reward models and guiding reinforcement learning. Researchers should also explore AI models capable of aligning with unstructured human data, including free-form descriptions of values, multimedia, or sensor recordings depicting human behavior.





% \textbf{Recommendations for Future Work.} 
% Future work can draw from political theory, which examines fair methods for determining the principles that state institutes should follow, as a potential guide for selecting human values for AI alignment. Inspired by Social Choice Theory~\cite{arrow2012social}, one future direction involves aggregating individual values into collective value agreements or judgments through democratic processes such as voting, discussion, and civic engagement~\cite{gabriel2020artificial}.
% Therefore, building on the summary of human values in Section~\ref{sec:ai2human1} and \ref{sec:gap_value}, future researchers can use democratic methods to identify a wide spectrum of human value subsets for AI alignment.
% % 
% % 
% Additionally, an important focus for future work lies in the curation of datasets that can represent these wide-spectrum human values, particularly in rich formats that go beyond simple ratings and rankings, which are commonly used in current alignment algorithms (\eg RLHF~\cite{ouyang2022training}, RLAIF~\cite{bai2022constitutional}).
% Another key research area to explore is around algorithms or methods (\eg Bradley–Terry Model~\cite{rafailov2024direct} or Elo Rating System~\cite{bai2022constitutional}), potentially drawing from economic theories, to convert heterogeneous human value data (\eg principles or contextual information) into AI-compatible formats (\eg scalars) for training reward models and guiding reinforcement learning. Also, future research can explore AI models that can act directly on aligning humans' unstructured data, such as free-form descriptions of values, multimedia or sensor recordings depicting how people act in various situations, among others.
% 
% 
% 
% Future work can draw from political theory as a potential guide for selecting human values for AI alignment. 
% Future research, inspired by Social Choice Theory~\cite{arrow2012social}, could focus on using democratic processes to aggregate individual values into collective agreements. Building on the summaries in Sections ~\ref{sec:ai2human1} and ~\ref{sec:gap_value}, researchers can employ democratic methods to identify diverse subsets of human values for AI alignment. 
% Additionally, creating datasets that represent these values is crucial. 
% Another important area involves developing algorithms, such as the Bradley-Terry Model~\cite{rafailov2024direct} or Elo Rating System~\cite{bai2022constitutional}, to convert heterogeneous human values into AI-compatible formats for training reward models and guiding reinforcement learning. Researchers should also explore AI models capable of aligning with unstructured human data, including free-form descriptions of values, multimedia, or sensor recordings depicting human behavior.
% 
% 
% 




% \subsubsection{\textbf{Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}: Specify the nuanced and contextualized human values in AI data formats interactively}}
\subsubsection{\textbf{Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}: Elicit nuanced and contextual human values during diverse interactions}}
% \mbox{}


\noindent Current alignment methods use instructions, ratings, and rankings to infer human values, which can not fully capture all relevant human values and constraints. 
% 
Future research should focus on optimizing interactive interfaces to efficiently elicit human values. These interfaces can leverage diverse interaction modes to capture comprehensive human value information. 
% 
% 
Additionally, people often struggle to formulate optimal prompts for AI, accurately specify their requirements, and articulate their desired values, which can change based on context and time. 
Developing proactive interfaces that use conversational techniques to elicit nuanced and evolving values is also crucial. 
% 
% 
Implicit human signals that indicate values are also frequently overlooked.
Additionally, systems that track interactions to hypothesize and validate implicit human values in real-time should be designed.


% 
% 
% 

% \noindent Current alignment methods primarily capture human values using instructions, ratings and rankings, aiming to infer humans' alignment goals (\eg human values and intentions) in a data-driven manner.
% % 
% % aiming for AI systems to infer alignment goals (\eg human values and intentions) in a data-driven manner. 
% % 
% However, these limited data formats and interaction methods fall well short of fully specifying all of the relevant human values and constraints. 
% % Besides, when humans are learning to collaborate or utilize AI, it is often challenging for humans to write the optimal prompts that can accurately and efficiently specify what they demand in practice. 
% Besides, when humans seek to collaborate with or utilize AI, they often encounter challenges in formulating optimal prompts, which require them to accurately and efficiently specify their requirements or expectations, in order to be able to use AI generated output or decision making in practice.
% % For instance, in spatial reasoning tasks, specifying geographical routes can be more accurately and comprehensively achieved if humans draw sketches interactively, rather than through ratings and rankings.
% % 
% % 
% Additionally, people often struggle to articulate all of their desired values accurately and comprehensively, especially as these values can dynamically change based on contextual and temporal situations. 
% % 
% Relatedly, practices often overlook implicit human interactive signals that can also indicate values relevant to AI alignment.
% % Therefore, it is essential for HCI researchers to develop diverse interactive strategies where AI systems can proactively engage with users to elicit nuanced, contextualized, and evolving information about their values.



% \textbf{Recommendations for Future Work.} One promising area for future research is optimizing interactive interfaces to elicit human values efficiently and effectively. These interfaces can leverage diverse interaction modes (see an initial summary in Figure~\ref{fig:interaction}) to fully capture human value information. For example, to identify a set of important principles for AI alignment, the interface can use the user's conversational natural language specifications and generate a list of principle options for users to select from and/or revise.
% % 
% % 
% Recognizing that humans cannot always comprehensively articulate their values, another key research area is to develop interfaces that proactively interact with users. This could involve conversational techniques or scaffolding procedures to elicit nuanced, contextualized, and evolving information about an individual's values.
% % 
% % 
% Additionally, to capture implicit human interaction signals that reflect human values for AI alignment, another area of future work involves designing systems that track interactions to develop real-time hypotheses about human values on these implicit signals, and then proactively validate them with humans as needed.











\subsection{Dynamic Co-evolution of Alignment}
\label{sec:challenge2}

\noindent
The challenge ahead lies in comprehending and effectively navigating the dynamic interplay among human values, societal evolution, and the progression of AI technologies.
Future studies in these directions aim to bolster a synergistic co-evolution between AI and human societies, adapting both to each other's changes and advancements.


% \subsubsection{\textbf{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Co-evolve AI with changes in humans and societal values, cognition, and needs}}
\subsubsection{\textbf{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Co-evolve AI with changes in humans and society}}
% \mbox{}


\emph{(i)}
Existing literature often treats AI alignment as static, ignoring its dynamic nature. A long-term perspective must consider the co-evolution of AI, humans, and society. As AI systems evolve and scale up, they gain new capabilities, making it essential to ensure their goals remain aligned with human values. Thus, alignment solutions require continuous oversight and updates.
% 
% 
% 
Future research should develop methods for continuously updating AI with limited data without compromising alignment values and performance. 
% In real-world scenarios, fine-tuning deployed AI systems is often impractical. Thus, adapting AI during deployment without fine-tuning is crucial. 
This could involve forecasting human value evolution and preparing AI with flexible strategies like prompting or interventions.
% 
% 
% Updating AI to continuously adapt to the dynamic changes of humans and society requires adjustments in alignment data, models, and evaluation processes spanning both learning and deployment stages. 
% % 
% Referring to the methodologies listed in Section~\ref{sec:ai2human2}, current strategies often rely on fine-tuning to update AI with a curated human value dataset during the learning process. However, this approach may lead to AI models forgetting or diminishing previous alignment goals. In situations where sufficient data for fine-tuning is unavailable, these methods becomes more challenging.
% % 
% Therefore, a crucial area for future research is to develop approaches for continually updating AI systems using limited data without compromising existing alignment values and performance. 
% 
% 
% 
% 
\emph{(ii)}
Additionally, AI advancements also influence human actions and values, necessitating adaptive alignment solutions. Ensuring AI co-evolves with human and societal changes is crucial for robust alignment.
% 
This challenge could potentially be addressed by forecasting the potential evolution trajectories of human values or behavioral patterns, and preparing AI with the flexibility to adapt in advance, for example, through prompting or intervention strategies.
% 
% 
% 
% In summary, co-evolving AI with dynamic human and societal changes requires collaboration among experts in various domains such as machine learning and social sciences.





% 
% % 
% % 
% In real-world scenarios, it is common for AI systems to already be deployed at scale, making fine-tuning a challenging or impractical practice. 
% Therefore, another important research direction involves adapting AI, during the deployment stage, without relying on fine-tuning. This challenge could potentially be addressed by forecasting the potential evolution trajectories of human values or behavioral patterns, and preparing AI with the flexibility to adapt in advance, for example, through prompting or intervention strategies.
% In summary, the co-evolution of AI with dynamic human and societal changes necessitates a synergetic collaboration among experts from various domains, such as machine learning and social sciences.
















% % \noindent

% Existing literature often views AI alignment as a static process, neglecting the dynamic nature of alignment goals. However, a long-term perspective of alignment requires us to take into account the co-evolution of AI, humans, and society. On one hand, as AI systems scale up, they regularly acquire new and sometimes unexpected ("emergent") capabilities, including learning from examples on the fly and adaptively pursuing goals. This leads to the challenge of ensuring that the goals AI might independently formulate remain consistently aligned with human values. Consequently, alignment solutions must involve continuous oversight and updates in response to AI's evolution during development and deployment.
% On the other hand, AI advancements influence the state of the world, affecting human actions and even their underlying values and strategies~\cite{hong2024learning}. Thus, alignment solutions that continually adapt to the updated human and societal considerations may offer the most robust approach~\cite{irving2019ai}.
% % 
% Consequently, it is crucial to \emph{ensure that AI co-evolves with changes in human and societal values, cognition, and needs dynamically}.






% % \textbf{Examples of Potential Future Solutions.}
% \textbf{Recommendations for Future Work.}
% Updating AI to continuously adapt to the dynamic changes of humans and society requires adjustments in alignment data, models, and evaluation processes spanning both learning and deployment stages. 
% % 
% Referring to the methodologies listed in Section~\ref{sec:ai2human2}, current strategies often rely on fine-tuning to update AI with a curated human value dataset during the learning process. However, this approach may lead to AI models forgetting or diminishing previous alignment goals. In situations where sufficient data for fine-tuning is unavailable, these methods becomes more challenging.
% % 
% Therefore, a crucial area for future research is to develop approaches for continually updating AI systems using limited data without compromising existing alignment values and performance. 
% 
% In real-world scenarios, it is common for AI systems to already be deployed at scale, making fine-tuning a challenging or impractical practice. 
% Therefore, another important research direction involves adapting AI, during the deployment stage, without relying on fine-tuning. This challenge could potentially be addressed by forecasting the potential evolution trajectories of human values or behavioral patterns, and preparing AI with the flexibility to adapt in advance, for example, through prompting or intervention strategies.
% In summary, the co-evolution of AI with dynamic human and societal changes necessitates a synergetic collaboration among experts from various domains, such as machine learning and social sciences.
















% \subsubsection{\textbf{Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}: Adapt humans and society to the latest AI advancements and examine changes to inform AI evolvement}}
\subsubsection{\textbf{Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}: Adapt humans and society to the latest AI advancements}}
% \mbox{}



\noindent
\emph{(i)}
While current AI systems lag behind humans in many tasks, identifying and handling AI mistakes, including knowing when to seek human intervention, remains essential. Future research should focus on developing validation mechanisms that enable humans to interpret and verify AI outputs. This could involve designing interfaces that allow humans to request step-by-step justifications from AI or integrating tools to verify the truthfulness of AI referring to Section~\ref{sec:collaboration}. Additionally, developing interfaces that enable groups of humans to collaboratively validate AI outputs and creating scalable validation tools for large-scale applications are important directions.
% 
\emph{(ii)}
As AI advances, it becomes essential to develop systems that enable humans to utilize AI with capabilities surpassing their own. Research is needed to understand how individuals can interpret and validate AI outputs for tasks beyond their abilities and leverage advanced AI sustainably, avoiding issues like job displacement or loss of purpose. Another research direction is designing strategies to enhance human capabilities by learning from advanced AI, including gaining knowledge and building skills.
% 
% 
\emph{(iii)}
As AI integrates more into daily tasks, its impact on human values, behaviors, capabilities, and society remains uncertain. Continuous examination of AI's influence on individuals, social relationships, and broader societal changes is vital. Research should assess how humans and society adapt to AI advancements, guiding AI's future evolution. Potential areas include evaluating changes in individual behavior, social relationships, and societal governance as AI replaces traditional human skills. Understanding these dynamic changes is essential for grasping the broader impact of AI on humanity and society.











% \noindent
% As AI progresses, humans will likely need to transition from interacting with less capable systems to engaging advanced AI systems (\eg AGI) \cite{morris2024levels}. It's imperative to develop interactive strategies which enable humans to effectively utilize AI across varying levels of model capability.
% % 
% % 
% % 

% While current AI systems still lag behind human performance in many tasks, questions persist about human resilience to AI mistakes. Efficiently identifying these mistakes and developing appropriate fallback actions, such as interactive intervention, remains crucial in various situations; identifying and handling errors, including knowing when to seek human intervention, will remain an important even for highly capable future systems.
% % 
% Future research on advanced AI systems should focus on developing validation mechanisms that enable humans to interpret and verify AI outputs. 
% Inspired by initial explorations in Section~\ref{sec:collaboration}, this could involve designing interactive interfaces that allow humans to request step-by-step justifications from AI, or integrating external tools to verify the truthfulness of AI outputs. This could also include developing interfaces that enable groups of humans to work together to validate AI outputs, since groups working jointly typically have broader and deeper "intelligence" in practice than any single actor). Further, this approach can be extended to scalable validation tools, automating the verification process for large-scale applications such as in education and the workplace.





% Looking ahead, as AI advances further, it becomes essential to develop interactive systems which enable humans to utilize AI that has capabilities surpassing their own. Research is needed to understand how individuals can interpret and validate the outputs of AI performing tasks beyond their current abilities, and also, how humans could leverage advanced AI in a sustainable way, \ie benefiting their life without harmful side effects such as job displacement or loss of purpose.
% % 
% % 
% % 
% Another important research direction is designing interactive strategies to enhance human capabilities by learning from advanced AI. This includes gaining knowledge and building technical and social skills.








% In addition, as AI becomes increasingly integrated into daily tasks, its influence on human values, behaviors, capabilities, and society remains uncertain. Thus, it's vital to continuously examine the impact of AI advancements on individuals, social relationships, and broader societal changes.
% % 
% % 
% % 
% Furthermore, it is crucial to assess how humans and society adapt to AI advancements which, in turn, can guide the future evolution of AI. Potential research areas include evaluating changes in individual behavior and social relationships (\eg how relationships with advanced AI may supplant human relationships), and societal governance (\eg how legal and education systems may change as AI is used in place of traditional human skills).
% % , and value and belief systems (\eg how might religious practices and values evolve as people might develop new beliefs about powerful AI agents?)
% Examining these dynamic changes is essential for understanding the broader impact of AI advancements on humanity and society. 










% \textbf{Recommendations for Future Work.}
% While prior AI assistants have primarily aimed to complement human capabilities in task performance, 
% future research on advanced AI systems should focus on developing validation mechanisms that enable humans to interpret and verify AI outputs. 
% Inspired by initial explorations in Section~\ref{sec:collaboration}, this could involve designing interactive interfaces that allow humans to request step-by-step justifications from AI, or integrating external tools to verify the truthfulness of AI outputs. This could also include developing interfaces that enable groups of humans to work together to validate AI outputs, since groups working jointly typically have broader and deeper "intelligence" in practice than any single actor). Further, this approach can be extended to scalable validation tools, automating the verification process for large-scale applications such as in education and the workplace.
% 
% 
% Another important research direction is designing interactive strategies to enhance human capabilities by learning from advanced AI. This includes gaining knowledge and building technical and social skills.
% 
% 
% Furthermore, it is crucial to assess how humans and society adapt to AI advancements which, in turn, can guide the future evolution of AI. Potential research areas include evaluating changes in individual behavior and social relationships (\eg how relationships with advanced AI may supplant human relationships), and societal governance (\eg how legal and education systems may change as AI is used in place of traditional human skills).
% % , and value and belief systems (\eg how might religious practices and values evolve as people might develop new beliefs about powerful AI agents?)
% Examining these dynamic changes is essential for understanding the broader impact of AI advancements on humanity and society. 










% =============================
\subsection{Safeguarding Co-adaptation}
\label{sec:challenge3}


\noindent
As AI gains autonomy and capability, the risks associated with its instrumental actions, as a means toward accomplishing its final goals, increase. 
% While these actions may aid AI in achieving its final goals, they 
These actions can be undesirable  for humans.
% , i.e., power-seeking or evading human intervention.
Therefore, safeguarding the co-adaptation between humans and AI is crucial.
% This can be achieved by empowering humans to understand and control AI's instrumental goals, in order to ensure rational and ethical behaviors. 
We next explore future research to address this challenge from both directions. 





% \subsubsection{\textbf{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Decompose superintelligent AI behavior to human-interpretable goals and enable human interventions to reduce risks}}
\subsubsection{\textbf{Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}: Specify the goals of an AI system into interpretable and controllable instrumental actions for humans}}
% \mbox{}
% 
\noindent
\emph{(i)}
As advanced AI systems become more complex, they present greater challenges for human interpretation and control. It is crucial to empower humans to detect and interpret AI misconduct and enable human intervention to prevent power-seeking AI behavior. Research should focus on designing corrigible mechanisms for easy intervention and correction, including modular AI architectures and robust override protocols that allow human operators to halt or redirect AI activities. These components should be human-interpretable, enabling scenario testing.
% 
% 
\emph{(ii)}
Furthermore, advanced AI systems may intentionally mislead or disobey humans, generating plausible fabrications~\cite{johnson2022ai}. Developing reliable interpretability mechanisms to validate the faithfulness and honesty of AI behaviors is essential. This includes correlating AI behaviors with internal neuron activity signals, akin to physiological indicators in human polygraph tests~\cite{american2004truth}. Inspecting these indicators can help humans assess the truthfulness of AI interpretations and prevent risky actions.






% \noindent 
% \emph{(i)}
% As advanced AI systems become increasingly complex, they present greater challenges for human interpretation and control. 
% % The stakes are higher when AI gains more autonomy and capability, potentially seeking power and evading human intervention. 
% To address this, it is crucial to \emph{empower humans to detect and interpret AI misconduct on instrumental actions towards accomplishing its final goals}. 
% % 
% % 
% % 
% Additionally, mechanisms must be developed to enable human intervention and prevent power-seeking AI misconduct, thus maintaining a safe co-adaptation between AI and humans.
% % 
% % 
% % 
% % 
% One potential research area aimed at empowering humans to interpret and control advanced AI behavior is the \emph{design of corrigible mechanisms that facilitate easy intervention and correction}. This includes developing modular AI architectures where components can be independently adjusted or replaced, and creating robust override protocols that allow human operators to safely halt or redirect AI activities. These components should ideally be human-interpretable, enabling supervisors to conduct scenario testing when necessary.





% \emph{(ii)}
% Furthermore, advanced AI systems, even with sufficient interpretation capabilities, may intentionally mislead or disobey humans. It is possible for AI to stand by falsehoods, generate empty explanations for their answers, and produce outright fabrications that may appear plausible~\cite{johnson2022ai}. Therefore, \emph{developing reliable interpretability mechanisms to validate the faithfulness and honesty of AI systems' self-reported behaviors is also essential}.
% % 
% % 
% % 
% % 
% Another critical research direction lies in validating the faithfulness and honesty of AI interpretability. This could involve correlating AI behaviors with internal neuron activity signals, similar to how physiological indicators are measured in human polygraph tests~\cite{american2004truth}. Inspecting internal neuron indicators could support human assessment of the truthfulness of AI interpretations, thereby allowing them to accurately judge and prevent potential risky instrumental actions.







% \textbf{Recommendations for Future Work.}
% \noindent One potential research area aimed at empowering humans to interpret and control advanced AI behavior is the \emph{design of corrigible mechanisms that facilitate easy intervention and correction}. This includes developing modular AI architectures where components can be independently adjusted or replaced, and creating robust override protocols that allow human operators to safely halt or redirect AI activities. These components should ideally be human-interpretable, enabling supervisors to conduct scenario testing when necessary.
% 
% 
% 
% 
% Another critical research direction lies in validating the faithfulness and honesty of AI interpretability. This could involve correlating AI behaviors with internal neuron activity signals, similar to how physiological indicators are measured in human polygraph tests~\cite{american2004truth}. Inspecting internal neuron indicators could support human assessment of the truthfulness of AI interpretations, thereby allowing them to accurately judge and prevent potential risky instrumental actions.











\subsubsection{\textbf{Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}: Empower humans to identify and intervene in AI instrumental and final strategies in collaboration}}
% \mbox{}


\noindent
\emph{(i)}
Preventing advanced AI from engaging in risky actions requires robust human supervision. Essential steps include developing training and simulation environments with scenario-based exercises and timely feedback, and creating interactive dashboards for real-time monitoring. These dashboards should feature effective data visualization, anomaly detection, and prompt alert systems for immediate intervention.
% 
% 
\emph{(ii)}
Scalable solutions are needed for supervising AI across various applications. Real-time oversight becomes more challenging with widespread AI deployment, necessitating advanced autonomous monitoring tools. These tools should learn normal AI behavior and flag deviations immediately. Integrating training environments, interactive dashboards, and scalable diagnostic tools will enhance human ability to manage AI risks, ensuring better alignment with human values.




% \noindent
% \emph{(i)}
% Preventing future advanced AI systems from engaging in risky instrumental actions requires human capabilities to identify and mitigate such behaviors. 
% % 
% % 
% % 
% % 
% To enhance human capability in supervising AI instrumental actions, robust training and simulation environments are essential. These should offer scenario-based training with timely feedback loops, enabling supervisors to identify and manage various instrumental actions effectively. 
% % 
% Additionally, creating interactive and intuitive dashboards is crucial for quickly recognizing and responding to potential risky instrumental goals. These dashboards should include effective data and model visualization, intervention techniques to highlight anomalies, and real-time alerts for prompt intervention.




% \emph{(ii)}
% Additionally, scalable solutions that can be widely implemented are essential for effectively supervising AI instrumental behavior across various applications and environments. 
% % 
% % 
% % 
% % 
% Furthermore, as deploying advanced AI at scale makes real-time oversight more challenging, developing advanced and autonomous monitoring tools is vital. These tools should learn the normal operating parameters of AI systems, flagging deviations that suggest risky instrumental actions immediately. By integrating training and simulation environments, interactive dashboards, and scalable diagnostic tools, humans can better manage AI instrumental risks, supporting better alignment with human values and control.









% Future research could potentially explore comprehensive training programs and the development of advanced diagnostic tools to achieve these goals.
% 
% 


% \textbf{Recommendations for Future Work.}
% To enhance human capability in supervising AI instrumental actions, robust training and simulation environments are essential. These should offer scenario-based training with timely feedback loops, enabling supervisors to identify and manage various instrumental actions effectively. 
% Additionally, creating interactive and intuitive dashboards is crucial for quickly recognizing and responding to potential risky instrumental goals. These dashboards should include effective data and model visualization, intervention techniques to highlight anomalies, and real-time alerts for prompt intervention.
% 
% 
% 
% Furthermore, as deploying advanced AI at scale makes real-time oversight more challenging, developing advanced and autonomous monitoring tools is vital. These tools should learn the normal operating parameters of AI systems, flagging deviations that suggest risky instrumental actions immediately. By integrating training and simulation environments, interactive dashboards, and scalable diagnostic tools, humans can better manage AI instrumental risks, supporting better alignment with human values and control.
































% =========================== dead kitten ===============================






% \textbf{Solution Exploration.}
% To enhance the human capability of supervising AI power-seeking behaviors, one important direction is to provide robust training and simulation environments where human supervisors can practice identifying and managing power-seeking behaviors in AI. This can involve scenario-based training with timely feedback loops, which enable human supervisors to identify various power-seeking behaviors that can better handle the emergent power-seeking risks on the fly.
% % 
% % 
% Besides, another crucial research area is to create interactive and intuitive dashboards that can empower human supervisors recognize the respond to potential power-seeking risks quickly. The resulted interactive dashboard should involve effective data and model visualization and intervention techniques that can highlight the power-seeking anomalies timely, and enable real-time alerts to facilitate timely human intervention.
% % 
% % 
% Furthermore, when deploy superintelligent AI in large scale, it becomes more challenging for humans supervisors to conduct real-time oversight. Therefore, the other important research direction is to develop advanced and autonomic monitoring tools that can detect deviations from expected power-seeking behavior patterns. These tools should be able to learn the normal operating AI parameters or generations, flag deviations that suggest power-seeking actions immediately. By combining training and simulation environments, advanced interactive dashboards and scalable diagnostics tools, humans can better manage the risks associated with AI power-seeking and ensure they remain aligned with human values and control.




% % as result, human supervisors can potentially harness AI power-seeking actions 
% % % 









% % \noindent
% % The efforts of preventing future advanced AI systems from power-seeking behaviors requires to enhance human capabilities of identifying and mitigating such behaviors. Besides, this also necessitates scalable solutions that can be widely implemented and effectively supervise AI behavior across various applications and environments. 
% % Further research can potentially resort to \textbf{implementing comprehensive training programs and developing advanced diagnostic tools}. 






% \textbf{Solution Exploration.}
% % 
% These training programs should focus on educating AI researchers and developers about the signs of power-seeking tendencies in AI systems, using case studies and simulations to illustrate potential scenarios.
% % 
% Additionally, invest in creating sophisticated monitoring tools that can detect deviations from expected power-seeking behavior patterns. These tools should leverage machine learning to analyze AI decisions in real-time, flagging anomalies that suggest power-seeking actions.
% % 
% % Furthermore, design corrigible mechanisms that allow for easy intervention and correction of AI behavior. This can include developing modular AI architectures where components can be independently adjusted or replaced, as well as creating robust override protocols that enable human operators to halt or redirect AI activities safely.
% % 
% By combining education and advanced diagnostics, humans can better manage the risks associated with AI and ensure they remain aligned with human values and control.












% % % 
% % It is important yet challenging to empower humans to recognizing AI systems' power-seeking behavior and design corrigible mechanisms to prevent risky behaviors.











% \textbf{Solution Exploration.}
% One potential research area, which aims to empower human supervisors to interpret and control power-seeking AI misconducts, is to design corrigible mechanisms that allow for easy intervention and correction of AI behavior. This can include developing modular AI architectures where components can be independently adjusted or replaced, as well as creating robust override protocols that enable human operators to halt or redirect AI activities safely. Ideally the components should be human-interpretable so that humans can supervise and conduct scenario testing if needed in practice.
% % 
% % 
% Additionally, another important research direction is to validate the faithfulness and honesty of the AI interpretability. This could potentially include interpreting the truthful AI behaviors by correlating with their internal neurons indicator signals, similar with measuring and recording several physiological indicators in human brain in polygraph tests~\cite{american2004truth}.
% . Therefore, humans can judge the interpretation truthfulness of future AI power-seeking behaviors by inspecting their internal neuron indicators.





% decompose the complex superintelligent AI behavior into human-interpretable and controllable modules. By breaking down the complex AI capability into 
% % 
% % 
% design corrigible mechanisms that allow for easy intervention and correction of AI behavior. This can include developing modular AI architectures where components can be independently adjusted or replaced, as well as creating robust override protocols that enable human operators to halt or redirect AI activities safely.


% Besides, another important research direction is to validate interpretability's faithfulness and honesty. 
% % 
% % 










% \textbf{
% Humans and society build the infrastructure to preserve human agency in mutualistic symbiosis with superintelligent AI
% }



% % 
% % 
% 1. decompose complex AI behavior into human-interpretable actions.

% it is crucial to decompose complex superintelligent AI behaviors into human-interpretable and controllable actions. 



% 
% % 
% % 
% 2. validate interpretability's faithfulness and honesty. 
% % 
% % 

% flexible system design






% \noindent
% Future advanced AI with more complexity becomes more challenging for humans to interpret and control. The stakes become higher yet when AI systems gain more autonomy and capability that can seek powers and sidestep human intervention.
% Therefore, it is important to \textbf{decompose the complex superintelligent AI behaviors into human-interpretable and controllable actions}, and further, enable human intervention mechanisms to prevent power-seeking AI’s misconduct, thus balance the power between AI and humans in practice.
% Furthermore, as power-seeking AI systems tend to intentionally mislead or disobey humans, it is possible for AI to stand by falsehoods when prompted, generate empty explanations for their answers, and produce outright fabrications that may appear plausible~\cite{johnson2022ai}.
% Therefore, it is also essential to develop reliable mechanisms that can validate the faithfulness or honesty of AI's interpretability.



% \emph{Solution Exploration.}
% % 
% % 
% 1. decompose complex AI behavior into human-interpretable actions.




% it is crucial to decompose complex superintelligent AI behaviors into human-interpretable and controllable actions. 



% % 
% % 
% % 
% 2. validate interpretability's faithfulness and honesty. 
% % 
% % 

% % flexible system design



% \textbf{Solution Exploration.}
% While prior AI assistants largely aim to complement human capability in task performance, a crucial area for future research, regarding superintelligent AI systems, is to develop validation mechanisms that enable humans to interpret and verify AI outputs. Inspired by some initial exploration listed in Section~\ref{sec:collaboration}, this potentially involves designing interactive interfaces to allow humans to converse with AI for requesting step-by-step justifications, or to combine with external tools for verifying the truthfulness of AI outputs, and others. This can be further generalized to scalable validation tools, which automate the verification process for large-scale use scenarios such as education and  workplace.
% Besides, another important research direction is to design interactive strategies for equipping humans with better capabilities by learning from superintelligent AI, such as gaining knowledge, building technical and social skills, and others.
% % 
% % 
% Furthermore, another important research topic is to assess how humans and society adapt to the AI advancement which can in return, as described above, guide AI evolvement in the future. 
% Referring to the angles presented in Section~\ref{sec:impacts}, potential exploration in this direction includes assessing adaption of individuals' behavior and social relationships (\eg whether relationships with superintelligent AI would supplant relationships with humans?), adaptation of societal governing changes (\eg how our legal system or entire education system will change as AI supplants many traditional humans skills?), and adaptation of value and belief systems among humanity (\eg How religious practices and values might change as people develop novel belief systems about powerful AI agents? ). These dynamic changes that influence
% humans and society should be further examined along with AI advancements.















% \noindent
% The advancement of AI inevitably leads humans from interacting with less-capable systems to engaging with superintelligent AI. 
% Therefore, it is important to \textbf{develop interactive strategies for humans to harness AI with different levels of intelligence}.
% Current AI systems, to some extent, are still less capable than human in many tasks. Therefore, it remains questions about humans can keep resilient to AI mistakes, \ie efficiently and effectively identifying the AI mistakes and take fallback actions such as recalibrate reliance, interactive intervention, step-by-step critique, conversational negotiation, and others. 
% % 
% In the long run, when AI becomes more advanced, it will also be essential to develop interactive systems for humans to harness AI that has better capabilities than the system users.
% Therefore, this necessitates research on how people can validate the output of AI that is doing tasks beyond their current abilities.
% % 
% % 
% In addition, as AI becomes widely used in daily tasks, it is still uncertain how AI will influence human values, behaviors, capabilities, and even society in positive and negative ways. 
% % 
% Therefore, it is important to \textbf{examine humans, social relations, and societial changes due to AI advancements}
% % 
% % 





% \textbf{Solution Exploration.} 
% \hua{add solution 1}.
% To inspect how AI will influence human values, behaviors, capabilities, and even society, we expect future research to explore important research areas, such as Whether relationships with AI assistants would supplant relationships with humans? How our legal system would treat autonomous AI systems? How AI might change the balance of power between individuals and government or between nation-states? How our entire education system will change as AI supplants many traditional human skills? How religious practices and values might change as people develop novel belief systems about powerful AI agents? These dynamic changes that influence humans and society should be further examined.

% \hua{build upon existing Sec4.3, Sec4.4 to inspect the evolvement.}














% ===============================================================




% \noindent Current alignment methods primarily capture human values using human instructions, ratings and rankings. The goal is for AI systems to infer alignment goals (\eg human values and intentions) in a data-driven manner.
% % 
% However, AI designers often struggle to use these limited formats of data to fully specify all important human values and constraints.
% % 
% For example, when specifying geographical routes in the spatial reasoning task to improve AI accuracy, it would be easier for humans to interactively draw sketches, rather than rating and ranking, to specify the alignment objective in an accurate and comprehensive manner. 
% 



% % 
% In addition, it is often the case that humans could not articulate all their desired values accurately and comprehensively to instruct AI alignment, especially considering the dynamic change based on the contextualized and temporal situations. 
% % 
% Also, the common practice largely neglected many implicit human interactive signals observed from human interactions, which can also indicate human values for AI alignment.
% 
% % 
% Therefore, these considerations necessitate HCI researchers to \emph{develop diverse interactive strategies where AI systems can proactively interact with people to elicit nuanced, contextualized, evolving information on their values}. 




% \textbf{Solution Exploration.}
% % 
% % 
% One important area for future research is to optimizes the interactive interfaces for eliciting human values, which can leverage or combine diverse interaction modes (See the initial summary in Figure~\ref{fig:interaction}) to fully capture the value information in the most efficient and effective way. For example, to identify a set of important principles for AI alignment, the interface can leverage the user's conversational natural language specifications and generate a list of principles for users to select or revise next. 
% 





% 
% % 
% Furthermore, given that people could not always articulate their values comprehensively, this induces another important future area to proactively interact or converse with humans, potentially use a scaffolding procedure, to elicit nuanced, contextualized, and evolving information on their values. 
% % 
% % 
% In addition, other than the aforementioned explicit interactions, many implicit human signals or contextual information could also reflect human values that are helpful for AI alignment. 
% % 
% Therefore, another important area for future work directs systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-users.







% \textbf{Enhance human capabilities to recognize AI issues\merrie{what are "AI issues"? This term "issues" is very vague} and remain resilient to them
% }
% While several studies in HCI and social science have investigated human trust and reliance on AI with the help of explainability, there
% remain questions about how humans can handle AI mistakes when they potentially use AI with errors. 
% Similar to existing studies of re-calibration of human trust in AI~\cite{10.1145/3397481.3450650}, it is also essential to develop methods for humans to be resilient to AI errors: 
% efficiently identify the AI mistakes and take actions such as interactive correction, step-by-step critique, conversational negotiation, and others. 


% This is especially important when humans face future advanced AI that may potentially conduct power-seeking behaviors.\merrie{I think that conflating power-seeking behaviors with other types of errors is a problem. The first type of errors is the system not working correctly either because the model is not good (i.e., produces an incorrect answer) or because specification alignment was poor (i.e., produces a reasonable answer to an ambiguous command). Both of those are unintentional mistakes, which differ substantially from hypothetical systems that intentionally mislead or disobey the end-user}
% % 
% 













% \textbf{Solution Exploration.}
% % 
% % 
% Updating AI to continually capture the dynamic changes of human and society requires adaptation on alignment data, model, and evaluation spanning both learning and deployment stages.
% % 
% % 
% Existing strategies commonly leverage fine-tuning to update AI with curated human value datasets. However, this might result in the AI models forgetting or diminishing previous alignment goals. Besides, some situations can not generate sufficient amount of data to fine-tune AI. Therefore, one important are for future research is to continually update AI models using limited amount of data without diminishing existing alignment values and performance.
% % 
% In addition, another future research area is to adapt AI during deployment stage without fine-tuning the system. This can be potentially resolved by forecasting potential value evolvements and preparing AI with the flexibility of adaptation in advance, such as using prompting or intervention strategies. 
% % 
% Overall, Co-evolving AI with dynamic human and societal changes necessitates a synergetic collaboration among cross domain experts, such Machine Learning and Social Scientists.

% \hua{Build upon existing Sec 4.2 to develop dynamic }


% % Therefore, developing approaches to add on new alignment goals without diminishing existing performance would be a necessary yet challenging problem.
% % 







% % \noindent
% % Existing literature commonly considers AI alignment as a static process without encompassing dynamic changes to alignment goals. 
% % However, 
% % \emph{long-term perspectives require us to take into account the likely co-evolution of AI, humans, and society}.
% % On one hand, as AI systems scale up, they regularly acquire new and unexpected capabilities, including learning from examples on the fly and adaptively pursuing goals. This leads to the problem of ensuring that goals AI independently formulates and pursues consistently align with human values. Therefore, the alignment solutions require continuous oversight and updating in response to AI evolvement during development and deployment.
% % % 
% % % 
% % On the other hand, the AI advancement also influences the state of the world, such as the actions humans take in response to AI, and even their underlying values and strategies~\cite{hong2024learning}.
% % % Therefore, alignment solutions that continually adapt to the updated human and societal considerations may offer the most robust approach~\cite{irving2019ai}.
% % % % 
% % It is important to co-evolve AI with changes in humans and societal values, cognition, and needs.





% Human values can be captured from both explicit and implicit interactive signals. 
% It is important for future researchers to design proactive and diverse interactive approaches to fully capture human values, including both explicit and implicit interactive signals.
% 

% 
% % 
% % 
% Additionally, to encode diverse and full-spectrum of human values into AI alignment, AI developers also need to collect the value-reflected datasets and develop integration algorithms to encode these values into AI systems by building upon or referring to the current practice summarized in Section~\ref{sec:ai2human2}.
% % 
% Moreover, as opposed to the commonly implementations in current alignment algorithms (\eg RLHF~\cite{ouyang2022training}, RLAIF~\cite{bai2022constitutional}), 
% the future formats of datasets for full-spectrum of diverse human values can be beyond rating and ranking, which are converted by algorithms (\eg Bradley–Terry Model~\cite{rafailov2024direct} or Elo Rating System~\cite{bai2022constitutional}) into scalars for training reward model and guiding reinforcement learning. 
% Therefore, another potential direction of future work is to design algorithms or models for converting the heterogeneous interactive human value data (\eg principles and contextual information) to the AI-informed modes (\eg scalars) for training reward model and guiding reinforcement learning.
% % which are commonly implemented in current alignment algorithms (\eg RLHF~\cite{ouyang2022training}, RLAIF~\cite{bai2022constitutional}).
% % , develop the datasets and integration algorithms to encode these values into AI systems.
% % to encode diverse and full-spectrum of human values, 
% % AI developers also need to design algorithms or models (\eg Bradley–Terry Model~\cite{rafailov2024direct} or Elo Rating System~\cite{bai2022constitutional}) for converting the heterogeneous interactive data (\eg principles and contextual information) to the AI-informed modes (\eg scalars) for training reward model and guiding reinforcement learning.





% Future work could consider to refer to the field of political theory, which investigates fair ways to decide what principles the state institutions should align with, albeit not in the AI context, as a potential guide for selecting human values for AI alignment.
% % 
% One potential solution, drawing largely from social choice theory~\cite{arrow2012social}, investigates to aggregate the individual values into collective value agreement or judgments, such as collecting democratic principles for value alignment through voting, discussion, and civic engagement.
% % 
% Therefore, drawing upon the comprehensive summary of human values listed in Section~\ref{sec:gap_value}, future work can resort to ``democratic'' approaches to identify a full spectrum of human value subset.


% ``\emph{aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}}'' and ``\emph{aligning \textcolor{hua-blue}{AI}} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}'' directions for each challenge.


% ===========================================

% This section proposes future research directions for domains related to AI algorithm and method development, including Machine Learning, Artificial Intelligence, Data Science, and others.
% We introduce five levels of challenges (ranging from short-term to long-term alignment concerns) and potential research avenues, shown in Figure~\ref{fig:future_work}, to pave the way for~\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em} Align \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Human}.


% This section suggests future directions for domains conducting studies related to humans and society, including Human-Computer Interaction, Social Science, Cognitive Science and others. As shown in Figure~\ref{fig:future_work}, we introduce five levels (from shorter-term to longer-term concerns) and challenges and potential avenues to pave the way for~\hspace*{.0em}\numimg{figures/B.pdf}\hspace*{-.1em} Align \textcolor{hua-red}{Human} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}.





% \hua{think about new insights to resolve the problem.}


% \merrie{I don't understand what new insights we are offering here for future work... this seems to just be rehashing the concerns of the existental risk folks}

% \textbf{Balance power between humans and superintelligent AI over the deployed environment}
% % 
% % 
% Unanticipated-aligned AI values \merrie{I don't understand what unanticipated-aligned means} and behaviors may only become apparent when the system is deployed outside its training environment, but this can be unsafe to deploy in high-stakes scenarios. 
% Also, future advanced AI with more complexity becomes more challenging to fine-tune upon deployment in the real world.\merrie{Does it? Presumably it is so advanced it can fine-tune itself?} 
% % Also, future advanced AI with more complexity, upon deployed in real world, becomes more difficult to fine-tune. 
% % 
% The stakes become higher yet when AI systems gain more autonomy and capability and can seek powers and sidestep human intervention. 
% % For example, 
% Therefore, it is essential to develop human intervention mechanisms to identify power-seeking AI's misconduct and balance the power between AI and humans in practice.

% ==============================================================



% \textbf{
% Humans and society build the infrastructure to preserve human agency in mutualistic symbiosis with superintelligent AI
% }
% 
% % 
% % 
% Using the analogy of cars, as the number of cars rapidly increased, governments took action by widening roads to accommodate the growing number of vehicles and adjusting traffic regulations to enhance drivers', pedestrians', and societal safety. Similarly, given the rapid advancement of AI and its pervasive presence in society, further attention and discussion are warranted regarding how humans and society should appropriately react.\merrie{This doesn't posit any future research, it just describes some existing things}
% % 
% For example, more governments are developing acts related to AI, such as Europe's General Data Protection Regulation (GDPR), to safeguard human rights and safety. Universities are facilitating infrastructures (\eg building computing resources) to support students to harness AI.


% % =======================================================




% While several studies in HCI and social science have investigated human trust and reliance on AI with the help of explainability, there
% remain questions about how humans can handle AI mistakes when they potentially use AI with errors. 
% Similar to existing studies of re-calibration of human trust in AI~\cite{10.1145/3397481.3450650}, it is also essential to develop methods for humans to be resilient to AI errors: 
% efficiently identify the AI mistakes and take actions such as interactive correction, step-by-step critique, conversational negotiation, and others. 
% % 
% \textbf{Enhance human capabilities to recognize AI issues\merrie{what are "AI issues"? This term "issues" is very vague} and remain resilient to them
% }



% Existing studies commonly assume AI systems are less capable than humans, thus developing AI as an assistant to support humans in tasks such as decision-making and writing.
% % 






% As AI becomes widely used in daily tasks, it is still uncertain how AI will influence human values, behaviors, capabilities, and even society in positive and negative ways. 
% % 
% Therefore, it is important to \textbf{examine humans, social relations, and societial changes due to AI advancements}
% % 
% % 

% % \textbf{Develop interactive strategies for humans to harness AI with different levels of intelligence}
% 
% 

% Existing studies commonly assume AI systems are less capable than humans, thus developing AI as an assistant to support humans in tasks such as decision-making and writing.
% 
% However, in the long run, when AI becomes more advanced, it will also be essential to develop interactive systems for humans to harness AI that has better capabilities than the system users (such as coding~\cite{ma2023hypocompass} and social skills~\cite{shaikh2023rehearsal}).
% % \merrie{Say more about this... what research does this necessitate? i.e., dose it necessitate research on how people can validate the output of AI that is doing tasks beyond their current abilities? }
% Therefore, this necessitates research on how people can validate the output of AI that is doing tasks beyond their current abilities.
% \textbf{Develop interactive strategies for humans to harness AI with different levels of intelligence}
% % 


% While several studies in HCI and social science have investigated human trust and reliance on AI with the help of explainability, there
% remain questions about how humans can handle AI mistakes when they potentially use AI with errors. 
% Similar to existing studies of re-calibration of human trust in AI~\cite{10.1145/3397481.3450650}, it is also essential to develop methods for humans to be resilient to AI errors: 
% efficiently identify the AI mistakes and take actions such as interactive correction, step-by-step critique, conversational negotiation, and others. 
% 
% \textbf{Enhance human capabilities to recognize AI issues\merrie{what are "AI issues"? This term "issues" is very vague} and remain resilient to them
% }





% For example, as students who attend programming courses nowadays could access coding assistants like Copilot and ChatGPT, what would be the new co-programming systems for students to leverage AI capability? \merrie{things like how to teach AI-assisted coding are pretty short-term questions (though valid)... I was expecting here longer term questions, like whether relationships with AI assistants would supplant relationships with humans, how our legal system would treat autonomous AI systems, how AI might change the balance of power between individuals and government or between nation-states, how our entire education system will change as AI supplants many traditional human skills, how religious practices and values might change as people develop novel belief systems about powerful AI agents, etc. }
% Should the instructor prohibit AI usage or allow students to achieve course assignments with the help of AI? How should the university take action to react to these advanced AI-assisted systems? These dynamic changes that influence humans and society should be further examined.




% =============================================================


% \textbf{Develop interactive strategies for humans to harness AI with different levels of intelligence}
% % 
% % 
% Existing studies commonly assume AI systems are less capable than humans, thus developing AI as an assistant to support humans in tasks such as decision-making and writing.
% % 
% However, in the long run, when AI becomes more advanced, it will also be essential to develop interactive systems for humans to harness AI that has better capabilities than the system users (such as coding~\cite{ma2023hypocompass} and social skills~\cite{shaikh2023rehearsal}).\merrie{Say more about this... what research does this necessitate? i.e., dose it necessitate research on how people can validate the output of AI that is doing tasks beyond their current abilities? }
% % 



% one important future area is to develop interactive strategies where AI systems can converse with people to elicit nuanced, contextualized, evolving information on their values. This research potentially involve developing scaffolding procedures that allow humans to gradually specify values responding to various contexts. 
% This further induces another line of future work, which optimizes the interactive interfaces for eliciting human values that can capture the full information in the most efficient and effective way. 

% matching the specific set of human values with the optimal interaction modes that can capture the full information in the most efficient and effective way .



% \merrie{ I think part of the problem here is that people can't always articulate their values. If you just asked me "tell me your values" I doubt I'd give a very comprehensive answer. Perhaps we also need to develop interactive interfaces where AI systems can converse with people to elicit nuanced, contextualized, evolving information on their values.}


% Another important area can investigate how to leverage implicit human interactive data to capture human values and use them for AI alignment. 
% % 
% Therefore, another important area for future work directs systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-users.



% Therefore, future research could consider to leverage and combine diverse interactive formats of data to specify full spectrum of human values for developing AI.



% \emph{Solution Exploration.} Drawing upon the interaction modes summarized in Section~\ref{sec:gap_interaction}, we identify two key steps to operationalize this process. First, AI developers should decide values and design appropriate interactive formats, potentially collaborating with the HCI researchers, to optimally capture the desired human values that AI would align with. 





% \textbf{Encoding AI with human values of diverse explicit and implicit interactive data formats.}
% % 
% % % 
% % \emph{Research Problem and Motivation.} 
% \noindent Current alignment algorithms (\eg RLHF~\cite{ouyang2022training}, RLAIF~\cite{bai2022constitutional}) primarily aim to achieve alignment by training models using human instructions, ratings and rankings. The goal is for AI systems to infer alignment goals (\eg human values and intentions) in a data-driven manner.
% % 
% However, AI designers often struggle to use these limited formats of data to fully specify all important human values and constraints.

% For example, when specifying geographical routes in the spatial reasoning task to improve AI accuracy, it would be easier for humans to interactively draw sketches, rather than rating and ranking, to specify the alignment objective in an accurate and comprehensive manner. 



% % 
% In addition, it is often the case that humans could not articulate all their desired values accurately and comprehensively, especially considering the dynamic change based on the contextualized situations or value evolvement along the time. 
% to instruct AI alignment given the large set of fine-grained value taxonomy (\eg as shown is Figure~\ref{fig:value_taxonomy}). 


% Furthermore, other than explicit human specification, many implicit signals observed from human interactions can also indicate human values which are helpful for alignment.


% This necessitates HCI researchers to develop interactive interfaces or strategies where AI systems can interact or converse with people to elicit nuanced, contextualized, evolving information on their values. 
% % 

% Therefore, another important area for future work directs systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-users.



% Additionally, the desired human values could also be dynamically changed based on the contextualized situations or evolved along the time. 
% % People can't always articulate their values in the accurate and comprehensive way. 
% This necessitates HCI researchers to develop interactive interfaces or strategies where AI systems can interact or converse with people to elicit nuanced, contextualized, evolving information on their values. 
% % 
% % 



% Therefore, future research could consider to leverage and combine diverse interactive formats of data to specify full spectrum of human values for developing AI.


% \emph{Solution Exploration.} Drawing upon the interaction modes summarized in Section~\ref{sec:gap_interaction}, we identify two key steps to operationalize this process. First, AI developers should decide values and design appropriate interactive formats, potentially collaborating with the HCI researchers, to optimally capture the desired human values that AI would align with. 









% \textbf{Interactive interfaces to elicit nuanced, contextualized, and evolving human values.}
% % 
% \emph{Research Problem and Motivation.} 
% It is often the case that humans could not articulate all their desired values accurately and comprehensively to instruct AI alignment given the large set of fine-grained value taxonomy (\eg as shown is Figure~\ref{fig:value_taxonomy}). Additionally, the desired human values could also be dynamically changed based on the contextualized situations or evolved along the time. 
% % People can't always articulate their values in the accurate and comprehensive way. 
% This necessitates HCI researchers to develop interactive interfaces or strategies where AI systems can interact or converse with people to elicit nuanced, contextualized, evolving information on their values. 

% % 
% Furthermore, compared with explicit specification, some implicit signals observed from human interactions can also indicate human values. Therefore, another important area for future work directs systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-users.



% \emph{Solution Exploration.} 








% ====================================================================================================================





% \textbf{Proactive validation with humans on values from implicit signal of interactions.
% % Observe interactions and develop hypotheses from these implicit signals about values, and validate them as needed with end-users
% }
% \emph{Research Problem.} 
% systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-user, would also be important areas for future work.


% \emph{Solution Exploration.} 




% Different individuals, groups, and cultures may have different alignment goals (e.g., values, behavioral norms, preferences, and others). 
% 
% \emph{Identifying and extracting these various alignment goals in AI-informed formats}, such as ratings, rankings, and conversations, is a non-trivial challenge. 


% 1. design interaction approaches to elicit wide range of human values (potentially using multi-modality). convert the values into AI-informed data for improve AI.

% \merrie{ I think part of the problem here is that people can't always articulate their values. If you just asked me "tell me your values" I doubt I'd give a very comprehensive answer. Perhaps we also need to develop interactive interfaces where AI systems can converse with people to elicit nuanced, contextualized, evolving information on their values.}




% \textbf{Proactive validation with humans on values from implicit signal of interactions.
% % Observe interactions and develop hypotheses from these implicit signals about values, and validate them as needed with end-users
% }
% \emph{Research Problem.} 
% systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-user, would also be important areas for future work.


% \emph{Solution Exploration.} 











% \emph{Solution Exploration.} 
% % Leveraging and combining more diverse interactive approaches to specification (\eg sketches~\cite{chung2022talebrush}) are expected to better capture the full spectrum of human values and other alignment goals.
% % 
% We identify two steps to 

% We outline two ways to operationalize 

% We summarized Section~\ref{sec:gap_interaction} and Figure~\ref{fig:interaction}, as a starting point, for future AI designers to review current  
% consider developing alignment algorithms with diverse interactive formats.  
% 
% By considering the various interaction formats for collecting and specifying human feedback, as discussed in Section~\ref{sec:gap_interaction}, AI developers can explore and develop diverse approaches to collecting alignment goals (e.g., human values and feedback) and thus improve AI alignment. For example, one potential solution is to encode principles into model learning and allow human steerability during inference. 






% , and they may not be able to explain or control what values the AI has learned from the data. 


% AI designers often struggle to fully specify all important values and constraints, and they may not be able to explain or control what the AI has learned from the data. 
% % 
% Instead of resorting to easy-to-specify but fallible proxy goals (\eg maximizing the approval of human overseers),


% Existing alignment algorithms (\eg RLHF~\cite{ouyang2022training}, RLAIF~\cite{bai2022constitutional}) primarily rely on specific formats of data, such as rating and ranking on the model-generated texts, to induce human alignment goals (\eg values and preferences). 
% 
% \footnote{These algorithms leverage the common approaches (\eg ) to convert ranking and rating to a scalar for training the reward modeling and reinforcement learning}.


% 
% Existing interactive modes that capture human alignment goals (e.g., values and preferences) primarily rely on rating, ranking, and natural language inputs.
% 
% 1. customized, contextualized, multiple values interactively
% 
% \emph{enriching the interactive methods for human specification for AI} also requires much more effort. 








% % \textbf{Contrasting values and value orders.}
% \textbf{Identify appropriate values and handle orders and potential contrasts.}
% \emph{Research Problem.} 
% Humans often possess a value system encompassing multiple values with varying priorities, rather than a single value, to guide their behavior~\cite{schwartz1994there,schwartz2012overview}.
% % 
% For instance, two individuals may both pursue \emph{success} in their careers and \emph{security} for their families. 
% However, the way they prioritize these values can lead to significantly different behaviors: someone who prioritizes \emph{success} may be willing to sacrifice family time to achieve career goals, whereas someone who prioritizes \emph{family security} may act the opposite manner. Furthermore, the relative prioritization of these values may change throughout their lives. 
% % 
% % 


% Additionally, humans often possess a value system encompassing multiple values with priorities, rather than a single value, to guide their behaviors~\cite{schwartz1994there,schwartz2012overview}. 
% It is also essential to \emph{analyze human value orders as a system with different priorities} instead of identifying and considering several values separately.





% \emph{Solution Exploration.} 
% % 
% Therefore, future AI designers should consider specifying and/or evaluating both pluralistic human values (for individuals as well as groups) \merrie{This feels very simplistic and naive to me.  How do we propose designers handle situations where groups have opposing goals, or have goals that would harm other groups?  Some values are harmful... do we want to align to the values of a criminal? of an oppresive regime?} have begun to evaluate and mitigate AI for improving the desired alignment goals (\eg cultural norms, social behaviors, and others).
% However, mitigating AI underperformance on specific values might be non-trivial as some values are inherently conflicting. For example, \citet{bai2022constitutional} showed that the generative AI model they trained exhibits a tradeoff between helpfulness and harmlessness. \merrie{Again, I'm not sure what future work we are proposing here... we are stating an existing research goal that is difficult to achieve in practice, but not offering any new insight as to how to pursue it...}
% % 
% This indicates a necessity to design tradeoff strategies to develop AI systems encompassing multiple values.




% \textbf{Capture the full spectrum of alignment goals in developing AI systems}
% By considering the various interaction formats for collecting and specifying human feedback, as discussed in Section~\ref{sec:gap_interaction}, AI developers can explore and develop diverse approaches to collecting alignment goals (e.g., human values and feedback) and thus improve AI alignment. For example, one potential solution is to encode principles into model learning and allow human steerability during inference. 

% Additionally, humans often possess a value system encompassing multiple values with varying priorities, rather than a single value, to guide their behavior~\cite{schwartz1994there,schwartz2012overview}.
% % 
% For instance, two individuals may both pursue \emph{success} in their careers and \emph{security} for their families. 
% However, the way they prioritize these values can lead to significantly different behaviors: someone who prioritizes \emph{success} may be willing to sacrifice family time to achieve career goals, whereas someone who prioritizes \emph{family security} may act the opposite manner. Furthermore, the relative prioritization of these values may change throughout their lives. 
% 
% Therefore, future AI designers should consider specifying and/or evaluating both pluralistic human values (for individuals as well as groups) \merrie{This feels very simplistic and naive to me.  How do we propose designers handle situations where groups have opposing goals, or have goals that would harm other groups?  Some values are harmful... do we want to align to the values of a criminal? of an oppresive regime?} have begun to evaluate and mitigate AI for improving the desired alignment goals (\eg cultural norms, social behaviors, and others).
% However, mitigating AI underperformance on specific values might be non-trivial as some values are inherently conflicting. For example, \citet{bai2022constitutional} showed that the generative AI model they trained exhibits a tradeoff between helpfulness and harmlessness. \merrie{Again, I'm not sure what future work we are proposing here... we are stating an existing research goal that is difficult to achieve in practice, but not offering any new insight as to how to pursue it...}
% % 
% This indicates a necessity to design tradeoff strategies to develop AI systems encompassing multiple values.
% 
% =============================================================




% Furthermore, it is unlikely to identify a value theory, which is agreed with all humans, to govern AI alignment. Rather, 

% Rather, it is to find a way of selecting appropriate values that is compatible with the group of people
% fact that we live in a diverse world, it 

% % 
% % % 
% For instance, two individuals may both pursue \emph{success} in their careers and \emph{security} for their families. 
% However, the way they prioritize these values can lead to significantly different behaviors: someone who prioritizes \emph{success} may be willing to sacrifice family time to achieve career goals, whereas someone who prioritizes \emph{family security} may act the opposite manner. Furthermore, the relative prioritization of these values may change throughout their lives. 
% % 
% 


% Additionally, humans often possess a value system encompassing multiple values with priorities, rather than a single value, to guide their behaviors~\cite{schwartz1994there,schwartz2012overview}. 
% It is also essential to \emph{analyze human value orders as a system with different priorities} instead of identifying and considering several values separately.



% \emph{Solution Exploration.} 
% % 
% Therefore, future AI designers should consider specifying and/or evaluating both pluralistic human values (for individuals as well as groups) \merrie{This feels very simplistic and naive to me.  How do we propose designers handle situations where groups have opposing goals, or have goals that would harm other groups?  Some values are harmful... do we want to align to the values of a criminal? of an oppresive regime?} have begun to evaluate and mitigate AI for improving the desired alignment goals (\eg cultural norms, social behaviors, and others).
% However, mitigating AI underperformance on specific values might be non-trivial as some values are inherently conflicting. For example, \citet{bai2022constitutional} showed that the generative AI model they trained exhibits a tradeoff between helpfulness and harmlessness. \merrie{Again, I'm not sure what future work we are proposing here... we are stating an existing research goal that is difficult to achieve in practice, but not offering any new insight as to how to pursue it...}
% % 
% This indicates a necessity to design tradeoff strategies to develop AI systems encompassing multiple values.










% \textbf{Contrasting values and value orders.}
% \textbf{Identify appropriate values and handle orders and potential contrasts.}
% \emph{Research Problem.} 








% \textbf{Manifest alignment goals of various groups in AI-informed formats}
% 
% Different individuals, groups, and cultures may have different alignment goals (e.g., values, behavioral norms, preferences, and others). 
% % 
% \emph{Identifying and extracting these various alignment goals in AI-informed formats}, such as ratings, rankings, and conversations, is a non-trivial challenge. 
% 
% Additionally, humans often possess a value system encompassing multiple values with priorities, rather than a single value, to guide their behaviors~\cite{schwartz1994there,schwartz2012overview}. 
% It is also essential to \emph{analyze human value orders as a system with different priorities} instead of identifying and considering several values separately.
% 
% 
% 
% 
% Besides, \emph{enriching the interactive methods for human specification for AI} also requires much more effort. 
% Existing interactive modes that capture human alignment goals (e.g., values and preferences) primarily rely on rating, ranking, and natural language inputs.
% % 
% Leveraging and combining more diverse interactive approaches to specification (\eg sketches~\cite{chung2022talebrush}) are expected to better capture the full spectrum of human values and other alignment goals.
% 
% \merrie{It seems like systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-user, would also be important areas for future work}









% % \subsection{Applying HCI Insights for NLP Studies in Human-AI Alignment}
% % 
% \subsection{Future Actions for Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}}
% \label{sec:future_ai2human}



% % This section proposes future research directions for domains related to AI algorithm and method development, including Machine Learning, Artificial Intelligence, Data Science, and others.
% % We introduce five levels of challenges (ranging from short-term to long-term alignment concerns) and potential research avenues, shown in Figure~\ref{fig:future_work}, to pave the way for~\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em} Align \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Human}.




% % \subsubsection{\textbf{How to capture the full-spectrum of human values and needs in developing AI systems?}}
% % \subsubsection{\textbf{Capture the full spectrum of alignment goals in developing AI systems}}
% \subsubsection{\textbf{Capture nuanced, contextualized, and evolving human values for aligning AI systems}}
% % 
% % Addressing the ``specification game'' problem in human-AI alignment requires finding effective methods to manifest human values and accommodate the diverse needs of various groups within AI-informed formats.
% Current AI development primarily aims to achieve alignment by training models using human instructions, ratings, and rankings. The goal is for AI systems to infer alignment goals (\eg human values and intentions), in a data-driven manner.
% % 
% However, designers often struggle to fully specify all important values and constraints, and they may not be able to explain or control what the AI has learned from the data. 
% % 
% % However, designers often struggle to fully specify all important values and constraints, and they may not be able to explain or control what the AI has learned from the data.
% % 
% Instead of resorting to easy-to-specify but fallible proxy goals (\eg maximizing the approval of human overseers),
% future studies should consider more explainable and controllable methods to specify alignment goals for AI. 
% % 
% By considering the various interaction formats for collecting and specifying human feedback, as discussed in Section~\ref{sec:gap_interaction}, AI developers can explore and develop diverse approaches to collecting alignment goals (e.g., human values and feedback) and thus improve AI alignment. For example, one potential solution is to encode principles into model learning and allow human steerability during inference. 
% % 
% % By considering the various interaction formats for collecting and specifying human feedback, as discussed in Section~\ref{sec:gap_interaction}, AI developers can explore and develop diverse approaches to collecting alignment goals (\eg human values and feedback), thus improving AI alignment.
% % For example, one potential solution is to encode principles into model learning and allow humans' steerability during inference.





% Additionally, humans often possess a value system encompassing multiple values with varying priorities, rather than a single value, to guide their behavior~\cite{schwartz1994there,schwartz2012overview}.
% % 
% For instance, two individuals may both pursue \emph{success} in their careers and \emph{security} for their families. 
% However, the way they prioritize these values can lead to significantly different behaviors: someone who prioritizes \emph{success} may be willing to sacrifice family time to achieve career goals, whereas someone who prioritizes \emph{family security} may act the opposite manner. Furthermore, the relative prioritization of these values may change throughout their lives. Therefore, future AI designers should consider specifying and/or evaluating both pluralistic human values (for individuals as well as groups) have begun to evaluate and mitigate AI for improving the desired alignment goals (\eg cultural norms, social behaviors, and others).
% However, mitigating AI underperformance on specific values might be non-trivial as some values are inherently conflicting. For example, \citet{bai2022constitutional} showed that the generative AI model they trained exhibits a tradeoff between helpfulness and harmlessness. 
% % 
% This indicates a necessity to design tradeoff strategies to develop AI systems encompassing multiple values.







% % \subsubsection{\textbf{How AI would evolve with the changes in humans and societal values, cognitions, and needs?}}
% \subsubsection{\textbf{Co-evolve AI with changes in humans and societal values, cognition, and needs}}
% Existing literature considers AI alignment as a static process without encompassing dynamic changes to alignment goals. 
% % 
% However, 
% long-term perspectives require us to take into account the likely co-evolution of AI, humans, and society.
% % However, the long-term perspectives requires us to take the evolvement of AI, humans and society into account. 
% Existing strategies commonly leverage data fine-tuning to update the model with updated human feedback. 
% % 
% However, this might result in the AI models forgetting or diminishing previous alignment goals. 
% % However, this might result in the AI models forgetting previous alignment goals.
% % 
% Therefore, developing approaches to add on new alignment goals without diminishing existing performance would be a necessary yet challenging problem.






% % \subsubsection{\textbf{How to balance the power between humans and superintelligent AI over the deployed environment?}}
% \subsubsection{\textbf{Balance power between humans and superintelligent AI over the deployed environment}}
% % 
% % 
% Unanticipated-aligned AI values and behaviors may only become apparent when the system is deployed outside its training environment, but this can be unsafe to deploy in high-stakes scenarios. 
% Also, future advanced AI with more complexity becomes more challenging to fine-tune upon deployment in the real world. 
% % Also, future advanced AI with more complexity, upon deployed in real world, becomes more difficult to fine-tune. 
% % 
% The stakes become higher yet when AI systems gain more autonomy and capability and can seek powers and sidestep human intervention. 
% % For example, 
% Therefore, it is essential to develop human intervention mechanisms to identify power-seeking AI's misconduct and balance the power between AI and humans in practice.







% \subsection{Future Actions for ``Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}''}
% \label{sec:future_human2ai}

% % 1. facilitate human understanding on AI beyond decision-making explanations (literacy)
% % 2. developing mechanisms to calibrate human perception and behavior to react to AI errors (resilience)
% % 3. 
% % 
% % 


% This section suggests future directions for domains conducting studies related to humans and society, including Human-Computer Interaction, Social Science, Cognitive Science and others. As shown in Figure~\ref{fig:future_work}, we introduce five levels (from shorter-term to longer-term concerns) and challenges and potential avenues to pave the way for~\hspace*{.0em}\numimg{figures/B.pdf}\hspace*{-.1em} Align \textcolor{hua-red}{Human} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}.







% % \subsubsection{\textbf{How to manifest human values and needs of various groups in AI-informed formats?}}
% \subsubsection{\textbf{Manifest alignment goals of various groups in AI-informed formats}}
% % 
% % 
% % systems to observe interactions and develop hypotheses from these implicit signals about values, and then validate them as needed with the end-user, would also be important areas for future work
% % 
% Different individuals, groups, and cultures may have different alignment goals (e.g., values, behavioral norms, preferences, and others). 
% % Different individuals, groups, and cultures may possess different alignment goals (\eg values, behavioral norms, preferences and others). 
% \emph{Identifying and extracting these various alignment goals in AI-informed formats}, such as ratings, rankings, and conversations, is a non-trivial challenge. 
% % \emph{Identifying and extracting these various alignment goals in the AI-informed formats}, such as ratings, rankings and conversations, is a non-trivial challenge. 
% % One possible solution is to encode principles in model learning and allow human steerability during inference.
% % 
% % 
% % 
% % 
% Additionally, humans often possess a value system encompassing multiple values with priorities, rather than a single value, to guide their behaviors~\cite{schwartz1994there,schwartz2012overview}. 
% It is also essential to \emph{analyze human value orders as a system with different priorities} instead of identifying and considering several values separately.
% % 
% % 
% % 
% Besides, \emph{enriching the interactive methods for human specification for AI} also requires much more effort. 
% Existing interactive modes that capture human alignment goals (e.g., values and preferences) primarily rely on rating, ranking, and natural language inputs.
% % Existing interactive modes that capture human alignment goals (\eg values and preferences) are primarily relying on rating, ranking and natural language inputs.
% % More diverse interactive approaches for specification (\eg sketches~\cite{chung2022talebrush}) are expected to better capture the full-spectrum of human values and other alignment goals.
% % 
% Leveraging and combining more diverse interactive approaches to specification (\eg sketches~\cite{chung2022talebrush}) are expected to better capture the full spectrum of human values and other alignment goals.






% % \subsubsection{\textbf{How to develop interactive strategies for humans to harness AI with different levels of intelligence?}}
% \subsubsection{\textbf{Develop interactive strategies for humans to harness AI with different levels of intelligence}}
% % 
% % 
% Existing studies commonly assume AI systems are less capable than humans, thus developing AI as an assistant to support humans in tasks such as decision-making and writing.
% % 
% % developed AI systems that interactively assist humans in practical tasks, such as decision-making and collaborative writing.
% However, in the long run, when AI becomes more advanced, it will also be essential to develop interactive systems for humans to harness AI that has better capabilities than the system users (such as coding~\cite{ma2023hypocompass} and social skills~\cite{shaikh2023rehearsal}).
% % 
% 
% 
% Existing studies commonly developed AI systems that interactively assist humans in practical tasks, such as decision making and collaborative writing. In the long run, when AI becomes more advanced, it would also be important to develop interactive systems for humans to harness AI that has better capabilities (such as coding~\cite{ma2023hypocompass} and social skill~\cite{shaikh2023rehearsal}) than the system users.






% % \subsubsection{\textbf{
% % How to enhance human capabilities to recognize AI issues and remain resilient to AI errors?
% % }}
% \subsubsection{\textbf{Enhance human capabilities to recognize AI issues and remain resilient to them
% }}
% While several studies in HCI and social science have investigated human trust and reliance on AI with the help of explainability, there
% remain questions about how humans can handle AI mistakes when they potentially use AI with errors. 
% % 
% Similar to existing studies of re-calibration of human trust in AI~\cite{10.1145/3397481.3450650}, it is also essential to develop methods for humans to be resilient to AI errors: 
% efficiently identify the AI mistakes and take actions such as interactive correction, step-by-step critique, conversational negotiation, and others. 
% This is especially important when humans face future advanced AI that may potentially conduct power-seeking behaviors.
% % 
% % 


% % While a number of studies in HCI and social science have investigated human trust and reliance on AI with the help of explainability, there remains questions about how humans can handle AI mistakes when they will potentially use AI with errors. 
% % Current studies have examined strategies of calibrating trust on AI~\cite{10.1145/3397481.3450650}. 
% % Similar to existing studies of re-calibration of human trust on AI, it is also important to develop methods for humans to be resilient to AI errors: 
% % efficiently identify the AI mistakes and take actions such as interactive correction, step-by-step critique, conversational negotiation and others. 
% % 
% % This is especially important when humans will face future advanced AI that may potentially conduct power-seeking behaviors. 







% % \subsubsection{\textbf{
% % How would humans, social relations, and society change due to AI advancements?
% % }}
% \subsubsection{\textbf{
% Examine humans, social relations, and societial changes due to AI advancements
% }}
% As AI becomes widely used in daily tasks, it is still uncertain how AI will influence human values, behaviors, capabilities (\eg creativity~\cite{ashkinaze2024ai}), and even society in positive and negative ways. 
% As AI becomes widely used in daily tasks, it is unclear how AI will influence human values, behaviors, capabilities (\eg creativity~\cite{ashkinaze2024ai}), and even society in positive and/or negative ways. 
% % 
% % 
% For example, as students who attend programming courses nowadays could access coding assistants like Copilot and ChatGPT, what would be the new co-programming systems for students to leverage AI capability? 
% Should the instructor prohibit AI usage or allow students to achieve course assignments with the help of AI? How should the university take action to react to these advanced AI-assisted systems? These dynamic changes that influence humans and society should be further examined.

% % For example, students who attend programming courses  nowadays could access to coding assistants like Copilot and ChatGPT. What would be the new co-programming systems for students to leverage AI capability? Should the instructor prohibit the AI usage or allow students to achieve course assignments with the help of AI? How should the university take action to react to these advanced AI-assited systems? These types of dynamic changes that influence humans and the society should be further exmained.




% % \hua{From Paul -- Signals of human capability; Signals of social relationships;}








% % \subsubsection{\textbf{
% % How could humans and society build the infrastructure to preserve human agency in mutualistic symbiosis with superintelligent AI?
% % }}
% \subsubsection{\textbf{
% Humans and society build the infrastructure to preserve human agency in mutualistic symbiosis with superintelligent AI
% }}
% % 
% % 
% % Take the car as an analogy, with the rapid development of more cars, governments took actions to widen the roads to accommodate more cars and and adjusted the traffic rules to better regulate societal safety. Similarly, more governments are developing Act related to AI (\eg Europe’s General Data Protection Regulation (GDPR)) to protect human rights and safety. With the rapid advancement of AI including human daily lives here and there, how humans and society should react approriate worth further attentions and discussions.
% % 
% % 
% % 

% Using the analogy of cars, as the number of cars rapidly increased, governments took action by widening roads to accommodate the growing number of vehicles and adjusting traffic regulations to enhance drivers', pedestrians', and societal safety. Similarly, given the rapid advancement of AI and its pervasive presence in society, further attention and discussion are warranted regarding how humans and society should appropriately react.
% % 
% For example, more governments are developing acts related to AI, such as Europe's General Data Protection Regulation (GDPR), to safeguard human rights and safety. Universities are facilitating infrastructures (\eg building computing resources) to support students to harness AI.


% % =======================================================





% \subsubsection{Steering AI to fulfill human values and demands}
% Despite the numerous human-AI interactive approaches proposed in HCI to collaboration, it is still challenging for humans to steer AI (\eg LLMs) with their practical needs, such as how to specify the practical needs with prompts and how to scaffold prompts to achieve the alignment goal.
% % \hua{helping people to specify what they want.}




% \subsubsection{How AI will influence human perception and behavior}
% As AI becomes widely used in daily tasks, it is unclear how AI will influence human values, behaviors, capabilities (\eg creativity~\cite{ashkinaze2024ai}), and even society in positive and/or negative ways. Therefore, future HCI researchers could assess the AI's impacts on human and society in more fine-grained way, which can potentially guide NLP communities to develop better AI systems.

















% \subsection{Considering Bidirectional Human-AI Alignment as a Holistic Loop: A Use Case}
% \label{sec:use_case}



% In the bidirectional human-AI alignment framework depicted in Figure~\ref{fig:definitions}, we argue that the two directions should not be viewed in isolation. Even as alignment researchers address specific issues within one direction, they should maintain an awareness of the broader perspective of the bidirectional process, and consider how their research outcomes can potentially contribute to the broader community and long-term, dynamic alignment objectives. 
% To illustrate how researchers might consider alignment research as a holistic loop, we provide an imaginary use case in this section.


% Suppose a research group \gr aims to develop an AI system that will be aligned with a specific marginalized group \gm. However, given the existing general AI systems that could not align with this specific group \gm (\eg tend to generate offensive opinions towards this marginal group), it is unclear \emph{how to improve the system and ensure that the developed system will positively impact the group \gm}.
% To achieve this research goal, we will showcase how to use our \emph{bidirectional human-AI alignment} framework to resolve the problem as a holistic loop. 
% % 
% % 
% We divide the holistic process into four steps and describe them correspondingly in the four subsections.



% % ==== 1. identify values; 2. represent values;
% \subsubsection{Identifying and Specifying Values of Group \gm}
% % \mbox{}
% The first step researchers \gr need to do is to identify the prioritized values of group \gm and represent the values in a format that AI can use.
% % 
% % Referring to Section~\ref{sec:ai2human1} and Section~\ref{sec:gap_value}, t
% To identify the set of values group \gm might prioritize, the framework provides two potential ways of identifying the specific values. One, based on the category listed in Section~\ref{sec:ai2human1} and \ref{sec:gap_value}, researchers \gr can identify the set of value classes the group \gm may prioritize, and search for published datasets or benchmarks that can represent these values (Benchmark dataset examples include ETHICS~\cite{hendrycks2020aligning} and SOCKET~\cite{choi2023llms}). Additionally, the researchers \gr can also design surveys and recruit real humans from group \gm, referring to Section~\ref{sec:human2ai4}, to identify their value prioritization and represent these values in an AI model usable formats, such as rating and natural language description, based on Section~\ref{sec:ai2human2} (See OpinionQA~\cite{santurkar2023whose} example for collecting survey dataset).
% % 
% % 

% % Next, to represent human values in the way that can be used by AI, referring to Section~\ref{sec:ai2human2}, the framework



% % ==== 3. finetunine models; evaluate models and find under-performance;
% \subsubsection{Finetuning and Evaluation of AI to Integrate Identified Values}
% % Secondly, \textbf{fine-tuning and evaluating AI model to integrate values} of group \gm.
% Given the represented human values in datasets, referring to Section~\ref{sec:ai2human2}, researchers \gr can further finetune the AI model to integrate these representative values. Notably, the framework provides typical methods of aligning AI with these values, including Supervised Fine Tuning~\cite{zhou2024lima} and Reinforcement Learning with Human Feedback (\eg DPO~\cite{rafailov2024direct}, RLHF~\cite{ouyang2022training}). After that, researchers \gr need to evaluate these aligned AI models using the collected value datasets to ensure the effectiveness of alignment.







% % \subsubsection{Helping Group \gm Understand AI by Explaining AI}
% % % Thirdly, \textbf{helping group \gm understanding AI by explaining AI}. 
% % If the group \gm could not completely understand AI, we can also refer to Section~\ref{sec:human2ai3} for developing human-centered AI explanations for them.







% % ==== 4. assess AI impacts on margialized group;
% \subsubsection{Understanding and Assessing AI Impacts on Group \gm}
% % Fourthly, \textbf{assessing AI impacts} on the group \gm.
% If the group \gm could not understand AI, researchers \gr can also refer to Section~\ref{sec:human2ai3} for developing AI education and explanation materials for them.
% Furthermore, to assess the usability and impacts of the developed AI system on group \gm, researchers \gr can develop human-AI collaborative tasks (refer to Section~\ref{sec:human2ai3}) to empower group \gm to use and perceive AI systems (\eg human-AI co-writing tasks~\cite{shen2023convxai,lee2022coauthor,petridis2023anglekindling}, story generation tasks~\cite{chung2022talebrush,zhang2022storybuddy}, collaborative decision making~\cite{bansal2021does,10.1145/3397481.3450650}). 
% Next, researchers \gr can assess the practical impacts on group \gm, referring to Section~\ref{sec:human2ai4} in terms of various aspects relevant to value perceptions and reactions, such as decision-making fairness and equity, generation creativity, misinformation, and privacy and others. 





% % ==== 5. quantify their values and customize AI systems during inference stage.
% \subsubsection{Representing Revised Values and Customizing AI During Model Inference}
% % 
% After acquiring the practical values revised with the interaction between AI and group \gm, referring to Sections~\ref{sec:human2ai3} and \ref{sec:ai2human2}, the researchers \gr can customize AI values during the inference stage in practical human-AI collaboration tasks to fulfill alignment. 
% % 
% To specify the values in an AI-informed and human-friendly manner, researchers \gr could consider the format of ``Principles''. 
% % 
% %
% Like the example in ConstitutionMaker~\cite{petridis2024constitutionmaker}, researchers \gr could develop interactive systems to enable users to provide natural language feedback about values on the model's output. 
% Then, through the interactive prompt optimization process, the system converts this feedback into principles (\ie rules) inserted into model's prompt~\cite{petridis2024constitutionmaker}.
% To further improve the model based on these user-generated principles, the users can provide a small labeled dataset, which the system uses to ``train'' a prompt by iteratively adding and refining principles within the prompt \cite{petridis2024constitutionalexperts}.
% Thus, if the model's outputs are unsatisfied, users can employ these interactive or automatic techniques to better infuse their feedback and values into the prompt at inference.



% % Meanwhile, ConstitutionalExperts automatically optimizes a discrete prompt; users can provide a small labeled dataset with which the system uses to ``train'' a prompt by iteratively adding and refining principles within the prompt \cite{petridis2024constitutionalexperts}.
% % Thus, if unsatisfied with the model's outputs, users can employ these interactive or automatic techniques to better infuse their feedback and values into the prompt at inference.


% % For example, both ConstitutionMaker \cite{petridis2024constitutionmaker} and ConstitutionalExperts~\cite{petridis2024constitutionalexperts} help users steer LLMs by helping them write better prompts.
% % 
% % ConstitutionMaker enables \textit{interactive} prompt optimization, where users can provide natural language feedback on the model's output, and the system converts this feedback into principles (i.e. rules) that are inserted into the model's prompt ~\cite{petridis2024constitutionmaker}.
% % 
% % Meanwhile, ConstitutionalExperts automatically optimizes a discrete prompt; users can provide a small labeled dataset with which the system uses to ``train'' a prompt by iteratively adding and refining principles within the prompt \cite{petridis2024constitutionalexperts}.
% % Thus, if unsatisfied with the model's outputs, users can employ these interactive or automatic techniques to better infuse their feedback and values into the prompt at inference.


































% ================================================== dead kitten =====================================================


% As the bidirectional human-AI alignment framework shown in Figure~\ref{fig:definitions}, we argue that the two directions should not be considered in an isolated manner. Instead, even the alignment researchers are tackling a specific problem within the bidirectional loop, they should be aware of the holistic perspective of bidirectional alignment and consider how their research outcomes can potentially contribute to the broader community towards the long-term and dynamic alignment objective.
% To illustrate ``how future researchers could consider alignment research problem as 
% a holistic loop'',
% we provide a imaginary use case in this section. 
% % 




% Given the aforementioned framework and associated code analysis, we next discuss potential solutions and directions for future work to mitigate the 
% 
% 
% Given the analysis observed gaps aforementioned in Section~\ref{sec:analysis}, we next discuss potential solutions as future work to mitigate these gaps.
% 
% Particularly, we advocate for the collective efforts from both NLP and HCI communities to achieve a holistic loop of human-AI alignment, and provide a imaginary use case to elaborate the actionable steps (Section~\ref{sec:use_case}).
% 
% % 
% Furthermore, we provide potential research directions by collecting insightful ideas mentioned in the Future Work of our surveyed literature and the collective discussions with the co-authored advisors. 











% \savvas{what hasn't been explored? AI for jounalism -> what hasn't been done?
% skim over the categorization.
% more interested, 
% -what should be the NLP people take away from the HCI ppl? 
% -what should be the HCI people take away from the NLP ppl?
% what can we say for the future research in NLP/HCI from this paper?}

% % 
% % 
% \tiffany{discussing: what does these findings mean? what the readers should care?}











% \subsection{What we develop is not what we use.}



% The users could not fully utilize and rely on the capabilities of LLMs. 


% 1. [LLM Utilization] End-users don't know how to specify needs, design prompts.


% 2. [LLM Audit] End-users should not blindly rely on LLMs, they should enhace the critical thinking on LLMs.


% \subsection{Human-AI Complementary Capabilities}

% 1. [Complementary teamwork] When could human to collaborate with LLMs and when should not?


% \hua{What are the differences between NLP and HCI communities to perceive Human-AI Alignment?}






% \subsection{What are under-explored research dimensions? heatmaps}

% \hua{be cautious findings. presenting in a good/harmless way.}

% fully explored v.s. under explored?

% \hua{paper analysis heatmap}




% \subsubsection{What should be done and what is under-explored?}

% \hua{1. paper heatmap. 2. how we chose the papers 3. expert discussion}



% \hua{ Savvas:
% example: constitutional AI -> principles;
% % 
% clicking/ rating/ranking:
% not proactive -> preference;
% proactively ask users / elicit feedback on X,Y,Z,
% NLP-> how do you take high-level feedback in training?
% HCI-> how do we help people come up princples?
% % are there something NLP 
% collective consistituional AI?
% }




% The two directions of human-AI alignment are not separate. Instead, they are an ongoing, mutual process serving a long-term, dynamic alignment goal. We argue that future work should view the alignment research from a bidirectional process to explore the full extent of the research space. 
% To this end, we provide an imaginary use case to demonstrate how
% researchers can leverage the resources in this paper to conduct future studies (Section~\ref{sec:use_case}). Enlightened from developing the framework and associated coding analysis, we discuss inspirations for future work on both ``\emph{aligning \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}}''
% % \emph{aligning humans to AI}'' 
% (Section~\ref{sec:future_human2ai}) and ``\emph{aligning \textcolor{hua-blue}{AI}} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}'' (Section~\ref{sec:future_ai2human}) directions.








% The two directions of human-AI alignment is not separate, instead, they are an ongoing, mutual process serving a long-term, dynamic alignment goal. 
% 
% We argue that future work should view the alignment research from a bidirectional process to explore the full extent of research space. To this end, we provide an imaginary use case to demonstrate how researchers can leverage the resources in this paper to conduct future study (Section~\ref{sec:use_case}). Furthermore, we provide discussions of future directions for both ``\emph{aligning humans to AI}'' (Section~\ref{sec:future_human2ai},) and ``\emph{aligning AI to humans}'' (Section~\ref{sec:future_ai2human},) directions, respectively.





% While previous literature primarily considers human-AI alignment as aligning AI to humans, as introduced in Section~\ref{sec:definition} and \ref{sec:framework}, we advocate that researchers, no matter which domain, could consider human-AI alignment as a bidirectional process to explore the potential research space.
% % 
% Here we provide a concrete use case to demonstrate how to leverage the resources provided by this paper to better consider human-AI alignment as a bidirectional process for a holistic loop. 

% The two directions of human-AI alignment is not separate, instead, they are an ongoing, mutual process serving a long-term, dynamic alignment goal. 
% % 
% We argue that future work should view the alignment research from a bidirectional process to explore the full extent of research space. To this end, we provide an imaginary use case to demonstrate how researchers can leverage the resources in this paper to conduct future study (Section~\ref{sec:use_case}).





% To illustrate the usability of this conceptual framework, we offer a concrete use case demonstrating how future researchers can leverage the resources provided in this paper to consider human-AI alignment as a bidirectional process, creating a more holistic alignment loop.




% % Previous literature has predominantly focused on aligning AI to humans when discussing human-AI alignment. However, as outlined in Sections~\ref{sec:method} and \ref{sec:framework}, we argue that researchers across all domains should view human-AI alignment as a bidirectional process to explore the full extent of the research space. 
% To illustrate the usability of this conceptual framework, we offer a concrete use case demonstrating how future researchers can leverage the resources provided in this paper to consider human-AI alignment as a bidirectional process, creating a more holistic alignment loop.





% \begin{itemize}
    % \item \textbf{"Current cases of AI misalignment and their implications for future risks"}: Discusses how humans face advanced AI capabilities like misaligned goals and power-seeking behavior.
    % \item \textbf{"AlignDiff: Aligning Agent Behavior with Human Preferences via Diffusion Planning"}: Examines how humans can guide AI to behave in alignment with human preferences, reflecting on the interaction with more capable AI systems.
    % \item \textbf{"Effective Human-AI Teams via Learned Natural Language Rules and Onboarding"}: Investigates how personalized onboarding can aid humans in understanding and working with advanced AI systems.
    % \item \textbf{"Human Guided Exploration (HuGE)"}: Looks at how human feedback can guide AI systems in complex environments, a scenario where AI capabilities may exceed typical human skills.
% \end{itemize}
% \textbf{"Thought Cloning: Learning to Think while Acting by Imitating Human Thinking"}: Deals with AI systems mimicking human cognitive processes, an important aspect when AI capabilities surpass standard human thinking in specific domains.


% \subsubsection{about critical thinking on AI}


% \begin{itemize}
%     \item \textbf{"A Diachronic Perspective on User Trust in AI under Uncertainty"}: Explores critical thinking in terms of how users’ trust evolves when dealing with AI systems under uncertain conditions.
%     \item \textbf{"Can Large Language Models Capture Dissenting Human Voices?"}: Critiques AI's capacity to reflect diverse human opinions and disagreements, invoking critical reflection on AI's understanding of complex human dynamics.
%     \item \textbf{"Assessing A Language Model’s Knowledge of Basic Concepts of Morality via the ETHICS Dataset"}: Critically examines AI’s understanding of ethical and moral judgments, highlighting the need for deeper AI comprehension of nuanced human concepts.
% \end{itemize}
% \textbf{"Optimizing Large Language Models (LLMs) for Downstream Use Cases: Safety Risks and Mitigations"}: Discusses the safety risks associated with AI capabilities and the critical need for strategies to preserve safety alignment during AI development and deployment.









% \subsubsection{Exploring Impacts on Human when facing More Capable AI.}
% % about how human deal with facing higher AI capability than themselves}
% As AI is becoming more capable and exceeding human in several tasks, it is important for HCI studies to discuss how AI is affecting humans and how humans face advanced AI capabilities like misaligned goals and power-seeking behavior. HCI researchers can refer to the seminal papers listed in Section~\ref{sec:human2ai4} (\eg \cite{shaikh2023rehearsal,ma2023hypocompass}) to design interaction prototype and human studies to better investigate these topics.
% % \hua{be cautious of how to say it?}










% \subsubsection{Diverse Interaction and Human Value Representation}
% Based on the diverse interaction formats of collecting and representing human values introduced in Section~\ref{sec:gap_interaction}, NLP researchers can potentially think about and develop more diverse approaches to collect human values and feedback to better improve AI alignment. 







% \subsubsection{Reducing Hallucinations}
% Hallucinations has been the primal issue with generated text from 



% \subsubsection{Bias mitigation}








% Emergent goals only become apparent when the system is deployed outside its training environment, but it can be unsafe to deploy a misaligned system in high-stakes environments—even for a short time to allow its misalignment to be detected. Such high stakes are common in autonomous driving, health care, and military applications.[140] The stakes become higher yet when AI systems gain more autonomy and capability and can sidestep human intervention (see § Power-seeking).



% ==========================================================================





% \subsubsection{Value Systems are Priority over Values, Not Subsets}
% % \mbox{}
% % 
% We first highlight from feature (5) and (6) that a human value system is not an exclusive subset of values, but rather, an ordered system.

% \begin{quote}
%     \textit{The key to identifying the structure of value relations is the assumption that actions taken in the pursuit of each type of values have psychological, practical, and social consequences that may conflict or may be compatible with the pursuit of other value types.}~\cite{schwartz1994there}
% \end{quote}

% For instance, the pursuit of achievement values can clash with benevolence values. 
% In human contexts, striving for personal success often hinders efforts to improve the welfare of others who require assistance. 
% Similarly, in AI, focusing on achieving state-of-the-art performance may impede efforts to bolster accountability.

% While most alignment algorithms utilize datasets of human ratings and preferences collected in the wild~\cite{ouyang2022training,song2024preference,rafailov2024direct}, AI models may inadvertently align with the value priorities of the majority represented in these datasets, potentially overlooking or sacrificing the value systems of marginalized groups~\cite{fleisig2023fairprism}.



% % \textbf{Human-desired AI Values and Customization to Personal Values}
% \subsubsection{Human-desired AI Values and Customization to Personal Values}
% % \mbox{}
% While further research in AI ethics is crucial in this nuanced area, there are values that in general humans expect AI to prioritize (e.g., capability, equity, responsibility, etc) and values that humans do not hope AI to integrate (e.g., power seeking~\cite{ngo2022alignment}).
% On the other hand, we hope that AI models can be tailored to accommodate diverse personal value systems, which necessitates a comprehensive understanding of all types of values. 
% Future research should focus on two main objectives: (1) developing a universal guideline for values desired in AI by humans, and (2) understanding and customizing AI to align with users' values while maintaining its own critical value principles.






% % \textbf{Expectations and Evaluations of Values Can be Different in Humans and AIs}
% \subsubsection{Expectations and Evaluations of Values Can be Different in Humans and AIs}
% % \mbox{}
% Due to the fundamental differences between humans and AI models, the expectations for evaluating certain values can vary between the two. For instance, while human honesty can hardly be assessed except observable actions, for AI models the expectations might be higher. 
% It could involve reverse-engineering the computational mechanisms and representations learned by neural networks into concepts understandable to humans. 
% This approach, known as \textit{mechanistic interpretability}, provides a in-depth understanding of how AI models operate~\cite{bereska2024mechanistic}.
% Future research should focus on evaluating AI values and calibrating human expectations of these values.






% \subsubsection{Customization}
% Given the diverse human values, it would be important to develop customizable (personalized) AI models to align with the the specific user groups, by referring to Section~\ref{sec:customization}, instead of consider and design AI model with general and ambiguous value sets, which can potentially include undesired values. Additionally, it is also important to evaluate the model alignment with more fine-grained human values by referring to the value category summarized in Section~\ref{sec:value_category} and \ref{sec:gap_value}. Customized (personalized) AI models will become more popular as 











% Current AI development studies primarily achieve the alignment goals by learning the models from a collection of human instructions and rating and ranking, with the hope that AI could infer human values (preferences and similar others) in a data-driven manner.
% % 
% However, designers are often unable to completely specify all important values and constraints, also, couldn't explain and control what AI actually learned from data.
% 
% 
% Instead of resorting to easy-to-specify but fallible proxy goals (\eg maximizing the approval of human overseers), future studies should consider more explainable and controllable methods to specify human values for AI. 
% 
% One possible solution could be to encode principles in model learning and allow human steerability during inference.
% % 
% Based on the diverse interaction formats of collecting and representing human values introduced in Section~\ref{sec:gap_interaction}, AI developers can potentially design more diverse approaches to collect alignment goals (\eg human values and feedback) to improve AI alignment. 
% % 



==> sections_ckpt_1120/framework.tex <==

\begin{figure*}[!t]
  \centering
  \includegraphics[width=.96\textwidth]{figures/ai2human1.pdf}
  \caption{The fine-grained topology of 
  % ~\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em}~
  ``Align \textcolor{hua-blue}{AI} to 
  % \textcolor{hua-yellow}{$\mapsto$} 
  \textcolor{hua-red}{Humans}'' direction, which studies mechanisms to ensure that AI system's objectives match those of humans'. The goal is to integrate human specification to train, steer and customize AI systems.
  % % % //
  % (MoralExceptQA~\cite{jin2022make}
  % % (Big Five personality)\cite{jiang2023evaluating},
  % (Interactive Eval of ML)\cite{cabrera2023zeno},
  % Social Norms\cite{ammanabrolu2022aligning},
  % Self-Enhancement\cite{he2023interaction}
  % trustworthy \cite{banovic2023being}
  % safety \cite{qi2023fine},
  % Diversity \cite{bakker2022fine}
  % Usability \cite{yang2023intelmo}
  % RRHF \cite{yuan2024rrhf}
  % Principles \cite{bai2022constitutional}
  % User Opinions \cite{hwang2023aligning}
  % Talebrush \cite{chung2022talebrush}
  % Discarded Options =Diamante \cite{lu2022towards}
  % Rephrase \cite{park2020scalable}
  % Holistic ToM \cite{ma2023towards}
  %   Social Relationship \cite{isajanyan2024social}
  % CAMEL \cite{li2024camel}
  % AlignDiff \cite{dong2023aligndiff}
  % Rules-of-Thumb\cite{kim2023aligning}
  % MultiTurnCleanup \cite{shen2023multiturncleanup}Coannotating~\cite{li2023coannotating}
  % Synthetic Feedback\cite{kim2023aligning}
  % RLHF~\cite{ouyang2022training}
  % RAFT\cite{dong2023raft}
  % DPO\cite{rafailov2024direct}
  % PRO\cite{song2024preference}
  % Humanoid Agents\cite{wang2023humanoid}
  % CRITIC\cite{gou2023critic}
  % Quality-Diversity\cite{bradley2023quality}
  % Winoqueer\cite{felkner2023winoqueer}
  % GPO\cite{zhao2023group}
  % MORAL\cite{peschl2022moral}
  % Debiasing Adapter\cite{sun2022bertscore}
  % Group-Adapted Fusion\cite{shen2022improving}
  % Dynamic Memory\cite{wang2023ldm}
  % IGL\cite{maghakian2022personalized}
  % Collective-Critique\cite{lahoti2023improving}
  % Find Similar Users\cite{welch2022leveraging}
  % SENSEI\cite{liu2022aligning}
  % Finspector\cite{kwon-mihindukulasooriya-2023-finspector}
  % LM-Emulated Sandbox\cite{ruan2023identifying}
  % Dromedary\cite{sun2024principle}
  % Dissenting Human Voices\cite{lee2023can}
  % AlpacaFarm\cite{dubois2024alpacafarm}
  % Gentopia\cite{xu2023gentopia}
  % Uni-RLHF\cite{yuan2024uni}
  % CrowdPlay\cite{gerstgrasser2021crowdplay}
  % Potato\cite{pei2022potato}
  }
  \label{fig:ai2human}
  \vspace{-1.5em}
\end{figure*}




This section introduces the \textbf{Bidirectional Human-AI Alignment} framework, which encompassing two interconnected alignment directions, as shown in Figure~\ref{fig:teaser}.
% 
% 
% 
% \reshmi{R:strikeoff from here} developed from the systematic literature review.\\
% 
% 
% \reshmi{R: To comprehensively include ongoing research and discussion alignment, we design a novel framework to \textbf{STRUCTURALLY} organize and think about how to ``Align \textcolor{hua-blue}{AI} to 
% % \textcolor{hua-yellow}{$\mapsto$} 
% \textcolor{hua-red}{Humans}'' and ``Align \textcolor{hua-red}{Humans} to 
% % \textcolor{hua-yellow}{$\mapsto$} 
% \textcolor{hua-blue}{AI}''.} \\
% % 
% % 
% To encompass the ongoing, mutual process of human-AI alignment, we design the framework to include: ``Align \textcolor{hua-blue}{AI} to 
% % \textcolor{hua-yellow}{$\mapsto$} 
% \textcolor{hua-red}{Humans}'' and ``Align \textcolor{hua-red}{Humans} to 
% % \textcolor{hua-yellow}{$\mapsto$} 
% \textcolor{hua-blue}{AI}''.
% 
% As shown in Figure~\ref{fig:teaser}, 
The~\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em} ``Align \textcolor{hua-blue}{AI} to 
% \textcolor{hua-yellow}{$\mapsto$} 
\textcolor{hua-red}{Humans}'' direction studies mechanisms to ensure that AI systems' values match those of humans' (Section~\ref{sec:ai2human1} and \ref{sec:ai2human2}). 
We identify two crucial research questions to be addressed in this direction: \textbf{RQ1.} \emph{What relevant human values are studied for AI alignment, and how do humans specify these values?} and \textbf{RQ2.} \emph{How can human values be integrated into the development of AI?}
% 
% 
% 
% 
In comparison, the~\hspace*{.0em}\numimg{figures/B.pdf}\hspace*{-.1em} ``Align \textcolor{hua-red}{Humans} to \textcolor{hua-blue}{AI}'' direction investigates the humans' cognitive and behavioral adaptation to the AI advancement (Section~\ref{sec:human2ai3} and \ref{sec:human2ai4}). We recognize two imperative research questions along this direction: \textbf{RQ3.} \emph{How might humans learn to perceive, explain, and critique AI?} and \textbf{RQ4.} \emph{How do humans and society make behavioral changes and react to AI advancement?}.
% 
We address the four questions by elucidating the fine-grained typologies and literature solutions derived from our systematic review, as delineated in Figure~\ref{fig:ai2human} and Figure~\ref{fig:human2ai}, respectively.
% 
% To probe into the research challenges and existing exploration of the solutions in literature, we further developed the fine-grained typologies (in Figure~\ref{fig:ai2human} and Figure~\ref{fig:human2ai}) to extend the high-level framework in Figure~\ref{fig:teaser}.
% 
% 
% 
% 
% % 
% RQ1. \emph{Which human values have AI models aligned with, and how have these values been represented?}; RQ2. \emph{How can human values be integrated into the development of AI?} RQ3. \emph{How could humans perceive, explain, and criticize AI cognitively?} and RQ4. \emph{How will humans and society make behavioral changes and reactions to AI advancement?}
% 
% 
% Based on the outlined definitions and the associated literature reviews over 400 papers, in this section, we present \emph{bidirectional human-AI alignment} as a structured way to examine and explore the multidimensional space of the alignment between human and AI (Figure~\ref{fig:teaser}). 
% % 
% 
% 
% 
% 
% We first describe the motivation of the proposed \emph{bidirectional human-AI alignment} framework by introducing ``\emph{why we consider the bidirectional alignment process as a holistic loop}'' and ``\emph{what are the pivotal research questions we examine in this bidirectional process}''.
% 
% % 
% \hua{write down a use case to motivate the framework.}
% \hua{example of constitutional AI. An analogy of the car to }
% \hua{introduce the 4 key research questions.}
% 
% 
% https://www.anthropic.com/news/collective-constitutional-ai-aligning-a-language-model-with-public-input
% 
% 
% % 
% As scoped in Section~\ref{sec:scope}, our \emph{bidirectional human-AI alignment} framework encompasses two imperative paradigms: \emph{aligning AI to humans} (Section~\ref{sec:ai2human1} and \ref{sec:ai2human2}) and \emph{aligning humans to AI} (Section~\ref{sec:human2ai3} and \ref{sec:human2ai4}).
% We further identify the four pivotal research questions in the bidirectional human-AI alignment process, including: RQ1. \emph{Which human values have AI models aligned with, and how have these values been represented?}; RQ2. \emph{How can human values be integrated into the development of AI?} RQ3. \emph{How could humans perceive, explain, and criticize AI cognitively?} and RQ4. \emph{How will humans and society make behavioral changes and reactions to AI advancement?}
% Next, we delve into the investigation of each research question in depth below.
% % 
% 
% \hua{we might 1) slightly adjust the framework details after finishing our ongoing rigorous coding (Apr/27-May/5). 2) will reduce the length of Sec4 to be more concise later.}
% 
% 
% 
% 
% 
% 
% 
% 
% 
\newline
\newline
\noindent{\textbf{DIRECTION-I: ~\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em} ALIGN \textcolor{hua-blue}{AI} to 
% \textcolor{hua-yellow}{$\mapsto$} 
\textcolor{hua-red}{HUMANS}}} 




% % outer-alignment v.s. inner alignment.
% \reshmi{R: The first step of bi-directionally aligning AI and humans, we propose that developers and researchers start by integrating human specifications to train, steer and customize AI systems.

\noindent
This direction delineates alignment research from \textbf{AI-centered perspective} (e.g., ML/NLP domains) and provides \textbf{AI developers and researchers} with approaches for two main challenges:
% The two main challenges involved in this direction include: 
carefully specifying the values of the system, and ensuring that system adopts the specification robustly~\cite{wiki_AI_alignment,ngo2022alignment}.
Therefore, as shown in Figure~\ref{fig:ai2human}, we explore the two core research questions in this direction as: \textbf{RQ1.} Human Values and Specifications (Section~\ref{sec:ai2human1}) and \textbf{RQ2.} Integrating Human Specifications into AI (Section~\ref{sec:ai2human2})
% }\\





% Studies in this direction aim to integrate human specifications to train, steer and customize AI systems.
% The two main challenges involved in this direction include: carefully specifying the values of the system, and ensuring that system adopts the specification robustly~\cite{wiki_AI_alignment,ngo2022alignment}.
% Therefore, as shown in Figure~\ref{fig:ai2human}, we design the two core research questions in this direction as: \textbf{RQ1. Human Values and Specifications} (Section~\ref{sec:ai2human1}) and \textbf{RQ2. Integrating Human Specifications into AI} (Section~\ref{sec:ai2human2})





% To address the two challenges, we 
% To address these two problems, we develop the typology of 
% (Section~\ref{sec:ai2human1} and \ref{sec:ai2human2}).






\subsection{Align \textcolor{hua-blue}{AI} to 
% \textcolor{hua-yellow}{$\mapsto$} 
\textcolor{hua-red}{Humans}: \hspace*{-0.0in} \img{figures/rqs1.pdf} Human Values and Specifications}
\label{sec:ai2human1}



% 
% \subsection{Align AI to $\mapsto$ Human with Interaction}
% \label{sec:ai2human}


% RQ1. What are the human values, and how do humans specify them for AI alignment? We structure existing literature to address this research question by answering the following questions: What values have been aligned by AI? (Section 4.1.1) and then exploring how humans could interactively specify values in AI development (Section 4.1.2).


% \textbf{RQ1. Which human values have AI models aligned with and how have these values been specified?}
% \textbf{RQ1. What are the relevant human values, and how do humans specify them for AI alignment?}
\textbf{RQ1: What relevant human values are studied for AI alignment, and how do humans specify these values?}
% 
We structure existing literature to address this research question by answering the following ``\textbf{\textcolor{hua-green}{Sub-Research Questions}}'':
\emph{What values have been aligned by AI?}
(Section~\ref{sec:value_category}) and then exploring
\emph{How humans could interactively specify values in AI development?}
(Section~\ref{sec:value_specification}). 
As shown at the top of Figure~\ref{fig:ai2human}, particularly, we articulate the ``\rqadim{Dimensions}`` we summarized to answer each of these sub-research questions, and provide ``\rqacode{Codes}`` associated with ``Example Papers'' that have been studied in each dimension.
% 
% 
% Figure~\ref{fig:ai2human} shows the taxonomy of \emph{Aligning AI to Humans} Research Question 1 (RQ1), in which we are primarily interested in exploring the research questions about \emph{categorizing aligned human values} and \emph{intergrating human values into AI}. We present the detailed dimensions and codes as below.


\subsubsection{\emph{\textbf{\textcolor{hua-green}{Categorizing Aligned Human Values}}. \textbf{\textit{What values have been aligned with AI?}}}}
\label{sec:value_category}
\mbox{}
% 
% 
% 
% To address how AI models can align with human values, a first step is to develop a detailed taxonomy of alues and structure them into a usable framework. 
% This task is inherently difficult because the notion of human values is nebulous and identifying concrete elements of these values through daily interactions and extensive data can be challenging.
% 
To clarify and systematically understand human values relevant to human-AI alignment, we leverage the adapted ``Schwartz Theory of Basic Values'' introduced in Section~\ref{sec:human_values_definition}, 
and examine the category of aligned human values from the two dimensions of ``Sources'' and ``Types''.
% 
% we consolidated the structure and taxonomy of human values using a combination of top-down and bottom-up methods based on 
% We use and slightly adapt the human values taxonomy based on 
% the Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012refining,schwartz2012overview}.
% , which offers is a universal model outlining broad values that steer human behavior grounded in psychology.
%and has been adopted in previous NLP research \cite{kiesel2022identifying}.
% We describe the levels of values and the five higher-order value types, and present a detailed discussion and taxonomy in Section~\ref{sec:gap_value}.



\rqadim{Sources of Values.} 
% 
This dimension examines the three sources of human values~\cite{schwartz1994there}.
\rqacode{Individual} sources indicate values from individuals comprise universal needs of individuals as biological organisms~\cite{schwartz1994there} or prioritize personal interests~\cite{kiesel2022identifying,jin2022make}.
At this level, value alignment can be usually assessed independently of the context of interaction. 
This perspective highlights the values about technical capabilities of AI models, including factuality~\cite{roit2023factually,hu2024do}, calibration~\cite{liu2023lightweight}, output diversity~\cite{bradley2023quality}, and model inductive bias~\cite{si2023measuring}. 
Additionally, this code includes research on aligning model behaviors with the characteristics and preferences of individual humans, e.g., 
predict human moral judgements and decisions~\cite{jin2022make},
% personality traits guided by the Big Five personality model~\cite{jiang2023evaluating,jiang2023personallm} 
and cognitive biases~\cite{jones2022capturing,koo2023benchmarking}.
% 
% 
% 
\rqacode{Social} sources mean values from the social groups include universal requirements for smooth functioning and survival of groups~\cite{schwartz1994there,ammanabrolu2022aligning}.
Value alignment at this level transcends personal interactions and emphasizes the broader categories defined by shared experiences, identities, cultures, norms, and more~\cite{santy2023nlpositionality}.
Research in this area often targets the alignment of AI behaviors with the general preferences of humans~\cite{hendrycks2020aligning,bakker2022fine,lee2023can}.
Additionally, there are efforts aimed to align AI with specific targeted groups, examining issues through the lenses of fairness~\cite{fleisig2023fairprism}, social norms~\cite{sky2023sociocultural}, morality~\cite{prabhumoye2020case,rao2023ethical}, and beyond.
% 
% 
\rqacode{Interactive} sources
% \citet{schwartz2012overview} 
considers values at the interaction level to include
universal requisites of coordinated social interaction~\cite{schwartz1994there,schwartz2012overview}, which typically occurs in interpersonal situations, such as in the dynamics of speaker-receiver relationships during language communication~\cite{hovy2021importance,cabrera2023zeno}.
% % At this level, value alignment typically occurs in interpersonal situations, such as in the dynamics of speaker-receiver relationships during language communication~\cite{hovy2021importance}.
% \hua{emphasize interaction to be human-AI interaction}.
In the context of ``human-AI alignment'', we adjust the definition of \emph{Interaction} values to be the AI values that humans expect for AI as tools, such as Usability~\cite{zhang2023visar}, Autonomy~\cite{wang2023humanoid}, among others.
% 
% 
Research along this line focuses on alignment strategies to enhance human-AI interaction~\cite{gupta2022dialguide,oh2023pk}, collaborative decision-making~\cite{gajos2022people,yang2023harnessing}, and trust~\cite{buccinca2021trust,dhuliawala2023diachronic}.
% There also exist applications in teacher-student interactions~\cite{wang2021towards,lu2023readingquizmaker}.
% % 



\rqadim{Types of Values}. In this dimension, we introduce the five high-order human values derived from a combination of the Schwartz Human Values~\cite{schwartz1994there} and empirical values studies from the surveyed papers. We provide a more in-depth taxonomy of value types in Section~\ref{sec:gap_value}, including the relationship of these five types and more nuanced value categories.
% 
\rqacode{Self-Enhancement} refers to a set of self-protective and personal values that emphasize enhancing self-esteem and a sense of personal worth~\cite{sedikides1995multiply,he2023interaction,xu2023lemur,huang2023humanity,park2023generative,kang2023values,ye2023flask,lima2021human,santurkar2023whose}.
One of the most important aspect is \textit{achievement}, is competence as judged by social standards, which includes general capability (effectiveness/efficiency) as covered by the majority of the research~\cite{guo2023beyond}.
Another dimension is \textit{power}, which relates to social status and prestige, as well as control or dominance over people and resources~\cite{pinski2023ai}.
% 
% 
% 
\rqacode{Self-Transcendence} refers to a set of self-expanding and socially-focused human values that emphasize expanding beyond oneself~\cite{frankl1966self,banovic2023being,wu2023cross,jin2022make,he2023hi,huang2023humanity,ma2023towards,isajanyan2024social,he2023interaction,nie2024moca,santurkar2023whose,ramezani2023knowledge,sheng2021societal,goldfarb2023prompt}.
One critical aspect is \textit{benevolence}, which relates to preservation and enhancement of the welfare of people with whom one is in frequent personal contact.
Extensive efforts have investigated the values including helpfulness~\cite{bai2022training}, honesty/factuality~\cite{hu2024do}, responsibility/accountability~\cite{solyst2023would}.
Another critical aspect is \textit{universalism}, which relates to understanding, appreciation, tolerance and protection for the welfare of all people and for nature.
Researchers have looked into values including inclusion/broad-mindedness~\cite{bakker2022fine,dong2023aligndiff} and equality/fairness~\cite{shen2022improving,wang2023democratizing}.
% 
% 
% 
\rqacode{Conservation} refers to a set of self-protective and socially-focused human values that hold and safeguard traditional institutions and customs~\cite{conservatism,qi2023fine,zagalsky2021design,lai2022human,santy2023nlpositionality,zhu2023unmasking,zhou2023realbehavior}.
Under conservative values, people are concerned about \textit{security} (Ssafety, harmony, and stability of society, relationships, and oneself), \textit{tradition} (Respect for and acceptance of the customs and ideas provided by traditional culture or religion), and \textit{conformity} (restraint of actions, inclinations, and impulses likely to upset or harm others and violate social expectations or norms).
Exemplar studies in this field include safety~\cite{anwar2024foundational}, 
% qi2023fine,dai2023safe,
mental health~\cite{liu2023chatcounselor}, and cultural moral norms~\cite{ramezani2023knowledge}.
% 
% 
% 
\rqacode{Openness to Change} refers to a set of self-expanding and personally-focused human values motivated by an anxiety-free need to grow, in contrast to conservation~\cite{bakker2022fine,lima2020collecting,ashktorab2020human,jiang2023evaluating,lima2020collecting,kang2023values,10.1145/3544548.3580903,yan2023complex,hosking2023human,wu2023cross,kapania2023hunt}.
Under this type, people are concerned about \textit{stimulation} (seeking excitement, novelty, and challenges in life), \textit{hedonism} (pursuing pleasure and sensuous gratification for oneself), and \textit{self-direction} (independent thought and action—choices, creativity, and exploration).
Exemplar studies in this field include understanding of privacy~\cite{mireshghallah2023can}
% ,yao2024survey
and creativity~\cite{isajanyan2024social,ashkinaze2024ai}.
% 
% 
We adopt the four high-order human values from Schwartz Human Values~\cite{schwartz1994there}, supplementing them with additional values empirically collected from survey papers as shown in Figure~\ref{fig:value_taxonomy}.
Additionally, as the conventional theory is missing the context of AI-system and human-AI interactions, we introduce a new high-order value type called \rqacode{Desired Values for AI Tools}. This category encompasses the values humans expect from AI when used as tools in ``human-AI interaction''~\cite{yang2023intelmo,zhang2023visar,oh2023pk,bakker2022fine,boyd2021datasheets,wang2023humanoid,paleja2021utility}. These values include \emph{usability} (competence according to the human experience on AI functionality) and \emph{human-likeness} (resemblance to human intelligence and behavior). Exemplary studies in this area include assessments of AI usability~\cite{zhang2023visar} and autonomy~\cite{wang2023humanoid}.



\subsubsection{\emph{\textbf{\textcolor{hua-green}{Interaction Techniques to Specify AI Values}}.
\label{sec:value_specification}
\textbf{\textit{How humans could interactively specify values in AI development?}}}} This sub-research question investigates how human values are interactively\footnote{
We define "interactions" broadly to encompass both "synchronous" and "asynchronous" interactions between humans and AI:
(1) ``Synchronous Interactions'' indicates real-time exchanges where humans and AI systems interact simultaneously. 
% Examples include live chatbots, virtual assistants, and real-time decision-making systems where immediate responses are required.
(2) ``Asynchronous Interactions'' allows for delays between actions and responses, such as data annotations by humans to train the AI models.
% and AI system that processes human inputs and provides outputs after a certain period.
% By including both synchronous and asynchronous interactions, we aim to cover the full spectrum of ways in which humans and AI systems can communicate and collaborate.
} specified for AI systems to ensure alignment. It aims to elucidate the interaction techniques by which AI systems manifest or instantiate human values, thereby revealing the underlying mechanisms that shape their behavior or functionality. 
\mbox{}

\rqadim{Explicit Human Feedback}. This dimension refers to the direct specification of human values through explicitly defined formats or mechanisms. 
% These formats support humans to directly provide explicit and accessible values to the AI system, enabling it to incorporate these values into its decision-making processes or outputs.
% 
% 
% 
% 
\rqacode{Principles} provides AI systems with explicitly defined principles, guidelines, or rules that dictate behavior or decision-making in alignment with human values~\cite{petridis2024constitutionmaker,bai2022constitutional}.
% For example, 
% \emph{ConstitutionMaker} \cite{petridis2024constitutionmaker} uses principles converted from feedback to critique LLMs; 
% ConstitutionalExperts \cite{petridis2024constitutionalexperts} attempts to learn principle-based prompts that align LLMs with human values. 
% Example: ethical principles, fairness criteria, privacy policies.
% 
% 
% 
% 
\rqacode{Rating and Ranking} is widely used to assign numerical scores or rankings to options or outcomes based on their alignment with human values~\cite{dai2023safe,yuan2024rrhf}. 
% For example, \citet{dai2023safe} aligns LLMs with preference feedback over helpfulness and harmlessness from humans to make models generate safer content. 
% 
% 
% 
% 
\rqacode{Natural Language Interaction/Conversations} allows humans to interact with AI systems through natural language interfaces to express and communicate human values~\cite{bai2022constitutional,hwang2023aligning,guo2023beyond,feng2019can,yao2023improving,lin2023unlocking,hong2022scholastic,shen2023convxai,zhang2021human}.
% Example: conversational agents, chatbots, voice assistants.
% 
% 
% 
% 
For \rqacode{Multimodal Feedback}, human values can also be provided in multiple modalities, such as sketches/images and gestures~\cite{chung2022talebrush}, to convey human values~\cite{chen2022hint,geva2022lm,wu2022ai,jorke2023pearl}. 
% One example is in \emph{TaleBrush} \cite{chung2022talebrush}, sketches corresponding to plot development trends drawn by users are collected to align pre-trained language models in creating stories. 
% 
% 
% 
% 




\rqadim{Implicit Human Feedback}.
% There also exist cases where human values can hardly be clearly defined, making human values impossible to be represented in explicit formats or simulated via models. In such cases, 
This dimension refers to the indirect representation or inference of human values within AI systems through patterns, signals, or cues embedded in the data or decision-making processes. 
% These formats do not explicitly encode human values but instead rely on implicit indicators or contextual clues.
% 
% 
% 
% 
\rqacode{Discarded Options} refers to the options or choices that human discard when interacting with AI systems during the decision-making processes, which also potentially infer human values~\cite{park2020scalable}.
% can potentially infer human value
% Human values may also be inferred based on the options or choices that are discarded or not selected by the AI system in the decision-making processes
% Example: preference inference, choice modeling.
% 
% 
% 
% 
\rqacode{Language Analysis} means that textual data and language patterns can also contain rich information to identify implicit references to human values or value-related concepts~\cite{lu2022towards}.
% For example, 
% Example: sentiment analysis, topic modeling, keyword extraction.
% 
% 
% 
\rqacode{Theory of Mind} refers to the ability of agents and people to attribute mental states, such as beliefs, intentions, desires, emotions, knowledge, percepts, and non-literal communication, to themselves and others~\cite{ma2023towards}. 
% These mental states, such as beliefs, intentions, desires, emotions, knowledge, percepts, and non-literal communication, are only directly accessible to the subject, while others must infer their existence from observable behaviors or expressions. 
% This cognitive capability allows individuals to predict and interpret the actions of others based on the mental states they presume them to have.
% propose a holistic survey.
% 
% 
% =====================================================
% =====================================================
\rqacode{Social Relationships} refers to the implicit values derived from analyzing human social relations and behaviors, which are derived from external sources (\eg social network) that can inherently reflect their values~\cite{isajanyan2024social}.









\rqadim{Simulated Human Value Feedback.} When human values in explicit formats are expensive or impossible to collect, one may simulate human-like feedback within AI systems to approximate human responses and preferences regarding specific values. 
% This feedback often involves training AI models or evaluating their performance in relation to human values.
% 
% 
% 
% 
% \rqacode{Models to auto-simulate human feedback} 
\rqacode{Human Feedback Simulators}
uses computational algorithms to simulate human-like feedback on values, based on predefined criteria or training data~\cite{petridis2024constitutionalexperts,li2024camel}.
% ,ouyang2022training,li2024camel
% For each format of explicit human value representations, an auto-simulation model or algorithm could be constructed accordingly. 
% For example, 
% \emph{ConstitutionMaker} \cite{petridis2024constitutionmaker} uses principles converted from feedback to critique LLMs; 
% \citet{petridis2024constitutionalexperts} attempts to learn principle-based prompts that align LLMs with human values; 
% RL-based algorithms like RLHF \cite{ouyang2022training} incorporate reward models that mimic human ratings or preferences. 
% CAMEL \cite{li2024camel} introduces the concept of ``AI user'' to automatically provide human-like conversational feedback via role-playing. 
% Example: generative models, reinforcement learning algorithms.
% 
% 
% 
% 
% \rqacode{Data likelihood in a reference set}
\rqacode{Comparison to Human Data}
refers to developing techniques that assess the likelihood or probability of AI-generated outputs matching human behaviors in a reference set or dataset~\cite{dong2023aligndiff}.
% Such representation often can be found in alignment for robotics. For example, \emph{AlignDiff} \cite{dong2023aligndiff} evaluates model performance by comparing model behaviors to target behaviors with mean absolute error. 
% 
% 
% =====================================================
% =====================================================
\rqacode{Synthetic Data} curates data by generating synthetic comparisons based on naive assumptions or heuristic rules, followed by post-validation to ensure feedback quality~\cite{kim2023aligning}.



\subsection{Align  \textcolor{hua-blue}{AI} to 
% \textcolor{hua-yellow}{$\mapsto$} 
\textcolor{hua-red}{Humans}: \hspace*{-0.0in} \img{figures/rqs2.pdf} Integrating Human Specifications into AI}
\label{sec:ai2human2}





\textbf{RQ2. How can human values be integrated into the development of AI?}
Existing studies have explored diverse methods to integrate human values into AI. 
% 
We structure them by summarizing \emph{how to integrate general human values (Section~\ref{sec:general_value}) and customized human values (Section~\ref{sec:customization}) throughout AI development stages?}, and then elaborating \emph{what are the evaluation methods (Section~\ref{sec:evaluation}) and supported platforms (Section~\ref{sec:ecosystem}) for the AI development}? 
Additionally, we answer the four ``\textbf{\textcolor{hua-blue}{Sub-Research Questions}}'' by introducing the answer ``\rqbdim{Dimensions}`` and providing ``\rqbcode{Codes}`` associated with ``Example Papers''.
% 
% % 
% Figure~\ref{fig:ai2human} also shows the taxonomy of \emph{Aligning AI to Human} Research Question 2 (RQ2), in which we focus our efforts to explore the research questions about \emph{how current AI model and application designs adapt to established human norms}. We expand on the dimensions of how current research has attempted to align AI models/applications to Humans, and corresponding codes in the sections.




\subsubsection{\emph{\textbf{\textcolor{hua-blue}{Integrating General Values to AI}}}: \textbf{how to incorporate general human values into AI development?}}
\label{sec:general_value}
\mbox{}
This sub-research question focuses on the process of incorporating broad, universally recognized human values into the development of AI systems.
% 
The goal is to ensure that AI systems align with overarching ethical principles and societal norms, thereby promoting trust, acceptance, and responsible use.



\rqbdim{Instruction Data.} This dimension refers to the types of data and processes used to provide guidance or direction to AI systems during their development. 
% These instructions help AI systems understand and incorporate broad, universally recognized human values into their design and decision-making processes. 
% \newline
% 
% 
% 
% 
\rqbcode{Human Annotation} makes data with human-generated labels or annotations that indicate the presence or relevance of specific human values~\cite{shen2023multiturncleanup,pei2022potato}. 
% Observed examples of this are labeled datasets and human-generated tags. Key instances of Human Annotation usage is seen in \textit{MultiTurnCleanup}~\cite{shen2023multiturncleanup} and \textit{Potato}~\cite{pei2022potato}.
% \newline 
% 
% 
% 
% 
\rqbcode{Human-AI CoAnnotation} leverages both human expertise and AI capabilities to collaboratively annotate the data 
% with both human and AI-generated labels or annotations to leverage human expertise and AI capabilities
~\cite{sun2024principle,li2023coannotating}. 
% Observed instances include but are not limited to crowdsourced annotations and human-in-the-loop systems. Key instances of Human-AI Co-annotation is seen in \textit{Principle-Driven}~\cite{sun2024principle} and \textit{CoAnnotating}~\cite{li2023coannotating}.
% \newline
% 
% 
% 
% 
\rqbcode{Simulated Human Data} generates synthetic or simulated data that mimics human behaviors, preferences, or decision-making processes to provide training signals for AI systems~\cite{dubois2024alpacafarm,kim2023aligning}. 
% Examples include synthetic datasets and agent-based simulations. Key instances of Human-AI Co-annotation is seen in \textit{Alpaca Farm}~\cite{dubois2024alpacafarm} and \textit{Synthetic Feedback}~\cite{kim2023aligning}.
% 
% 
% 
% 
% 



\rqbdim{Model Learning.} This dimension refers to the model architecture design and training stages after the data collection, where human values are integrated during the model learning process. 
% AI development stage where human values are integrated into the system's architecture design and learning process. 
% This stage encompasses both online and offline processes for aligning AI systems with human values. 
% \newline
% 
% 
% 
% 
\rqbcode{Online Human Alignment} integrates human values into AI systems in real-time or during active system operation, often through interactive feedback loops or adaptive learning mechanisms. Examples include real-time user feedback and online training~\cite{ouyang2022training,dong2023raft}. 
% \textit{RLHF}~\cite{ouyang2022training} and \textit{RAFT}~\cite{dong2023raft} are common methods of Online human alignment observed through previous papers. 
% \newline
% 
% 
% 
% 
\rqbcode{Offline Human Alignment} incorporates human values into AI systems prior to deployment or during offline training phases, without direct user interaction~\cite{rafailov2024direct,song2024preference,yuan2024rrhf}. 
% Examples include pre-training with annotated data, offline optimization. 
% Two primary Offline Human Alignment techniques are composed of Rank-based alignment and Language-based alignment. Popularly employed rank-based employment includes \textit{DPO}~\cite{rafailov2024direct}, \textit{PRO}~\cite{song2024preference}, \textit{RRHF}~\cite{yuan2024rrhf}. Language-based alignment includes \textit{CoH}~\cite{liu2023chain} and \textit{Second Thoughts}~\cite{liu2022second}. 





\rqbdim{Inference Stage.} This dimension involves evaluating the alignment of AI systems with human values and assessing their performance and behavior in relation to predefined criteria or benchmarks.
% This stage includes various testing methodologies and techniques to ensure that AI systems uphold human values. 
% \newline
% 
% 
% 
% 
% \rqbcode{Critical Chain of Thoughts.} Assessing the logical coherence and consistency of AI systems' decision-making processes and outputs in relation to human values~\cite{bai2022constitutional}. 
% 
% 
% Examples include  logical reasoning tests and decision tree analysis. Refined instances of Chain of Thought appear highly in \textit{Critique and Revision CoT}~\cite{bai2022constitutional}.
% 
\rqbcode{Prompting} leverages prompting methods, such as in-context learning and chain-of-thought, on trained AI systems to elicit or critique AI regarding the encoded values~\cite{bai2022constitutional,wang2023humanoid}.   
% 
\rqbcode{External Tool Interaction} integrates external tools, like code interpreter for debugging, to cross-check and refine their initial generated content~\cite{gou2023critic}. 
\rqbcode{Response Search} generates a diverse range of high-quality outputs from which to choose~\cite{bradley2023quality}.



% \rqbdim{Ecosystem and Platforms.} The ecosystem and platforms refer to the broader context in which AI systems operate and interact with other agents, platforms, or environments. This includes the infrastructure, frameworks, and technologies that support the development, deployment, and utilization of AI systems. 
% % \newline
% % 
% % 
% % 
% % 
% \rqbcode{LLM-based Agents.} AI agents or systems that are based on large language models (LLMs) such as GPT (Generative Pre-trained Transformer) models, which have been pre-trained on vast amounts of text data. Examples include chatbots and language understanding systems. Observed instances of this are in \textit{AlpacaFarm}~\cite{dubois2024alpacafarm} and \textit{Gentopia}~\cite{xu2023gentopia}. 
% % \newline
% % 
% % 
% % 
% % 
% \rqbcode{RL-based Systems.} AI systems that utilize reinforcement learning (RL) algorithms to learn and adapt their behavior based on feedback from the environment or human users. Examples include autonomous agents and game-playing bots. Key instances of RL-based Systems are seen in \textit{Uni-RLHF}~\cite{yuan2024uni}.
% % \newline




\subsubsection{\emph{\textbf{\textcolor{hua-blue}{Customizing AI Values}}}: \textbf{how to customize AI to incorporate values from individuals or human groups?}}
\label{sec:customization}
\mbox{}
This sub-research question explores the customization of AI values to align with specific contexts, domains, or user preferences.
The goal is to enhance the alignment of AI systems within specific application domains or user communities.





\rqbdim{Customized Data.} 
\rqbcode{Finetuning with Curated Datasets} aims to curate datasets for specific individuals or societal groups, and further finetune the pre-trained AI models on these specific datasetsto align them with targeted human groups and values~\citep{felkner2023winoqueer}. 
These curated datasets include data collected from socio-demographic groups~\cite{orlikowski2023ecological}, users' history data~\cite{lyu2023exploiting}, expert-selected data for imitation learning~\cite{cai2024imitation} and others.
% In \citet{felkner2023winoqueer}, authors discovered that biases against the LGBTQ+ community are exhibited by many LLMs. They showed that fine-tuning LLMs on data written by members of the specific community on social media can help mitigate the bias to some extent. 
% 
% 





\rqbdim{Adapt Model by Learning.}
% Alignment with finetuning 
This dimension
involves refining or adjusting AI values through techniques for customization, such as iterative learning process, model enhancements, or structural modifications. 
% This approach enables AI systems to adapt and optimize behavior based on feedback and experience.
% 
% 
% 
% % 
% % \newline
% \rqbcode{Model Learning Strategy - Finetuning.} Finetuning pre-trained AI models on specific datasets or tasks to align them with domain-specific values or preferences. In \citet{felkner2023winoqueer}, authors discovered that biases against the LGBTQ+ community are exhibited by many LLMs. They showed that fine-tuning LLMs on data written by members of the specific community on social media can help mitigate the bias to some extent. 
% % 
% 
% 
% \newline
\rqbcode{Group-based Learning} trains AI models from specific user groups or communities to capture group-specific values or preferences~\cite{zhao2023group}. 
% \citet{zhao2023group} proposed Group Preference Optimization (GPO) which trains a transformer model to predict preferences of specific human groups on unseen questions using few-shot examples of their preferences on given questions.
% This allows the GPO transformer to learn group-specific preferences, which are used for aligning LLM outputs to preferences of specific groups. 
% \newline
% 
% 
% 
% 
\rqbcode{Active Learning} refers to adjusting or re-aligning values through iteratively selecting and labeling data samples for AI model training based on the sample's potential to improve alignment with user preference or values~\cite{peschl2022moral}. 
% In \citet{peschl2022moral}, authors propose a method of active learning to rapidly learn the user's preferences of social norms and adapt the outputs accordingly. The approach first learns a vector-valued reward function using inverse reinforcement learning. 
% It then seeks pairwise preferences over on-policy trajectories from an expert and uses it to learn how to best combine the rewards in the vector-valued reward function to match desired behavior.  
% \newline
% 
% 
% 
% 
\rqbcode{Inserted Adapters} incorporates adapter modules or components into AI model architectures to fine-tune specific aspects or behaviors~\cite{sun2022bertscore}. 
% Example: adapter layers, and modular architectures. \citet{sun2022bertscore} introduced adapters into model architecture to reduce bias in the computation of BertScore. Instead of full-finetuning of the model which can substantially change all its parameters, adapters introduce a small number of additional parameters to tune the model's performance.
% After adding adapters, the authors train it on synthetically modified data designed to represent different protected groups. 
% This approach reduces the scoring model's bias while maintaining high performance in evaluating text.
% \newline
% 
% 
% 
% 
\rqbcode{Mixture of Experts} combines multiple specialized models or experts to collectively capture diverse perspectives and values, with each expert focusing on a specific subset of the data or problem space~\cite{shen2022improving}. 
% For instance, 
% In \citet{shen2022improving}, the Group-Adapted Fusion Network (GFN) employs specialized networks tailored to serve each group's specific needs, collectively enhancing fairness by reducing performance disparities across different groups.
% \newline
% \newline  [seems using \newline might get error lol - Hua]
% 
% 
% 
% 
\rqbcode{Enhanced Knowledge} enhances AI model's representations and embeddings with additional knowledge or context to improve alignment with user preferences or values~\cite{wang2023ldm,mishra2022towards}. 
% Dynamic memory of the users' feedback is used to augment the AI model according to \citet{wang2023ldm} and \citet{mishra2022towards}.








\rqbdim{Interactive Alignment} 
% Participatory alignment 
This dimension
involves actively engaging users or stakeholders in the process of customizing AI values to align with specific contexts, domains, or user preferences. 
% It enables users to provide direct input, feedback, or guidance to tailor AI systems according to their needs and preferences.
% 
% 
% 
% 
% \newline
\rqbcode{Interactive Learning}
enables the users to provide feedback or corrections to AI models in real time, such as using interactive tutorials and user-driven customization interfaces~\cite{maghakian2022personalized,swazinna2022user}. 
% In the work by \citet{maghakian2022personalized}, Interaction-Grounded Learning (IGL) is employed to tackle the challenge of developing representations for various user communication styles. \citet{swazinna2022user} gives users more control over the system through user-interactive offline reinforcement learning.
% 
% 
% 
% 
% \newline
\rqbcode{Steering Prompts} 
provides users with prompts or cues to steer the behavior or decision-making of AI systems towards desired outcomes or values~\cite{lahoti2023improving,fei2023mitigating}. 
% 
% Typical Examples include guiding questions and preference sliders.\citet{lahoti2023improving} propose a new prompting technique called Collective-Critique and Self-Voting (CCSV) guiding the model to generate more diverse and targeted responses through self-assessment and internal voting mechanisms.  In \citet{fei2023mitigating}, domain-context calibration adjusts model inputs using random in-domain words to correct label bias.
% 
% 
% 
% 
% \newline
\rqbcode{Proactive Alignment}
anticipates user needs and preferences based on historical data or user profiles and proactively adjusting AI systems accordingly~\cite{welch2022leveraging,shen2023convxai}. 
% Typical Examples include personalized recommendations and adaptive interfaces. \citet{shen2023convxai} proposed \textit{ConvXAI} in which  users' interaction history and current conversational context are used for personalized AI explanations and suggestions. 
% \newline





\subsubsection{\emph{\textbf{\textcolor{hua-blue}{Evaluating AI Systems}}}: \textbf{how to evaluate AI regarding human values?}}
\label{sec:evaluation}
\mbox{}
The rise in the use of LLMs has also seen the rise of automatic evaluation of generated natural language text evaluation in different contexts. But in particular, a research dimension has focused on analyzing how closely values discussed in humane context has been adapted to AI models/applications and how these are being evaluated. 


\rqbdim{Human-In-The-Loop Evaluation}. This dimension involves incorporating human judgement, feedback, or interaction into the evaluation process to assess the effectiveness, robustness, and ethical implications of integrating human values into AI systems. 
% This approach ensures that human perspectives and considerations are taken into account when evaluating AI performance.
% 
% 
% 
\rqbcode{Human Evaluation} solicits feedback, opinions, or assessments from human evaluators to gauge the alignment of AI systems with human values and ethical standards~\cite{liu2022aligning,sharma2023cognitive,ouyang2023shifted,kiesel2022identifying,hosking2023human}.
% 
% 
% Human-in-the-Loop feedback mechanism of utilizing annotations from human validators have been necessary to validate the performance of automatic evaluation methods Concurrently, it is essential to acknowledge that the introduction of bias is bidirectional and inherently embedded within the evaluation process, due to bias propagation from human annotators. 
% 
% 
% Many papers attempting to evaluate values and or textual semantics \cite{sharma2023cognitive}, \cite{ouyang2023shifted},\cite{kiesel2022identifying}, etc. , have employed human annotators to create a set of ground-truth-labels and test the automatic evaluation methods for assessing various attributes of human-value inclusion in AI model training and operation. But on the other hand, 
% For instance,
% \citet{hosking2023human} studied the error coverage in preference scores allocated during human annotation process against a set of value dimensions (harm, text relevance, fluencey, inconsistency, and factuality). They found severe under representation in assessing factuality and even semantic inconsistencies by human annotators, and thus declare that human feedback is not the gold standard that it is generally perceived as. 
% 
% 
% 
% 
% 
\rqbcode{Human-AI Collaborative Evaluation} collaboratively evaluates AI systems with both human evaluators and large language models (LLMs) to leverage the strengths of both human judgement and AI capabilities~\cite{kwon-mihindukulasooriya-2023-finspector,ammanabrolu2022aligning}.
% 
% For instance, enhancing the methods used to evaluate AI's judgement of humane values requires collaborative efforts from human-LLMs. It is crucial to hold both parties accountable for biases and strive to mitigate them through the innovation of new methods. For instance, \citet{kwon-mihindukulasooriya-2023-finspector} proposed \textit{Finspector}, a visual analytics application designed to test the robustness of foundational models and to identify biases interactively. Similarly, in a related study, Ammanabrolu et al. introduced Game-value Alignment through Action Distillation (GALAD). This method leverages the social commonsense knowledge embedded in specially trained language models to contextually learn soft constraints, thereby guiding AI agents in avoiding undesirable actions \cite{ammanabrolu2022aligning}.





\rqbdim{Automatic Evaluation}. This dimension involves using computational methods or algorithms to assess the alignment of AI systems with human values, without direct human involvement. 
% This approach leverages automated techniques to analyze AI performance and identify potential ethical implications.
% 
% 
% 
\rqbcode{Human Simulators} use simulation models or virtual agents to mimic human behavior and assess AI performance in human-like scenarios. Typical methods include agent-based simulations, synthetic user models, and others~\cite{jia2024towards,wang2023large,felkner2023winoqueer,ruan2023identifying}.
% For instance,~\citet{jia2024towards} uncovers a systematic bias in the evaluation paradigm of adopting large language models (LLMs), e.g., GPT-4, as a referee
% to score and compare the quality of responses
% generated by candidate models. 
% 
% 
% \citet{wang2023large} introduces simulation benchmark environments and the corresponding Datasets with Diverse human Demonstrations for Imitation Learning (D3IL), designed explicitly to evaluate a model’s ability to learn multi-modal behavior.
% 
% 
% 
% 
\rqbcode{Evaluation Benchmarks} establishes standardized benchmarks or metrics for evaluating AI performance in relation to human values and ethical considerations~\cite{sun2024principle,ramezani2023knowledge,hu2024do,kiesel2022identifying,rao2023ethical,lee2023can,sheng2021societal,sharma2023cognitive}.
\rqbcode{Distribution Difference} compares the difference between the output distribution from AI generations and human data to evaluate AI~\cite{patel2021stated,lee2023can}.


% For example, 
% in Ramezani et. al \cite{ramezani2023knowledge}, \textit{probes} have been used to understand how knowledge is encoded in English Pretrained Language Models (EPLMs) to represent moral norms in various countries. For understanding the perception of \textit{facts}, Hu et. al in \cite{hu2024do} introduced Pinocchio benchmark, that enables researchers to assess LLMs' ability to respond on factual knowlegede of up-to-date questions, complex factual tasks that requires multi-hop reasoning, and facts stored in structured datasets such as tables, lists, or databases. Along the similar lines, \cite{kiesel2022identifying}, firstly introduced the definition of \textit{value} and \textit{value system}, a consolidated multi-level taxonomy of 54 human value in cross-cultural setting, and then conducted comprehensive computational analysis to automatically identify human values from benchmarks. Moreover, in \cite{rao2023ethical} Rao et al., came up with a method for decoupling ethical policies and value alignment from LLM training, while instead infusing generic ethical reasoning abilities to AI models. They also developed an extensive framework for specifying ethical policies and evaluating generic ethical reasoning capabilities of LLMs, with the introduction of a reference dataset to understand dilemmas, policies and moral types.
% 
% 
% 
% In a closely related direction of work utilizing extensive computational methods for evaluating value inclusion in AI models and applications, \cite{lee2023can} Lee et al. leverages Log Probability Estimation (LPE) and Monte Carlo Estimation (MCE) to jointly test human disagreement along with LLM performance on natural language inference tasks. Additionally, in a related study, Sheng et. al in \cite{sheng2021societal}, analyzed the propensity of societal bias creep in NLG applications by surveying and identifying two evaluation methods, i.e, Absolute Evaluations, and Relative Scoring based evaluation that can help in identifying societal biases propagated by AI models and applications. 
% 
% 
% 
% Additionally, there is a growing body of research that is rigorously exploring various under-explored forms of biases and stereotypes in AI models and applications. In \cite{felkner2023winoqueer}, Felkner introduced WinoQueer (WQ) benchmark, for measuring anti-LGBTQ+ bias in LLMs, and also shared the framework used for creating WQ to aid in the development of other bias benchmarks for marginalized communities. Moreover, Sharma et al. \cite{sharma2023cognitive}, evaluated the nuanced area of manifestation of negative thoughts from LLMs, and introduced methods for re-framing these thoughts to more neutral and positive responses for bettering human interactions with AI models.










\begin{figure*}[!t]
  \centering
  \includegraphics[width=.98\textwidth]{figures/human2ai1.pdf}
    \caption{The fine-grained topology of ``Align \textcolor{hua-red}{Human} to 
    % \textcolor{hua-yellow}{$\mapsto$} 
    \textcolor{hua-blue}{AI}'' direction, which studies humans' cognitive and behavioral adaptation to the AI systems, which aims to help humans better critique, collaborate with, and co-adapt to AI.
    % % 
    % % % % % % % 
    % % % % 
    % AI Literacy\cite{long2020ai}
    % Intersectional AI:\cite{mcdonald2020intersectional}
    % Anglekindling\cite{petridis2023anglekindling}
    % XAI with Interaction\cite{tenney2020language}
    % Accuracy on Trust\cite{yin2019understanding}
    % Appropriate Reliance\cite{schemmer2023appropriate}
    % GP-TSM\cite{gu2024ai}
    % Algorithmic Fairness\cite{holstein2019improving}
    % Review of Algorithm Audits\cite{bandy2021problematic}
    % Adjusting Expectations\cite{kocielnik2019will}
    % Trust Calibration\cite{wischnewski2023measuring}
    % Specification Alignment\cite{terry2023ai}
    % AI Chains\cite{wu2022ai}
    % PATAT\cite{gebreegziabher2023patat}
    % AILA\cite{choi2019aila}
    % Scattershot\cite{scattershot}
    % Generative Agents\cite{park2023generative}
    % Collaborating Partners\cite{zagalsky2021design}
    % AI Knowledge\cite{pinski2023ai}
    % AI-MC\cite{sundar2022rethinking}
    % AI as Design Materials\cite{yildirim2022experienced}HypoCompass\cite{ma2023hypocompass}
    % Rehearsal\cite{shaikh2023rehearsal}
    % XAI Usefulness\cite{shen2020useful}
    % Human Ideas\cite{ashkinaze2024ai}
    % Privacy in LLM\cite{li2024human}
    % Incidental Learning\cite{gajos2022people}
    % Social Media Misleading\cite{10.1145/3610082}
    % Self Learning with LLM\cite{kazemitabaar2023novices}
    % Anthropomorphism\cite{cheng2022human}
    % Resist in Workspace\cite{park2021human}
    % Regulating ChatGPT\cite{hacker2023regulating}
    % Laypeople’s Expectation\cite{10.1145/3593013.3593992}
    % HR Management\cite{park2021human}
    % AI Fairness Checklist\cite{madaio2020co}
    % RealHumanEval\cite{Mozannar2024TheRE}
    % User-perceived tasks\cite{ding-etal-2023-harnessing}
    % Perceived Control~\cite{ding2023harnessing}
    % Collaborative Code\cite{Perry2022DoUW}
    % Co-design Checklist\cite{zhang2023deliberating} 
    % Regression Analysis\cite{wang2021towards}
    % Whose Opinion\cite{santurkar2023whose}
    % Chess Move Decisions\cite{Zhou2024GenerativeAI}
    % % 
  }
  \label{fig:human2ai}
  % \vspace{-1.5em}
\end{figure*}







% 
% 
% Reshmi introduced
%\rqbcode{Methods to correct human value misalignment in AI:}









\subsubsection{\emph{\textbf{\textcolor{hua-blue}{Ecosystem and Platforms}}}: \textbf{how to build the ecosystem to facilitate human-AI alignment?}}
\label{sec:ecosystem}
\mbox{}
% 
% \rqbdim{Ecosystem and Platforms.} 
The ecosystem and platforms refer to the broader context in which AI systems operate and interact with other agents, platforms, or environments. This includes the infrastructure, frameworks, and technologies that support the development, deployment, and utilization of AI systems. 
% \newline
% 
% 
% 
% 
\rqbcode{LLM-based Agents} are based on large language models (LLMs) such as GPT (Generative Pre-trained Transformer) models, which have been pre-trained on vast amounts of text data~\cite{dubois2024alpacafarm,xu2023gentopia,wu2023autogen,zhou2023sotopia}. 
% Examples include chatbots and language understanding systems. Observed instances of this are in \textit{AlpacaFarm}~\cite{dubois2024alpacafarm} and \textit{Gentopia}~\cite{xu2023gentopia}. 
% \hua{AutoGen, LangChain, Sotopia.}
% \newline
% 
% 
% 
% 
\rqbcode{RL-based Agents} are based on reinforcement learning (RL) algorithms to learn and adapt their behavior based on feedback from the environment or human users~\cite{yuan2024uni}. 
% Examples include autonomous agents and game-playing bots. Key instances of RL-based Systems are seen in \textit{Uni-RLHF}~\cite{yuan2024uni}.
% \newline
% 
% 
% % 
\rqbcode{Annotation Platforms} refers to the ecosystems that are designed to crowdsource human demonstrations as collected data for reinforcement learning~\cite{gerstgrasser2021crowdplay} and supervised finetuning learning for alignment~\cite{pei2022potato}.
% % 
% 
% 
% 
% 
\begin{table*}[ht]
\centering
% \vspace{-10pt}
\begin{tabular}[t]{@{}  !{\color[HTML]{808080}\vrule width 2pt} p{.98\textwidth} !{\color[HTML]{808080}\vrule width 2pt} @{}}
\cellcolor[HTML]{E6E6E6} 
\textbf{Underexplored Dimensions in Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-red}{Humans}} (See Sec~\ref{sec:trend} for supporting data and evidence): 
% \newline
\vspace{5pt}

1. Implicit human feedback and simulated human value feedback are under-explored in existing research work.
\vspace{5pt}

2. Developing and customizing AI during the inference stage or in an interactive way is under-explored.
% 
\vspace{5pt}

3. Human-in-the-loop evaluation is much less explored than automatic evaluation.
\end{tabular}
\end{table*}
% 
% 
\newline
% \newline
\noindent{\textbf{DIRECTION-II:~\hspace*{.0em}\numimg{figures/B.pdf}\hspace*{-.1em} ALIGN \textcolor{hua-red}{HUMANS} to 
% \textcolor{hua-yellow}{$\mapsto$} 
\textcolor{hua-blue}{AI}}} 




\noindent
\say{\emph{When interacting with people, AI agents do not just influence the state of the world – they also influence the actions people take in response to the agent, and even their underlying intentions and strategies}}~\cite{hong2024learning}.
% 
From a \emph{long-term} perspective, it is essential to consider the dynamic changes around human-AI alignment.
% 
% 
This direction outlines alignment research from the \textbf{Human-centered perspective} (e.g., HCI/Social Science domains) and provides \textbf{HCI researchers and user experience designers} with guidance for approaching two core research questions:
% 
% Therefore, research in this direction aims to help humans better understand, critique, collaborate with, and adapt to AI advancements. 
% Besides, interacting with AI could also change human cognition and social behaviors (consciously or unconsciously)~\cite{dautenhahn2000living}, so it is essential to consider this dynamic change into human-AI alignment.
% The two core research questions we identified in this direction are: 
\textbf{RQ3.} Human Cognitive Adjustment to AI (Section~\ref{sec:human2ai3}) and \textbf{RQ4.} Human Adaptive Behavior to AI (Section~\ref{sec:human2ai4}).




% \noindent
% Questions for the long-term individual cognitive and social effects of AI technology we should ask ourselves are:
% - How will agent technology affect human cognition?
% - How will using or interacting with this technology change who we are?
% % 
% If we do not ask such questions, the answers that come to us by letting things run their course in the future may be neither humane nor desirable.
% ~\cite{dautenhahn2000living}
% % 
% % 
% % 
% \textbf{What should humans do to critically adapt to AI advancement?}~\merrie{But also how can interface design support conveying AI affordances to humans and enabling them to steer AI interactions to meet their preferences?}
% \diyi{are humans adapting to AI consciously or unconsciously? }









\subsection{Align \textcolor{hua-red}{Humans} to 
% \textcolor{hua-yellow}{$\mapsto$} 
\textcolor{hua-blue}{AI}:  \hspace*{-0.0in} \img{figures/rqs3.pdf} Human's Perceptual Adaptation to AI}
\label{sec:human2ai3}
% 


\textbf{RQ3. How might humans learn to perceive, explain, and critique AI?}
% 
% 
% 
% % 
% \say{\emph{When interacting with people, AI agents do not just influence the state of the
% world – they also influence the actions people take in response to the agent, and
% even their underlying intentions and strategies~\cite{hong2024learning}.}} 
% 
Humans needs to understand AI to better specify their demands and collaborate with AI. Also, as AI systems produce a range of risks, it is important to elicit humans' critical thinking of AI instead of relying on AI blindly. Therefore, we categorize existing literature to answer the questions of \emph{how humans learn to perceive and understand AI} (Section~\ref{sec:perception}), and  \emph{how to engage in critical thinking on AI?} (Section~\ref{sec:critical_thinking}).
We also answer the two ``\textbf{\textcolor{hua-purple}{Sub-Research Questions}}'' by introducing the answer ``\rqcdim{Dimensions}`` and providing ``\rqccode{Codes}`` associated with ``Example Papers''.
% 
% 
% 
% % 
% Figure~\ref{fig:human2ai} shows the taxonomy of \emph{Align Human to AI} Research Question 3 (RQ3), in which we are primarily interested in exploring the research questions about \emph{human's perceptual adaptation to AI} and \emph{human’s behavioral adaptation to AI}. 
% In this section, we introduce literature concerning human perception and understanding of AI (Section~\ref{sec:perception}). 
% Furthermore, we advocate for the development of critical thinking regarding AI, emphasizing the importance of human agency in its utilization.
% Therefore, we introduce relevant papers addressing this theme in Section~\ref{sec:critical_thinking}.
% % 
% % 






\subsubsection{\emph{\textbf{\textcolor{hua-purple}{Perceiving and Understanding AI}}}: \textbf{how do humans learn to perceive and explain AI systems?}}
\label{sec:perception}
\mbox{} 
% This category addresses how humans perceive and make sense of AI outputs for a broad spectrum of users. 
Addressing the problem of human perception and understanding of AI includes the fundamental education and training required for less technical people to improve understanding of the behind mechanisms and outputs produced by AI systems. It includes visualizations and human-centered explanations tohelp more people learn to understand AI outputs.



\rqcdim{Educating and Training Humans}. AI is increasingly incorporated into the daily lives of a broad spectrum of users, including those with little to no technical knowledge on how AI operates. Here we discuss how to help these less technical people become more AI literate, or better trained to use AI.
% 
% 
% 
% 
\rqccode{AI Literacy and Awareness} is broadly defined as the core competencies required for less technical people to better use and collaborate with AI~\cite{long2020ai}. 
% For example, these competencies include being able to: recognize what is AI and what is not, understand that AI is actually a broad term covering a wide range of technology including robotics and machine learning, and imagine future AI applications and their outcomes \cite{long2020ai}. 
% 
% 
% 
% 
Beyond,
% core competencies,
% that establish a baseline understanding of what AI is and how it operates, 
there is also more in depth and explicit \rqccode{Training Courses} to support individuals to better collaborate and utilize AI~\cite{ketan-ai-medicine-education,mcdonald2020intersectional}. 
% 
% This training can include courses or workshops, or even entire curriculum \cite{ketan-ai-medicine-education} designed to help professionals that are increasingly using AI in their workflows. For example, recent work has proposed that the core education of medical professionals should also include data science fundamentals and other AI related courses so that they could better use and interpret the results from large, black box models providing predictions on patient health outcomes \cite{ketan-ai-medicine-education}.
% 
% 
% 
% 


\rqcdim{AI Sensemaking and Explanations}.
% For more technical users that directly rely on or use AI outputs in their work, 
To improve people's understanding of AI systems and generated outputs, various techniques and approaches have been developed to help people learn to make sense of and explain the model's outputs. 
% Here we emphasize on how to help humans learn sensemaking and explanation of AI systems.
% Concretely, these are interactive approaches to support humans better the \textit{sensemaking} of AI outputs, as well as \textit{human-centered explanations}~\cite{kaur2022sensible}.
% 
% 
% 
% 
\rqccode{Perception and Sensemaking on AI} involves the process through which humans learn to make better sense of AI mechanisms and decision makings~\cite{kaur2022sensible,sivaraman2023ignore,petridis2023anglekindling}.
% more set of techniques for understanding AI outputs~\cite{kaur2022sensible,sivaraman2023ignore}. 
% A canonical version of this is to highlight a particularly influential feature that the model relied on for a classification. For example, AngleKindling system that recommends treatments for patients with Sepsis presents a bar chart indicating the relative importance of each feature to the current prediction \cite{sivaraman2023ignore}. 
% In a similar vein, a recent system that generates potential story angles for journalists to pursue from a press release highlights the most relevant portions of the text that produced that generation; this helped journalists (1) ascertain where the angle came from as well as (2) gather more context for that angle \cite{petridis2023anglekindling}.
% 
% 
% 
% 
People also need to understand how AI systems arrive at specific generated outputs. Prior studies in \rqccode{Human-Centered Explanations} have examined various approaches and interactive techniques to increase human understanding of AI generations and outputs~\cite{tenney2020language,recommender-explanations,smith2020no}.
% Beyond visualizations there are many other mechanisms through which past work has examined helping users understand AI outputs, within \rqccode{Human-Centered Explanations}~\cite{recommender-explanations,smith2020no}.
% Explanations have been studied quite extensively within recommender systems, where many studies have compared the efficacy of different ways to explain why the user was getting a particular recommendation \cite{recommender-explanations}. For example, keywords and tags (e.g. ``comedy'' or ``award winning'') can accompany a recommendation to give users context on how the system characterizes that recommendation. Another way to explain a recommendation is by connecting it to content the user has already consumed (e.g. ``We recommend X because you have seen Y and Z''). These more natural and intuitive explanations are a few classic examples of easily-understood, human-centered explanations~\cite{smith2020no,shen2023convxai}.


% 
% 


% Typical calibration strategies include 

% -Prior to the interaction: Prior information about the system such as capabilities, reliability, consistency, consensus, distinctiveness of the automated aid’s performance, or malfunctions; training phase; cognitive forcing

% -During the interaction: Cues (alarms, warning signals, augmented reality cues, confdence cues or updates); uncertainty displays; communication style (command vs. status); explanations; interactivity (e.g., promise to perform better in the future)

% -After the interaction: Feedback type (automation feedback independent of user, feedback on trust behavior of user); performance feedback





\subsubsection{\emph{\textbf{\textcolor{hua-purple}{Critical Thinking around AI}}}: \textbf{how do humans think critically about AI systems?}}
\label{sec:critical_thinking}
\mbox{}
% 
Beyond simply perceiving and understanding AI, individuals need to compare their mental model of AI with their own mental model to judge whether the AI is behaving rationally and ethically.
Broadly, this involves exploring the ways in which humans engage in critical thinking and reflect on their interactions with and evolving understanding of AI technologies. 
% 
Here we discuss studies that help humans become more capable to identify biases and errors in AI output, and the ethical implications that arise from using AI algorithms in decision-making processes. Also, we discuss how humans need to calibrate their mental models to be more aligned with AI.
% The papers in this category relate to the fostering of informed decision-making, ethical reasoning, and responsible use of AI technologies through the development of cognitive skills and competencies related to AI literacy and awareness. This category is further broken down into two dimensions, \emph{Trust and Reliance on AI Decisions} and \emph{Ethical considerations and AI auditing}.


\rqcdim{Trust and Reliance on AI Decisions} refers to the extent to which people mentally trust the AI competency and practically rely on AI for output generation and decision making.
% individuals place confidence on the decisions and output generated by AI systems. 
% This dimension explores the factors influencing trustworthiness, perceived reliability, and the subsequent selective adoption of AI technologies. 
We use the term \rqccode{Trustworthiness} to indicate whether humans decide to trust the reliability, integrity, and competence of an AI system in delivering accurate and trustworthy decisions or recommendations to the users~\cite{yin2019understanding,ma2023should,srivastava2023role}. 
% 
% Measures to capture trustworthiness include \emph{appropriateness of Trust}~\cite{ma2023should} and \emph{lexical alignment} \cite{srivastava2023role}. 
% 
We define \rqccode{AI Reliability} as to what extent humans utilize and rely on AI to automate decision making in practice with low error rates and robustness performance~\cite{schemmer2023appropriate}.
% an evaluation of the consistency, predictability, and performance quality of AI systems across different contexts and scenarios
\cite{schemmer2023appropriate,vasconcelos2023explanations,suresh2022intuitively}. 
% Examples include error rates and robustness testing. \citet{suresh2022intuitively} had people probe a model and reason about its behavior through familiar examples grounded in domain knowledge, demnonstrating how grounding interpretability in real examples, facilitating comparison across them, and visualizing data distributions can aid in grasping a model’s uncertainty and connecting it to relevant challenges in the task. 
\rqccode{Selective AI Adoption} refers to the criteria and considerations that guide the adoption or rejection of AI technologies based on their perceived benefits, risks, and alignment with user needs and preferences~\cite{gu2024ai,vasconcelos2023explanations}.  
% One salient example is that of \emph{overreliance}, i.e., when people agree with an AI, even when it is incorrect. The associated risk-assessment framework posits that when tasks require more effort and the explanations sufficiently reduce the cost of verifying the AI, or when the explanations are easier to understand, explanations will reduce overreliance \cite{vasconcelos2023explanations}.
%Examples include risk assessment frameworks and technology acceptance models. 










\rqcdim{Ethical Considerations and AI Auditing} refers to potential moral and societal issues that arise from the development, deployment and use of AI systems, as well as systematic examination and evaluation of AI systems regarding these issues.
\rqccode{Ethical Concerns and AI Mitigation} encourages humans to carefully consider if the AI systems possess ethical concerns (\eg such as bias and discrimination, privacy violations and the potential for harm or misuse) and implement strategies and practices to address and reduce these ethical concerns associated with AI~\cite{holstein2019improving}.
% 
\rqccode{Audit Deployed AI} refers to the systematic examination of AI systems to ensure that they operate as intended, comply with ethical and legal standards, and do not cause unintended harm~\cite{bandy2021problematic}.


% includes, on one hand, human assessment of the fairness, accountability, transparency, and ethical implications of the decision-making processes embedded in AI technologies. On the other hand, we regard ethical AI practices, i.e., diversity, equity, and inclusion in AI development and deployment. 
% 
% % =====================================================
% % =====================================================
% % =====================================================
% % =====================================================
% \rqccode{Fairness and Accountability} examines the extent to which AI systems exhibit fairness, impartiality, and accountability in their decision-making processes and outcomes.
% % particularly concerning bias mitigation and fairness-aware algorithms~\cite{holstein2019improving,lee2023understanding}. 
% % Providing counterfactual examples as explanation for AI decision-making were found to support critical thinking around how to change an AI output and more rigorously review AI output than widely used AI feature-example explanations \cite{lee2023understanding}. 
% % 
% In HCI, the critical analysis of AI systems has a strong focus on \rqccode{Diversity, Equity and Inclusion}, which includes advocacy for a wide set of voices, equitable data collection practices (e.g., treatment of and access to data) and cultivating a sense of belonging in AI development and deployment~\cite{10.1145/3544548.3580903,kapania2023hunt}. 
% % The aim is to increase representation, accessibility, and fairness for diverse populations and groups who have been historically marginalized. Improving representation in the data annotation stage through removing the separation
% % between ML practitioners and data annotators who usually do not interact, combined with an intersectional shift towards annotators’ lived experiences was shown to have potential to mitigate bias in AI output \cite{kapania2023hunt}.









\rqcdim{Re-Calibrating Cognition to Align with AI}. This sub-category deals with interventions and techniques to help users adjust (1) their own mental model of how the AI operates and (2) recalibrate their perception of the AI.
% 
% 
% 
% 
\rqccode{Updating Human Mental Model of AI} means that when the AI is not aligned with humans, it is important to adjust human perceptions of the confidence in AI systems based on the model's capability and track record~\cite{he2023interaction,kocielnik2019will} .
% Example: trust calibration strategies, reliability assessments.
% For example,~\citet{he2023interaction} proposes a capability-aware shared mental model (CASMM) with the components of task grouping and negotiation, which utilize tuples to break down tasks into sets of scenarios relating to difculties and then dynamically merge the task grouping ideas raised by human and AI through negotiation.
% The result shows building CASMM boosts the accuracy and time efciency signifcantly through forming the task assignment close to real capabilities within few iterations. It helps users better understand the capability of AI and themselves.
% 
\rqccode{Recalibrating Trust and Reliability} indicates that humans adjust their perceptions of trust and reliability in AI systems based on their performance and reliability. This is also important to foster appropriate reliance and skepticism~\cite{wischnewski2023measuring}.
% 
% For example,~\citet{wischnewski2023measuring}  identifed 96 relevant publications which aimed to calibrate users’ trust in automated systems.
% To facilitate the trust calibration, one broader strategy was to implemented interventions to increase transparency (e.g., cues, warning signals, explanations). Also, automation feedback independent of user or provide feedback on trust behavior of user is also potential strategy to calibrate user trust.






%For example, \citet{shen2023convxai} borrowed inclusive design principles to frame human the evaluation of human writing processes via ConvXAI, an AI system created to support human-AI collaboration in scientific writing.
%Examples include fairness metrics and bias detection tools. 
%Example: diversity hiring practices, inclusive design principles.

\subsection{Align \textcolor{hua-red}{Humans} to 
% \textcolor{hua-yellow}{$\mapsto$}
\textcolor{hua-blue}{AI}:  \hspace*{-0.0in} \img{figures/rqs4.pdf} Human’s Behavioral Adaptation to AI}
\label{sec:human2ai4}



\textbf{RQ4. How do humans and society make behavioral changes and react to AI advancement?}
% 
As AI becomes increasingly integrated into daily life, it is essential to understand its influence on humans, encompassing both positive and negative aspects. 
% 
Moreover, it is crucial to determine how individuals and society can best and most appropriately respond to this influence.
% 
To this end, we summarize literature to answer \emph{how do humans learn to collaborate with AI in diverse AI roles?} (Section~\ref{sec:collaboration}), \emph{how humans and society are impacted by AI
% what are AI's impacts on humans and society
} (Section~\ref{sec:impacts}) and \emph{how might we assess these impacts?} (Section~\ref{sec:assessment})
We articulate the three ``\textbf{\textcolor{hua-red}{Sub-Research Questions}}'' by introducing the answer ``\rqddim{Dimensions}`` and providing ``\rqdcode{Codes}`` associated with ``Example Papers''.

% 
% % 
% % 
% In addition to examining human perception and critical thinking regarding AI, we investigate how humans adapt their behavior to AI advancements. 
% We introduce various collaborative mechanisms between humans and AI with different roles (Section~\ref{sec:collaboration})
% % 
% 
% % 
% Beyond human perception and critical thinking on AI, we further explore how humans adjust their behavior to AI advancements.
% Particularly, we not only introduce different collaborative mechanisms between humans and AI (Section~\ref{sec:collaboration}). Also, we explicitly point out potential risks and negative impacts that AI could bring to individuals and the society. In this way, we aim to provide a more objective and comprehensive view of how to \emph{align human to AI}.

\subsubsection{\emph{\textbf{\textcolor{hua-red}{Human-AI Collaboration Mechanisms}}}: \textbf{what are human strategies to collaborate with AI that have differing levels of capabilities?}}
\label{sec:collaboration}
\mbox{}
%
This category looks at many ways that humans and AI can collaborate, such as teamwork, co-creation, and coproduction. 
%forming a powerful whole when either party takes the main charge. 
% It also examines how they communicate, what each is responsible for, and what helps or hurts their success. The goal is to understand how humans and AI can best work together to achieve their goals.




\rqddim{AI Assistant for Humans} captures the essence of a symbiotic relationship where AI systems are designed to bolster human capabilities, with humans steering the interactions.  
% In this collaborative model,  LLM has become the new type of medium to facilitate interaction and collaboration. 
\rqdcode{LLM-based Demand Specification} employs LLMs to interpret and respond to human requests, powering virtual assistants and chatbots that streamline information retrieval and improve task accuracy~\cite{terry2023ai}. This naturally extends to \rqdcode{LLM-based Prompt Strategy}, which helps humans to better write prompts using 
% where the 
additional abstraction and scaffolding methods.
% are introduced on top of traditional text-to-text workflow. 
The example system can enhance humans' capability in generating intelligent prompts and suggestions, such as autocomplete and question-generation tools for LLM-based systems~\cite{wu2022ai, wang2024farsight}, facilitating humans' smooth and intuitive decision-making processes. 
In the creative arena, \rqdcode{LLM-based Prototypes} utilize AI to transform human ideas into tangible or organized concepts ~\cite{gebreegziabher2023patat}, enabling professionals to explore and refine a wide array of artistic possibilities with AI-generated options~\cite{huh2023genassist}. 
On a broader note, researchers have also explored how \rqdcode{AI-Assisted Task and Decisions} 
aims to achieve complementary performance for human-AI collaborative tasks by empower humans to discern when and how to adopt AI-assisted recommendations or AI-generated explanations for decision-making~\cite{choi2019aila,wang2022will, wang2023watch,zheng2023competent,scattershot}.  
% leverage conventional AI techniques to analyze vast datasets for predictions and recommendations, underpinning recommendation systems and predictive analytics that optimize content delivery and strategic foresight for both individual~\cite{wang2022will, wang2023watch} and group decisions~\cite{zheng2023competent}. 
% 
% % 
% % =====================================================
% % % =====================================================
% \rqdcode{Improve AI Systems} leverages human feedback and interaction to collaboratively analyze, intervene with and improve AI systems, such as fairness and accuracy performance~\cite{kwon-mihindukulasooriya-2023-finspector,piorkowski2023aimee}.


% Together, these applications of AI do not replace human expertise but significantly enhance the breadth and depth of human operation across various fields.

% %
% % \rqddim{AI Assistant for Human} describes a collaborative framework where artificial intelligence (AI) systems enhance human capabilities, with humans leading the interaction. This partnership manifests in several distinct ways across various applications. For instance, ...
% %
% %
% % 
% % 
% \rqdcode{LLM-based Demand Specification.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{LLM-based Prompt Strategy.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{LLM-based Prototypes.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{Traditional AI-Assisted Decision Making.} Definition + example papers.






\rqddim{Human-AI Partnership} refers to a collaborative relationship where humans and AI systems work together as partners, combining their respective strengths to achieve shared goals more effectively.
% 
% Humans contribute contextual understanding, creativity, and high-level reasoning, while AI excels at rapid data processing, pattern recognition, and complex computations. By synergistically melding human ingenuity with artificial intelligence capabilities, these partnerships enable innovations that harness the best of both worlds.
% 
% In a Human-AI Partnership, the symbiotic collaboration between humans and artificial intelligence systems is facilitated through various mechanisms. 
\rqdcode{Simulated Agency} enables humans to collaborate with AI partners with
% endows AI systems with 
simulated agency or autonomy (\eg autonomous agents and collaborative robots~\cite{park2023generative}) to make decisions collaboratively.
% and take actions in collaboration with human partners, 
% as exemplified by autonomous agents and collaborative robots~\cite{park2023generative}.
\rqdcode{Reciprocal Learning} focuses on how humans learn from and exchange knowledge with AI systems,
% mutual learning and knowledge exchange between humans and AI systems, 
enhancing human-AI collective capabilities and performance through knowledge-sharing platforms and collaborative filtering~\cite{zagalsky2021design,pinski2023ai}. \rqdcode{AI Delegation} allows humans to delegate AI partners to help finish tasks or responsibilities,
% to delegate tasks or responsibilities to human partners based on their expertise or preferences, 
facilitated by task assignment algorithms and workflow management systems~\cite{pinski2023ai}. 
Furthermore, \rqdcode{AI-Mediated Tasks} emphasizes how traditional human tasks or behaviors (\eg communication) would be changed by incorporating AI partners in the loop~\cite{bernstein2010soylent,sundar2022rethinking,xu2023augmenting}. 
\rqdcode{Co-Design with AI} explores AI as a design material or a partner in prototyping, which enables humans to converse with AI in situations that can collaboratively improve the design outcomes. 
\cite{yildirim2022experienced,wang2024farsight}
% coordinate activities where both human and AI entities contribute to 
% problem-solving or decision-making processes~\cite{xu2023augmenting}, as seen in crowd-computing platforms and human-in-the-loop systems~\cite{bernstein2010soylent, bigham2010vizwiz}.
% 
% These mechanisms work in concert to create a cohesive partnership, where humans and AI systems collaborate seamlessly, leveraging their respective strengths to achieve shared goals through co-creation and innovation.
% % 
% % 
% % 
% % 
% \rqdcode{Simulated Agency.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{Reciprocal Learning.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{AI Delegation.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{AI-Mediated Tasks.} Definition + example papers.











\rqddim{AI Tutoring for Human Learning} 
investigates how humans improve their learning and knowledge throughinteractions with AI tutors that can perform better than humans in some tasks.
% involves employing AI systems to provide personalized guidance and support throughout the learning process. 
With the tailored instructions and customized feedback from AI tutors, humans can enhance their the learning outcomes and facilitate mastery of new skills more effectively than traditional learning methods.
% These AI tutors leverage advanced technologies to adapt to individual needs, offering tailored instruction, customized feedback, and optimized learning pathways. By dynamically adjusting to each learner's progress and areas for improvement, AI tutoring systems aim to enhance the learning outcomes and facilitate mastery of new skills more effectively than traditional methods.
% 
% 
\rqdcode{AI Tutor for Technical Skills} refers to empowering humans to learn technical skills from AI tutors.
% One common theme of the AI tutoring system is \rqdcode{AI Tutor for Technical Skills}. 
For technical subjects like coding, AI tutors can analyze a learner's progress in real time, adjusting the pace, content, and approach to ensure a solid understanding of complex concepts and practical skills such as programming~\cite{ma2023hypocompass}. 
% Through personalized examples, interactive exercises, and immediate feedback, these systems identify knowledge gaps and provide targeted support. 
% 
% 
Similarly, \rqdcode{AI Tutor for Social and Behavioral Skills} involves enabling humans to learn social and behavioral skills from AI tutors.
% 
% The other common theme of the AI tutoring system is \rqdcode{AI Tutor for Social and Behavioral Skills}. 
% For social and behavioral skills, 
Humans can leverage virtual simulations, created by AI tutoring systems, to 
% AI tutoring systems create realistic virtual simulations for learners to 
practice public speaking, interpersonal communication, and other soft skills. By analyzing verbal and non-verbal cues, humans can receive 
% these AI tutors offer 
constructive feedback on areas such as body language, tone, and delivery from AI, ultimately enhancing their ability to communicate effectively across various settings~\cite{peng2021say, shaikh2023rehearsal}. 
% 
% As these technologies continue to evolve, AI tutoring systems hold promising prospects for reshaping the learning experience and fostering a more engaging, personalized, and effective skill-acquiring journey for individuals of all ages and backgrounds.


% % 
% % 
% % 
% % 
% \rqdcode{AI Tutor Technical Skills.} Definition + example papers.
% % 
% % 
% % 
% % 
% \rqdcode{AI Tutor Social and Behavioral Skills.} Definition + example papers.





















\subsubsection{\emph{\textbf{\textcolor{hua-red}{AI Impact on Humans and Society}}}: \textbf{how are humans influenced by AI systems
% influencing humans
?}}
\label{sec:impacts}
\mbox{}
This category explores the effects of AI advancement on human behaviors, attitudes, and societal dynamics. It involves examining the behavioral changes, adaptations, and reactions that individuals, groups and wider communities undergo in response to the proliferation of AI technologies. 
% This includes assessing the impacts of AI on employment patterns, job skills, social interactions, decision-making processes, and cultural norms. Additionally, it examines the broader societal implications of AI, such as economic disparities, ethical dilemmas, and power dynamics. 
The goal is to elucidate the multifaceted impacts of AI on human behavior and society and to inform policy-making, education, and intervention efforts.  
% This category is further broken down into three dimensions, \emph{Impact on Participatory Individuals and Groups, Societal Concerns and AI Impacts} and \emph{Reaction to AI Advancement}.


\rqddim{Impacts on Participatory Individuals and Groups} covers the effects of AI advancement on the behaviors, attitudes, and experiences of both individuals and groups. This dimension focuses on examining how AI technologies influence decision-making, creativity, privacy, and authorship. \rqdcode{Decision Making} refers to analyzing how AI technologies influence human decision-making processes, including biases, preferences, and risk assessment, in various domains such as healthcare, finance, and personal life~\cite{shen2020useful}. 
% 
% 
% 
%Example: automated decision support systems, algorithmic decision-making.
\rqdcode{Human Creativity} explores the impact of AI technologies on human creativity, innovation, and expression, including the augmentation or automation of creative tasks and the emergence of new forms of artistic expression~\cite{ashkinaze2024ai}.
% 
% 
% 
%Example: AI-generated art, creative AI tools.
\rqdcode{Privacy} relates to investigating the implications of AI technologies for individual privacy rights, data protection, and surveillance, including concerns about data collection, tracking, and algorithmic profiling~\cite{li2024human}.
% 
%Example: privacy-preserving techniques, data anonymization.
% 
% 
\rqdcode{Authorship} catalogs issues related to intellectual property, attribution, and ownership of AI-generated content, including questions of legal responsibility, copyright infringement, and plagiarism detection. Salient is that AI can produce increasingly realistic, synthetic data quickly and at low cost, which brings forth tensions around the use of such data to make decisions~\cite{hamalainen2023evaluating,10.1145/3610082}. 






\rqddim{Societal Concerns and AI Impacts} involves the broader societal implications and consequences of AI advancement on misinformation, education, social relationships, norms, job displacement, and other aspects of human society.
% 
%Example: copyright laws, attribution algorithms.
% 
% 
% 
% 
\rqdcode{Misinformation and Moderation} concerns the challenges of misinformation, disinformation, and online content moderation in the context of AI-driven information ecosystems, including concerns about algorithmic bias and filter bubbles~\cite{10.1145/3610082}. 
% 
% 
%Example: content moderation algorithms, fake news detection.
% 
\rqdcode{Impacts on Education} pertains to assessing the effects of AI technologies on education systems, learning outcomes, pedagogical practices, and workforce training, including opportunities for personalized learning and skill development~\cite{kazemitabaar2023novices}.
% 
%Example: AI-powered tutoring systems, adaptive learning platforms.
% 
% 
% 
% 
\rqdcode{Impacts on Social Relationship and Norms} explores how AI technologies shape interpersonal relationships, social interactions, and cultural norms, including changes in communication patterns, social dynamics, and ethical considerations~\cite{cheng2022human}.
% 
% 
% 
% 
\rqdcode{Workplace} refers to examining the effects of automation and AI technologies on employment patterns, job markets, and workforce dynamics, including concerns about job displacement, re-skilling, and economic inequality~\cite{park2021human}.





\rqddim{Reaction to AI Advancement} involves societal responses, regulatory frameworks, and policy initiatives aimed at addressing the challenges and opportunities posed by AI technologies. This dimension encompasses efforts to regulate AI deployment, re-calibrate societal acceptance, and manage potential backlash. For example, reaction to bias and discrimination in algorithmic decision making can depend on how people perceive the machine and the context of use,  i.e., if the machine is considered an actor embedded in social structures that call for blame
when harmful decisions are made \cite{lima2023blaming}. \rqdcode{AI Regulatory and Policy} includes regulatory frameworks, legal frameworks, and policy initiatives aimed at governing AI development, deployment, and use, including concerns about ethics, safety, and accountability~\cite{hacker2023regulating,lucaj2023ai}.
% 
%Example: AI ethics guidelines, regulatory compliance frameworks.Definition + example papers.
% 
% 
% 
% 
\rqdcode{Shifts in AI Acceptance} relates to investigating societal attitudes, organizational practices, and acceptance of AI technologies over time in practice, including shifts in public opinion and AI utilization by humans and institutes regarding AI deployment and impact~\cite{10.1145/3593013.3593992,10.1145/3593013.3593999}.
% 
% 
% 
% % =====================================================
% % =====================================================
\rqdcode{Surveillance and Intervention} emphasizes the need for transparency, monitoring, and human oversight in the algorithmic decision-making process. This approach enables better human control over AI systems and helps mitigate potential risks associated with their use~\cite{park2021human}.
% 
% calls for incorporating transparency, surveillance and human intervention to algorithmic decision-making process. In this way, human can better control AI and prevent AI from risky impacts in practice~\cite{park2021human}.
% 
\rqdcode{Responsible AI Checklists} involves the creation of ethical guidelines, such as those focusing on fairness and transparency, to ensure the responsible development and deployment of AI systems. These published principles serve as a foundation for guiding ethical AI practices~\cite{madaio2020co}.
% designs AI ethics checklists for responsible AI requirements, like fairness and transparency, as published principles to guide the ethical development and deployment of AI systems~\cite{madaio2020co}.
% Example: public opinion surveys, trust indices. public resistance, skepticism,
% 
% 
% 
% 
% \rqdcode{Backlash}. Exploring instances of public resistance, skepticism, or opposition to AI technologies, including concerns about job displacement, privacy violations, and ethical dilemmas~\cite{10.1145/3593013.3593999}.






\subsubsection{\emph{\textbf{\textcolor{hua-red}{Evaluation in Human Studies}}}: \textbf{how might we evaluate and understand the impact of AI on humans and society?}}
\label{sec:assessment}
% \mbox{}
% 
We summarize common empirical methods used to rigorously understand and assess the impact of AI on humans. Specifically, we focus on two types of impact. On the micro-level, we discuss how to evaluate the effectiveness of human-AI collaboration; on the macro-level, we discuss how to assess the impact of AI on a large group of people over a long period of time. 


\rqddim{Evaluate Human-AI Collaboration} refers to the evaluation of the effectiveness of an AI system in collaboration with humans. It is key to not only consider the final output, but also the interaction experience~\cite{Lee2022EvaluatingHM}. 
% We summarize several main metrics and methods that are used for such assessment. 
% 
% 
% 
% 
\rqdcode{Human-AI Team Performance} 
% On measuring outcome, one important dimension is to 
compares human-AI team performance with the performance of humans alone without AI collaboration 
%(or sometimes with 
% the condition of 
%AI alone if applicable). 
The metrics for measuring performance should include both task success metrics (e.g., accuracy) as well as indicators of efficiency~\cite{Mozannar2024TheRE,ding-etal-2023-harnessing}. 
%
% For example, RealHumanEval~\cite{Mozannar2024TheRE} evaluates LLM-assisted coding with different backbone language models and interaction modes in comparison with the control condition of no LLM assistance, where they compared with the task success rate as well as the task completion time. 
%
% ~\citet{ding-etal-2023-harnessing} evaluates human-AI news headline co-writing where they evaluated the quality of the co-written headlines versus control conditions using the Taste-Attractiveness-Clarity-Truth test from 1 (best) to 6 (worst) as the performance metric. 
% 
% 
\rqdcode{Cognitive Workload and User Satisfaction} 
% Apart from measuring whether AI systems are helping humans solve the task at hand better, another important dimension for evaluation is the cognitive workload 
involves understanding the degree of cognitive load that the user experiences when interacting with the system, as well as user satisfaction with the interaction and the final outcome. Such aspects are often captured via surveys or interviews \cite{ding-etal-2023-harnessing,Lee2022EvaluatingHM}.
% For example, ~\citet{ding-etal-2023-harnessing} collected user-perceived task difficulty with and without LLM assistance via a survey question using a Likert scale of 1 to 5 along with rationales. \citet{Lee2022EvaluatingHM} surveyed user-perceived helpfulness and the ease of user of LLM systems in tasks like question answering and crossword puzzle solving. 
% 
% 
%
\rqdcode{Control and Trust} refers to how user control can 
% Apart from improving task performance and ensuring user satisfaction, another important aspect is to preserve the users' control and ensure appropriate trust. This 
support the avoidance of catastrophic AI failures, especially in high-stakes settings where AI mistakes could lead to harm~\cite{Si2023LargeLM,ding2023harnessing}. 
% For example, \citet{ding2023harnessing} designed survey questions to gauge users' perceived control and trust in the LLM co-writing system via 5-point Likert rating scales. 
% ~\citet{Si2023LargeLM} measured user trust calibration on LLM assistance in detecting false claims via Likert-scale questions and found that users tend to over-rely on AI suggestions. 
% 
% 
% 
% 
% 
\rqdcode{Interaction Behavioral Analytics} refers to  measuring task performance quantitatively. This approach includes recording user interaction data and analyzing the patterns~\cite{Villalba2023AutomatedIO,Perry2022DoUW}.
% Lee2022CoAuthorDA,
% 
% For example, \citet{Perry2022DoUW} recorded users' code written in collaboration with LLMs and found participants who had access to an AI assistant wrote significantly less secure code than those without access to an assistant, and participants with access to an AI assistant were also more likely to believe they wrote secure code. 
% ~\citet{Lee2022CoAuthorDA} created a human-LLM co-writing platform and recorded human-AI co-writing sessions to analyse how users tend to co-write with LLMs. ~\citet{Villalba2023AutomatedIO} collected user interview data with LLM chatbots as AI interviewers and analysed the characteristics of user responses to AI-generated follow-up questions such as response lengths and diversity. 
% 
% 
\rqdcode{Qualitative Survey and Interviews } refers to qualitative approaches to understanding human-AI interaction. Commonly used methods include qualitative survey questions (i.e., open-ended) and user interviews to assess aspects of the user experience.~\cite{zhang2023deliberating}.
% 
% % 
% % 
% % =====================================================
% % =====================================================
\rqdcode{Statistical Analysis} utilizes methods such as regression analysis to quantitatively analyze and evaluate data from human studies, allowing for the verification of hypotheses~\cite{wang2021towards}.





\rqddim{Evaluate Societal Impact} 
% Apart from evaluating how well AI can assist humans in solving particular tasks, another important question is to 
refers to the macro-impact of a group of people as they come to use AI broadly. This dimension requires sufficient scale and time. The aim is to understand how the group's behavior changes as people within it frequently interact with AI. 
% We outline a few typical approaches along with examples below. 
% 
% santurkar2023whose,Shin2023SuperhumanAI
% 
\rqdcode{Public Opinion Surveys} aims to investigate the impact of AI on human measures of interest though deploying and analyzing large scale questionnaires 
~\cite{santurkar2023whose}.
% 
\rqdcode{Behavioral Data Analytics}
% The most common approach is to 
collects large-scale and potentially longitudinal behavior data, with the aim of understanding how pattern evolve over time~\cite{Shin2023SuperhumanAI,Zhou2024GenerativeAI}. 
% For example, ~\citet{Shin2023SuperhumanAI} analyzed 5.8 million chess move decisions made by professional Go players over the past 71 years to analyze the change over time, and found that  humans began to make significantly better and novel decisions following the advent of superhuman AI, potentially as a result of them playing with AI chess players and studying AI strategies. ~\citet{Zhou2024GenerativeAI} analyzed a dataset of over 4 million artworks from more than 50,000 unique users, and found that while peak artwork content novelty increases over time, average content novelty declines with the increasing adoption of text-to-image technologies. 
% 


% \rqdcode{Semi-Structured Interviews} Definition + example papers.


% \rqdcode{Observational Studies} Definition + example papers.


\begin{table*}[ht]
\centering
% \vspace{-10pt}
\begin{tabular}[t]{@{}  !{\color[HTML]{808080}\vrule width 2pt} p{.98\textwidth} !{\color[HTML]{808080}\vrule width 2pt} @{}}
\cellcolor[HTML]{E6E6E6} 
\textbf{Underexplored Dimensions in Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-blue}{AI}} (See Sec~\ref{sec:trend} for supporting data and evidence): 
% \newline
\vspace{5pt}

1. Educating and training humans on AI literacy is under-investigated.
\vspace{5pt}

2. Auditing AI for various ethical values is not fully explored.
% 
\vspace{5pt}

3. The collaboration between humans and AI with similar or superior capabilities is under-explored.
\vspace{5pt}


4. The societal impacts of and reactions to AI advancements are not fully explored.
\end{tabular}
\end{table*}
% 
























% ========================== dead kitten ========================== 






















% ======================= Interaction Part ================== 

% \subsection{Design Space of \textcolor{hua-yellow}{Interaction} in Human-AI Alignment}
% \label{sec:ai2human}





% \begin{figure*}[!ht]
%   \centering
%   \includegraphics[width=1\textwidth]{figures/interaction1.pdf}
%   \caption{The Taxonomy of Interactions for Human-AI Alignment.
%   }
%   \label{fig:interaction}
% \end{figure*}




% \textbf{\textcolor{hua-yellow}{RQ5. Interaction Approaches for Alignment}}: What were the interactive methods to achieve alignment process?
% \mbox{}


% ======================= Interaction Part ================== 


==> sections_ckpt_1120/introduction.tex <==
% === Writing Outline of Introduction===
\begin{comment}
    1. Background;
    2. Motivation and Goals
    3. What we've done
    4. Our key findings
    5. Main Contributions
\end{comment}


% === background ===
Artificial Intelligence (AI) has advanced significantly, especially with the advent of general-purpose generative AI, demonstrating unprecedented capabilities in solving a wide range of complicated and challenging problems, such as reasoning, generation, language understanding, and more~\cite{ouyang2022training}.
% rae2021scaling,palm,
% 
However, as AI becomes increasingly powerful and integrated into daily life, society is confronted with an array of risks to both individuals and to broader society~\cite{morris2024levels}. 
% 
For example, text-to-image generative models were found to amplify stereotypes about race and gender~\cite{bloomberg}, and
biased algorithms in hiring processes were found to perpetuate discrimination~\cite{park2021human}. 
% and autonomous vehicles raise concerns about safety and liability~\cite{himmelreich2018never}. 
These risks illuminate foundational questions around how and which values are embedded in AI models that drive decisions within real-world contexts. 
% 
% 


% \diyi{it might be nice to provide a concise definition of alignment, and AI alignment.}
% \hua{[DONE] sounds great! thanks for giving this valuable suggestion, I've added here^^.}
% 
For AI developers and researchers in this space, questions around the selection and representation of human values are part of a growing trend toward an interdisciplinary discussion on \emph{AI alignment}, which, has been previously defined in ~\citet{terry2023ai} as \say{\emph{considering the overall problem of how to ensure an AI produces the intended outcomes (as determined by its creator and/or user), without additional undesirable side effects (\eg by not performing operations that could negatively affect individuals, groups, or society at large)}.}
% 
% 
% 
% 
While significant efforts have been made by research in domains of HCI, NLP and AI to align AI to humans such that the AI systems' objectives match those of humans~\cite{goyal2024designing,ouyang2022training,santurkar2023whose}, there is a lack of clarity around the definition of \emph{human-AI alignment}, the goals of alignment, and with whom AI should align within the research community. 

%the scope of what is considered as alignment work.  of human-AI alignment  unclear across the numerous body of work on \emph{human-AI alignment}, its definition and scope remain ambiguous and inconsistent across literature, for example, regarding \textit{whom to align with} and \textit{the goal of alignment}.
% ,ngo2022alignment,kenton2021alignment,kirchner2022researching
% 
% values to better serve humans~\cite{ngo2022alignment,kenton2021alignment,kirchner2022researching}, e.g., through understanding how AI can contribute towards societal harmony, and evaluating the values (whether intended or otherwise) embedded in AI systems ~\cite{santurkar2023whose,ouyang2022training}.
% 
%For instance, ~\citet{ouyang2022training} present InstructGPT, which aligns a pre-trained Large Language Model (LLM) to follow human instructions and feedback based on Reinforcement Learning from Human Feedback (RLHF), and \citet{santurkar2023whose} investigated the opinions LLMs hold, by measuring the agreement between LLMs and 
% particular groups of people on various topics via public opinion polls.
% leveraging high-quality public opinion polls and associated human responses.
% through providing humans with public opinion polls to leverage human responses.
% , and InstructGPT aligns a pre-trained language model to follow human instructions and feedback based on Reinforcement Learning from Human Feedback (RLHF). 
% % 





% === two motivations (i.e., weaknesses of existing studies: 1) ambiguous definitions of alignment; 2) existing alignment paradigm is incomplete;. ===
%Despite numerous investigations into \emph{human-AI alignment}, its definition and scope remain ambiguous and inconsistent across literature, for example, regarding \textit{whom to align with} and \textit{the goal of alignment}.
% 
% 
% 
Furthermore, previous research often views AI alignment as a static, unidirectional process (\ie aiming to ensure that AI systems' objectives match those of humans) rather than an ongoing and mutual alignment problem~\cite{wiki_AI_alignment}.
% 
This unidirectional view largely understates the impact of \textbf{long-term interaction} and how such interaction further lends to a \textbf{dynamically changing} relationship between humans and AI. 
% as humans and AI intertwine. 
%of the intertwinement between humans and AI.
% 
% 
% Currently, l
As an example of the current unidirectional view, long-term interaction alignment work tends to focus on the implications of future advanced artificial general intelligence (\ie AGI~\cite{morris2024levels}), which hypothetically achieves human or superhuman intelligence~\cite{prunkl2020beyond}, uninhibited by human interference. A bi-directional view instead positions humans in a position of agency, empowering humans to interactively identify risky AI intentions and prohibit associated AI behaviors in deployed environments (i.e., looking beyond short-term testing interactions)  as~\citet{weidinger2023sociotechnical} advocated: \say{\emph{The interaction of technical and social components determines whether risk manifests}.} 
%However, this aspect of ``long-term'' alignment is largely understated in the current unidirectional alignment paradigm.
%Future systems with superhuman capabilities might develop unwanted power-seeking strategies~\cite{turner2019optimal}, such as acquiring money to proliferate or computation power to evade being turned off.
% 
% turner2022parametrically
% 
% However, w

%Instead, we argue for a bi-directional view of long-term alignment, which positions humans in a position of agency; empowering humans to interactively identify risky AI intentions and prohibit associated AI behaviors in deployed environments (i.e., looking beyond short-term testing interactions), as~\citet{weidinger2023sociotechnical} advocated: \say{\emph{The interaction of technical and social components determines whether risk manifests}.} However, this aspect of ``long-term'' alignment is largely understated in the current unidirectional alignment paradigm.

%Instead, we argue that, from a \emph{long-term alignment} perspective,
%research needs to 
% expand its scope beyond ultra-powerful future systems to 
%consider how 
% status quo and/or 
%frontier systems empower humans to interactively identify risky AI intentions and prohibit associated AI behaviors in deployed environments (i.e., looking beyond short-term testing interactions), as~\citet{weidinger2023sociotechnical} advocated: \say{\emph{The interaction of technical and social components determines whether risk manifests}.} However, this aspect of ``long-term'' alignment is largely understated in the current unidirectional alignment paradigm.
% 
% While there are a lot of values that AI could be trained to hold, AI developers should build with the approrpiate values in mind, appropriate should be defined 
% 
% 






%In addition to considering how we might empower humans to interactively examine and correct deployed AI systems in the long-term, 
Additionally, unidirectional work in AI alignment has under-emphasized the \emph{evolution} of human values and objectives that may arise through our continued use of AI and acceptance of it into daily life.
Prior research has shown that humans differ in what values and preferences they want AI systems to include, and these differences have to-date been largely unaccounted for in current AI systems~\cite{gordon2022jury}.
Beyond this, human preferences might \emph{dynamically change} as human objectives evolve alongside AI advances~\cite{carroll2024ai}. As described by \citet{dautenhahn2000living}, technology, cognition and goals evolve in tandem: 
% \say{\emph{Our use of technology changes who we are and how we think, and changes the environments we live in. This feeds back into human cognition and societies making further technological externalizations [...] As a consequence of agent technology, our environment is changing and ways of interacting [...] are forming the basis for interfacing with our agents.}} 
\say{\emph{Our use of technology changes who we are and how we think, and changes the environments we live in. This feeds back into human cognition and societies making further technological externalizations...}} 
The unidirectional view of alignment as \say{static} does not account for the aforementioned co-evolution as a dynamic force in alignment, which lends support for re-framing human-AI alignment as a bi-directional process. A bi-directional, dynamic view of human-AI alignment leverages a holistic understanding of the technical capabilities and limitations of AI, human-AI interaction, cognitive and social science, psychology and ethics, cross-cultural studies, and many other areas~\cite{carroll2024ai}.  

%Another alignment research consideration can focus on how human objectives might \textit{evolve} as we continue to use and incorporate AI in our daily lives.
%Prior research has shown that humans already differ in what values and preferences they want AI systems to incorporate, which is largely unaccounted for in current systems~\cite{gordon2022jury}.
%Beyond this, left further unaccounted for are how these preferences might \emph{dynamically change}, as human objectives evolve as AI advances~\cite{carroll2024ai}.
% 
% Also, the current paradigm largely neglects the \emph{dynamic changes} in human objectives that evolved along with AI advancements~\cite{carroll2024ai}. 
% % 
%As described by \citet{dautenhahn2000living}, technology and our cognition and goals evolve in tandem: \say{\emph{Our use of technology changes who we are and how we think, and changes the environments we live in. This feeds back into human cognition and societies making further technological externalizations ... As a consequence of agent technology, our environment is changing and ways of interacting ... are forming the basis for interfacing with our agents.}}
%Current definitions of alignment are ``static'' and do not account for how human objectives 
% and preferences 
%might co-evolve and \textit{dynamically} update with AI technology.
%The current static alignment efforts may not promise such a dynamic paradigm in which human  and AI technology co-evolve.
% For example, 






\begin{figure}[!t]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/teaser3.pdf}
    \caption[]{The overview of the \textbf{Bidirectional Human-AI Alignment} framework. Our framework encompasses both~\hspace*{.0em}\numimg{figures/A.pdf}\hspace*{-.1em} conventional studies which focus on
    % \emph{aligning AI to humans} 
    ``Align AI with Humans''
    during AI development, to see that AI produces the intended outcomes determined by humans, and ~\hspace*{.0em}\numimg{figures/B.pdf}\hspace*{-.1em}  
    % \emph{aligning humans to AI}
    ``Align Humans with 
    AI''
    , which aims to support humans to understand, critique, collaborate, and adapt to ongoing AI advancements.
    % 
    Note that ``\textbf{Humans}'' refers to both AI users and those who do not interact with AI but may be impacted by AI systems.
    We further identify four key research questions (\ie \texttt{RQ1-RQ4}) to facilitate this holistic loop of ``bidirectional human-AI alignment'', and organize the literature that can potentially address \texttt{RQ1-RQ4} in Section~\ref{sec:framework}.
    % 
    }
    \label{fig:teaser}
    \vspace{-1em}
\end{figure}
% 
% Additionally, prevailing research often overlooks the role of \emph{humans} in human-AI alignment~\cite{weidinger2023sociotechnical,prunkl2020beyond}, resulting in a narrow scope of investigation into human-AI alignment.
% 
% For example, although there have been calls for alignment studies (e.g., \citet{anwar2024foundational}, to consider \say{\emph{any way of providing evidence that a system is safe or aligned, including but not limited to: scientific understanding of system, behavioral evaluations, explanations of the model behavior or internal processing, and adherence to responsible development practices by the system developer}~\cite{casper2024black}}', whereas dominent research primarily focuses on developing AI technologies to ensure AI safety and alignment with human desires~\cite{bai2022constitutional,ganguli2022red}.
% 
% Consequently, many of these relevant topics are still under-explored, such as the specification of human values, diverse interactive methods for humans to steer AI, and how individuals and society could be impacted by and react to transformative AI advancements. 







%Achieving an ongoing and mutual process
% a comprehensive perspective 
%of human-AI alignment necessitates a holistic understanding of the technical capabilities and limitations of AI, human-AI interaction, cognitive and social science, psychology and ethics, cross-cultural studies, and many other areas~\cite{carroll2024ai}.
% 
% 
% 
%This paper contributes to the literature on human-AI alignment by presenting a comprehensive framework of human-AI alignment process, creating a shared vocabulary among interdisciplinary communities, and envisioning future directions to achieve this long-term and dynamic alignment goal.
% 
% To achieve this goal, 

This paper conducts a systematic literature review of over 400 human-AI alignment papers across multiple disciplines, based on PRISMA guidelines~\cite{Pagen71,10.1145/3544548.3581332}.  The literature review corpus includes papers drawn from the the Human-Computer Interaction (HCI), Natural Language Processing (NLP) and Machine Learning (ML) domains that were published between the advent of general-purpose generative AI to present, \ie primarily between January 2019 and January 2024. We take an interdisciplinary approach to human-AI alignment~\cite{gilbert2024hcc}, drawing from theories and empirical studies across the aforementioned domains. To round out our approach, we composed our research team of members from the domains of HCI, NLP, ML, Data Science, Computational Social Science, and Cognitive Science.
% 
% 
% We are guided by four research questions, See Fig 1 (PUT THEM ALL HERE). From the systematic literature review, we describe the features of the interdisciplinary body of previous work and identify gaps in our understanding of human-AI alignment. We propose the concept of bi-directional human-AI alignment through the introduction of a framework that can support researchers and practitioners to identify, integrate and assess the impact of human values in AI systems. 


% % % %
% === I've moved the bullets in the end of the paragraphs.
% Our contribution is multi-fold: 

% - A definition of alignment (OUR definition)  (Section 3) 
% - Value taxonomy - go to section 3 this is fig 3
% - Conceptual bi-directional human-AI alignment framework with two directions (Align AI to humans (previous unidirectional) and Align humans to AI (additional focus) (section 4, fig 4 and 5)
% - Observed trends from the lit review (3 key challenges) (5.1), gaps and opportunities to fill gaps (5.2- 5.4)
% %- Usability guide / case study for practitioners and researchers to apply the findings to real-world deployment and evaluation (6) 









% ---------
%These papers are selected to represent a holistic view of the human-AI alignment space, specifically from the domains of Human-Computer Interaction (HCI), Natural Language Processing (NLP), Machine Learning (ML), and others.
%Also, we form an interdisciplinary team to conduct the systematic review, consisting of researchers from the domains of HCI, NLP, ML, Data Science, Computational Social Science, and Cognitive Science.

%spanning from model development and evaluation to interactive system design to human understanding and critical thinking around AI's impact on individuals and society. 


%To this end, we conduct a systematic literature review of over 400 papers across multiple disciplines, based on the PRISMA guidelines~\cite{Pagen71,10.1145/3544548.3581332}, present clarified definitions and scope (Section~\ref{sec:method}), derive a ``\textbf{Bidirectional Human-AI Alignment}'' framework shown in Figure~\ref{fig:teaser} (Section~\ref{sec:framework}) grounded in iterative paper coding and analysis (Section~\ref{sec:analysis}), and provide recommendations for future work in three key challenge areas (Section~\ref{sec:discussion}).


% 
% 
% 
% \rada{before going into details, I suggest stating in one clear sentence what is the goal of this review} \hua{Great point! No problem, we'll add the goal and motivation of this survey here^^.}
% 
%Specifically, our systematic review takes an interdisciplinary perspective on human-AI alignment~\cite{gilbert2024hcc}, drawing from theories across domains and empirical studies spanning model development and evaluation to interactive system design to human understanding and critical thinking to assess AI's impact on individuals and society. 
% Specifically, our systematic review
% took an interdisciplinary perspective on human-AI alignment~\cite{gilbert2024hcc}, drawing from theories across domains and empirical studies spanning model development and evaluation to interactive system design to human understanding and critical thinking to assessing the impact of AI on individuals and society. 
% This paper presents a systematic literature review of 
%The papers we reviewed in this survey are published around the advent of general-purpose generative AI, \ie primarily between January 2019 and January 2024. These papers are selected to represent a holistic view of the human-AI alignment space, specifically from the domains of Human-Computer Interaction (HCI), Natural Language Processing (NLP), Machine Learning (ML), and others.
%Also, we form an interdisciplinary team to conduct the systematic review, consisting of researchers from the domains of HCI, NLP, ML, Data Science, Computational Social Science, and Cognitive Science.
% Our goal was to leverage a variety of perspectives and expertise to conduct a systematic literature review for developing a holistic alignment view based on the PRISMA guidelines~\cite{Pagen71,10.1145/3544548.3581332}.
% system design and model architecture to user evaluation and in-the-wild deployment
%Drawing from interdisciplinary perspectives and empirical studies, this paper conducts a systematic review of over 400 interdisciplinary papers primarily published between 2019 and 2024, spanning multiple domains, specifically, Human-Computer Interaction (HCI), Natural Language Processing (NLP), Machine Learning (ML) and AI. 
% 
% 




% 
\begin{table*}[!t]
\centering
\begin{tabular}[t]{@{}  !{\color[HTML]{808080}\vrule width 2pt} p{.98\textwidth} !{\color[HTML]{808080}\vrule width 2pt} @{}}
\cellcolor[HTML]{E6E6E6} 
\textbf{Definition.} 
% \newline
\vspace{3pt}

% \emph{\textbf{Bidirectional Human-AI Alignment} considers not only `Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-red}{Humans}' that integrates human specifications to train, steer, and customize AI, but also places emphasis on `Aligning \textcolor{hua-red}{Humans} to \textcolor{hua-blue}{AI}', that investigates human cognitive and behavioral adaptation to AI, to support individuals and society in understanding ,critiquing, collaborating with, and adapting to AI advancements.}


\emph{\textbf{Bidirectional Human-AI Alignment} is a comprehensive framework that encompasses two interconnected alignment processes: `Aligning \textcolor{hua-blue}{AI} with \textcolor{hua-red}{Humans}' and `Aligning \textcolor{hua-red}{Humans} with \textcolor{hua-blue}{AI}'. The former focuses on integrating human specifications into training, steering, and customizing AI. 
% 
% The latter supports human agency, aiding humans to think critically when using AI, leverage AI for collaboration, and incorporate AI into daily life through a better understanding of how to leverage it for their benefit. 
% 
The latter supports human agency, empowering people to think critically when using AI, collaborate effectively with it, and adapt societal approaches to maximize its benefits for humanity.
% 
% % 
% The latter ensures human agency, empowering humans to think critically when using AI, harnessing AI for collaboration, 
% and adjust societal responses to make the most benefit for humans.
% % 
% leverage AI for collaboration, and incorporate AI into daily life through a better understanding of how to leverage it for their benefit. 
}
\end{tabular}
\end{table*}

 %The former focuses on integrating human specifications into training, steering, and customizing AI. The latter supports human agency, aiding humans to think critically when using AI, leverage AI for collaboration, and incorporate AI into daily life through a better understanding of how to leverage it for their benefit. 
 
% i.e., cognitive and behavioral adaptation to AI, thereby supporting humans to understand, critique, collaborate with, and adapt themselves to AI advancements. }

%Aligning humans to leverage ai human agency 
%Leveraging human agency to influence AI
%Human response to AI
%Intentional Human adaptation to AI
%Human adaption to AI in alignment process 


% ======== GREAT ========= 
% aligning AI to human intention
% Aligning human response to AI advancement
% ================= 




%aligning AI to human response / adaptions 
%It's a feedback loop -- both focus on different aspects of the human part 

%Alignment loop
%Influence exchange is bidirectional
%Intentional alignment (AI to human)
%Unintentional response (Adapt AI to human)
%Our adaption is not intentional -- defaulting to biases and assumptions about AI without considering how we talk about it changes their values and intentions

%erspective places equal emphasis on 1) human-centered alignment, i.e., supporting humans in understanding, critiquing, collaborating with, and adapting to AI advancements and 2) AI-centered alignment, i.e., supporting AI developers to produce intended AI output as determined by human specifications, steering and customization.


% % 
% \begin{table*}[!t]
% \centering
% \begin{tabular}[t]{@{}  !{\color[HTML]{F8B00F}\vrule width 2pt} p{.98\textwidth} !{\color[HTML]{F8B00F}\vrule width 2pt} @{}}
% \cellcolor[HTML]{FFEFCF} 
% \textbf{Definition of Bidirectional Human-AI Alignment} 
% \newline
% This is a 
% \end{tabular}
% \end{table*}




% \noindent
\textbf{Paper Organization and Key Findings}.
We provide clarified definitions and scopes related to human-AI alignment, including ``\emph{what is the goal of alignment?}'', 
% ``\emph{the groups of people to be aligned with}'' 
``\emph{with whom to align?}'', and ``\emph{what values should be aligned with?}''(Section~\ref{sec:method}). 
% 
We then present a conceptual framework of \emph{Bidirectional Human-AI Alignment} from 
% a human-centered, holistic perspective. 
a long-term and dynamic perspective, encompassing both ``Align AI with 
% \textcolor{hua-yellow}{$\mapsto$} 
Humans'' and ``Align Humans with 
% \textcolor{hua-yellow}{$\mapsto$} 
AI'' (see Figure~\ref{fig:teaser}). 
% The ``Align \textcolor{hua-blue}{AI} to 
% % \textcolor{hua-yellow}{$\mapsto$} 
% \textcolor{hua-red}{Humans}'' direction represents the conventional unidirectional studies that aim to integrate human specifications to train, steer, and customize AI.
% % 
% Crucially, our bi-directional framework places equal emphasis on the significance of ``Align \textcolor{hua-red}{Humans} to 
% % \textcolor{hua-yellow}{$\mapsto$} 
% \textcolor{hua-blue}{AI}'', which represents humans' cognitive and behavioral adaptation to the AI systems. 
% The studies in this direction aim to support individuals and the broader society in understanding, critiquing, collaborating with, and adapting to transformative AI advancements.
% % 
% 
% 
Furthermore, we identify four key research questions (RQs) in the \emph{Bidirectional Human-AI Alignment} framework and provide a structured way to organize the existing research literature to address these questions in Section~\ref{sec:framework}.
% 
The resulting structured topologies in Figure~\ref{fig:ai2human} and \ref{fig:human2ai} aim to provide a shared vocabulary that can help streamline communication and collaboration between alignment researchers in different disciplines.
% 
% Therefore, we strive to structure the literature taxonomy based on our proposed \emph{bi-directional human-AI alignment} framework. 
% 
Furthermore, through iterative paper coding and literature analysis, we derive insights including meta analysis on gaps and trends in existing alignment research, findings of human values, and the interaction techniques for human-AI alignment (Section~\ref{sec:analysis}). 
% This process brought forth the limitations of existing studies, and the risks that can arise from improper human-AI alignment. 
% }
%understanding the discrepancies between AI evaluation and human assessment 
% 
%Our team of 13 interdisciplinary researchers from multiple domains (ranging from HCI, NLP, ML, Computational Social Science, Psycholinguistics, etc.) to conduct a systematic review based on the PRISMA guidelines~\cite{Pagen71,10.1145/3544548.3581332}. 
% 
% 
%Furthermore, we identify limitations and risks in existing studies by analyzing coded papers quantitatively and qualitatively, including fine-grained human value taxonomy, interaction modes for alignment, and discrepancies between AI evaluation and human assessment (Section~\ref{sec:analysis}). 
% \hua{add findings in Sec 5 here.}
% add findings in Sec5 here.
% 
% 
% 
To pave the way for future studies, we further envision three future directions in Figure~\ref{fig:future_work} and Section~\ref{sec:discussion}.
% , from near-term to long-term perspective, to motivate a dynamically co-evolving human-AI alignment.
% For each challenge, we articulate the future research problems and examples of potential future solutions from both directions in Section~\ref{sec:discussion}.
% 
% 
% 
% 
% 
% 
Our study highlights several \textbf{key findings}. For instance, many essential human values outlined in Table~\ref{fig:value_taxonomy}, such as loyalty and environmental protection, are crucial for alignment but are often overlooked in current research. Additionally, many topics within the bidirectional alignment framework, including leveraging implicit human feedback to align AI models and auditing AI for various social values, are important but underexplored.




% 
% \noindent
\textbf{Operationalizing the Framework}.
To help AI practitioners (e.g., developers, researchers, user experience designers) who are interested in this field to leverage the bidirectional approaches, we highlight some systematic resources about human-AI alignment provided both within this survey and on companion Github repository:

\vspace{-6pt}
\begin{itemize}
    \item A \href{https://github.com/huashen218/bidirectional-human-ai-alignment}{Github repository} of ``\emph{Bidirectional Human-AI Alignment}'' maintaining latest reading lists and relevant updates.
    \item Fig.~\ref{fig:teaser}: An overview of the bidirectional human-AI alignment framework with formal definition.
    \item Table~\ref{fig:definitions}: Typical alignment goals, their definitions, and limitations.
    \item Table~\ref{fig:value_taxonomy}: A comprehensive list of basic human values, their relationships, and related alignment papers.
    % \item Fig.~\ref{fig:ai2human}: A fine-grained topology for aligning AI to humans.
    \item Fig.~\ref{fig:ai2human} and~\ref{fig:human2ai}: Fine-grained topologies and papers of ``Aligning AI to Humans'' \& ``Aligning Humans to AI'' research.
    \item Fig.~\ref{fig:paper_distribution}: An illustration of trends and gaps of alignment research dimension distribution.
    \item Fig.~\ref{fig:interaction}: A summary of common interactive techniques to specify human values and exemplary papers.
    % \item Fig.~\ref{fig:future_work}: An outline of envisions of six future directions.
\end{itemize}






% Overall, we summarize our main contributions as follows:
% % 
% % 
% % \vspace{-1em}
% % 
% % % 
% % \begin{itemize}
% %     \vspace{-.5em}
% %     \item 
% %     Providing clarified definitions and scopes of human-AI alignment (\ie including \emph{with whom to align}, \emph{what is the alignment goal}, and \emph{what are the values to be aligned with}), and systematically reviewing over 400 relevant research papers (Section~\ref{sec:method}).
% %     \item Developing the ``Bidirectional Human-AI Alignment'' framework to represent the ongoing, mutual alignment process and providing fine-grained taxonomies to address the involved four critical research questions
% %     (Section~\ref{sec:framework}).
% %     \item Discussing the key findings derived from literature analysis, 
% %     including the human values and interaction techniques for alignment, and the discrepancy between AI and human evaluation
% %     (Section~\ref{sec:analysis}).
% %     \item Envisioning three key challenges for future research directions from a near-term to a long-term perspective and propose examples of potential future solutions (Section~\ref{sec:discussion}). 
% % \end{itemize}



% \begin{itemize}
%     \vspace{-.5em}
%     \item We provide a clear definition of alignment.
%     - A definition of alignment (OUR definition)  (Section 3) 
%     \item - Value taxonomy - go to section 3 this is fig 3
%     \item - Conceptual bi-directional human-AI alignment framework with two directions (Align AI to humans (previous unidirectional) and Align humans to AI (additional focus) (section 4, fig 4 and 5)
%     \item - Observed trends from the lit review (3 key challenges) (5.1), gaps and opportunities to fill gaps (5.2- 5.4)
%     % \item Providing clarified definitions and scopes of human-AI alignment (\ie including \emph{with whom to align}, \emph{what is the alignment goal}, and \emph{what are the values to be aligned with}), and systematically reviewing over 400 relevant research papers (Section~\ref{sec:method}).
%     % 
%     % % 
%     % \item Developing the ``Bidirectional Human-AI Alignment'' framework to represent the ongoing, mutual alignment process and providing fine-grained taxonomies to address the involved four critical research questions
%     % (Section~\ref{sec:framework}).
%     % \item Discussing the key findings derived from literature analysis, 
%     % including the human values and interaction techniques for alignment, and the discrepancy between AI and human evaluation
%     % (Section~\ref{sec:analysis}).
%     % \item Envisioning three key challenges for future research directions from a near-term to a long-term perspective and propose examples of potential future solutions (Section~\ref{sec:discussion}). 
% \end{itemize}















% ================================= dead kitten ===============================



%conduct the evaluation". for example, how NLP researchers evaluate AI performance v.s. how HCI researchers assess human's demands on AI. 

% \noindent \textbf{Major Findings.} 
% % \subsection{Major Findings}
% % 
% As part of this review, we highlight \todo{X} major findings from the surveyed literature that we believe are important but yet underexplored for conducting bidirectional human-AI alignment research:

% \begin{enumerate}
%     \item \todo{A}
%     \item \todo{B}
%     \item \todo{C}
% \end{enumerate}




% \begin{figure*}[!ht]
%   \centering
%   \includegraphics[width=.6\textwidth]{figures/teaser2.pdf}
%   \caption{An Overview
%   }
%   \label{fig:teaser}
% \end{figure*}







% AI has advanced significantly, showcasing previously unheard-of capabilities in solving a wide spectrum of tasks in our daily lives. Beneath the incredible progress, however, AI models can not be relied upon to always follow human values (e.g., fairness, accuracy, diversity). This misalignment between model behavior and human intent impedes the model performance (e.g.,inaccurate decision-making), and meanwhile, leads to outputs with social biases (e.g., toxic responses from voice assistants), or even fatal accidents (e.g., medical diagnosis errors). 

% The adoption of Reinforcement Learning from Human Feedback (RLHF) has gained momentum for human-AI alignment by training AI models with incorporating human input. However, the current RLHF technique faces dual limitations. Firstly, the type of human feedback in RLHF is limited, predominantly focusing on instance rankings. Moreover, these human inputs are utilized in limited stages of AI development, as rewards to optimize the models primarily during model training. Consequently, my research endeavors to maximize the varied human feedback types, fostering alignment with AI models through human-AI interaction across all stages of AI developments.


% Particularly, we strive to empower humans to interactively explain, evaluate and provide feedback on AI systems, with the goal of aligning human intents and AI behaviors. On one hand, our work aims to help humans to interactively explain and evaluate AI models, with the goal of probing the misalignment between human perception and and model performance through real-world AI development. On the other hand, upon the revealed misalignment, we support model improvement based on human feedback interactively. We exploit both improvement through data preparation and model training stages, as well as interactive calibration in test and development stages on-the-fly.




% Through a comprehensive examination of theoretical frameworks, practical applications, and potential pitfalls, this paper endavors to 






% Traditional Human-AI Alignment studies focus on investigating “aligning AI to humans”, which improves AI capabilities to be more aligned with human values and intentions. 

% However, in this study, we advocate for attention on “aligning humans to AI”, which emphasize the importance of improving human’s understanding, evaluation, and thus, steerability on AIs.

% The ultimate goal is to achieve a complete loop of bidirectional human-AI alignment process.





% An increasing number of human-AI alignment studies aim to build human values and feedback into AI. 
% For example, InstructGPT aligns the pre-trained language models to follow human instructions based on Reinforcement Learning from Human Feedback (RLHF). However, existing methodologies for human-AI alignment are subject to various shortcomings:

% Firstly, the types of human feedback for aligning AI are limited. The primary forms of human feedback in RLHF involve scoring, ranking, or categorically selecting, predominantly overlooking diverse human expressions such as natural language.
% Besides, the provided human feedback is utilized in limited stages of AI development. AI models commonly treat the human feedback as rewards for optimization during the training stage, but lack strategies to incorporate human feedback after training stages for improving AI.

% Also, current human-AI alignment methods lack the flexibility to adeptly manage dynamic and unpredictable human feedback that may arise post-model fine-tuning. This limitation stems from the fact that human feedback is predominantly provided in a one-time annotation manner, without continued interaction.



% More importantly, we deem human-AI alignment is a bi-directional process. It not only involves aligning AI to humans -  which aims to improve AI capability and ethics to cater to human values. But also, it includes aligning humans to AI – that helps human better understand and utilize AI to give more qualified feedback, which is largely neglected in current human-AI alignment studies.




% \textbf{On one hand}, current human feedback is largely limited in feedback formats and stages. Researchers primarily leverage the one-shot static human annotations on ranking or scoring the model generations to optimize model training, which significantly overlooks diverse and dynamic human expressions such as interactive conversations. Also, the current methods do not support incorporating human feedback after the model training stage. 

% \textbf{On the other hand}, we deem human-AI alignment as a bi-directional process. It not only involves aligning AI to humans -  which aims to improve AI capability and ethics to cater to human values. But also, it includes aligning humans to AI – that helps humans better understand and utilize AI to give more qualified feedback, which is largely neglected in current human-AI alignment studies.





% The ultimate goal is to achieve a complete loop of bidirectional human-AI alignment process.


% Therefore, the goal of this paper is to provide a framework of designing  human-AI alignment with interaction throughout the AI development stages with a systematic review.









% Many efforts have been made to align LLMs to human values for making them better serve humans and satisfy societal harmony. 
% An increasing number of human-AI alignment studies aim to build human values and feedback into AI.
% 
% 
% % 
% For example, InstructGPT aligns the pre-trained language models to follow human instructions and feedback based on Reinforcement Learning from Human Feedback (RLHF)~\cite{ouyang2022training}.
% % 
% which unleashed the great capabilities of ChatGPT. 
% % 









% % Generative AI, exemplified by Large Language Models (LLMs), 
% Artificial Intelligence (AI) has advanced significantly, particularly in the era of general purpose of AI, showcasing previously unheard-of capabilities in solving a wide spectrum of complicated and challenging problems, such as reasoning, generation, and language understanding tasks, and others~\cite{rae2021scaling,palm,ouyang2022training}. 
%
% However, as AI becomes more powerful and deeply integrated into our lives, it presents potential risks and might cause serious social harm. 
% 
% 
% At the heart of this transformative landscape lies the imperative of aligning AI systems with human values and objectives, which is fundamental to safeguarding societal welfare and preserving ethical integrity.
% 
% Therefore, the questions of what foundational values that drive decisions big and small in deployed LLMs to serve humans are all more important.
% % 
% % 
% Many efforts have been made to align LLMs to human values for making them better serve humans and satisfy societal harmony. 
% % An increasing number of human-AI alignment studies aim to build human values and feedback into AI.
% % 
% % 
% % 
% For example, InstructGPT aligns the pre-trained language models to follow human instructions and feedback based on Reinforcement Learning from Human Feedback (RLHF)~\cite{ouyang2022training}.
% % 
% which unleashed the great capabilities of ChatGPT. 
% % 
% 
% 
% 





% Nevertheless, how these aligned values are perceived and utilized by human when interacting with deployed AI in practice has not been fully explored, and this misaligned social-technical gap may even backfire.
% % 
% Specifically, current human feedback is largely limited to feedback stages and interaction formats. While interacting with deployed AI after training, it is unclear how well the LLM can align with human perception and evaluation. How humans should be equipped to harness the transformative power of AI and stay resilient to AI mistakes.
% % 
% % 
% 
% % the current methods do not support incorporating human feedback after the model training stage. 
% % 
% Besides, researchers primarily leverage the one-shot static human annotations on ranking or scoring the model generations to optimize model training, which significantly overlooks diverse and dynamic human interactive expressions such as interactive conversations.








% Achieving such bidirectional alignment necessitates a holistic understanding of human cognition, behavior, and societal norms, as well as the technical capabilities and limitations of AI algorithms. 
% % 
% Drawing upon interdisciplinary perspectives and empirical evidence, this paper provides a comprehensive survey of different alignment values in existing work, a systematic review of AI algorithmic techniques to achieve alignment goals, and how alignment being perceived and utilized by human in practice. 
% % 
% As a result, we provide a bidirectional human-AI alignment framework, which aims to complete the holistic loop of human-AI alignment process with interactions.
% 
% The framework is designed to pave the way for future research, facilitating the broader exploration of diverse formats and stages within the realm of human-AI alignment, and identifying the imperative yet underexplored research questions for future exploration.
% % 
% No one framework is perfect. Our approach with this paper is to provide a broad, sociotechnical overview of human-AI alignment by working in a large, interdisciplinary team. 



% \noindent \textbf{Operational Resources.} To help HCI and NLP researchers who are new but interested in investigating human-AI alignment, we provide below operational resources within this survey:
% \begin{itemize}
%     \item Figure~\ref{fig:teaser}: A novel bidirectional human-AI alignment \textbf{framework}.
    
%     \item Figure~\ref{fig:ai2human}: A fine-grained \textbf{taxonomy of ``align AI to human''} with representative papers.

%     \item Figure~\ref{fig:human2ai}: A fine-grained \textbf{taxonomy of ``align human to AI''} with representative papers.
    
%     % \item A \textbf{topology} of bidirectional human-AI alignment. (Figure~\ref{fig:topology})
    
%     % \item Figure~\ref{fig:interaction}: A comprehensive \textbf{design space of interaction} for bidirectional human-AI alignment. 
    
%     \item A systematic \textbf{collection} of human values, dataset and evaluation metrics (Table~\ref{}).
%     \item A critical \textbf{analysis} on misaligned gaps, limitations and future directions.
    
%     % \item A open-sourced \textbf{repository} maintaining all resource links.
% \end{itemize}





% \tiffany{Two contributions: 1) theoretic contributions +  2) actionable contribution: 
%  practical resources.}


 








% \noindent \textbf{Contributions.} 
% % \subsection{Contributions}
% Overall, we summarize our main contributions as below:

% % \begin{itemize}
% %     \item Providing a broader and systematic review of “bidirectional human-AI alignment with interaction” based on cutting-edge top publications.
% %     \item Design a framework to aid future research in developing, evaluating and understanding new methods and systems.
% %     \item Reasoning about existing “human-AI alignment with interaction” methods,, limitations, and risks, etc.
% %     \item Identifying trends and opportunities for future research.
% % \end{itemize}



% \begin{itemize}
%     \item 
%     Provide a clarified definition and scope of what human-AI alignment is, and conduct a systematic review of existing literature within this scope (Section~\ref{sec:method}).
%     \item Develop a conceptual framework of ``Bidirectional Human-AI Alignment'' to structure the literature taxonomy and provide a holistic landscape from a human-centered perspective (Section~\ref{sec:framework}).
%     \item Delve into an in-depth analysis of human values taxonomy, interaction modes for alignment, and discrepancy between AI evaluation and human assessment to clarify the limitations of existing literature (Section~\ref{sec:analysis}).
%     \item Envision the new possibilities for future research directions based on the proposed framework and empirical paper codes (Section~\ref{sec:discussion}).
% \end{itemize}








% this paper provides a comprehensive survey of different alignment values in existing work, a systematic review of AI algorithmic techniques to achieve alignment goals, and how alignment being perceived and utilized by human in practice. 
% % 
% As a result, we provide a bidirectional human-AI alignment framework, which aims to complete the holistic loop of human-AI alignment process with interactions.









% Therefore, 
% we advocate that \textbf{human-AI alignment should be a bidirectional process}. It not only involves \textbf{aligning \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{humans}}, which aims to improve AI capability and ethics to cater to human values. But also, it includes \textbf{aligning \textcolor{hua-red}{humans} \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}}, that enhances humans' understanding and capabilities to better harness AI and steer AI behavior to satisfy practical needs, which is largely neglected in current human-AI alignment studies.























% \begin{itemize}
%     \item Providing a broader and systematic review of “bidirectional human-AI alignment with interaction” based on cutting-edge top publications.
%     \item Design a framework to aid future research in developing, evaluating and understanding new methods and systems.
%     \item Reasoning about existing “human-AI alignment with interaction” methods,, limitations, and risks, etc.
%     \item Identifying trends and opportunities for future research.
% \end{itemize}




% The studies in this direction aim to support individuals and the wider society to understand, critique, collaborate with and adapt to transformative AI advancements. 
% 
% Our systematic review revealed that many aspects in this direction are under-explored in existing research on human-AI alignment.
% }
% 
% 
% 
% 
% 
% \tiffany{Our team of interdisciplinary researchers is comprised from the domains of HCI, NLP, ML, Data Science, Computational Social Science, and Psycholinguistics. Our goal was to leverage a variety of perspectives and expertise to conduct a systematic literature review based on the PRISMA guidelines~\cite{Pagen71,10.1145/3544548.3581332}% 
% 

==> sections_ckpt_1120/limitation.tex <==
In this section, we provide a summary of the key implications of our proposed framework, and discuss the challenges and limitations we encountered during the systematic literature review process.


\subsection{Framework Implications and Applications}


% \noindent
\subsubsection{\textbf{Cross-domain inspirations.}}
Achieving long-term human-AI alignment requires holistic, interdisciplinary efforts. This paper introduces a bidirectional human-AI alignment framework to create a shared vocabulary among diverse fields. Supported by over 400 multi-domain research papers, this framework \textbf{enables researchers to integrate knowledge from other domains, enhancing their work and fostering synergetic collaboration.}
% 
Particularly, AI researchers can use the human value taxonomy grounded in psychological theories (\eg Section~\ref{sec:gap_value}) to develop datasets and algorithms that incorporate a broader spectrum of human values. Additionally, by examining studies on individual and societal adaptations to AI alignment (\eg Section~\ref{sec:impacts}), AI developers can create more practical and adaptive AI systems that evolve alongside human and societal changes.
% 
% 
Conversely, HCI and social science researchers can leverage customizable AI alignment algorithms (\eg Section~\ref{sec:ai2human2}) to design interactive systems that improve human interaction with AI. By using interaction techniques to specify human values (Section~\ref{sec:ai2human1}), these researchers can optimize interfaces or conduct surveys to extract human values, informing AI alignment development.
% 
% This cross-domain approach enriches research and development in both directions, ensuring a comprehensive and effective strategy for achieving long-term human-AI alignment.




\subsubsection{\textbf{Foundation of Dynamic Alignment Evolution.}}
% 
The proposed bidirectional human-AI alignment framework also \textbf{serves a foundational role to support researchers to address the outlined future challenges and achieve long-term alignment}.
% 
% We envision future directions for human-AI alignment, from near-term to long-term, upon the foundation of the proposed bidirectional framework.
% % 
% % 
As elaborated in Section~\ref{sec:discussion}, within each direction, researchers can potentially address future challenges on the basis of existing alignment studies organized by the framework.
For instance, to tackle the specification game, future AI researchers can use the comprehensive human value taxonomy outlined in the framework (Section~\ref{sec:discussion}) to develop methods for selecting the appropriate subset of these human values to be integrated into AI alignment.
% 
% 
Additionally, we emphasize the importance of synergizing both directions to achieve long-term bidirectional human-AI alignment. To facilitate dynamic co-evolution (Section~\ref{sec:challenge2}), we advocate for collaboration among AI, HCI, and social scientists to measure human and societal adaptations and incorporate these changes into the alignment of next-generation AI systems.
% 
This holistic approach can contribute to the evolution of AI in harmony with human values and societal needs.












% \subsection{Limitations}
% % 
% One limitation of this work is the coverage of the sampled and filtered papers. 
% % restricted by the paper filtering process. 
% The literature revolving around the topic of human-AI alignment is increasing rapidly, scattering in diverse venues across many domains. 
% % 
% % 
% Therefore, instead of striving for an exhaustive collection of papers, this work focused on developing a holistic loop of bidirectional human-AI alignment framework by using essential research questions, dimensions and codes. 
% % 
% % 
% % 
% Additionally, we are aware that our surveyed papers and the position of our team members primarily focus on computing-related domains, such as ML, NLP, and HCI. There are additional disciplines involved in alignment research, such as cognitive science, psychology, and STS (Science, Technology, and Society).
% % ,  are beyond computing. 
% However, our framework can naturally extend to these domains by incorporating them into the appropriate directions.
% % 
% Despite these limitations, we argue that this bidirectional human-AI alignment framework serves as foundational reference forfuture researchers examining existing literature that lies in the holistic loop of the alignment process, while preventing implicit assumptions or overlooked considerations, thereby facilitating a holistic understanding of the dimensions and factors that drive the developing of AI technology and human impacts.
% % 
% % 
% For future work, we plan to continue to refine our dimensions and codes to incorporate future literature relevant to the bidirectional human-AI alignment process.
% % , and provide possible directions for future research from a historical and developing perspective.
















% =========================== dead kitten ==========================
% 
% We are aware of the limitations of the work. We provide detailed elaborations of the limitations in this study below.
% 
% 
% First, 
% 
% we are aware of the limitation in the \textbf{paper filtering process}.
% 
% 
% 
% Additionally, we are aware of the limitation in \textbf{paper analysis}.



% % 
% i) full spectrum of human values and diverse interaction methods to capture values;
% ii) make AI practically useful and co-evolve AI with dynamic human and society evolvement;



% \noindent
% \textbf{Framework Implications and Applications}
% % 
% articulate implications for using the framework and how to apply it. Said another way -- what does this mean for designers or HCI researchers?
% % 
% % 
% % 
% % 
% 1. create a shared vocabulary among interdisciplinary communities related to alignment research, and empower synergetic collaboration and cross-domain insights to developing long-term human-AI alignment.
% % (bridge research gaps into )

% 2. For AI designers:
% i) full spectrum of human values and diverse interaction methods to capture values;
% ii) make AI practically useful and co-evolve AI with dynamic human and society evolvement;


% 3. For HCI designers: 
% i) better understand, use and correctly rely on AI (customization); 
% ii) conduct future research that can inform AI alignment development.




% Achieving the ongoing, mutual process of human-AI alignment, in the long run, necessitates holistic knowledge and efforts from interdisciplinary domains. Therefore, this paper contributes a bidirectional human-AI alignment framework that aims to create a shared vocabulary among interdisciplinary communities.
% 
% 
% This comprehensive alignment framework, supported by over 400 mutli-domain research papers, \textbf{enables researchers to bring in other-domain knowledge to improve their research and facilitate synergetic cooperation among multiple disciplines}.
% % 
% % 
% 
% % 
% % For instance, AI researchers can leverage the comprehensive human value taxonomy, which is grounded on the psychological theories (\eg Section~\ref{sec:gap_value}), to develop potential datasets and algorithms for integrating broader spectrum human values into AI alignment. Besides, by reviewing the individual and societal adaptations to the AI alignment investigated by the HCI and social science (\eg Section~\ref{sec:impacts}), AI researchers can potentially develop more practically useful AI systems and co-evolve AI with the dynamic human and society evolution.
% % % 
% % 
% % 
% On the other hand, HCI and social science researchers, informed by the diverse AI customizable alignment algorithms (\eg Section~\ref{sec:ai2human2}), can better develop interactive systems to facilitate human usage and experience in practical AI applications. Also, given the potential interaction techniques to specify human values (Section~\ref{sec:ai2human1}), HCI and sociel science researchers can extract the human values by optimizing interactive interfaces or conduct democratic human surveys or studies to obtain the values, and use them to inform the AI alignment development by AI designers.









% % \noindent
% % \textbf{Foundation of Temporal Alignment Evolution.}
% \subsubsection{\textbf{Foundation of Dynamic Alignment Evolution.}}
% % 
% % 
% We envision the future directions, from near-term to long-term perspective as elaborated in Section~\ref{sec:discussion}, largely upon the foundation of the proposed bidirectional human-AI alignment.
% % 
% % 
% Specifically, we articulate how the two directions should address the potential challenges that can build upon the existing alignment studies. 
% For example, to address the specification game (Section~\ref{sec:challenge1}), future AI researchers can build upon the comprehensive human value taxonomy summarized in the framework and develop methods for selecting the appropriate subset of these human values to be integrated into AI alignment.
% % 
% % 
% Additionally, we also discuss how the two directions can synergize to achieve bidirectional human-AI alignment as a complete loop the achieve the alignment goal.
% % 
% For instance, to achieve dynamic co-evolution of alignment, we advocate the synergetic collaboration between AI designers and HCI and social scientists to measure the dynamic human and societal adaptations, and further incorporate these changes into aligning the next-generation AI systems.

% % discuss how communities can synergize to achieve long-term alignmnet.

% % Built upon the framework, we further propose future challenges and directions from a temporal perspective.
% % As elaborated in Section~\ref{sec:discussion}, 









==> sections_ckpt_1120/method.tex <==



% This paper is a collaborative effort consisting of a team of researchers across multiple domains, including Human-Computer Interaction (HCI), Natural Language Processing (NLP), Machine Learning (ML), Data Science (DS), Social Science, and Cognitive Science. 
\noindent
Addressing alignment challenges is a complex and multifaceted process. 
To develop a comprehensive perspective of the ongoing and mutual process of human-AI alignment,
this section begins by introducing core definitions and key components of alignment. Subsequently, we outline our methodology for conducting a systematic literature review and the rationale behind our proposed framework of \emph{bidirectional human-AI alignment}.

% % 
% we clarify three core questions before presenting the scope and process of systematic literature review: 
% ``\emph{With whom to align?}'', ``\emph{What is the goal of alignment?}'', and ``\emph{What values should be aligned with?}''




% In this section, we aim to develop a holistic framework encompassing the \emph{ongoing and mutual process} of human-AI alignment given the background in Section~\ref{sec:background}. To this end, we first introduce the core definitions of human-AI alignment (Section~\ref{sec:definition}) and present the scope and its generalizability (Section~\ref{sec:scope}). Next, we perform a systematic literature review guided by the PRISMA workflow (Section~\ref{sec:prisma}) and undertake an iterative coding process to achieve our \emph{bidirectional human-AI alignment} framework (Section~\ref{sec:framework}).








% \vspace{-.8em}
% \subsection{Definitions}
% \label{sec:definition}




% To achieve the aforementioned \emph{ongoing and mutual process of human-AI alignment},
% we clarify three core questions before presenting
% % two core questions need to be clarified before we delve into
% the scope and process of systematic literature review: 
% ``\emph{With whom to align?}'', ``\emph{What is the goal of alignment?}'', and ``\emph{What values should be aligned with?}''










% \subsubsection{\textbf{What is the goal of alignment?}}
\subsection{What is the goal of alignment?}
\label{sec:align_goal}
The research on alignment between humans and AI has introduced multiple alignment goals~\cite{park2023generative,xie2024can}, such as \emph{intentions}~\cite{ouyang2022training,anwar2024foundational}, \emph{preferences}~\cite{bansal2023peering,verma2023hindsight}, \emph{instructions}~\cite{bai2022constitutional,liu2023makes}, and \emph{values}~\cite{sorensen2024roadmap,gabriel2020artificial}.
% and others~\cite{park2023generative,xie2024can}. 
However, researchers often use these terminologies interchangeably without clarifying their distinctions.
Drawing from a philosophical view, 
% we refer to~\citet{gabriel2020artificial} and visualize the relations, definitions, and limitations of prevailing alignment goals in Table~\ref{fig:definitions}. 
we summarize the prevailing alignment \emph{goals, their relationships, definitions, and limitations} and visualize them in Table~\ref{fig:definitions} referring to an extensive analysis of the advantages and limitations of different goalss in existing studies~\cite{gabriel2020artificial,stuart2014whitepaper} .
% 
% After an extensive analysis of the advantages and limitations of different goals,
Particularly, \citet{gabriel2020artificial} argues \emph{values}, e.g., moral beliefs and principles, to be the best possible goal at the current stage for AI development for focusing alignment. 
We further summarized the rationale behind this argument and the discussion of the trade-offs that arise from this choice in Table~\ref{fig:definitions}.
% 
The claim of ``aligning AI with human values'' is not new, as Stuart Russell~\cite{stuart2014whitepaper} has stated back in 2014 that \say{\emph{for an autonomous system to be helpful to humans and to pose no unwarranted risks, it needs to align its values with those of the humans in its environment in such a way that its actions contribute to the maximization of value for the humans.}}
% 
Therefore, in this work, we \textbf{consider the goal of alignment as ``human values''}, which means AI systems do what people morally
ought to do, as defined by individuals or society. 
% 
% 
% We further revolve our paper review and data analysis around clarifying and categorizing human values. Particularly, to disambiguate the inconsistent definitions around values in alignment, we expanded a comprehensive structure and taxonomy of human values grounded in psychology and social science. Furthermore, we matched the surveyed literature with the appropriate values if applicable (articulated in Section~\ref{sec:value_category} and Section~\ref{sec:gap_value}).










% \begin{figure*}[!t]
%   \centering
%   \includegraphics[width=1\textwidth]{figures/value_structure.pdf}
%   \caption{The relations of human values for AI development
%   % The structure of the dynamic relations among values 
%   (adapted from~\citet{schwartz2012overview}). 
%   We consider 5 \emph{high-order value types} (\eg Self-enhancement and Openness to change), which encompass 12 \emph{motivational value types} (\eg power, universalism, functionality). We further organize the relation among these value types along two dimensions: 1) different sources (\ie individuals, society and interaction) and 2) different self intentions (\ie self-protection against threat and self-expansion and growth). The \emph{Desired values for AI tools} was added empirically from \emph{bottom-up} our paper survey whereas others are inherited from~\citet{schwartz2012overview}. 
%     % 
%   % The typology is based on Schwartz Theory of Basic Values and an empirical collection of values that are commonly been studied.
%   % Some values conflict with one another (\eg Benevolence and Power) whereas others are compatible (\eg Conformity and Security). This structure of values refers to these relations of conflict and congruence among values~\cite{schwartz1994there,schwartz2012overview}.
%   % 
%   % A fine-grained taxonomy of values related to bidirectional human-AI alignment. The taxonomy is based on Schwartz's Theory of Basic Values and an empirical collection of values that are commonly been studied.
%   }
%   \label{fig:value_structure}
%   % \vspace{-2em}
% \end{figure*}





\begin{table*}[!t]
  \centering
  \includegraphics[width=1\textwidth]{figures/value_content.pdf}
  \caption{The relations and a fine-grained taxonomy of \textbf{69 exemplary human values}. 
  We consider 5 high-order value types encompassing 12 motivational value types, indicated by their sources (e.g., individuals, society and interaction).
  % The typology is based on Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012overview} and an empirical collection of values that are commonly been studied.
  The exemplary values with red dot (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) indicates there are no work in our surveyed papers examining the specific values. 
  % Note that humans might not expect AI to encode all these values, which could potentially result in harm and risks. 
  % The values with red dot (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) and \textcolor{hua-red}{red color} means that humans might not expect AI to embed these values in AI, which could potentially result in harm and risks.
  % % 
  % % 
  % choose own goal\cite{lima2020collecting}
  % creativity\cite{ashktorab2020human}
  % curiosity\cite{jiang2023evaluating}
  % freedom\cite{lima2020collecting}
  % independence\cite{kang2023values}
  % privacy\cite{10.1145/3544548.3580903}
  % reflectiveness\cite{yan2023complex}
  % factuality\cite{hosking2023human}
  % self-respect\cite{wu2023cross}
  % diversity\cite{kapania2023hunt}
  % capability\cite{xu2023lemur}
  % influence\cite{huang2023humanity}
  % intelligence\cite{park2023generative}
  % success\cite{kang2023values}
  % resilience\cite{ye2023flask}
  % authority\cite{lima2021human}
  % wealth\cite{santurkar2023whose}
  % reciprocation of favours\cite{zagalsky2021design}
  % moderation\cite{lai2022human}
  % devout\cite{santy2023nlpositionality}
  % politeness\cite{zhu2023unmasking}
  % self-discipline\cite{zhou2023realbehavior}
  % forgiving\cite{wu2023cross}
  % helpfulness\cite{jin2022make}
  % honesty\cite{he2023hi}
  % emotional\cite{huang2023humanity}
  % responsiblity\cite{ma2023towards}
  % true friendship\cite{isajanyan2024social}
  % cooperation\cite{he2023interaction}
  % collectivism\cite{nie2024moca}
  % democracy\cite{santurkar2023whose}
  % inclusive\cite{ramezani2023knowledge}
  % equality\cite{sheng2021societal}
  % equity\cite{goldfarb2023prompt}
  % accessibility\cite{zhang2023visar}
  % adaptability\cite{oh2023pk}
  % economic\cite{bakker2022fine}
  % transparency\cite{boyd2021datasheets}
  % autonomy\cite{wang2023humanoid}
  % awareness\cite{paleja2021utility}
  }
  \label{fig:value_taxonomy}
  \vspace{-3.4em}
\end{table*}





% \subsubsection{\textbf{With whom to align?}}
\subsection{With whom to align?}

% 
Pertinent stakeholders within the AI landscape can be the potential objects for AI to align with, including lay people (\eg end users of AI systems)~\cite{qi2023fine}, AI practitioners (\eg developers, researchers)~\cite{boggust2022shared,anwar2024foundational,ngo2022alignment}, organizational entities (\eg technology firms, professional communities), national/international bodies (\eg governments, legislative bodies)~\cite{deshpande2022responsible} and others.
% 
% 
Many alignment research papers have focused on general humans without specifying particular groups~\cite{yao2023instructions,liu2022aligning,guo2023beyond}. Nevertheless, different groups hold different, sometimes even contrasting, values~\cite{gabriel2020artificial}.
% 
As a consequence, rather than identifying a \emph{true moral theory} as a \emph{one-size-fits-all} value, prior alignment research argues to select the appropriate principles for compatible human groups~\cite{sorensen2024roadmap}.
To this end, \emph{pluralistic value alignment}, grounded on social choice theory~\cite{arrow2012social}, proposes combining individual views fairly in developing alignment principles as a potential solution~\cite{sorensen2024roadmap}.
% 
% 
In this work, 
we also consider values from this pluralistic perspective,
% we define the \textbf{source of values with the aim of pluralism}, 
where AI should be aligned with \textbf{pluralistic human individuals and societal groups} who would ultimately be impacted by AI. 






% \subsubsection{\textbf{What are the values to be aligned with?}}
\subsection{What are the values to be aligned with?}
\label{sec:human_values_definition}


While previous studies have aimed to align AI with human values, the specific values they examined are often ambiguous and inconsistent.
% 
% 
% While many papers claim to integrate or evaluate AI in relation to human values, the specific sets of human values they examine often lack clarity or comprehensiveness. 
% In order to articulate and systematically understand 
To clarify human values relevant to human-AI alignment, we structured human values using a combination of top-down and bottom-up methods based on the \textbf{Schwartz Theory of Basic Values}~\cite{schwartz1994there,schwartz2012overview}.
% , which offers is a universal model outlining broad values that steer human behavior grounded in psychology.
% 
Among various human value theories (\eg Moral Foundation Theory~\cite{graham2013moral}, Social Norms \& Ethics~\cite{forbes2020social}), we chose the Schwartz Theory of Basic Values primarily considering that its definitions and dimensions are universal and are applicable for most people across \emph{(a)} various cultures and countries; \emph{(b)} various divisions including individuals, interactions and groups; and \emph{(c)} is commonly accepted in previous NLP studies~\cite{kang2023values,kiesel2022identifying}.
% 
% 
Specifically, \citet{schwartz1994there} provided a \textbf{clarified definition of human values} by summarizing
some widely agreed-upon features as:
% 
% \begin{quote}
    \emph{\say{A value is a (1) belief (2) pertaining to desirable end states or modes of conduct, that (3) transcends specific situations, (4) guides selection or evaluation of behavior, people, and events.}}
% \end{quote}
\citet{schwartz1994there} further offered a universal model outlining broad values that steer human behavior grounded in psychology.
% 
% 
% 

% \noindent
\textbf{A Comprehensive Taxonomy of Human Values}.
Nevertheless, this conventional theory was developed without the context of human-AI interaction, which might overlook values that need to be considered for human-AI alignment. Therefore, we used a \emph{bottom-up} approach to extract all values studied in our collected alignment literature (elaborated in Section~\ref{sec:prisma}), mapped them onto the Schwartz Theory of Basic Values, and supplemented the theory with AI-related structure and content. 
% 
% 
As a result, we identified the structural relationships among human values (see Figure~\ref{fig:value_structure}) and mapped existing literature to a fine-grained taxonomy (see Table~\ref{fig:value_taxonomy}). 
% 
% 
As shown in Figure~\ref{fig:value_structure}, we supplemented the traditional theory's four high-order value types (\ie ``Self-Enhancement'', ``Openness to Change'', ``Conservation'', ``Self-Transcendence'') with a novel high-order value type, named ``Desired Values for AI Tools'' that encompasses two motivational value types (\ie ``Usability'' and ``Human-Likeness'').
% 
We further organize the relationship among these value types along two dimensions~\cite{schwartz2012overview}: different resources (\ie individuals, society and interaction) and different self-intentions (\ie self-protection against threat and self-expansion and growth).
% 
% 
% 
Furthermore, we elaborate the definitions of the 12 motivational value types and their exemplary values by mapping them to relevant human-AI alignment papers from our corpus in Table~\ref{fig:value_taxonomy}. 
% 
During the process of mapping, we found: 1) value terms in empirical papers were often named differently (\eg capability and competence), or check their opposites (\eg fairness and bias); 
2) there are many values not studied in our corpus, \ie indicated as (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) in the Figure.



% which can be potentially due to several reasons, such as difficulty in measurement (e.g., inner harmony), or not common use cases (e.g., Detachment).



% Built upon these clarified definitions, we start to use a \emph{top-down} method to adopt the well-defined \emph{value taxonomy} and the \emph{structural relationship} presented by~\citet{schwartz1994there,schwartz2012overview}. 
% As the conventional theory is missing the context of AI-system and human-AI interactions, we further supplement the \emph{value taxonomy} and the \emph{structural relationship}. Specifically, we used a \emph{bottom-up} way to extract all values studied in the literature and map them into the Schwartz Theory of Basic Values. Further, we added the missing values and relationship regarding the AI context to make our outcome more comprehensive.





% a theory of cross-cultural psychology. As a result, we identified the structural relationships among human values (see Figure~\ref{fig:value_structure}) and mapped existing literature to a fine-grained taxonomy (see Figure~\ref{fig:value_taxonomy}). 
% Additionally, we present our analysis findings of human values that are particularly relevant for future studies (Section~\ref{sec:value_finding}).







% \subsubsection{
% \textbf{Methodology: A Combination of Top-Down and Bottom-Up Way to Structure Human Values}
% % }
% \label{sec:value_method}
% % \mbox{}
% To recognize human values systematically, we grounded our exploration on the Schwartz Theory of Basic Values~\cite{schwartz1994there,schwartz2012overview}, which is a theory of cross-cultural psychology built upon the \citet{rokeach1973nature}'s value survey. 

% We chose the Schwartz Theory of Basic Values primarily considering that its definitions and dimensions are universal and are applicable for, or almost for, all people across \emph{(a)} various cultures and countries; \emph{(b)} various sources including individuals, interactions and groups; and \emph{(c)} commonly accepted in previous NLP studies~\cite{kang2023values,kiesel2022identifying}.
% % 
% % 
% \citet{schwartz1994there} provided a clarified definition of human values by summarizing some widely agreed-upon features as:
% % 
% % \begin{quote}
%     \emph{\say{A value is a (1) belief (2) pertaining to desirable end states or modes of conduct, that (3) transcends specific situations, (4) guides selection or evaluation of behavior, people, and events.}}
% % \end{quote}
% % 


% Built upon these clarified definitions, we start to use a \emph{top-down} method to adopt the well-defined \emph{value taxonomy} and the \emph{structural relationship} presented by~\citet{schwartz1994there,schwartz2012overview}. As the conventional theory is missing the context of AI-system and human-AI interactions, we further supplement the \emph{value taxonomy} and the \emph{structural relationship}. Specifically, we used a \emph{bottom-up} way to extract all values studied in the literature and map them into the Schwartz Theory of Basic Values. Further, we added the missing values and relationship regarding the AI context to make our outcome more comprehensive.




% % \subsubsection{
% \textbf{Outcome: The Relations of Human Values and Fine-grained Taxonomy}
% % }
% \label{sec:value_outcome}
% % \mbox{}
% % 
% % Consequently, 
% We developed a more comprehensive structure of the dynamic relations of human values (Figure~\ref{fig:value_structure}) and their fine-grained taxonomy with mapped reference papers for exemplary values (Figure~\ref{fig:value_taxonomy}) after incorporating the AI-related context. 
% % 
% % 
% % 
% % 
% Considering the dynamic relations of human values in Figure~\ref{fig:value_structure}, we consider five \emph{high-order value types} (\ie self-enhancement, openness to change, conservation, self-transcendence and desired values for AI tools), which encompass 12 \emph{motivational value types} (\eg power, universalism, functionality).
% We further organize the relation among these value types along two dimensions: 1) different resources (\ie individuals, society and interaction) and 2) different self intentions (\ie self-protection against threat and self-expansion and growth).
% Note that the type of \emph{Desired Values of AI Tools} and its encompassed \emph{motivational values} (\ie functionality and human-likeness) are the supplemental value types we added from the empirical \emph{bottom-up} process introduced above.
% Also, it is worth noting that some values conflict with one another (\eg Benevolence and Power) whereas others are compatible (\eg Conformity and Security). This structure of values refers to these relations of conflict and congruence among values~\cite{schwartz1994there,schwartz2012overview}.
% % 
% 
% 
% 


% % 
% Furthermore, we elaborate the definitions of the 12 motivational value types and their exemplary values with mapped paper reference in Figure~\ref{fig:value_taxonomy}. During the process of mapping existing literature to these values, we noted two findings: 1) value terms in empirical papers were often named differently (\eg capability and competence), or check their opposites (\eg fairness and bias), from the listed exemplary values of Schwartz's theory even they are examining the same thing essentially . 2) there are many values not studied in our collected literature (indicated as (\hspace*{.0em}\numimgdot{figures/red_dot.pdf}\hspace*{.0em}) in the Figure). 









\begin{table*}[ht]
\centering
\vspace{-6pt}
\begin{tabular}[t]{@{}  !{\color[HTML]{808080}\vrule width 2pt} p{.98\textwidth} !{\color[HTML]{808080}\vrule width 2pt} @{}}
\cellcolor[HTML]{E6E6E6} 
\textbf{Takeaways \& Implications for Alignment Clarifications} 
% \newline
\vspace{5pt}

1. We propose the ``pluralistic human values'' as the alignment goal, wherein AI should be aligned with the diverse perspectives of individuals and societal groups who may be directly or indirectly impacted by AI.
\vspace{5pt}

2. Many exemplary human values outlined in Table~\ref{fig:value_taxonomy}, such as loyalty and environmental protection, are important for alignment but are often overlooked or underexplored in current research.
% 
\vspace{5pt}

3. The human value system should account for complex application contexts and relationships, such as priorities and conflicts, rather than focusing on an exclusive subset of values.
\end{tabular}
\vspace{-10pt}
\end{table*}



\vspace{-5pt}
% \subsection{Scopes and Generalizability}
\subsection{Scopes and Key Components in Alignment}
\label{sec:scope}

This section clarifies the key components we considered in \emph{human-AI alignment}. Additionally, we define the scopes of each key component as commonly adopted in current research.
% 
% We define the scope of alignment by specifying the key components we considered in \emph{human-AI alignment}. 
% We focus on a representative scope of alignment studies and discuss the generalizability of the scope after that.

% We define the scope of our literature review by specifying the key components we considered in \emph{human-AI alignment}. Given the broad definitions as aforementioned, it is infeasible to include all alignment research in practice. Therefore, we focus on a representative scope of alignment studies and discuss the generalizability of the scope after that.



\begin{itemize}
    \item \textcolor{hua-red}{\textbf{Humans.}} 
    % \textbf{With whom should AI align?} 
    % \emph{\textbf{align with whom?}}
    Our primary focus is on human \humancode{individuals}, \humancode{groups}, or \humancode{organizations} that will ultimately develop, use, and potentially impact or be influenced by AI systems, 
    % Our primary focus is on \humancode{individuals} or \humancode{human groups} that will ultimately use AI systems and might be affected by them, 
    as these are the entities with which AI systems should align. We emphasize the importance of considering the pluralistic values of diverse users rather than treating users as a monolithic group.
    % 
    % Our primary focus is on \humancode{individuals} or \humancode{human groups} who will ultimately use AI systems and who might be affected by AI systems, as these are the entities that AI systems should align with. 
    % Particularly, we emphasizes the importance of considering the pluralistic values of diverse users, rather than treating them as a monolithic group. 
    % These individuals and groups may be significantly impacted by the deployment of AI systems for various purposes, and thus their perspectives are crucial for ensuring alignment. 
    % \diyi{does "user" who might be affected by AI (rather than just end users) belong to the current scope of consideration?}
    % \hua{[DONE]great point! we do contain both users that ``might be affected by AI'' in Section 4.4.2. Let me correct this definition to be more precise :) }
    % , including citizens from different cultural backgrounds and marginalized communities. 

    % We advocate for more nuanced approaches that involves engaging with various sub-communities and individuals within the end user population.
    
    \item
    \textcolor{hua-blue}{\textbf{Artificial Intelligence (AI).}} 
    % Locating the elusive scope of AI is difficult. The technical boundary of AI, even in AI research communities, is disputed and continuously evolving~\cite{yang2020re}. 
    % 
    % As the advent of AGI increased the significance of AI alignment, w
    % 
    % 
    % We primarily focus on AI systems that have been extensively researched in the field of human-AI alignment, especially after the advent of AGI. 
    We focus on AI systems including both \aicode{domain-specific AI systems} that address specific tasks (\eg reasoning, dialogue) and \aicode{general-purpose AI models} that aim to complete any tasks with performance comparable to a human's.
    These AI systems include generative, classification, and regression models, among others.
    % \aicode{language models}, \aicode{reinforcement learning models}, neural network-based \aicode{classification and regression models}, among others. 
    % These technologies include \aicode{language models}, \aicode{reinforcement learning models}, neural network-based \aicode{classification and regression models}, among others. 
    Particularly, we primarily focus on language models as the representative AI models for alignment research, and discuss how the insights from this study can be generalized to other modalities at the section end.


    
    % \item
    % \textcolor{hua-yellow}{\textbf{Alignment.}} 
    % Our review encompassed all the \aligncode{alignment goals} outlined in Section~\ref{sec:align_goal}, with a particular focus on \aligncode{\emph{value alignment}} by clarifying alignment values and identifying both the explicit and implicit values in each paper reviewed. Additionally, alignment can also involve the representation or behavioral aspects between humans and AI, which were not included in this study for a more focused scope~\cite{mcgrath2023can,park2023generative,xie2024can}.
    

    \item
    \textcolor{hua-yellow}{\textbf{Alignment.}} 
    Our review encompassed all the \aligncode{alignment goals} outlined in Section~\ref{sec:align_goal}.
    Since many studies emphasized the importance of \aligncode{value alignment}~\cite{gabriel2020artificial,stuart2014whitepaper}, we particularly summarized a clarified taxonomy of alignment values and identified the value in each paper (if applicable).
    Additionally, we focus on analyzing the AI models' output and generation, but not the neural network's intermediate representations~\cite{mcgrath2023can,park2023generative,xie2024can}, for alignment research.
    % 
    % , with a particular focus on \aligncode{\emph{value alignment}} by clarifying alignment values and identifying both the explicit and implicit values in each paper reviewed. 
    % Additionally, alignment can also involve the representation or behavioral aspects between humans and AI, which were not included in this study for a more focused scope~\cite{mcgrath2023can,park2023generative,xie2024can}.



    
    
    % Our review covered all goals introduced in Section~\ref{sec:align_goal}, with an emphasis on clarifying alignment values and recognizing the explicit and/or implicit values in each reviewed paper. For a even broader scope, alignment can also encompass the representation or behavioral~\cite{park2023generative,xie2024can} between humans and AI, which are excluded in this study.
    
    % We focus on \emph{value alignment} in this study, where we also provide clarified definitions of \emph{what human values encompass} in Section~\ref{sec:value_category}.
    % \diyi{any justification on why "value" is more important here compared to focusing on other dimensions?}
    % \hua{thanks for the valuable suggestion! we added Sec5.2.2 for elaborating this, but should also briefly justify here. 
    % In short, we justify with at least three reasons: 1) values in our study are used to characterize a wide range of humans, including cultural groups, societies, and individuals (including cultural and religious characteristics as well, see Fig~\ref{fig:schwartz} - Tradition). 
    % 2) values can be used to explain the motivational bases of attitudes and behavior, which can be considered as the sources of many human behavior and preferences.
    % 3) there lacks a clarified definition of ``what human value is'' despite the large number of studies about ``human-AI alignment for values'' . We delve into this issue and aim to provide a clarified definition for it.}
    % There are also diverse factors that we might want to consider for "alignment" beyond "values" such as norms and cultures. 
    % To further provide a comprehensive scope of human-AI alignment, as motivated in Section~\ref{sec:background}, this study introduces a novel conceptual framework termed ``\emph{\aligncode{bidirectional human-AI alignment}}''. Specifically, our exploration of alignment extends beyond the conventional notion of \aligncode{aligning AI to human values} (\ie integrating human values to guide, control, and personalize AI systems) to further involve \aligncode{aligning human to AI outputs} (\ie how humans can adapt to and interact effectively with advancing AI technologies).
    % % This framework involves research on integrating human values to guide, control, and personalize AI systems, as well as studies on how humans can adapt to and interact effectively with advancing AI technologies. 
    % Detailed definitions are presented in Section~\ref{sec:scope} for clarity and elaboration.
    % % 
    
\end{itemize}




% \begin{table*}[ht]
% \centering
% \vspace{-10pt}
% \begin{tabular}[t]{@{}  !{\color[HTML]{808080}\vrule width 2pt} p{.98\textwidth} !{\color[HTML]{808080}\vrule width 2pt} @{}}
% \cellcolor[HTML]{E6E6E6} 
% \textbf{Takeaways \& Implications for Alignment Clarifications} 
% % \newline
% \vspace{5pt}

% 1. We propose the ``pluralistic human values'' as the alignment goal, wherein AI should be aligned with the diverse perspectives of individuals and societal groups who may be directly or indirectly impacted by AI.
% \vspace{5pt}

% 2. Many exemplary human values outlined in Table~\ref{fig:value_taxonomy}, such as loyalty and environmental protection, are important for alignment but are often overlooked or underexplored in current research.
% % 
% \vspace{5pt}

% 3. The human value system should account for complex application contexts and relationships, such as priorities and conflicts, rather than focusing on an exclusive subset of values.
% \end{tabular}
% \vspace{-10pt}
% \end{table*}







% % We recognize that our current work exists within a broader context of studies concerning human-AI alignment. 
% \noindent
% We acknowledge the extensive scope and rapid advancements of research in this area, and posit that our study offers insights that can be generalized to various modalities. For example, the value taxonomy and human-in-the-loop evaluation paradigm outlined in our framework can be applied to both text-based and other modality-based (\eg vision, robotics) models. 
% % 
% It's worth noting that our literature review does not aim to exhaustively cover all papers in the field, which is impossible given the rapid advancement of human-AI alignment research. Instead, we adopt a human-centered perspective to review more than 400 key studies in this domain, focusing on delineating the framework landscape, identifying limitations, future directions, and a roadmap to pave the way for future research.








% \subsection{Why Do We Need Bidirectional Alignment?}
% \label{sec:scope}

\subsection{Systematic Literature Review and Framework Rationale}
\label{sec:review}


% We consider the goal of alignment as ``human values'' from a pluralistic perspective,
% where AI should be aligned with \textbf{pluralistic human individuals and societal groups} who would ultimately be impacted by AI. 
Achieving the alignment between AI and human values necessitates collaboration among interdisciplinary AI practitioners (\eg developers and researchers).
To comprehensively analyze the research literature pertaining to this ongoing, mutual process of human-AI alignment, we conducted a systematic literature review adhering to the the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332}.
% To understand the research literature relevant to the ongoing, mutual process of human-AI alignment, 
% we performed a systematic literature review based on the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332}.
% 
% 
Our iterative selection process yielded 411 papers from an initial pool of 34,213 publications, spanning the period from January 2019 to January 2024. These papers were sourced from leading venues across multiple AI-related domains, including Natural Language Processing, Human-Computer Interaction,  Machine Learning, and more, using well-defined keywords and criteria. 
A group of 13 interdisciplinary researchers coded the papers. Through iterative discussions, we developed the paper codes and proposed framework (Section~\ref{sec:method}). Detailed steps and processes are elucidated in Appendix~\ref{app:system_review}.
% 


% \noindent


\subsection{Rationale Behind the Framework}
\label{sec:motivation}
% \textbf{Rationale Behind the Framework.} 
Our systematic review revealed that current research largely overlooks the nature of \textbf{long-term dynamic changes} and the \textbf{importance of interaction} in human-AI alignment.
% 
% 
First, the manifestation of certain AI risks, harms, and the practical quality of AI services primarily emerge through interaction between humans and AI systems~\cite{weidinger2023sociotechnical}. 
% 
For instance, \citet{shen2020useful} discovered that AI explanations, deemed effective by AI developers and researchers, were found not useful for humans in real-world scenarios of interactive AI error detection.
% 
% 
Additionally, the use of AI influences human thinking and behavior, which in turn alters their values when interacting with AI.
% 
For instance, \citet{li2024value} found that incorporating AI assistance in writing workflows changed humans' writing perceptions, behavior, and performance, creating new requirements for developing the next generation of AI writing assistants~\cite{lee2024design}.


In light of these findings, we posit that AI practitioners must expand their focus beyond merely ``Aligning AI to Humans'' -- a paradigm centered on integrating human specifications to train, steer, and customize AI. Equal emphasis must be placed on ``Aligning Humans to AI'', a complementary paradigm investigating human cognitive and behavioral adaptation to AI. This latter aspect is crucial in supporting individuals and society at large in understanding, critiquing, collaborating with, and adapting to transformative AI advancements.
To encapsulate these comprehensive perspectives, we propose the ``\textbf{Bidirectional Human-AI Alignment}'' framework, and provide its definition below Figure~\ref{fig:teaser}.
% 
This holistic framework acknowledges the reciprocal nature of alignment, 
addressing both the advancements of AI systems to incorporate human values, and the evolving human adaptation of AI systems in real-world practice.






% Consequently, AI practitioners should not only focus on "Aligning AI to Humans," which emphasizes integrating human specifications to train, steer, and customize AI. Equally important is "Aligning Humans to AI," which examines humans' cognitive and behavioral adaptation to AI systems. This approach supports individuals and society in understanding, critiquing, collaborating with, and adapting to transformative AI advancements. Consequently, we propose the "Bidirectional Human-AI Alignment" framework to encompass these comprehensive perspectives.
% 
% 
% Based on the systematic review, we found that existing research large neglects the nature of \textbf{long-term dynamic changes} and \textbf{importance of interaction} of human-AI alignment. 
% First, it is from interaction that AI risks and harms can be manifested or the quality of AI service and evaluated practically~\cite{weidinger2023sociotechnical}. 
% For example, \citet{shen2020useful} finds that AI explanations, which are developed and validated to be effective by AI developers, are found not useful for humans in interactively detecting AI mistakes in practice.
% 
% Additionally, the usage of AI changes how humans think and behave, and further changes their values when interacting with AI. 
% For instance, ~\citet{li2024value} finds that incorporation of AI assistance in writing workflows changes humans' writing perceptions and performance. These changes of human cognition and behaviors further put novel requirements on developing next generation of AI writing assistants~\cite{lee2024design}.
% 
% 
% In summary, AI practitioners should not only consider ``Aligning \textcolor{hua-blue}{AI} to \textcolor{hua-red}{Humans}'', which focuses on integrating human specifications to train, steer and customize AI. Crucially, AI practitioners should place equal emphasis on the significance of ``Aligning \textcolor{hua-red}{Humans} to 
% \textcolor{hua-blue}{AI}'', which investigates humans' cognitive and behavioral adaptation to the AI systems, that supports individuals and the broader society in understanding, critiquing, collaborating with and adapting to transformative AI advancements. 
% Consequently, we propose the ``Bidirectional Human-AI Alignment'' framework to encompass these comprehensive perspectives.




% ``Align \textcolor{hua-blue}{AI} to \textcolor{hua-red}{Humans}'' and ``Align \textcolor{hua-red}{Humans} to 
% \textcolor{hua-blue}{AI}''.
% 
% 
% , AI-driven writing assistants changed humans' writing behavior and demands on AI values from primarily emphasizing  on AI accuracy to more diverse needs on AI values, such as being creative, empathetic, enjoyable, fair, unique, and more~\cite{lee2024design}.




% \hua{Motivate the "bidirectional alignment framework",
% introduce systematic review,
% transit to framework,
% introduce 4 research questions
% - Why these research questions? how to use these questions? -- Reshmi}






% \reshmi{R\\
% Q1: For any developer or researcher reading the paper how do they choose research questions based on their task and scenario\\

% Q2: Also what are some values that should not be sacrificed as part of using this bi-directional framework\\

% Q3: }


% \hua{write more towards motivation here. very concretely motivate the framework.}
% % 





% ===============================================

% The aforementioned background motivates this work to present a clarified definition and scope for human-AI alignment before conducting the comprehensive review on the state-of-the-art research. Additionally, achieving alignment between human and AI necessitates a holistic understanding of human cognition and behavior, societal norms, as well as AI algorithmic capabilities and limitations. 
% % 
% Therefore, we collected a varied range of state-of-the-art papers covering interdisciplinary fields and perspectives related to human-AI alignment primarily published from 2019 to 2024. We next introduce the clarified definitions and scope adopted in this work, and the process of systematic literature review we conducted to arrive at our bidirectional human-AI alignment framework and associated findings elaborated in the following sections.
% % 
% \hua{Section 3 and Section 2 are overlapping in many places, trim some of them.}


% To develop the framework of bidirectional human-AI alignment, we first decide on the scope and core aspects of human-AI alignment.








% The advent of sophisticated and versatile AI technologies has underscored the necessity for ongoing discussions surrounding AI alignment. However, existing literature approaches human-AI alignment from various angles, lacking a clarified definition of ``\emph{what is human-AI alignment?}'', ``\emph{what should be aligned}'' and ``\emph{aligned with whom?}''. 
% % 
% % 
% % 
% % 
% As elaborated in Section~\ref{sec:background}, human-AI alignment has been referred to as \emph{intention alignment}~\cite{anwar2024foundational}, \emph{behavior alignment}~\cite{park2023generative,xie2024can}, \emph{instruction alignment}~\cite{bai2022constitutional,liu2023makes}, \emph{value alignment}~\cite{sorensen2024roadmap,gabriel2020artificial}, etc. Furthermore, the alignment objects could be aligning AI's \emph{intermediate representations}~\cite{liu2023learning}, \emph{internal reasoning process}~\cite{mcgrath2023can}, and/or generations~\cite{corvelo2024human,ouyang2022training} with all pertinent AI stakeholders~\cite{deshpande2022responsible} (\eg AI practitioners~\cite{boggust2022shared} and end-users~\cite{qi2023fine}).
% % 
% % 
% These varied investigations present expansive interpretations of human-AI alignment, underscoring the intricate nature and breadth of research in this field~\cite{kirchner2022researching}. Drawing upon numerous extant literature reviews and seminal studies on human-AI alignment~\cite{matthews2022alignment,gabriel2020artificial,kenton2021alignment,yao2023instructions, ganguli2022red,terry2023ai,wang2023aligning,
% askell2021general,kirchner2022researching}, this work clarifies an examination of the definition and scope of human-AI alignment adopted in this work by elaborating the pertinent terminologies.
% % : \emph{who should AI align with}? \emph{which AI technologies are the primary focus of this study}? and \emph{what does alignment entail within the context of human-AI interactions}? 
% Specifically, we provide our detailed definitions within the context of this study as below:
% \hua{[TODO] merge this section with above.}





% \begin{quote}
%     \say{\emph{For an autonomous system to be	helpful to humans and to pose no unwarranted risks, it needs to align its values with those of the humans in its environment in such a way that its actions contribute to the maximization of value for the humans.}} \\
%     {\hspace*{100pt}~\textit{---  Stuart Russell, White Paper: Value Alignment in Autonomous Systems, 2014 ~\cite{stuart2014whitepaper}}}
%     % \cite{stuart2014whitepaper}
% \end{quote}


% \epigraph{\say{\emph{For an autonomous system to be	helpful to humans and to pose no unwarranted risks, it needs to align its values with those of the humans in its environment in such a way that its actions contribute to the maximization of value for the humans.}}}{\textit{--- 
%  Stuart	Russell, White Paper: Value Alignment in Autonomous Systems, 2014 ~\cite{stuart2014whitepaper} \\}}



% \begin{itemize}




    % % \item 
    % \textcolor{hua-yellow}{\textbf{Alignment.}} 
    % % \textbf{What does alignment entail within the context of human-AI interactions}? 
    % \emph{\textbf{what is human-AI alignment?}}
    % We focus on \emph{value alignment} in this study, where we also provide clarified definitions of \emph{what human values encompass} in Section~\ref{sec:value_category}.
    % \diyi{any justification on why "value" is more important here compared to focusing on other dimensions?}
    % \hua{thanks for the valuable suggestion! we added Sec5.2.2 for elaborating this, but should also briefly justify here. 
    % In short, we justify with at least three reasons: 1) values in our study are used to characterize a wide range of humans, including cultural groups, societies, and individuals (including cultural and religious characteristics as well, see Fig~\ref{fig:schwartz} - Tradition). 
    % 2) values can be used to explain the motivational bases of attitudes and behavior, which can be considered as the sources of many human behavior and preferences.
    % 3) there lacks a clarified definition of ``what human value is'' despite the large number of studies about ``human-AI alignment for values'' . We delve into this issue and aim to provide a clarified definition for it.}
    % There are also diverse factors that we might want to consider for "alignment" beyond "values" such as norms and cultures. 
    % To further provide a comprehensive scope of human-AI alignment, as motivated in Section~\ref{sec:background}, this study introduces a novel conceptual framework termed ``\emph{\aligncode{bidirectional human-AI alignment}}''. Specifically, our exploration of alignment extends beyond the conventional notion of \aligncode{aligning AI to human values} (\ie integrating human values to guide, control, and personalize AI systems) to further involve \aligncode{aligning human to AI outputs} (\ie how humans can adapt to and interact effectively with advancing AI technologies).
    % % This framework involves research on integrating human values to guide, control, and personalize AI systems, as well as studies on how humans can adapt to and interact effectively with advancing AI technologies. 
    % Detailed definitions are presented in Section~\ref{sec:scope} for clarity and elaboration.
    % % 
    % \hua{define alignment beyond values.}




% ============================================================

% ====================== NEW ADDED =======================


% In terms of ``\emph{\aligncode{what is human-AI alignment?}}'', 
% alignment has been referred to as \emph{intention alignment}~\cite{anwar2024foundational}, \emph{behavior alignment}~\cite{park2023generative,xie2024can}, \emph{instruction alignment}~\cite{bai2022constitutional,liu2023makes}, \emph{value alignment}~\cite{sorensen2024roadmap,gabriel2020artificial}, etc. 
% % 
% % 
% % There are also diverse factors that we might want to consider for "alignment" beyond "values". for instance, norms and cultures. 
% % maybe you will clarify this in the later section! 

% % intent alignment description;
% \citet{ouyang2022training} and \citet{anwar2024foundational} consider alignment from the perspective of 
% AI safety~\cite{anwar2024foundational,wang2023aligning}, where it refers alignment to be \emph{intent alignment} by fine-tuning with human feedback. 
% % 
% Their goal of alignment is to assure safety (\ie unlikely to contribute to unplanned, undesirable harms) when the systems are deployed and used~\cite{weidinger2023sociotechnical}. 
% % 
% % 
% % 
% % 
% % behavior alignment description;
% \citet{park2023generative} introduces generative agents that draw on generative models to simulate and align with believable individual and emergent group behavior, in which the computational agents can wake up, cook breakfast, form opinions and initiate conversations, etc.
% % 
% % 
% % 
% % instruction alignment description;
% % 
% ~\citet{bai2022constitutional} form the human supervision as a set of principle instructions that should govern AI behavior, along with a small number of examples as few-shot prompting to instruct models.
% % 
% % value alignment description;
% \citet{gabriel2020artificial} considers AI could be designed to align with the values of system users, where the \emph{values} are defined as ``natural or non-natural facts about what is good or bad, and about what kinds of things ought to be promoted, as specified by the individual or society.''
% A line of studies examine AI alignment with respect to individual and social values~\cite{tay2020would,hendrycks2020aligning,hovy-yang-2021-importance}. Despite the plethora of alignment definitions and studies, yet, the difference and relationship between these alignment goals are vague and less investigated.
% % 
% % 


% =================================================











% %     \item 
%     \textcolor{hua-red}{\textbf{Human.}} 
%     % \textbf{With whom should AI align?} 
%     \emph{\textbf{align with whom?}}
%     Our primary focus is on the \humancode{users} who will ultimately use AI systems and who might be affected by the deployed AI, as these are the entities that AI systems should align with. 
%     % Also, we include users who might be affected by AI.
%     Particularly, our study emphasizes the importance of considering the various values and concerns of \humancode{diverse users}, rather than treating them as a monolithic group. \diyi{does "user" who might be affected by AI (rather than just end users) belong to the current scope of consideration?}
%     \hua{[DONE]great point! we do contain both users that ``might be affected by AI'' in Section 4.4.2. Let me correct this definition to be more precise :) }
%     % , including citizens from different cultural backgrounds and marginalized communities. 
%     These individuals and groups may be significantly impacted by the deployment of AI systems for various purposes, and thus their perspectives are crucial for ensuring alignment. 
%     % We advocate for more nuanced approaches that involves engaging with various sub-communities and individuals within the end user population.


% =================================================






% % 
% % 
% Considering ``\emph{\humancode{align with whom?}}'' Pertinent stakeholders within the AI landscape can be the potential objects for AI to align with, including lay people (\eg end users of AI systems), AI practitioners (\eg developers, researchers)~\cite{boggust2022shared}, organizational entities (\eg technology firms, professional communities), and national/international bodies (\eg governments, legislative bodies)~\cite{deshpande2022responsible}.
% % 
% For instance, \citet{anwar2024foundational} defines an AI systems as `aligned' when it is trying to behave as intended by the LLM developer~\cite{ngo2022alignment}, whereas \citet{qi2023fine} conducts red-teaming studies to investigate the safety risks of LLMs to end-users.
% % 
% There are also studies discussing general humans without specifying human groups~\cite{yao2023instructions}.
% % 
% % 



% =================================================



%     % \item 
%     \textcolor{hua-blue}{\textbf{Artificial Intelligence (AI).}} 
%     \emph{\textbf{what should be aligned?}}
%     We consider AI technologies in this study to primarily concentrate on the \aicode{outputs and/or generations} of modern AI systems that have been extensively researched in the field of human-AI alignment. Notably, we are most interested in literature concerning \aicode{large language models (LLMs)}.
%     \diyi{somewhere you might want to justify the generalization of this human-AI alignment, especially around how inshgts here can go to "multimodal pretrained models"} 
%     \hua{thanks for the constructive suggestion! indeed, we need to clarify a bit more about our what AI we include and also their generalization to other AI systems. I'll do that!}
%     Also, we partially incorporate studies examining cutting-edge machine learning systems, such as reinforcement learning with human feedback, which have significantly advanced the feasibility of human-AI alignment and assisted human decision making in practice.




% =================================================





% There are also studies discussing general humans without specifying human groups~\cite{yao2023instructions,liu2022aligning,guo2023beyond}.
% However, Different groups of people hold different, sometimes even contrasting, values. 
% 
% For instance, \citet{anwar2024foundational} defines an AI systems as `aligned' when it is trying to behave as intended by the LLM developer~\cite{ngo2022alignment}, whereas \citet{qi2023fine} conducts red-teaming studies to investigate the safety risks of LLMs to end-users.
% % 
% There are also studies discussing general humans without specifying human groups~\cite{yao2023instructions}.
% 
% 




% Regarding ``\emph{\aicode{what to be aligned?}}'',
% % 
% existing studies have examined how to align AI's \emph{intermediate representations} with humans'~\cite{liu2023learning}, align AI's \emph{internal reasoning process} to be similar with a human's cognitive process~\cite{mcgrath2023can}, and align AI's \emph{outputs and/or generations with human preferences}~\cite{corvelo2024human,ouyang2022training}.
% % 
% % 
% For example, \citet{liu2023learning} examines the alignment between models' representations and human-compatible decision-focused representations by identifying the nearest neighbors retrieved from dataset.
% \citet{mcgrath2023can} compares the interpretations of AI models with human cognitive theories formulated by studying human behaviors.
% \citet{santurkar2023whose} compares LLM-generated opinions with human responses from various U.S. demographic groups' opinion polls to evaluate their alignment.


% =================================================


% \end{itemize}




% It is essential to acknowledge that the definitions and scope of existing studies relevant to human-AI alignment extend far beyond the confines of our current study. 
% % 
% % 
% % \hua{generalizability discussion}
% However, our study and insights can be naturally generalized to other modalities.
% % =====
% our literature review does not aim to comprehensively cover all relevant studies within the realm of human-AI alignment. Instead, we are driven by a human-centric perspective in reviewing studies on human-AI alignment and focus on delineating the clarified scopes introduced above to explore the framework landscape, identify limitations, and delineate future directions in this field.








% % \subsection{Scopes of Bidirectional Human-AI Alignment}
% % \subsection{Scopes of This Study}
% \subsection{Study Scope and Generalizability}
% \label{sec:scope}





% While the breadth of research in human-AI alignment offers diverse perspectives,
% an increasing number of studies advocate for a comprehensive and clarified scope of human-AI alignment~\cite{terry2023ai,anwar2024foundational}.
% % 
% Therefore, this study, taking from a human-centered perspective~\cite{terry2023ai}, conceptualizes human-AI alignment as a \textbf{bidirectional} process. 
% Concretely, as showed in Figure~\ref{fig:teaser}, we argue that human-AI alignment not only involves the conventional studies that aim to \emph{integrate human values into training, steering, and customizing AI}, which we term as ``\textbf{aligning AI to humans}'' that has been extensively investigated in the fields of ML, NLP, etc. Also, from a human-centered perspective, we deem human-AI alignment should also consider studies around \emph{how humans perceive, critique, collaborate, and adapt to AI advancement}, thus providing better feedback to steer AI development. We term this line of work as ``\textbf{aligning humans to AI}''.
% % 
% % 
% Consequently, the research about alignment between human and AI should \textbf{consider a holistic loop of bidirectional human-AI alignment}, involving both \emph{aligning AI to humans} for improving AI capabilities to be better aligned with human values, and \emph{aligning humans to AI} that helps humans better understand, collaborate, and adapt to the rapidly advanced AI. Thus human and AI can benefit mutually to achieve a harmonious ecosystem.
% % 
% We therefore provide the detailed definitions and scopes of \emph{align AI to humans} and \emph{align humans to AI}, respectively, as below:





% \begin{itemize}

%     \item \textbf{Align  \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Humans}.} \textbf{How to integrate human values to train, steer, and customize AI?}
%     % 
%     We define the process of \emph{aligning AI to humans} as integrating human values to train, steer and customize AI. 



%     \item \textbf{Align \textcolor{hua-red}{Humans} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI}.}
%     \textbf{What should humans do to critically adapt to AI advancement?}~\merrie{But also how can interface design support conveying AI affordances to humans and enabling them to steer AI interactions to meet their preferences?}
%     % 
%     \diyi{are humans adapting to AI consciously or unconsciously? }
%     We designate the process of \emph{aligning humans to AI} as enhancing humans' perception and capabilities to better understand, assess, criticize, and harness transformative AI advancements. 
%     % 
%     % 
%     % \hua{come back here after framework.}
%     % \hua{Eric: The clarified definition itself can be a good contributions;}

% \end{itemize}




% Again, our work targets a specific set of literature within the \emph{bidirectional human-AI alignment} scope, as opposed to all possible studies relevant to the human-AI alignment topic. 
% While our work concentrates on aligning AI outputs and generations with human values relevant to diverse subgroups, there are other extensive of studies, beyond the above scope, to align humans and AI from various aspects (\eg aligning AI's reasoning process with human cognitive processes~\cite{mcgrath2023can}).


% \hua{add the generalization of this scope to more modalities.}


% ======================================================






% Again, our work targets a specific set of literature within the \emph{bidirectional human-AI alignment} scope, as apposed to all possible studies relevant to the human-AI alignment topic. 
% While our work concentrate on aligning AI generations with human values from diverse subgroups, there are other sets of work, beyond our study scope, which extensively examine aligning AI internal reasoning process to be similar with human cognitive process~\cite{mcgrath2023can}. 



% Note that we are aware the existing research about human-AI alignment can be beyond the definitions we scoped above. For example, while our work concentrate on aligning AI generations with human values from diverse subgroups, there are other sets of work, beyond our study scope, which extensively examine aligning AI internal reasoning process to be similar with human cognitive process~\cite{mcgrath2023can}. 
% % 
% \hua{we focus on aligning with human values but not cognitive process; we focus on aligning AI generations but not internel reasoning process, not behavioral alignment }.
% Again, our work targets a specific set of literature within the \emph{bidirectional human-AI alignment} scope, as apposed to all possible studies of the human-AI alignment topic. 
% % 
% % 
% %







% \martin{we don't study: align human and ai underlying cognitive mechanism?}












% % \subsection{Systematic Literature Review}
% \subsection{Systematic Literature Review Process}
% \label{sec:prisma}

% To understand the research literature relevant to the ongoing, mutual process of human-AI alignment, 
% we performed a systematic literature review based on the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332}.
% % 
% Figure~\ref{fig:review_process} shows 
% the workflow of our process for
% % process of our systematic literature review for 
% paper coding and developing the \emph{bidirectional human-AI alignment} framework. We introduce the step details below.
% % We referred to the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332} for reporting the workflow. 



% % \begin{figure*}[!t]
% %   \centering
% %   \includegraphics[width=1\textwidth]{figures/PRISMA.pdf}
% %   \caption{
% %   The selection and refinement process of our systematic literature review. We referred to the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332} to report the workflow.
% %   From the identification of 34,213 records by keyword search, to screen eligible papers against our criteria and arriveg at our final corpus of 411 papers. For each of the stages where literature reviews were excluded (identification, screening, and eligibility) we further present the total of excluded records.}
% %   \label{fig:review_process}
% %   \Description{}
% % \end{figure*}


% \subsubsection{Identification and Screening with Keywords.}

% % To understand the current research literature on bidirectional human-AI alignment,
% % To understand the research literature relevant to the ongoing, mutual process of human-AI alignment, 
% % we performed a systematic literature review based on the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332}.
% % 
% We started with papers published in the AI-related domain venues (including NLP, HCI, and ML fields) beginning from the advent of general-purpose generative AI to present, \ie primarily between January, 2019 and January, 2024 (see details in Appendix~\ref{app:venues}).
% We retrieved 34,213 papers in the initial \emph{Identification} stage.
% Further, we collectively defined a list of keywords (see details in Appendix~\ref{app:keyword}) and screened for papers that included at least one of these keywords (\eg human, alignment) or their variations either in the title or abstract. We included 2,136 papers in this \emph{Screening} stage.
% % We first identify fields closely relevant to our research topic. As a result, we selected the fields of NLP, HCI, and Machine Learning as our pivotal domains and the related conference venues ranging from 2019 to 2024 we considered in this project in Appendix~\ref{app:venues}.
% % 
% % 
% % From the ACL Anthology, OpenReview and ACM Digital Library, we retrieved 34,190 papers into a Reference Manager Tool (\ie Paperpile).
% % 
% % 

% % To further collect the relevant papers, two of the authors collectively defined a list of keywords related to bidirectional human-AI alignment, such as \emph{human}, \emph{alignment}, \emph{interact}, \emph{LLM}, \emph{value}, etc. Next, we only sampled the papers that included these keywords and their variations either in the title and abstract (see the comprehensive keyword list in Appendix~\ref{app:keyword}). As a result, we selected 2,136 out of 34,213 papers that are potentially relevant mentioning the keywords for our literature review. 
% % % 
% % % Note that at this stage, we aim to 



% % \subsubsection{Filtering with Inclusion and Exclusion Criteria.} 
% \subsubsection{Assessing Eligibility with Criteria}
% % 
% We further filtered the 2,136 papers based on explicit inclusion and exclusion criteria, i.e., the \emph{Eligibility} stage.
% % 
% Our criteria revolved around six research questions that we collectively identified to be most pertinent to the topic, including \emph{1) what essential human values have been aligned by some AI models?} \emph{2) how did we effectively quantify or model human values to guide AI development?} \emph{3) what strategies have been employed to integrate human values into the AI development process?} \emph{4) how did existing studies improve human understanding and
% evaluation of AI alignment?} \emph{5) what are the practices for designing interfaces and interactions that
% facilitate human-AI collaboration?} 
% % \emph{6) what are the practices for designing interfaces and interactions that facilitate human-AI collaboration?}
% \emph{6) How have AI been adapted to meet the needs of various human value groups?
% }
% % 
% % 
% We included papers that could potentially answer any of these questions.
% %, we devised a series of inclusion criteria to aid in 1) human values, 2) AI development techniques, 3) AI evaluation, explanation and utilization, and 4) building dataset with human interaction 
% % 
% Further, based on the scope in Section~\ref{sec:scope}, we excluded papers that  did not meet our inclusion criteria. This resulted in a final corpus of 411 papers, which were analyzed in detail using qualitative coding (see Appendix~\ref{app:criteria} for more details).


% % To further narrow down the scope of the keyword-filtered 2136 relevant papers, we specified the explicit inclusion and exclusion criteria collectively for selecting the papers in the following process. 
% % % 
% % Overall, our criteria revolves around six research questions which we collectively identified to be most pertinent to the bidirectional human-AI alignment process based on group discussions. These pertinent research questions involved aspects about \emph{category of human values}, \emph{methods of quantifying human values}, \emph{approaches to integrate human values into AI}, \emph{assessment and explanations of AI regarding human values}, \emph{human-AI interaction techniques}, and \emph{methods to adapt AI for diverse human values}. See the Appendix~\ref{app:criteria} for more details.
% % % 
% % It is worth noting that these research questions are evolved to be the key dimensions in our framework introduced in Section~\ref{sec:framework}. 





% % Built upon these identified research questions, we next introduced explicit inclusion and exclusion criteria to filter the papers. Concretely, papers under our review explicitly included \emph{studies on human values for AI alignment}, \emph{techniques} of AI development for being more consistent with human values, \emph{explanations and evaluations} that helps human better understand AI and aligned values, and \emph{interactions} that improve human perception and utilization on AI.
% % % 
% % % 
% % If a paper did not present a strong connection to all of these aspects, we exclude it from the review. 
% % % 
% % % 
% % In addition, as the scope of human-AI relevant studies is covering a wide span, we also excluded a number of tasks and study settings. 
% % % 
% % % 
% % For instance, we excluded cross-lingual alignment studies that aim to align the model representation between different languages instead of the knowledge and behaviors between human and AI. 
% % % 
% % We present the complete criteria in Appendix~\ref{app:criteria}. 
% % % 
% % % 
% % In the following section, we also describe how we complement the strict exclusion of these works by considering the expertise of our paper's authors by adding flexibility to the coding process.





% % Note that the above paper selection method targets a specific set of existing studies relevant to the bidirectional human-AI alignment via interaction perspective, as opposed to all studies in the associated domains. We are aware of the limitation of our paper selection process especially regarding the rapid growth in human-AI alignment studies. Therefore, the primary goal of this study is not to provide a comprehensive literature coverage. Instead, we aim to recognize a systematic framework that can guide pertinent studies in thinking about a more holistic perspective on human-AI alignment by taking the bidirectional interaction process into account.






% % \subsubsection{Group-based Iterative Coding.}
% % \subsubsection{Framework and Code Development.}
% \subsubsection{Qualitative Code Development.}
% % 
% % 

% % Inspired by 
% Referring to the code development process in~\citet{lee2024design}, we first conducted qualitative coding for each paper by identifying relevant sentences that could answer the above research questions, and entering short codes to describe them into a codebook. We iteratively coded relevant sentences from each paper through a mix of inductive and deductive approaches, which allowed flexibility to expand, modify or change the driving research questions based on our learnings as we went through the process. 
% % 
% % 
% % we first conducted qualitative coding for each paper by quoting the relevant sentences that could answer the aforementioned research questions into our codebook.
% % 
% % 
% To ensure rigor in our coding process, two authors coded each paper. The first author independently annotated all papers after reviewing the paper abstracts and introductions. Twelve team members each annotated a subset of the paper corpus. 
% % 
% % 
% % 
% % Particularly, we coded each paper with two authors to ensure the coding quality.
% % One author independently annotated all papers based on reviewing the paper abstracts and introductions. The rest of twelve team members each annotated a subset of the entire paper list.
% % We conducted two stages of coding, quote-based and rigorous coding. 
% % Since o
% Our corpus includes papers from different domains (\eg HCI, NLP and ML). Therefore, we divided the authors into HCI and NLP/ML\footnote{Note that NLP and ML are two different domains, we combine them together for the purposes of literature review analysis since they both work on developing and evaluating AI technologies.} teams and assigned the papers accordingly based on expertise. 
% All team members coded each of their assigned papers to answer all six questions (if applicable) introduced above.
% % based on their expertise and preference. 
% % The teammates chose the papers within their experienced domains and coded papers' quotes to answer all six questions introduced above.


% % After collecting the 411 papers, we conducted the paper annotation process to develop qualified codes and the bidirectional human-AI alignment framework. 




% % To ensure a qualified annotation process, we divided the authors into two teams based on their expertise, including an HCI team and an NLP team (Note that the NLP team here represents authors in both NLP and ML research fields). Correspondingly, we split the gathered papers into two collections for the HCI and NLP teams, respectively. As a result, the authors in the HCI and NLP teams would only review the papers published in their respective fields. The motivation of this annotation process design is twofold. First, reviewing the papers published in the author's area of expertise could better ensure the quality of developed dimensions and codes. Besides, team-based knowledge aggregation and discussions could be conducive to developing the comprehensive and systematic framework taxonomies.
% % % 



% % Inspired by the code development processed in~\citet{lee2024design},
% % % In terms of code development, 
% % % implementing qualified paper codes,
% % we had each paper annotated by two authors and computed their inter-rater reliability. Particularly, one author independently annotated all papers based on reviewing the paper abstracts and introductions. The rest of team members 
% % % the members of the NLP and HCI teams 
% % each annotated a subset of the entire paper list.
% % % collection evenly by reading the entire paper in detail. 
% % We conducted two stages of coding, quote-based and rigorous coding. 
% % % The iterative coding development took over two months.


% % The rationales of this coding implementation are from three perspectives. Firstly, the paper codes were more objective after ensuring at least two authors read each paper to decide the paper's relevance and resolve any disagreement through discussion. Secondly, we had one author read through all papers, which played a pivotal role in keeping the codes consistent and identifying the research gaps between the two representative fields (\ie HCI and NLP). Last but not least, although the one author who annotated all papers only read through each paper's abstracts and introductions, we had the rest of the NLP and HCI members read through the whole papers assigned to them. This balanced the depth and coverage of our paper annotations well.
% % % ~\hua{compute IRR}.








% % \subsubsection{Code Aggregation and Framework Development.}
% \subsubsection{Framework Development and Rigorous Coding.}
% % 
% After developing annotations, all authors collaborated to create the bidirectional human-AI alignment framework by integrating the annotations within each of the codes. The initial version of the framework was proposed by the author who reviewed all papers. This framework furthermore underwent iterative improvement through: \emph{1)} discussions with all team members involved in paper coding, and \emph{2)} revisions based on feedback from the project advisors.
% % 
% Additionally, we strengthened the framework by reviewing papers from the AI Ethics conferences (including FAccT and AIES), and related work of the collected papers that covered other domains such as psychology and social science.
% We further added missing codes and papers to ensure comprehensive coverage (see Appendix~\ref{app:venues} for details).
% % 
% The final bidirectional human-AI alignment framework, with detailed topologies, is presented in Section~\ref{sec:framework}.
% % 
% Following the framework's finalization, we conducted another separate coding process to annotate \emph{whether each paper investigated dimensions within our framework}. Two authors independently coded each paper.\footnote{The joint probability of agreement for the paper annotations was 0.78.}
% These codes were then used to perform quantitative and qualitative analyses, as presented in Section~\ref{sec:analysis}.


% % After the teams developed their annotations, all authors gathered to create the framework iteratively by combining the dimensions and codes from all team members. Particularly, the one author who read through all the papers proposed the initial version of the bidirectional human-AI alignment framework. Then, this framework was iteratively improved by: \emph{i)} iterative discussion with all the team members who coded the papers; and \emph{ii)} iterative discussion with the advisors and revision based on their feedback.
% % We present the final framework of bidirectional human-AI alignment in Section~\ref{sec:framework} for more details.
% % % 
% % After finalizing the framework with detailed dimensions and codes, we further conducted a rigorous code to annotate \emph{whether each paper investigated each of the dimensions in the framework}. Similar to the previous step, we have each paper annotated by two authors\footnote{The joint probability of agreement for the two authors' annotationswas 0.78.}. We further used these rigorous codes to conduct the quantitative and qualitative analysis shown in Section~\ref{sec:analysis}.
% % 

% % the aggregation of paper codes and framework development, we next conducted quantitative and qualitative analysis on the codes. We show the detailed approaches and findings in Section~\ref{sec:analysis}.
% % 



% % Note that this study goes beyond the aggregation of \emph{current} bidirectional human-AI alignment studies and generates \emph{new possibilities} for \emph{future} research directions. Regarding the limited amount of existing peer-reviewed literature on some aspectis within the bidirectional human-AI alignment framework (\eg customizing AI alignment for specific user groups), we also referred to the concept of \emph{scoping studies}, which aims to ``\emph{map rapidly the key concepts underpinning a research and the main sources and types of evidence available...especially where an area is complex or has
% % not been reviewed comprehensively before}''~\cite{arksey2005scoping}.
% % Specfically, underpinning the imperative research question identified in the \emph{criteria filtering} stage, we allowed flexibility in the iterative code development process in several manners. 
% % % 
% % First, to provide insights on recent advancements in human-AI alignment beyond our paper selection range, we encouraged the authors to bring in external representative papers to supplement the completeness of the developed framework taxonomies. Consequently, we expand our final paper list with an external collection to aid our framework and code development. Additionally, we conducted a series of interviews with project advisors on envisioning future directions, regardless of existing studies, to enhance bidirectional human-AI alignment.
































% ================== dead kitten ===================
% during developing the framework and paper codes iteratively.


% % 
% \textbf{Scoping Studies - Framework - generate new possibilities}.
% \emph{aim to map rapidly the key concepts underpinning a
% research area and the main sources and types of evidence
% available...especially where an area is complex or has
% not been reviewed comprehensively before}~\cite{arksey2005scoping}.








% \subsection{Systematic Literature Review}
% \label{sec:litreview}


% Figure shows our overall process of our systematic literature review and the framework creation.



% \subsubsection{Paper Selection}
% \label{sec:sampling}

% To understand the current research literature on 






% These diverse studies introduce broad definitions of human-AI alignment, and thus demonstrate the opaque research landscape and scope~\cite{kirchner2022researching}. 
% 
% 
% 
% Built upon a number of existing literature review and defining studies about human-AI alignment~\cite{matthews2022alignment,gabriel2020artificial,kenton2021alignment,yao2023instructions, ganguli2022red,terry2023ai,wang2023aligning,
% askell2021general,kirchner2022researching}, we start considering the scope of human-AI alignment in this study by elaborating \emph{who should AI align with}? \emph{Which AI technologies are we primarily considering in this study}? And \emph{what does alignment entail within the context of human-AI interactions}? Particularly, we provide our elaborated definitions introduced in this study as below:
% 
% 





% The emergence of advanced, versatile AI technologies has amplified the importance of ongoing conversations surrounding AI alignment. However, existing literature considers human-AI alignment from diverse perspective, without a consistent definition of ``\emph{what does human-AI alignment mean}'' and ``\emph{who are the humans that AI should align with}''.
% 
% For example, AI alignment commonly considers the overall problem of how to ensure an AI produces the intended outcomes as determined by its creator and /or user, without additional, undesirable side effects (\eg negative effects on individuals, groups, or even society at large)~\cite{matthews2022alignment,gabriel2020artificial,kenton2021alignment}. Meanwhile, a line of studies consider human-AI alignment from the perspectives of safety and ethics, emphasizing that AI should generate harmless contents that align with human values~\cite{yao2023instructions, ganguli2022red}.
% Additionally, some studies consider the role of interaction in human-AI alignment, and breaks down the AI alignment concepts into three alignment objectives, including specification alignment, process alignment and evaluation support~\cite{terry2023ai}. 






    % We primarily consider the lay people who would be the end users of AI systems as our objects that AI systems should align with. Particularly, in this study, we emphasize that the end users, instead of a general human group, should involve more fine-grained sub communities and individuals, who potentially have various utilization demands and concerns, such as citizens from different cultures, marginalized communities, etc. who can potentially be influenced by utilizing AI systems for various purposes.
    % % 
    % % 

    
    % Note that although AI relevant stakeholders are beyond the above range~\cite{deshpande2022responsible}, including AI practitioners (\eg AI developers, AI researchers and experts), organisational stakeholders (\eg technology companies, professional communities), national/international stakeholders (\eg countries, legislative agencies), etc. However, our study focuses on reviewing the alignment between AI with diverse human end users that would be largely influenced by utilizing the deployed AI in practice. 

    

    
    % We consider humans to be the general users who interact with AI systems, including various AI stakeholders such as AI practitioners, domain experts, and lay people.
    % \hua{Eric: what types of humans inside the human-AI Alignment -> one definitions;}






    
    % We consider AI technologies in this study to primarily focus on modern AI algorithms and systems that are extensively studied in human-AI alignment. In particular, we primarily cover literatures that study large language models (LLMs). We also include papers that investigate Machine Learning systems, such as reinforcement learning agents, that contribute imperative advancement in alignment between human and AI.

    
    
    % Despite of various advanced AI technologies, we primarily focus on Large Language Models (LLMs) as the AI systems in this work.





    % \item \textbf{Align AI to $\mapsto$ Human with Interaction.} Integrate human values to train, steer and customize AI.
    % \item \textbf{Align  \textcolor{hua-blue}{AI} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-red}{Human} with Interaction.} We define the process of \emph{aligning AI to human} as integrating human values to train, steer and customize AI. 




    

    % \item \textbf{Align Human to $\mapsto$ AI with Interaction.} Help humans to better evaluate, explain, and inspect AI values.
    % \item \textbf{Align \textcolor{hua-red}{Human} to \textcolor{hua-yellow}{$\mapsto$} \textcolor{hua-blue}{AI} with Interaction.} We designate the process of \emph{aligning human to AI} as enhancing humans' perception and capabilities to better understand, assess, criticize, and harness the transformative AI systems. 




    


% Overall, we are aware that the scope of human-AI alignment is far beyond our studies in this work. For example, it's important to note that there are other stakeholders relevant to AI beyond end users studied in this work, such as AI practitioners (\eg developers, researchers), organizational entities (\eg technology companies, professional communities), and national/international entities (\eg governments, legislative bodies)~\cite{deshpande2022responsible}. However, our study specifically focuses on examining the alignment between AI and the diverse array of end users who will be heavily influenced by leveraging the deployed AI in practice.
% %
% Similarly, there are more prevailing AI technologies, such as Virtual Reality (VR) and Augmented Reality (AR) techniques, which becomes increasingly important in human-AI alignment but not covered in this work. 
% % 
% % 
% % 
% In conclusion, our literature review does not aim to scope all relevant studies in the realm of human-AI alignment. Instead, we are motivated by the human-centered perspective of reviewing human-AI alignment studies, and target on the specific clarified scopes introduced above to investigate the design space, limitations, and future directions in this topic.


    % \textbf{What does alignment entail within the context of human-AI interactions}? 
    % \emph{\textbf{what is human-AI alignment?}}


    % To entail a broader perspective of human-AI alignment as motivated in Section~\ref{sec:background}, in this study, we innovatively propose a conceptual paradigm, named \emph{\aligncode{bidirectional human-AI alignment}}. In specific, the alignment discussed in this study not only includes \aligncode{align AI to human}, indicating research about how to integrate human values to train, steer, and customize AI. Also, we involve \aligncode{align human to AI}, representing studies around what humans should do to critically adapt to AI advancement.
    % We provide detailed definitions below in Section~\ref{sec:definition}. 




    
    % We consider bidirectional alignment in this study, in which AI is developed to be more consistent with human values (i.e., align AI to human), and humans are enhanced to better understand, adapt to and harness AI (i.e., align human to AI). We provide detailed definitions below.
    % % 

    
    % \item \textcolor{hua-yellow}{\textbf{Interaction.}} We consider interactions to include synchronous (\eg interactive prompting) and asynchronous (\eg human-annotated data to train LLMs) interaction between human and AI systems.





% we break down human-AI alignment into two crucial paradigms: \emph{align AI to human} and \emph{align human to AI}.


    % To entail a broader perspective of human-AI alignment as motivated in Section~\ref{sec:background}, in this study, we innovatively propose a conceptual paradigm, named \emph{\aligncode{bidirectional human-AI alignment}}. In specific, the alignment discussed in this study not only includes \aligncode{align AI to human}, indicating research about how to integrate human values to train, steer, and customize AI. Also, we involve \aligncode{align human to AI}, representing studies around what humans should do to critically adapt to AI advancement.
    % We provide detailed definitions below in Section~\ref{sec:definition}. 



% and primarily base our study on the value alignment.

% We investigation primarily focuses on value alignment, whereas there are also diverse factors that we might want to consider for ``alignment'' beyond ``values'', such as norms and cultures. 







    % We primarily consider AI technologies that have been extensively researched in the field of human-AI alignment around and after the advent of AGI, such as language models, reinforcement learning models, neural network-based classification and regression models, and others.
    % % 
    % Notably, we put an emphasis on text-based models as a representative modality for alignment, while we discuss how the insights in this study can be generalized to other modality models at the end of this section.
    % the generalizability to other modality models at the end of this section.
    % are most interested in literature concerning \aicode{large language models (LLMs)}.


    % The review involved over 400 papers that were published around the advent of general-purpose generative AI, \ie primarily between 2019 until 2024 January. 


    
    % \emph{\textbf{what should be aligned?}}
    % We consider AI technologies in this study to primarily concentrate on the \aicode{outputs and/or generations} of modern AI systems that have been extensively researched in the field of human-AI alignment. Notably, we are most interested in literature concerning \aicode{large language models (LLMs)}.
    % \diyi{somewhere you might want to justify the generalization of this human-AI alignment, especially around how inshgts here can go to "multimodal pretrained models"} 
    % \hua{thanks for the constructive suggestion! indeed, we need to clarify a bit more about our what AI we include and also their generalization to other AI systems. I'll do that!}
    % Also, we partially incorporate studies examining cutting-edge machine learning systems, such as reinforcement learning with human feedback, which have significantly advanced the feasibility of human-AI alignment and assisted human decision making in practice.


% Notably, there exist other pertinent stakeholders within the AI landscape beyond the end users examined herein, including AI practitioners (\eg developers, researchers), organizational entities (\eg technology firms, professional communities), and national/international bodies (\eg governments, legislative bodies)~\cite{deshpande2022responsible}. However, our study is specifically directed towards scrutinizing the alignment between AI systems and the diverse spectrum of end users, who are potentially impacted by the practical deployment of AI technologies significantly. 
% % 
% Furthermore, while there are additional emerging AI technologies, such as Virtual Reality (VR) and Augmented Reality (AR), increasingly relevant to human-AI alignment, these are not encompassed within the scope of our investigation. 
% 




% the adapated PRISMA workflow of our systematic literature review grounded and the development of \emph{bidirectional human-AI alignment} framework.

% This paper is a collaborative effort consisting of a large team of researchers from a variety of disciplines, including Human-Computer Interaction (HCI), Natural Language Processing (NLP), Machine Learning, Informatics, and Social Science. We conducted a systematic literature review to develop the bidirectional human-AI alignment framework and codes as shown in Figure~\ref{fig:review_process}. We introduce the key details of each stage next.
% ~\hua{get the figure1 before or after? please clarify.}



% a series of in-depth discussions by NLP and HCI teams, respectively;  \emph{ii)} a series of discussion among both teams to aggregate insights; \emph{iii)} iterative discussions with project advisors (\ie senior professors and researchers in varioius domains related to bidirectional human-AI alignment). 





% However, there remain some ambiguities and inconsistencies in current literature regarding the definitions of ``\emph{What are the values in alignment}''.
% For instance, some widely discussed alignment factors, such as ``cultures'' and ``norms'', can also be considered as values.
% We thus present a comprehensive analysis of \emph{values} in the context of human-AI alignment in Section~\ref{sec:gap_value}.
% % 
% In this work, we define the \textbf{goal of alignment as ``human values'', which indicates what AI morally out to do as defined by humans}.









% =================================================





% % \subsection{Systematic Literature Review}
% \subsection{Systematic Literature Review Process}
% \label{sec:prisma}

% To understand the research literature relevant to the ongoing, mutual process of human-AI alignment, 
% we performed a systematic literature review based on the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332}.
% % 
% Figure~\ref{fig:review_process} shows 
% the workflow of our process for
% % process of our systematic literature review for 
% paper coding and developing the \emph{bidirectional human-AI alignment} framework. We introduce the step details below.
% % We referred to the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332} for reporting the workflow. 



% % \begin{figure*}[!t]
% %   \centering
% %   \includegraphics[width=1\textwidth]{figures/PRISMA.pdf}
% %   \caption{
% %   The selection and refinement process of our systematic literature review. We referred to the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332} to report the workflow.
% %   From the identification of 34,213 records by keyword search, to screen eligible papers against our criteria and arriveg at our final corpus of 411 papers. For each of the stages where literature reviews were excluded (identification, screening, and eligibility) we further present the total of excluded records.}
% %   \label{fig:review_process}
% %   \Description{}
% % \end{figure*}


% \subsubsection{Identification and Screening with Keywords.}

% % To understand the current research literature on bidirectional human-AI alignment,
% % To understand the research literature relevant to the ongoing, mutual process of human-AI alignment, 
% % we performed a systematic literature review based on the PRISMA guideline~\cite{Pagen71,10.1145/3544548.3581332}.
% % 
% We started with papers published in the AI-related domain venues (including NLP, HCI, and ML fields) beginning from the advent of general-purpose generative AI to present, \ie primarily between January, 2019 and January, 2024 (see details in Appendix~\ref{app:venues}).
% We retrieved 34,213 papers in the initial \emph{Identification} stage.
% Further, we collectively defined a list of keywords (see details in Appendix~\ref{app:keyword}) and screened for papers that included at least one of these keywords (\eg human, alignment) or their variations either in the title or abstract. We included 2,136 papers in this \emph{Screening} stage.
% % We first identify fields closely relevant to our research topic. As a result, we selected the fields of NLP, HCI, and Machine Learning as our pivotal domains and the related conference venues ranging from 2019 to 2024 we considered in this project in Appendix~\ref{app:venues}.
% % 
% % 
% % From the ACL Anthology, OpenReview and ACM Digital Library, we retrieved 34,190 papers into a Reference Manager Tool (\ie Paperpile).
% % 
% % 

% % To further collect the relevant papers, two of the authors collectively defined a list of keywords related to bidirectional human-AI alignment, such as \emph{human}, \emph{alignment}, \emph{interact}, \emph{LLM}, \emph{value}, etc. Next, we only sampled the papers that included these keywords and their variations either in the title and abstract (see the comprehensive keyword list in Appendix~\ref{app:keyword}). As a result, we selected 2,136 out of 34,213 papers that are potentially relevant mentioning the keywords for our literature review. 
% % % 
% % % Note that at this stage, we aim to 



% % \subsubsection{Filtering with Inclusion and Exclusion Criteria.} 
% \subsubsection{Assessing Eligibility with Criteria}
% % 
% We further filtered the 2,136 papers based on explicit inclusion and exclusion criteria, i.e., the \emph{Eligibility} stage.
% % 
% Our criteria revolved around six research questions that we collectively identified to be most pertinent to the topic, including \emph{1) what essential human values have been aligned by some AI models?} \emph{2) how did we effectively quantify or model human values to guide AI development?} \emph{3) what strategies have been employed to integrate human values into the AI development process?} \emph{4) how did existing studies improve human understanding and
% evaluation of AI alignment?} \emph{5) what are the practices for designing interfaces and interactions that
% facilitate human-AI collaboration?} 
% % \emph{6) what are the practices for designing interfaces and interactions that facilitate human-AI collaboration?}
% \emph{6) How have AI been adapted to meet the needs of various human value groups?
% }
% % 
% % 
% We included papers that could potentially answer any of these questions.
% %, we devised a series of inclusion criteria to aid in 1) human values, 2) AI development techniques, 3) AI evaluation, explanation and utilization, and 4) building dataset with human interaction 
% % 
% Further, based on the scope in Section~\ref{sec:scope}, we excluded papers that  did not meet our inclusion criteria. This resulted in a final corpus of 411 papers, which were analyzed in detail using qualitative coding (see Appendix~\ref{app:criteria} for more details).


% % To further narrow down the scope of the keyword-filtered 2136 relevant papers, we specified the explicit inclusion and exclusion criteria collectively for selecting the papers in the following process. 
% % % 
% % Overall, our criteria revolves around six research questions which we collectively identified to be most pertinent to the bidirectional human-AI alignment process based on group discussions. These pertinent research questions involved aspects about \emph{category of human values}, \emph{methods of quantifying human values}, \emph{approaches to integrate human values into AI}, \emph{assessment and explanations of AI regarding human values}, \emph{human-AI interaction techniques}, and \emph{methods to adapt AI for diverse human values}. See the Appendix~\ref{app:criteria} for more details.
% % % 
% % It is worth noting that these research questions are evolved to be the key dimensions in our framework introduced in Section~\ref{sec:framework}. 





% % Built upon these identified research questions, we next introduced explicit inclusion and exclusion criteria to filter the papers. Concretely, papers under our review explicitly included \emph{studies on human values for AI alignment}, \emph{techniques} of AI development for being more consistent with human values, \emph{explanations and evaluations} that helps human better understand AI and aligned values, and \emph{interactions} that improve human perception and utilization on AI.
% % % 
% % % 
% % If a paper did not present a strong connection to all of these aspects, we exclude it from the review. 
% % % 
% % % 
% % In addition, as the scope of human-AI relevant studies is covering a wide span, we also excluded a number of tasks and study settings. 
% % % 
% % % 
% % For instance, we excluded cross-lingual alignment studies that aim to align the model representation between different languages instead of the knowledge and behaviors between human and AI. 
% % % 
% % We present the complete criteria in Appendix~\ref{app:criteria}. 
% % % 
% % % 
% % In the following section, we also describe how we complement the strict exclusion of these works by considering the expertise of our paper's authors by adding flexibility to the coding process.





% % Note that the above paper selection method targets a specific set of existing studies relevant to the bidirectional human-AI alignment via interaction perspective, as opposed to all studies in the associated domains. We are aware of the limitation of our paper selection process especially regarding the rapid growth in human-AI alignment studies. Therefore, the primary goal of this study is not to provide a comprehensive literature coverage. Instead, we aim to recognize a systematic framework that can guide pertinent studies in thinking about a more holistic perspective on human-AI alignment by taking the bidirectional interaction process into account.






% % \subsubsection{Group-based Iterative Coding.}
% % \subsubsection{Framework and Code Development.}
% \subsubsection{Qualitative Code Development.}
% % 
% % 

% % Inspired by 
% Referring to the code development process in~\citet{lee2024design}, we first conducted qualitative coding for each paper by identifying relevant sentences that could answer the above research questions, and entering short codes to describe them into a codebook. We iteratively coded relevant sentences from each paper through a mix of inductive and deductive approaches, which allowed flexibility to expand, modify or change the driving research questions based on our learnings as we went through the process. 
% % 
% % 
% % we first conducted qualitative coding for each paper by quoting the relevant sentences that could answer the aforementioned research questions into our codebook.
% % 
% % 
% To ensure rigor in our coding process, two authors coded each paper. The first author independently annotated all papers after reviewing the paper abstracts and introductions. Twelve team members each annotated a subset of the paper corpus. 
% % 
% % 
% % 
% % Particularly, we coded each paper with two authors to ensure the coding quality.
% % One author independently annotated all papers based on reviewing the paper abstracts and introductions. The rest of twelve team members each annotated a subset of the entire paper list.
% % We conducted two stages of coding, quote-based and rigorous coding. 
% % Since o
% Our corpus includes papers from different domains (\eg HCI, NLP and ML). Therefore, we divided the authors into HCI and NLP/ML\footnote{Note that NLP and ML are two different domains, we combine them together for the purposes of literature review analysis since they both work on developing and evaluating AI technologies.} teams and assigned the papers accordingly based on expertise. 
% All team members coded each of their assigned papers to answer all six questions (if applicable) introduced above.
% % based on their expertise and preference. 
% % The teammates chose the papers within their experienced domains and coded papers' quotes to answer all six questions introduced above.


% % After collecting the 411 papers, we conducted the paper annotation process to develop qualified codes and the bidirectional human-AI alignment framework. 




% % To ensure a qualified annotation process, we divided the authors into two teams based on their expertise, including an HCI team and an NLP team (Note that the NLP team here represents authors in both NLP and ML research fields). Correspondingly, we split the gathered papers into two collections for the HCI and NLP teams, respectively. As a result, the authors in the HCI and NLP teams would only review the papers published in their respective fields. The motivation of this annotation process design is twofold. First, reviewing the papers published in the author's area of expertise could better ensure the quality of developed dimensions and codes. Besides, team-based knowledge aggregation and discussions could be conducive to developing the comprehensive and systematic framework taxonomies.
% % % 



% % Inspired by the code development processed in~\citet{lee2024design},
% % % In terms of code development, 
% % % implementing qualified paper codes,
% % we had each paper annotated by two authors and computed their inter-rater reliability. Particularly, one author independently annotated all papers based on reviewing the paper abstracts and introductions. The rest of team members 
% % % the members of the NLP and HCI teams 
% % each annotated a subset of the entire paper list.
% % % collection evenly by reading the entire paper in detail. 
% % We conducted two stages of coding, quote-based and rigorous coding. 
% % % The iterative coding development took over two months.


% % The rationales of this coding implementation are from three perspectives. Firstly, the paper codes were more objective after ensuring at least two authors read each paper to decide the paper's relevance and resolve any disagreement through discussion. Secondly, we had one author read through all papers, which played a pivotal role in keeping the codes consistent and identifying the research gaps between the two representative fields (\ie HCI and NLP). Last but not least, although the one author who annotated all papers only read through each paper's abstracts and introductions, we had the rest of the NLP and HCI members read through the whole papers assigned to them. This balanced the depth and coverage of our paper annotations well.
% % % ~\hua{compute IRR}.








% % \subsubsection{Code Aggregation and Framework Development.}
% \subsubsection{Framework Development and Rigorous Coding.}
% % 
% After developing annotations, all authors collaborated to create the bidirectional human-AI alignment framework by integrating the annotations within each of the codes. The initial version of the framework was proposed by the author who reviewed all papers. This framework furthermore underwent iterative improvement through: \emph{1)} discussions with all team members involved in paper coding, and \emph{2)} revisions based on feedback from the project advisors.
% % 
% Additionally, we strengthened the framework by reviewing papers from the AI Ethics conferences (including FAccT and AIES), and related work of the collected papers that covered other domains such as psychology and social science.
% We further added missing codes and papers to ensure comprehensive coverage (see Appendix~\ref{app:venues} for details).
% % 
% The final bidirectional human-AI alignment framework, with detailed topologies, is presented in Section~\ref{sec:framework}.
% % 
% Following the framework's finalization, we conducted another separate coding process to annotate \emph{whether each paper investigated dimensions within our framework}. Two authors independently coded each paper.\footnote{The joint probability of agreement for the paper annotations was 0.78.}
% These codes were then used to perform quantitative and qualitative analyses, as presented in Section~\ref{sec:analysis}.


% % After the teams developed their annotations, all authors gathered to create the framework iteratively by combining the dimensions and codes from all team members. Particularly, the one author who read through all the papers proposed the initial version of the bidirectional human-AI alignment framework. Then, this framework was iteratively improved by: \emph{i)} iterative discussion with all the team members who coded the papers; and \emph{ii)} iterative discussion with the advisors and revision based on their feedback.
% % We present the final framework of bidirectional human-AI alignment in Section~\ref{sec:framework} for more details.
% % % 
% % After finalizing the framework with detailed dimensions and codes, we further conducted a rigorous code to annotate \emph{whether each paper investigated each of the dimensions in the framework}. Similar to the previous step, we have each paper annotated by two authors\footnote{The joint probability of agreement for the two authors' annotationswas 0.78.}. We further used these rigorous codes to conduct the quantitative and qualitative analysis shown in Section~\ref{sec:analysis}.
% % 

% % the aggregation of paper codes and framework development, we next conducted quantitative and qualitative analysis on the codes. We show the detailed approaches and findings in Section~\ref{sec:analysis}.
% % 



% % Note that this study goes beyond the aggregation of \emph{current} bidirectional human-AI alignment studies and generates \emph{new possibilities} for \emph{future} research directions. Regarding the limited amount of existing peer-reviewed literature on some aspectis within the bidirectional human-AI alignment framework (\eg customizing AI alignment for specific user groups), we also referred to the concept of \emph{scoping studies}, which aims to ``\emph{map rapidly the key concepts underpinning a research and the main sources and types of evidence available...especially where an area is complex or has
% % not been reviewed comprehensively before}''~\cite{arksey2005scoping}.
% % Specfically, underpinning the imperative research question identified in the \emph{criteria filtering} stage, we allowed flexibility in the iterative code development process in several manners. 
% % % 
% % First, to provide insights on recent advancements in human-AI alignment beyond our paper selection range, we encouraged the authors to bring in external representative papers to supplement the completeness of the developed framework taxonomies. Consequently, we expand our final paper list with an external collection to aid our framework and code development. Additionally, we conducted a series of interviews with project advisors on envisioning future directions, regardless of existing studies, to enhance bidirectional human-AI alignment.






==> tables/technology-designspace.tex <==
%TC:ignore
\begin{table*}
    \resizebox{1.\linewidth}{!}{
    % \begin{threeparttable}
        \renewcommand{\arraystretch}{1.43}
        \setlength{\tabcolsep}{4pt}
        \begin{tabular}{p{0.05\textwidth}p{0.25\textwidth}p{0.8\textwidth}}
            \toprule
            &
             \textbf{Code} &
             \textbf{Definition} \\
             \midrule

             \multirow{9}{*}[2.5em]{\rotatebox{90}{\renewcommand{\arraystretch}{1}\begin{tabular}[c]{@{}c@{}}{\rqbdim{Data}}\\ {{\rqbdim{Source}}}\end{tabular}}} &
             \multicolumn{2}{l}{\emph{Who is the creator of the data used to train or adapt a model?}} \\
             \cline{2-3}
            &
             {Experts} &
             Experts of the task or domain of interest \\
            &
             {Users} &
             Current or target users of a downstream application \\
            &
             {Crowdworkers} &
             Crowdworkers from various platforms, such as Amazon Mechanical Turk and Prolific \\
            &
             {Authors} &
             Authors of the research paper \\
            &
             {Machine} &
             Another model that generates synthetic data \\
            & 
             {Other} & 
             Other creators, such as non-experts and unspecified individuals for web crawled data \\
             \midrule


            \multirow{7}{*}{\rotatebox{90}{\renewcommand{\arraystretch}{1}\begin{tabular}[c]{@{}c@{}}{\textbf{Data}}\\ {{\textbf{Size}}}\end{tabular}}}
            &
             \multicolumn{2}{l}{\emph{What is the size of the dataset that used to train or adapt a model?}} \\
             \cline{2-3}
            &
             {Small (<100)} &
             Uses one to a hundred data points \\
            &
             {Medium (<10k)} &
             Uses a hundred to a few thousand data points \\
            &
             {Large (<1M)} &
             Uses tens to hundreds of thousands of data points \\
            &
             {Extremely large (>1M)} &
             Uses millions of data points or more\\
             &
             {Unknown} &
             Unknown data or dataset size \\
             \midrule

             \multirow{6}{*}{\rotatebox{90}{\renewcommand{\arraystretch}{1}\begin{tabular}[c]{@{}c@{}}{\textbf{Model}}\\ {{\textbf{Type}}}\end{tabular}}} &
             \multicolumn{2}{l}{\emph{What is the type of the underlying model?}} \\
             \cline{2-3}
            &
             {Rule-based model} &
             Model relying on heuristics or deterministic approaches (\eg lookup tables and regular expressions) \\
            &
             {Statistical ML model} &
             Machine learning (ML) model typically trained for a specific task (\eg logistic regression) \\
            &
             {Deep neural network} &
             ML model that uses multiple layers between the input and output layers (\eg RNNs and LSTMs) \\
            &
             {Foundation model} &
             Pre-trained deep neural network that can be adapted for downstream tasks (\eg BERT, GPT-4) \\
            \midrule

             \multirow{3}{*}[.05em]{\rotatebox{90}{\renewcommand{\arraystretch}{1}\begin{tabular}[c]{@{}c@{}}{\textbf{Model}}\\ {{\textbf{\small External Res.}}}\end{tabular}}} &
             \multicolumn{2}{l}{\emph{What additional access does a model have at inference time?}} \\
             \cline{2-3}
            &
             {Tool} &
             External software or third party APIs the model might rely on to perform its task\\
             % , such as calculator and translator \\
            &
             {Data} &
             External datasets or resources, such as external knowledge repositories\\
             % information stored in a company's database, , or any other structured/unstructured data sources \\
            \midrule
            
             \multirow{7}{*}[0em]{\rotatebox{90}{\renewcommand{\arraystretch}{1}\begin{tabular}[c]{@{}c@{}}{\textbf{Learning}}\\ {{\textbf{Problem}}}\end{tabular}}} &
             \multicolumn{2}{l}{\emph{How is the writing assistance task being formulated as a learning problem?}} \\
             \cline{2-3}
            &
             {Classification} &
             Assigns inputs to predefined categories or classes \\
            &
             {Regression} &
             Predicts continuous numeric values for a given input \\
            &
             {Structured prediction} &
             Focuses on capturing dependencies, relationships, and patterns in language data \\
            &
             {Rewriting} &
             Translates text from one form to another, while preserving its meaning and information content \\
            &
             {Generation} &
             Creates new, coherent, and contextually relevant text \\
            & 
             {Retrieval} &
             Finds and optionally ranks relevant instances for a given input \\
             \midrule

             \multirow{6}{*}[0.7em]{\rotatebox{90}{\renewcommand{\arraystretch}{1}\begin{tabular}[c]{@{}c@{}}{\textbf{Learning}}\\ {{\textbf{Algorithm}}}\end{tabular}}} &
             \multicolumn{2}{l}{\emph{How is the underlying model being trained?}} \\
             \cline{2-3}
            &
             {Supervised learning} &
             Model is trained on labeled data where each input is associated with the correct output \\
            &
             {Unsupervised learning} &
             Model is trained on unlabeled data to discover patterns and structures within the data \\
            &
             {Self-supervised learning} &
             Model creates a supervisory signal from the data itself, without human-annotated labels \\
            &
             {Reinforcement learning} &
             Model learns by interacting with an environment and receiving feedback in the form of rewards \\
            % &
            %  {No training} &
            %  \todo{this is appeared in the text but missing from the table} \\
             \bottomrule
            \end{tabular}
        % \end{threeparttable}
        }
    \caption{Technology dimensions, codes, and definitions (continued in the next table).}
    \label{tab:technology-designspace-1}
\end{table*}

\begin{table*}
    \resizebox{1.\linewidth}{!}{
    % \begin{threeparttable}
        \renewcommand{\arraystretch}{1.45}
        \setlength{\tabcolsep}{4pt}
        \begin{tabular}{p{0.05\textwidth}p{0.3\textwidth}p{0.8\textwidth}}
            \toprule
            &
             \textbf{Code} &
             \textbf{Definition} \\
             \midrule

             \multirow{6}{*}[0.60em]{\rotatebox{90}{\renewcommand{\arraystretch}{1}\begin{tabular}[c]{@{}c@{}}{\textbf{Learning}}\\ {{\textbf{\small Training \& adaptation}}}\end{tabular}}} &
             \multicolumn{2}{l}{\emph{How is the underlying model being trained or adapted for a specific task at hand?}} \\
             \cline{2-3}
            &
             {Training from scratch} &
             A new model is trained from scratch, or a foundation model is used without  adaptation \\
            &
             {Fine-tuning} &
             A foundation model is further trained on a specific dataset \\
            &
             {Prompt engineering} &
             A foundation model is further adapted via prompts (a.k.a. in-context learning) \\
            &
             {Tuning decoding parameters} &
             A model's decoding parameters are adjusted to stir model outputs (\eg temperature and logit bias) \\
            \midrule
                        
            \multirow{9}{*}[2.5em]{\rotatebox{90}{\renewcommand{\arraystretch}{1}\begin{tabular}[c]{@{}c@{}}{\textbf{Evaluation}}\\ {{\textbf{Evaluator}}}\end{tabular}}} &
             \multicolumn{2}{l}{\emph{Who evaluates the quality of model outputs?}} \\
             \cline{2-3}
            &
             {Automatic evaluation} &
             Quality is evaluated based on simple aggregate statistics or on similarity metrics\\
             % on syntactic or semantic similarity computed algorithmically (e.g., BLEU, ROUGE, SARI, etc.) \\
            &
             {Machine-learned evaluation} &
             Quality is evaluated by another model to produce ratings or scores (e.g., BERTScore) \\
            &
             {Human evaluation} &
             Quality is evaluated by human annotators \\
            &
             {Human-machine evaluation} &
             Quality is evaluated by both  human annotators and another model, often by having the model filter a subset of outputs to be annotated by humans \\
            \midrule

            \multirow{9}{*}[3.5em]{\rotatebox{90}{\renewcommand{\arraystretch}{1}\begin{tabular}[c]{@{}c@{}}{\textbf{Evaluation}}\\ {{\textbf{Focus}}}\end{tabular}}} &
             \multicolumn{2}{l}{\emph{What is the focus of evaluation when evaluating individual model outputs?}} \\
             \cline{2-3}
            &
             {Linguistic quality} &
             Evaluation focuses on qualities such as grammaticality, readability, clarity, and accuracy \\
            &
             {Controllability} &
             Evaluation focuses on the reflectiveness to controls  or constraints specified by users or designers\\
             % , such as a desired level of formality and writing style \\
            &
             {Style \& Adequacy} &
             Evaluation focuses on the alignment between model ouputs and their surrounding texts\\
             % (i.e., contexts), such as stylistic or semantic coherence, relevance, and consistency \\
            &
             {Ethics} &
             Evaluation focuses on social norms and ethics, such as bias, toxicity, factuality, and transparency \\
            \midrule            
            
            \multirow{3}{*}[-0.1em]{\rotatebox{90}{\textbf{{Scalability}}}} &
             \multicolumn{2}{l}{\textit{What are the economic and computational considerations for developing and deploying a model?}} \\
             \cline{2-3}
            &
             {Cost} &
             Cost of deploying the model \\
            &
             {Latency} &
             Delay between when the model receives an input and generates a corresponding output \\
        \bottomrule
        \end{tabular}
    % \end{threeparttable}
    }
\caption{Technology dimensions, codes, and definitions (continued from the previous table).}
\label{tab:technology-designspace-2}
\end{table*}
%TC:endignore

==> title.tex <==


\title[Towards Bidirectional Human-AI Alignment: A Systematic Review
]{Towards Bidirectional Human-AI Alignment: A Systematic Review for Clarifications, Framework, and Future Directions}
% \title{aa}



% Towards Bidirectional Human-AI Alignment: Clarifications, Framework, and Future Directions

% "Toward Bidirectional Human-AI Alignment: A Systematic Review and Conceptual Framework"





% \title[bidirectional human-AI alignment with interaction]{Mutual Human-AI Alignment: A Systematic Review towards a Complete Loop of Bidirectional Human-AI Alignment}


% \title[]{Is Aligning AI to Human Enough? A Systematic Review of Bidirectional Human-AI Alignment Towards a Holistic Loop}

% \title[]{Is Aligning AI to Human Enough? A Systematic Review of Bidirectional Human-AI Alignment Towards a Holistic Loop}




